Profiling Apple Silicon Performance for ML Training

Apple Silicon has attracted much attention for its performance and role in machine learning (ML) training. Unlike NVIDIA GPUs, which have traditionally dominated ML training, Apple Silicon has a significant difference in memory architecture. It uses Unified Memory, which integrates CPU and GPU memory instead of separate CPU memory and GPU VRAM. However, it is difficult to tell whether Unified Memory means more performance benefits. This paper investigates the performance differences by training several large language model (LLM) workloads end-to-end under different memory scenarios. The results show a significant performance gap between Apple Silicon and NVIDIA GPUs. This paper attributes this gap to system-level factors such as page faults, power consumption, and kernel launch time. In addition, the performance difference of basic linear algebra subprograms (BLAS) on the NVIDIA GPUs and Apple Silicon chips is analyzed to further explain the observed gap.

==> contrib.tex <==
% !TeX root = main.tex

\section{Contributions}

The proposed project makes the following contributions:
\begin{myitemize}
	\item 
	It will identify and characterize the cold start inference problem on multiple platforms;
	it will obtain diverse IO/Compute profiles measured on real hardwares, such as Odroid~\cite{odroid-web}, Raspberry Pi~\cite{rpi3-web}, and Beagleboard X15~\cite{x15-web}.

	
	\item 
	A novel system design for accelerating \tfm{} cold start inference of pretrained models on edge devices.
	It features two novel techniques: 
	1) \textit{structured model sharding}, which partitions the whole pretrained model into multiple attention heads, quantized into different bitwidths;
	2) \textit{device heterogeneity-aware shard planning}, which schedules shards for both low latency and maximum accuracy, based on the specific IO/Compute profile of the hardware and a deadline.
	
	\item
	The implementation and evaluation of the proposed system.
	It will evaluate the system on the pretrained  BERT~\cite{bert} model using the GLUE benchmark suite~\cite{glue-benchmark}.
	The implementation will be made open-source to facilitate future research on the cold start inference problem. 
	
%	\begin{itemize}
%		\item 
%		Pipelining 
%		
%		\item 
%		Deadline-driven dynamic bitwidth selection for encoder layers. 
%		
%		\item 
%		Hierarchical word embedding cache layers. 
%	\end{itemize}
%	Backing the techniques is a co-designed system memory management layer.. 
%	Compared with the vanilla page cache, it is model aware and finer grained: at the granularity of an attention head instead of whole model file; 
%	cache replacement strategy is pipeline-aware...
%	
%	\item 
%	Case studies of \sys{} on a wide range of devices that have diverse hardware characteristics. 
	
\end{myitemize}


%\paragraph{Key ideas.}
%To address the above challenges, we propose \sys{}, a novel transformer-OS co-design.
%The mechanism is as follows.
%\begin{myenumerate}
%	\item
%	Hierarchical, frequency-based word embedding storage. 
%	To start as soon as possible, \sys{} caches XXX most recently used word embeddings in memory ($<1\%$, XXX KB) (Zipf law), and clusters the rest based on their frequency.
%	\sys{} stores each cluster in a number sequential disk blocks (XXX MB, XXX words), which minimizes the loading latency for the platform\Note{platform aware...}.
%	The hierarchical embedding reduces the latency by XX\%.
%	
%	
%	\item 
%	Progressive(evolutionary) weight sharing. 
%	During cold inference, \sys{} only loads one transformer layer, whose parameters are shared across all others, inspired by~\cite{albert};
%	upon each future inference, \sys{} loads one more transformer layer by overlapping its IO with compute on existing, loaded, and shared layers.  
%	Such a model can be viewed as supernet of $N$ transformer layers, which consists of $N$ subnets, each of 1 to $N$ distinct layers.
%	
%	
%	\item 
%	Layer-aware page caching.
%	To support \sys{}, we specialize kernel memory management. 
%	It unifies the model file \textit{with} flatten/loaded model parameters\Note{XXX:forecast double copy}, making them a unified copy;
%	instead of caching the model file as a whole, it caches individual transformer layers. 
%	Doing so saves XXX\% memory during inference. 
%\end{myenumerate}


==> design-bert.tex <==
% !TeX root = main.tex

\subsection{Progressive BERT}


The key idea is 1) to progressively load a BERT model from the smallest to the full one, and 2) to start inference as soon as possible by overlapping an IO task with Compute.

\subsubsection{Key challenges.}
The design raises following challenges:
\begin{myenumerate}
	\item 
	\textit{How to decide an IO/Compute task?}
%	\textit{How to avoid starvation?}
	It is crucial to pipeline efficiency. 
	Displacement of IO/Compute task (e.g. layerwise) leads to starvation and poor performance, as discussed in \sect{motiv:design-explore}. 
%	The problem is high IO/Compute ratio (as high as 10:1, shown in \sect{motiv:char}), which leads to starvation. 
	The ratio needs at least to be close for an effective overlap.

	
	\item 
	\textit{How to cater to different platforms?}
	IO vs Compute ratio is platform-specific, especially for mobile devices which have diverse hardware.
	A universal pipelining strategy cannot fit the different nature of mobile devices. 

	\item
	\textit{How to progressively load parameters?}
	\Note{how to train such a model...}
	The key of our design is weights from sub-trasnformers can be used to collectively and progressively to create a larger super-transformer. 
\end{myenumerate}

\subsubsection{Solutions.}

To address the above challenges, our ideas are as follows. 

\paragraph{Pipelining Transformer slice.}
We set to use an attention head and the slice of its underlying FFN, a \textit{slice} of a transfomer block, as the IO/Compute task.
We pipeline the slice instead of whole layers.
Our rationals are as follows:
\begin{myenumerate}
	\item 
	The slice is finer grained, offering has a much closer IO/Compute gap. 
	\Note{More importantly,} Compute scales much slower than IO.
	For instance, compute on 1 slice vs 5 slices only leads to XX\% increase, which is still closer than IO of 1 slice\Note{need a figure}. 
	This allows us to approximate pipelining strategy on different hardwares. 

	\item 
	Attention heads have been shown to have high redundancy\cite{16heads};
	weight sharing of them all is promising~\cite{albert}.
	This gives us assurance on performance during cold inference, even at the first inference when only one attention head is used. 
\end{myenumerate}

Formally, we define the \textit{slice} as follows:
a (vertical) slice of a transformer block consists of a single attention head of \Note{XXX} dimensions as specified in BERT~\cite{bert}, and the corresponding FFNs of 256 neurons (one twelve-th of 3076 dimensions). 


\paragraph{IO/Compute-adaptive pipelining strategy.}
This is to have an high-overlapping pipeline, adaptive to different hardwares of mobile devices. 
\sys{} profiles the IO and Compute time of a whole vertical slice defined above, then the IO and Compute for FFN of the slice. 
Due to the careful selection, the IO/Compute ratio is in the same magnitude or very close to each other;
from our measurement the ratio varies between \Note{XXX-YYY}.
For instance, it is 1:1 on Odroid.
\sys{} hence adaptively pipelines w.r.t three difference cases: 
\begin{myenumerate}
	\item 
	$IO = Compute$: 
	close enough ratio, \Note{e.g. 1:1 - 2:1}. 
	Pipeline the following: Compute of the \textit{current} loaded vertical slice with IO of \textit{next} to be loaded vertical slice.
	
	\item
	$IO < Compute$:
	\Note{range is ???}
	Pipeline:  Compute of \textit{current} loaded vertical slice with IO of \textit{next} $n$ vertical slices.
	The goal is not to starve IO;
	the $n$ depends on actual  
	
	\item 
	$IO > Compute$:
	\Note{range is XXX}.
	Pipeline: Compute of \textit{current} loaded vertical slice with IO of \textit{next} FFN, while reusing attention from previous slice. 
	The rational is stated before -- redundancy of attention heads makes weight sharing possible. 
\end{myenumerate}

From the three different cases, \sys{} produces the pipelining strategy for individual mobile devices of different IO/Compute ratio, based on the profile of a transfomer slice. 

\paragraph{Progressive Bert SuperTransformer.}
Our Progressive Bert \textit{Super}Transformer has the same architecture as BERT: 12 layers in total, each transformer layer contains \Note{XXX} attention heads, each of XXX dimensions, and 3076 hidden dimensions for FFNs. 

Its key property is: 
each subTransformer is a slice of the superTransformer;
each inference only loads \textit{one extra} slice of the superTransformer, based on the pipelining strategy;
from cold to hot, multiple inferences compose the slices of a full superTransformer architecture which is BERT.

Advancement from the prior arts is how to collocate and unify the multiple pipelining (i.e. weight sharing) strategy under one superTransformer.
Recall HAT has fixed weight sharing of FFN but not attention; 
DynaBert has fixed weight sharing of attention but not FFN. 
Ours -- two different weight sharing strategies, determined by the hardware it runs on: 1) subTransformers do not share param, or 2) share attention \Note{what about share FFN}.


\textbf{Training methods.}
We adopt following training techniques from previous works.

\textbf{Ranking importance of attention heads.}
So that the most important attention head can be loaded as early as possible for cold inference accuracy. 

\textbf{Sampling FFNs.} 
Similar to Albert~\cite{albert}, HAT~\cite{hat}, LayerDrop~\cite{layerdrop}, for the subTransformers which \textit{may} or \textit{may not} share FFN layer, we randomly sample them to share weights during training time.
This helps smooth the parameter distribution in the resultant superTransformer.


\Note{merge below}
\paragraph{Key difference with existing techniques.}
\begin{myitemize}
	\item 
	\textbf{HAT.} hardware-aware, based on a latency goal. But fix the weight sharing strategy to all FFNs, front part of the embedding. 
	To load the next subTransformer, need re-load attention parameters, resulting in cold inference and long latency.
	
	\item 
	\textbf{DynaBert.} Can adjust width \& depth simultaneously. 
	Also does weight sharing of subtransformers, in terms of attention heads and FFN. 
	Can do attention-head-based pipelining. 
	But is not hardware-aware and has the fixed weight sharing strategy -- a special case when IO = Compute. 
	
	\item 
	\textbf{Ours.} Adaptive pipelining strategy -- different weight sharing mechanism w.r.t. different IO/Compute profiles on diverse hardwares, which is our key novelty.
\end{myitemize}


==> design-embedding.tex <==
% !TeX root = main.tex

\section{Confining disk IO of embeddings}
\xzlNote{become part of implementation}

\Note{highlight the uniqueness of word frequencies}
During cold inference, embedding lookup is blocking and slow. 
When untreated, it significantly reduces usable spare IO (\S\ref{sec:design:planning}), e.g. by XXX\%;
the compute might not have enough budgets, leading to inferior accuracy...

\sys{} reduces the disk IO of embedding, which is a key blocker during cold inference.
It does so by reducing both the total number of disk accesses (caching and embedding quantization), as well as access latency by turning slow, random accesses into fast, sequence ones.

\Note{merge below}
During cold inference, embedding lookup is blocking and slow. 
When untreated, it significantly reduces usable spare IO (\S\ref{sec:design:planning}), e.g. by XXX\%. 
To this end, \sys{} retrofits the known storage optimization techniques:
it quantizes them in low-bit (e.g. 3 bits), reducing their sizes by XX $\times$; 
it employs a small cache (5\% of total size) to absorb most accesses; 
it continuous updates their disk layout based on embedding frequency, optimizing for sequential access.

Embedding table -- a solved problem in storage + recommender system community~\cite{recssd, flashembedding, bandana}.
Likely due to embedding table is the major bottleneck for the community.


\subsection{A primer on embeddings}

In NLP, each word is represented by one embedding vector, usually of a few hundred dimensions (e.g. 768). 
The embedding table is a large lookup table storing all embedding vectors of the vocabulary, sizing from 30K to billions in commercial cloud...
Upon each new input (e.g. 128 words), inference engine looks up each vector in the table, and gather them into a tensor (e.g. $1x128x768$ for a single input) for \tfm{} consumption.


\subsection{Key challenges}


The goal is to reduce disk IO incurred by embedding look up, such that spare IO can be spent on compute for maximizing model accuracy.

We face the following challenges. 
\begin{myitemize}
	\item
	\textit{Embedding IO must block.}
	Inference must wait for aggregated embedding vectors to start.
	Yet, the embedding table constitutes one third of the total parameters, consequently taking over 1s to fully load.
	Meanwhile, it cannot be treated like encoder layer (e.g. pipelining by layers), because there is no compute to overlap because embedding table lookup is negligible compared with IO.
		
	\item 
	\textit{Slow random access.}
	Based on input, one may load individual word embeddings on-demand.
	However, each embedding vector contains 768x4 bytes, consuming a 4KB block.
	On-demand loading results in random 4K block accesses, which is an order of magnitude slower than sequential access (XXX vs YYY) on flash storage. 
\end{myitemize}

\subsection{Reducing disk IO size}

\paragraph{Quantize embeddings into low precisions}
As have been demonstrated in~\cite{binarybert,bibert,qbert} and will be further demonstrated by us in \sect{eval}, embedding layer can afford low-bit representations while having minimal impacts on model accuracy;
there is no need for mixed precision because ...

Therefore we quantize the embedding layer in fixed low-bit precision with the same technique described in~\sect{design:sharding:quantize};
we decide its precision based on sensitivity analysis presented in \sect{design:planning}.

This reduces the embedding vectors size by XX$\times$. 
As a result, a 4K disk block can locate XXX embedding vectors, reducing the block access by XXX$\times$.


\subsection{Catering to embedding access pattern}

For compulsory embedding cache misses, \sys{} reduces their disk access delays in the following ways.

\paragraph{Storing embeddings based on frequencies}
\sys{} adds a new frequency column to the existing embedding table, e.g. like a new dimension to each vector.
It stores the embedding table sorted by frequency on disk in contiguous blocks;
it bookkeeping the file offsets of each word, e.g. ``5-th word is stored at offset 1024'', such that words can be looked up individually.
Doing so ensures the spatial locality of disk accesses of embeddings~\cite{flashembedding,recssd} -- words of phrases are likely used together and shall be stored closely. 
For instance, pronouns such as ``I, you, he, she, they'', are likely to be used often, which may be followed by commonly used verbs such as ``eat, see, walk, run''.

During inferences, \sys{} keeps track of the frequencies of individual embedding vectors being used.
When the inference session ends (e.g. app being killed) or remain quiescent for a period (e.g. 60s), \sys{} updates the frequencies of the on-disk embedding table with new ones.
Meanwhile, \sys{} also updates their disk locations by sorting respective entries.
The procedure is brief and low-cost, as we will evaluate in XXX...

\paragraph{Buffered embedding read}
Upon new inputs, \sys{} collects all cache misses.
Instead of issuing lookups for each embedding in an adhoc manner, \sys{} buffers them, sorts them by their file offsets, and attempts to merge any adjacent reads.

For instance, individually reads file offset "4096, 0, 8192" may be translated into three discrete 4K block reads by the block layer. 
With the buffer, \sys{} merges them into one large read spanning three contiguous 4K disk blocks, greatly reducing the disk access delay.
\sect{eval} will present more evidence...

\Note{to merge}
\paragraph{A small embedding cache}
\sys{} employs an in-memory cache, which is a smaller embedding lookup table occupying a small portion of the whole embedding table (e.g. 5\%, only tens of KB);
for simplicity, \sys{} uses an LRU policy for cache eviction, which are effective on words embeddings~\cite{embedding-cache}.
The rationale is the power law (zipf law) of word frequency distribution~\cite{groupreduce,recssd,flashembedding}: XX\% of accesses happen to only YY\% of words.

As will be evaluated, the embedding cache absorbs most accesses, effectively reduces the disk accesses by XXX$\times$, leaving spare IO largely untapped...



==> design-mm.tex <==
% !TeX root = main.tex

\section{Managing model memory}


Model memory management in the background for resident model under different system pressure..
Resemble memory balloons in VM: deflate (downgrade) shards when sys memory pressure is high, inflate (upgrade) shards when memory pres. low...


\paragraph{Use cases}
\begin{myitemize}
	\item 
	Who cares? The system, not the user: 1) user is oblivious to resident model; 2) in the background, does not concern current inference (although it will concern \textit{next} inference) because ...  
	
	\item 
	APIs: Retrofit the ideas from balloon driver. Two primitives: inflate (upgrade)/deflate (downgrade), with one argument -- memory constraint, i.e. how much memory does the system expect the resident model to occupy?
\end{myitemize}



==> design-model.tex <==
% !TeX root = main.tex

\subsection{System model}

We target Arm SoCs capable of floating-point operations. 


==> design-overview.tex <==
% !TeX root = main.tex

\section{Design overview}

%
%\Note{Outline} 
%
%\begin{myitemize}
%	\item 
%	System model: what is used during inference...what is assumed... 
%	
%	\item 
%	Workflow: sharding, execution, planning.
%	
%\end{myitemize}

%\subsection{The \sys{} engine}
%\subsection{The architecture}
\subsection{subsection}

 
% Yet, they often demand much less resource. 

%\paragraph{Target hardware}
%It targets commodity mobile SoCs commonly seen on today's smartphones. 
%The NLP inference can run on either CPU or GPU. 
%An SoC has no more than several GBs of DRAM~\cite{marvin-atc20} \xzlNote{better citation} and flash storage with throughput no more than 100 MB/sec~\cite{erofs-atc19}.



%We target on-device inference on a commodity, off-the-shelf mobile SoC, e.g. \cite{odroid-web,rpi3-web,jetson-nano-web}.
%It is equipped with multi-core Cortex-A CPUs~\cite{cortex-a53-web};
%the CPU is capable of floating point operations with typically 1-10 FLOPs~\cite{cortex-flops}.
%It supports DVFS for energy efficiency but will not change its operating frequency during an ongoing inference.
%Optionally, the SoC may have a GPU for accelerating inference~\cite{adreno-driver,mali-vulkan-sdk}.
%%\textbf{Computation may be done CPU or GPU}.
%It has a few GBs of memory~\cite{marvin-atc20} and a few hundred GBs of disk/flash storage with tens of MB/s throughput~\cite{erofs-atc19}.
%We assume Computation and IO resources are fully dedicated to \sys{} during inference.
%\Note{it is worth noting that}: our system does \textit{not} claim to overcome timing jitters originated from underlying OS or drivers. (from DART~\cite{dart}, re-phrase)

 
	% e.g. by receiving a budget from the app or the OS.
 	
% 	We assume the OS to designate a small memory pool sized by $M$ (e.g. as small as 1MB) to \sys{} for hosting the preload buffer. 
% 	The OS may adapt $M$ to system memory pressure as it sees fit.
 	% delegates the management of the memory pool to \sys{} by asking \sys{} , e.g. deflate, inflate. 
 	
 	 
% 	The buffer size is constant. 
 	
% 	The OS provides a working buffer (transient) which is sufficient (i.e. tens of MB) for hosting parameters used in one layer of computation.
 	%containing one layer of full-fidelity \tfm{} layer used during inference.
% 	The buffer is transient and OS is free to reclaim it when inference ends.

 

% \Note{merged}
%\begin{myitemize}
%	\item 
%	Resident memory: used by our model memory management. Long-lived in memory. It stores compressed model skeleton. 10X smaller than a full model (i.e. tens of MBs).
%	
%	\item 
%	Working memory(buffer): large enough to hold 1) one layer of full weights (why not one shard? data too small to exploit data parallelism), 2) decompression costs. Should also be tens of MBs.
%	\begin{myitemize}
%		\item 
%		Working buffer is only used when inference, lasting a few hundred milliseconds. Can be thrown away afterwards. 
%		
%		\item 
%		Though conceptually shards can be computed one by one, bringing the working buffer size to as small as one shard, the performance likely suffers much. This is because one shard is small and has limited data-parallelism; compute on one shard at a time will be significantly slower than compute on a layer of shards. 
%		
%		Mention even for one layer of shards, the data parallelism is limited (hence data parallelism within a shard is even worse). E.g. compute on 1 shard takes 30ms while compute on 12 shards take 100ms.  
%		
%	\end{myitemize}
%	
%\end{myitemize}

%Explain what is a ``resident model'' ... model structure/skeleton... always in-memory...  
%The workflow: foreground planning ... background recycling...



%\subsection{System overview}
%\sys{} incarnates as a planner/executor for the \tfm{} model shards. 

%It features two components:
%reacts to user and OS requests in the foreground and background respectively.

% to revisit
\begin{comment}
\xzlNote{much of the below already covered in intro; consider something different:}
\begin{itemize}
\item who is responsible for sharding,
\item  can sharding be done on device, cost
\item what model(s) can \sys{} work with
\item minimum resource requirement of \sys{}
\item how does \sys{} handle multiple models (one preload buffer? multiple buffers?
\item who sets the deadline T? what if T too long? too short (infeasible?)

We provide a practical range of T... on a low-cost mobile device, it can be as low as 300ms ... on a higher-end one, it may support tens of ms ... 
If too large T  (dont care about ddl..) , one can load model on demand... Our system helps the memory need with preload buffer... our system saves the disk IO, saving energy....

\item too little memory for preload shards? too much memory? (large enough for all shards, compressed? large enough for all shards, decompressed?)

\textbf{When} we will lose benefits... How much memory would render our system useless?  ... Conceptually if one has enough memory to always hold all uncompressed parameter, our system will not have benefits.... Until then, we can always leverage the IO to upgrade some parts of the model to have higher accuracy. 

\item accuracy guarantee? 

By design we do not have the guarantee.... some work (edgebert) has because accuracy guarantee is the part of the system design... 
We cannot have that because the shard configuration is too large... unless we enumerate through every pair... there's no way to tell the accuracy ahead of time... 

\item 
Smart phone is time-sharing... Your system does not guarantee a strict $T$...

\textbf{Admit that T is not strict.}
It is orthogonal (we provide guarantee on this workload, the $T$ is...) 
OS needs provide orthogonal scheduling techniques to ensure, e.g. use PSB to provide execution isolation...  
At least we provide a building block, without our techn ique, previous system cannot achieve .... 

\item 
How does GPU help in our system? Does our system work with GPU?\
GPU accelerates computation but not IO, in fact it exacerbates the skewness... 
Using GPU improves accuracy w.r.t. CPU because computes may be done on a larger submodel given same $T$... 

\end{itemize}
\end{comment}

%\paragraph{How to use}
\subsection{subsection}

 % as the basis for its pipeline planning. 

% it fills the layers with dummy parameters which do not affect the measured delays. 



%Accordingly, \sys{} plans an execution pipeline and preloads model shards. 
%In case the app expects to execute multiple possible models, \sys{} plans separate pipelines with separate preload buffers. 
%The planning happens ahead of the pipeline execution. 

%Prior to deployment on a mobile device, 
%first, it decomposes the model into $n \times m \times k$ via multi-version sharding; 
%second, it measures shard importance via ablation study on a small dev set.
%Due to the pre-processing is a one-time effort, it does so on a separate server. 
%Upon being shipped to the mobile device, \sys{} measures the device's hardware capability and launches a long-running service, which acquires a small preload buffer (e.g. a few MBs) from the OS and preloads it with shards.




%At run time, \sys{} serves inference request under a target latency $T$ specified by user.
%For each $T$ its planner produces an optimal execution plan and sends it to pipeline for execution. %with a shard configuration that maximizes the accuracy

%\Note{merged}
%\paragraph{Resource requirements}
%Since \sys{} plans on a per-device basis, a moderate $T$ on a higher-end device may appear too small on a wimpy one, resulting in a much smaller submodel with poor accuracy.
%\xzlNote{requiring user inputs/involvement as follows may backfire...}
%\Note{revised}
%To avoid such cases, \sys{} sets the minimum $T$ of the device as the execution delay of a $3 \times 3$ submodel which incurs $\sim 15\%$ accuracy degradation than the full one;
%%Upon $T$s below the threshold, \sys{} prompts to user about the possible inaccurate results. %but proceeds with minimum $T$...
%upon any $T$s below the threshold, \sys{} executes with the minimum $T$ instead. %but proceeds with minimum $T$...
%\sys{} does not set a maximum $T$. 
%If $T$ is larger than the full model execution delay, \sys{} still executes the full model but leverages the IO before execution to loads extra high-fidelity shards, or even the full model (e.g. when $T$ is larger than cold start latency).
%%Planner hence produces an optimal shard configuration of the submodel w.r.t. $T$, leveraging measure hardware \& importance...
%%It executes the plan/configuration with preload shards in the pipeline... 
%
%By design, the buffer sized by $M$ contains the shards at first few layers of the submodel to bootstrap inference, allowing IO/computation overlapping to happen at early stages, without stalling the pipeline. %without starving either...
%\Note{Before $M$ is large enough to host all full fidelity shards of the model, our system is beneficial for the inference to achieve maximum accuracy by upgrading shards.}
%Due to high memory pressure, OS may adjust $M$ to be too small (e.g. a few KBs) to host one layer of shards. 
%On such occasions \sys{} incurs compulsory pipeline stall to load missing shards at the first layer; 
%subsequent layers remain unaffected. % (compute starves in the first layers).. Subsequent layers can overlap fine... 
%When $M$ is large, e.g. full layers of shards are preloaded in 6-bit fidelity, \sys{} keeps upgrading them during execution until all reach full 32-bit.
%\xzlNote{still: with what M will our system loses benefits over baselines? promise something?}
%%... IO starves ... it is ok because compute does not and accuracy is maximum...
%%When execution finishes, \sys{} reacts to changing $M$ preserving more (higher-fidelity) shards or downgrading/evicting...
%%\paragraph{}
%
%%Background...OS gives $M$.... deflate/inflate the buffer...
%%\sys{} can also adapt to $M$ changes requested by OS in the background.
%%As $M$ increase, it \textit{inflates} the buffer by preloading more shards. 
%%To do so, it does a dry run of planning and filling the buffer with shards suggested by the planner, also from bottom layers until $M$.
%%%which is the same as when inference ends.
%%When $M$ decreases, it \textit{deflates} the buffer by downgrading or evicting shards from the top layers until $M$ is met.

\subsection{subsection}

%\paragraph{One-shot execution with preload shards}
%\paragraph{One execution per engagement}

%One-shot execution is one of the most common usage patterns of mobile apps~\cite{mobile-usage-sigir20}.

%It delivers the results in high accuracy (XX\%) under $T$ consistently, which cannot be achieved without elastic IO/compute pipelining.

%Among rounds of disconnected one-shot executions, with $M$,  
%pipelining shards allows \sys{} to deliver the results under $T$ consistently, which can not be achieved through existing approach (no pipelining) or even naive pipelining.
%Benefited from the planning, it achieves a decent accuracy, too.
%Clarify: what happen to the preloaded shards after the execution. Will they change? 

%\paragraph{A few back-to-back executions with preloaded shards}
%\paragraph{A few back-to-back executions per engagement}

%Seeing such needs, OS allocates more $M$ between executions, allowing \sys{} to preserve more loaded shards after each execution.

%With same $T$, the increasing $M$ allows \sys{} to distribute more IO on \textit{less} unloaded shards, resulting in higher fidelity per shard and improving the accuracy.
%With same $T$, the increasing $M$ allows \sys{} to concentrate its IO on less unloaded shards but in higher fidelity, which improves the accuracy.
%For instance, when $M$ contains only the first layer's shards, \sys{} must allocate IO to load all remaining 11 layers, each shard having low fidelity.
%When $M$ increases to contain the shards of first six layers, \sys{} allocates the same IO to load the remaining 6 layers, each shard having higher fidelity.
%To echo the intro: each engagement has 2-3 interactions.
%(M unchanged in between executions? M increases in between executions?)


%\paragraph{Cold start with no preloaded shards (M=0)}
%In our design, preloaded shards are scalable to the available memory. 
%In previous scenarios, we show that as low as XXX MBs can eliminate pipeline stalling. 
%An extreme case is when no preloaded shards ($M=0$). 
%In this case, stalling in early stages (bottom layers) is inevitable; 
%however, our key designs (pipeline scheduling via shard selection) is still significantly beneficial, which can launch the pipeline with low-fidelity shards of early stages and load higher-fidelity shards for later. 


\subsection{subsection}
%For the accuracy to be practical, \sys{} sets the minimum $T$ as the execution delay of a $3 \times 3$ model which incurs \~15\% accuracy degradation than the full model.
%The minimum $T$ is set as execution delay of $6\times 3$ submodel which incurs moderate accuracy degradation 10\%...
%The multi-version sharding of \sys{} does not require tedious and time-consuming fine-tuning.
%By design, it works with a pretrained \tfm{} model so long as the model supports adaptive widths and depths, such as~\cite{dynabert,hat}.
%Other transformer-based models....


%On our test hardware (Table~\ref{tab:platform}), \sys{} supports target latencies ranging from 150 ms to several hundred ms, a range known for high user satisfaction~\cite{nlp-delay-study}. 
%Yet, \sys{} do not deliver good accuracy with latency under 100ms -- there is not enough compute bandwidth. 
%However, this is a limit in our test hardware, which will mitigate with faster CPU/GPU. 
%\sys{} can work under more relaxed target latencies, e.g. seconds. However, such latencies cannot ensure good user experience. 
%other low-efficient methods, e.g. load before execution, also diminishes. 
%\sys{}'s advantage over other methods, e.g. load before execution, also diminishes. 


%\Note{it is worth noting that}: our system does \textit{not} claim to overcome timing jitters originated from underlying OS or drivers. (from DART~\cite{dart}, re-phrase)
%	T is not strict because mobile devices are time-sharing.
%	We argue our system is orthogonal to such a challenge... (we provide guarantee on this workload, the $T$ is...) 
%	OS needs provide orthogonal scheduling techniques to ensure, e.g. use PSB to provide execution isolation...  
%	At least we provide a building block, without our techn ique, previous system cannot achieve .... 
%	\Note{may not need this if we use target latency}

%	T is not strict because mobile devices are time-sharing.
%	We argue our system is orthogonal to such a challenge... (we provide guarantee on this workload, the $T$ is...) 
%	OS needs provide orthogonal scheduling techniques to ensure, e.g. use PSB to provide execution isolation...  
%	At least we provide a building block, without our techn ique, previous system cannot achieve .... 
%	\Note{may not need this if we use target latency}


% a key advantage in a multiprogrammed, memory-constrained mobile device. 

%\sys{} works for both CPU and GPU, as \sect{eval} will show. 

%\sys{}'s planner applies to both CPU and GPU.
%Despite we only characterize the IO/computation skewness on CPU in \sect{motiv}, 
%As we will show in \sect{eval}, GPU only reduces computation delay but not IO, exacerbates such skewness, and calls for a greater need for \sys{}.
%GPU accelerates computation but not IO, in fact it exacerbates the skewness... 
%Using GPU improves accuracy w.r.t. CPU because computes may be done on a larger submodel given same $T$... 



% --- below can be in rebuttal --- 

%\begin{myitemize}
%	\item 
%	\textbf{T guarantee.}
%	T is not strict because mobile devices are time-sharing.
%	We argue our system is orthogonal to such a challenge... (we provide guarantee on this workload, the $T$ is...) 
%	OS needs provide orthogonal scheduling techniques to ensure, e.g. use PSB to provide execution isolation...  
%	At least we provide a building block, without our techn ique, previous system cannot achieve .... 
%	\Note{may not need this if we use target latency}
%	
%	\item 
%	\textbf{Accuracy guarantee.} \xzlNote{can go to rebuttal}
%	By design we do not have the guarantee.... some work (edgebert) has because accuracy guarantee is the part of the system design... 
%	We cannot have that because the shard configuration is too large... unless we enumerate through every pair... there's no way to tell the accuracy ahead of time... (except a 2bit baseline) 
%	
%\end{myitemize}

%\textbf{Why NLP}
%The above challenges are specified to NLP but not CV.
%Specifically, CV models have following properties:
%\begin{itemize}
%	\item 
%	Much smaller (tens of MBs). 
%	Can be pinned, even under high memory pressure.
%	Won't affect other apps by swapping out their files.
%	
%	\item 
%	Balanced IO vs computation delays.
%	Layerwise pipelining suffices. 
%	
%	\item 
%	No significant parameter redundancy. 
%	Performance sensitive to compression.
%\end{itemize}


\begin{comment}
\Note{to merge}

\noindent
\circled{1}~\textit{Model sharding (ahead of time).}\Note{model preprocessor?} 
\Note{multi-version sharding}
\sys{} preprocesses the pretrained \tfm{} model by partitioning each of $N$ layer into $M$ vertical slices, called model shards.
With minimum accuracy loss, it compresses each shard into $K$ fidelity versions and stores the $N \times M \times K$ shards on disk.
At run time, \sys{} cherry picks and loads them to compose an executable model.
%They serve as the key building block for the elastic pipeline, which \sys{} overlaps their IO with computation.
%Each model shard contains the model parameters in different precisions, i.e. either the full-precision FP32 or low-bit representations;
%they will be loaded incrementally during inferences..
%Model shards explore the fine-grained tradeoffs between IO vs accuracy. 

\noindent
\circled{2}~\textit{STI planner (at run time)}.
It serves inference requests in deadline $T$. 
Upon receiving one request, it first goes through a 2-stage planning: computation and IO.
%The former decides the maximum dimensions of the submodel $R$ which executes under $T$, based on measured hardware capability.
%The latter selects the optimal shard configurations/combinations for $R$ which achieves maximum accuracy, based on the importance of individual shards and the existing ones in preload buffer.
Based on measured hardware capability and shard importance, the two stages jointly decide an execution plan;
the plan specifies a submodel $R$ and its shard configuration $S$, which maximizes the resource utilization hence the accuracy. 
It then executes the plan in the layerwise pipeline, overlapping the computation on $k$-th layer with shard loading of the $k+1$-th layer.
It leverages the preload buffer to bootstrap inference and uses a transient working buffer to deposit decompressed weights of one layer used in execution. %and executes the plan by layers.
%After the inference finishes, it delivers the results, deallocates the working buffer, and updates preload buffer w.r.t. a memory constraint $M$.
When the inference finishes, it updates preload buffer to fit a memory constraint $M$ by filling the buffer with loaded shards, descending from bottom layers. 
\end{comment}

%where each shard is a vertical slice of the model comprising an attention head plus underlying FFN neurons;
%The system shards a full model, where each shard is a vertical slice of the model comprising an attention head plus underlying FFN neurons;
%it then quantizes the shards into different bitwidths.





%\subsection{Benefits} 
%\xzlNote{Should have been covered in intro already}
%
%\begin{myitemize}
%	\item 
%	\textbf{Maximum accuracy under a given deadline}
%	XXX
%	
%	\item 
%	\textbf{Pipeline-ability (?)}
%	It enables the pipeline construction, such that io and compute can overlap. 
%	E.g. a naive partitioning strategy is by layer. 
%	However the time is bound by io because io is tens of $\times$ larger.  
%	
%	\item 
%	\textbf{Elastic IO.}
%	Model shards (of different bits) translate to different IOs. 
%	Compare with fixed/mixed precision model compression/quantization, this endows the pipeline with flexibility in handling with various deadlines, as well as device heterogeneity. 
%	
%	\item 
%	\textbf{Improvable accuracy with minimum loss.}
%	Compared with full-fledged model, \sys{} maintains a minimum loss (<2\%?), which can be constantly improved through subsequent inferences. 
%	
%%	Search in a hyper-exponential space is costly. 
%%	The heuristic-guided sampling approach offers a tradeoff between accuracy and efficiency...
%	
%	\item 
%	\textbf{Less latency variability}
%	The inference is determined by the deadline chosen by the user and thus has less latency variability caused by frequent pagecache swapping. 
%	
%	\item 
%	\textbf{Lower memory utilization}
%	Compared with the prior cold vs hot dichotomy, \sys{} better leverages the scarce memory resources. 
%	This is because it unifies cold vs hot inference -- previously it is either with (400MB) or without (0MB) the model file in cache, now \sys{} provides a middle ground, e.g. (100MB) during ``warm'' inferences.
%	This is especially helpful when inference invocations are less frequent. 
%	
%\end{myitemize}




\begin{comment}
\begin{myitemize}
	\item 
	\textbf{Task I: Sharding pretrained \tfm{} models without retraining.} 
	We intend to be free of retraining and support \textit{unmodified} pretrained models, for wider applicability and faster deployment. 
	To this end, we first propose a \tfm{}-structure-aware sharding strategy: the system shards the full pretrained model in \textit{attention head} granularity; 
	each shard hence is a vertical slice of a \tfm{} layer, comprising equal-size slices of Q, K, V matrix plus the underlying FFN neurons. 
	We then propose to further compress the shards with an outlier-aware quantization techniques~\cite{transformer-compression,efficient-transformer-survey} to reduce their sizes while maintaining the model performance.
	
	\item 
	\textbf{Task II: Planning shard pipeline for heterogeneous devices.}
	To reduce the latency, we first propose to pipeline the shard loading (IO) with computation on existing shards (Compute).
	This exploits the missed opportunity by existing work, which always executes IO and Compute tasks synchronously and sequentially. 
	Given the deadline, we seek to maximize model performance (e.g. accuracy) while supporting platforms with devices that have diverse IO/Compute speed.
	To this end, we propose a greedy planning algorithm for the system: 
	offline, it first profiles the IO and Compute of \tfm{} shards on the platform; 
	online, it prioritizes the loading of shards with highest possible resolution. 
		
\end{myitemize}
\end{comment}



%The system sets up a deadline for cold start inferences to meet.
%The system shards a full model in attention head granularity; 
%%where each shard is a vertical slice of the model comprising an attention head plus underlying FFN neurons;
%%The system shards a full model, where each shard is a vertical slice of the model comprising an attention head plus underlying FFN neurons;
%it then quantizes the shards into different bitwidths.
%At run time, instead of waiting to load the full model to begin inference, the system starts as soon as a minimal number of shards (typically 3) are loaded. 
%Depending on the deadline and current time budget, it dynamically schedules whether the shard will be loaded and in what bitwidth. 
%To further reduce overhead, it overlaps the shard loading with computation on existing shards. 
%The workflow is shown in Figure~\ref{fig:design:overview}.

%% resident model recycled

%The resident model cannot be used directly for inference, as model shards are compressed.  
%The system decompresses the resident model $R$ into the working buffer for inference, 
%as model shards are quantized w.r.t. different fidelities, whose weights are centroid indexes. 
%To use, the system first forms an empty, ``rectangular'' shaped model $R'$, whose widths and depths are determined by largest $(n,m)$ in $R$.
%The system then decompresses individual $S(n,m,b)$ and fills the decompressed weights into $R'$ in corresponding $(n,m)$.
%To decompress, it simply replaces compressed weights with centroids and patch the outliers. 
%Afterwards, the system then executes normally based on the 32-bit weights restored from centroids and outliers. %in the working buffer, whose execution time is dependent on sentence input lengths, number of shards per layer, and the number of layer. 

%Prior to inference, the system allocates a working buffer which is large enough to host a layer of $M$ full-fidelity shards.
%It decompresses each shard $S(m,n,b)$ in $R$ by projecting centroids onto the weight matrix of the shard, replacing the $b$-bit integers with 32-bit floating points. 
%It then restores the outliers by patching respective indexes of the matrix. 
%The process is efficient and takes a few ms on a 6-core dev board per shard.
%The process is efficient and takes $10\sim20$ ms on a 6-core dev board per 12-shard layer.

%During inference, the system executes normally based on the 32-bit weights restored from centroids and outliers in the working buffer, whose execution time is dependent on sentence input lengths, number of shards per layer, and the number of layer. 
%
%After inference, the system deallocates the working buffer while keeping the resident model in memory.

%Model shards breaks down a large model into fine-grained $K \times M$ grids, where each cell 
%Hence a resident model $R$ is defined as a set of shards: $R=\{S(i,j,b) | \}$

%\xzlNote{move here, to merge}
%\Note{explain why fidelity knob does not affect computation??}
% below obsolete 
%
%\Note{key difference with prior work:}
%
%The key difference to prior work: 
%1) finer-grained, vertical slice. Others -- horizontal slice, e.g. quantization by layer, by component (weight matrix); 
%2) quantization is not ``done deal''. 
%All quantization versions of are stored but only some will be picked and selected at run time.\Note{can be optimized?} 

%% obsolete 
%\begin{myitemize}
%	\item 
%	During one inference, \# of shards is the same across all layers
%	
%	\item 
%	Overlap what? IO of \textit{next} layer and compute of \textit{current} layer
%	
%	\item 
%	What is being computed on? Restored, full-precision weights. 
%	After quantization, shard stores the index to centroids (FP32).
%	\sys{} restore them (with minimal cost).
%	
%%	is our system does not quantize the attention heads uniformly into $n$-bit. 
%%	Instead, each shard may be quantized into different bitwidths; 
%%	the eventual model comprises shards with different precisions.
%
%\end{myitemize}

%\begin{myenumerate}
%	\item 
%
%	\item 
%	\textit{Device profiling \& shard planning.}
%	prior to the very first inference, \sys{} profiles the io and compute capability of the edge device, and generates a profile about it -- how many ms it takes to load a shard (and in what precisions) and compute on them per layer. 
%	Taking the profile, \sys{} searches for shard planning strategies under various practical deadlines (e.g. 50ms - 500ms) by answering the question: given the deadline, what shard configurations (i.e. how many shards will be used during the inference and in what corresponding precisions) achieve best accuracy?
%	
%
%	\item 
%	\textit{Runtime scheduling.}
%	To use, the user sets up a deadline for our system to meet during cold start inferences.
%	Based on the deadline, \sys{} selects a planning strategy generated from stage II.
%	Instead of waiting to load the full model to begin inference, the system starts as soon as the shards at first layer are loaded, and overlap io/compute by \textit{layers}:
%	it overlaps the loading (IO) of \textit{next} shards with compute on already loaded shards in \textit{current} layer. 
%\end{myenumerate}



==> design-sharding.tex <==
% !TeX root = main.tex

\section{Elastic model sharding}
%\section{Managing the model in elastic shards}
%\section{Managing \Tfm{}s in fine elasticity}
%\section{Building an elastic IO/compute pipeline}
\label{sec:design:sharding}


%\textbf{Key points (structured around resident model):}1
%\begin{itemize}
%	\item 
%	Challenge: how to properly select a model shard? Must meet a list of criteria..
%	
%	\item
%	Model shards. Two things: partition by vertical slice (insights, formal definition), quantization technique (rationale, operation)
%	
%	\item
%	Resident model structure: in-memory representation, how to use, 
%	misc: activations (fixed high bits due to small, negligible).
%\end{itemize}


%\xzlNote{moved here, to merge}
%where each shard spans one Transformer attention head and $1/M$ FFN neurons of this layer. 
%For each shard, it creates $K$ fidelity versions, which are lower-bit representations of this shard's weights. 
%For instance, a full-fidelity version that represents each weight with 32 bits, a two-bit version that does so with 2 bits. 
%We therefore store $NxMxK$ shard versions on disk. 
%The preprocessing is a one-time effort per model; being light transformation of an existing model without pre-training, it can be done on device at the model installation time. 
%\Note{Model shards trade inexpensive disk storage for expensive, scarce memory... }


%The preprocessing is a one-time effort per model; 
%lightweight and requiring no model re-retraining, it can be done on mobile devices. 




%\Note{needed?}
\subsection{subsection}
%\Note{merge challenges to below}
%We solve a key challenge in constructing a resident model: how to choose the proper parameter composition of a shard? %(as a smallest tunable unit for resident model)? 
%We solve a key challenge in constructing a resident model: how to instantiate a model shard? %(as a smallest tunable unit for resident model)? 
%We solve a key challenge: how to instantiate an elastic shard? %(as a smallest tunable unit for resident model)? 
 %(as a smallest tunable unit for resident model)? 
%As they are set to enable the engine to manage resident model in fine-granularity: depths, width, and fidelity. \Note{why use multiple fidelity has to be motivated early on}
%As they are 
%Set to enable the elasticity of a model (i.e. depths, widths, fidelity) and management (i.e. IO/computation/memory), they must meet the following criteria: 

%	Can execute partially (with existing shards) and incrementally (with newly loaded shards). %Independent, compatible with each other 
	
	
	%Compression should not require further fine-tuning for fast deployment.
%	must not starve computation. 
%	This is to counter skewed IO delays. 
%	\xzlNote{IO delays must be tunable -- accommodate different hardware}
	
%	\item 
%	Support variable compression ratio, no re-finetuning, minimum accuracy loss. 
%	\xzlNote{overlap with point 2? I can see the point of shard importance}


%To exploit the pipeline parallelism and construct the io/compute pipeline, we face the following two challenges.
%\Note{skewed io/compute: within a model; across diff. devices...}

% obsolete 
%\textit{First, pipelining at what granularity?}
%The key requirement is to allow for partial model execution.
%I.e. the inference may start as soon as the small part of the model is loaded.
%In hindsight, one may partition and pipeline the model by layers. 
%Yet, due to large model size, the \tfm{} models have a highly \textit{skewed} io/compute time\Note{TODO: there are more fundamental reasons for this}.
%For instance, io and compute latency of a layer differs by over 10$\times$ as demonstrated in~\S\ref{sec:motiv:char}.
%The naive layerwise partitioning leads to excessive, large pipeline bubbles and starves the CPU;
%as a result, the pipeline is no different from serial execution, failing the deadline..
%This is demonstrated in Figure \Note{XXX}.

%\textit{Second, how to handle device heterogeneity?}
%\Note{Do not need much exposure...}
%Not only the model itself are skewed in io/compute, edge devices are also known to have diverse hardware\Note{cite}. 
%Due to their different io/compute capability, there is no silver-bullet partitioning strategy given a deadline.
%As shown in \sect{motiv:char}, Rpi3 has much slower io compared with Odroid -- one partitioning strategy may have small pipeline bubbles on the latter but much larger bubbles on the former, starving CPUs.

%The \underline{second} research question is how to compress the shards?
%Broadly, three techniques can be used to compress the shards:
%shards may be pruned and discarded~\cite{cnn-entropy-filter-pruning, cnn-prune-nvidia}; 

%We set to shard \textit{pretrained} language models (e.g. BERT) without retraining. 
%The \underline{first} research question is at 
%To do so, there are two design choices. 
%One is \textit{unstructured} sharding~\cite{gordonCompressingBERTStudying2020,ladabert}, that is, viewing the whole (over 100 million) parameters as a large flat data array and splitting it in trunks. % which is common in network pruning

%they may share weights with each other~\cite{transformer-attention-share,nn-weight-share};
%they may be quantized into a lower bitwidth~\cite{binarybert,ibert,bibert}.
%%Our system must navigate through the compression techniques to ensure that shards 
%Our system must shard a model cautiously, navigate through the compression techniques, and ensure a decent model performance. %shards should work well with each other



\subsection{subsection}
\label{sec:design:sharding:shard}
%For pretrained \tfm{} models, we propose a retraining-free sharding approach, which is a novel combination of width-adaptive \tfm{} and outlier-aware quantization.
%\textbf{structured}, \textbf{outlier-aware quantization} approach for sharding the pretrained \tfm{} model. 
%Our key idea is to shard the model by layers, and by their attention heads.
%\Note{Our key construct is ...}
%In response, our key construct is \textit{model shards}, where we partition the transformer layers into mixed-precision, finer grained pieces.

%To address the challenges, our key idea is to leverage a novel combination of two techniques: dynamic \tfm{}~\cite{dynabert,hat} and dictionary-based quantization~\cite{deep-compression}. 

%compress a dynamic \tfm{} (e.g. DynaBERT~\cite{dynabert}, HAT~\cite{hat}) with Gaussian-outlier-aware simulated quantization~\cite{quantization-survey}.
%To address the challenges, our key insight is to leverage a dynamic \tfm{} with adaptive widths and depths (e.g. DynaBERT~\cite{dynabert}, HAT~\cite{hat}), with Gaussian-outlier-aware simulated quantization~\cite{gobo}.
%Our rationale is dynamic \tfm{} enables partial and incremental model execution because sub\Tfm{}s (\xzlNote{??}) share weights with the super\Tfm{}; 
%Gaussian-based simulated quantization works with pretrained models and incurs little accuracy degradation by accurately approximating parameter distribution~\cite{gobo,deep-compression}.
%We next describe the details.
%\Note{rationale, merge}
%The former enables partial and incremental model execution because sub\Tfm{}s share weights with the super\Tfm{}; 
%the latter works with pretrained models and incurs little accuracy degradation by exploiting parameter redundancy (\S\ref{sec:motiv:primer}).
%\Note{rationale merge}
%We do so because the parameter distribution of a \tfm{} layer is known to resemble Gaussian distribution~\cite{gobo};
%hence we can approximate the majority of values with a few representatives called centroids, while preserving the rest outliers (i.e. outside the Gaussian distribution). 
%The whole process resembles lossy compression and does not require fine tuning..

%We then partition each version into vertical slices by layers, which are model shards. 
%To address the challenges, our key insight is to leverage a dynamic \tfm{} with adaptive widths and depths (e.g. DynaBERT~\cite{dynabert}, HAT~\cite{hat}), and compress it into different fidelity versions using Gaussian-outlier-aware simulated quantization;
%we then partition each version into vertical slices by layers, which are model shards.

%Our rationale are as follows. 
%Dynamic \tfm{} allows for partial model execution;
%the parameter distribution of a \tfm{} layer 
%by approximating it with Gaussian distribution while preserving outliers resembles lossy compression which incurs little accuracy degradation. 

%integrating a novel combination of two known techniques: structured pruning \& outlier-aware quantization. 

%Compared with partitioning by layers, model shards bridges the gap between the skewed io vs compute (XXX vs XXX), allowing for efficient pipeline execution with small bubbles;
%their variable fidelity further enables elastic IO time.  %adapting to various deadlines on heterogeneous devices.
%\Note{merge below}
%% obsolete 
%\paragraph{\textit{Benefits}} are as follows.
%\begin{myitemize}
%	\item 
%	\textit{Partial model execution.}
%	First (cold) inference may start execution on only a few (e.g. 3) shards per layer, while subsequent inferences may incrementally load more.
%	
%	%Our rationale is as follows.
%	%First, an attention head is an atomic structure of the MHA mechanism~\cite{transformer}, which is learned at training time;
%	%shards conforming to the structure preserves the same mechanism.
%	%%shards can work seamlessly with each other. 
%	
%	\item 
%	\textit{Close and elastic IO/compute.}
%	A typical shard contains only one twelve-th parameter as a layer, thus having the same small portion of its IO (e.g. 40ms), approximating the compute time on a shard per layer (e.g. 30ms).
%	Mixed-precisions allow for multiple other devices..
%	
%\end{myitemize}


%\xzlNote{each techniques below shall map back to challenges.}


%\Note{update Figure 5}

%\xzlNote{This this should go before quantization}
%The system then partitions each of $B$ fidelity versions into $M$ vertical slices by $K$ layers (in total $b\times m \times k$ such slices). 
 %(e.g. models from Huggingface~\cite{huggingface)}.
%such models they may be publicly accessible  
%The model must have adaptive widths and depths, that is, at run time it may decide differently how many parameters of a layer to use (i.e. widths), as well as the number of layers (i.e. depths).
%The model must have adaptive widths and depths, that is, at run time it may decide differently how many number of attention heads and FFN neurons of a layer (i.e. widths), as well as the number of layers (i.e. depths) to use.
%The system adopts a pretrained dynamic \tfm{} model as the backbone network,  which is already fine-tuned on a downstream task (e.g. sentiment analysis) to have adaptive widths and depths. 
%That is, it can vary the number of attention heads and FFN neurons of a layer, as well as the number of layers.

 %by total $N$ layers.
 %whose parameters compose a shard.

%as can be seen, the partitioning equally slices the layer 

%Doing so warrants model shards elasticity and the same capability to extract linguistic features from inputs, as done by the attention mechanism: 
%Doing so warrants model shards attending to linguistic features of input tokens: 
%Doing so warrants model shards with same attention mechanism linguistic features : 

%jointly, multiple shards recover full semantic features of inputs.
%A slice/shard $S$ can be uniquely identified by a three-tuple $S=(m,k,b)$, where $m, k$ are the indexes for the slice and layer respectively, and $b$ is its fidelity.
 % and their results can be combined to produce meaningful output.
%\Note{to add: say shard identity is relative to BERT model, e.g. shard at 2nd layer 1st slice...}

%Doing so preserves the language features in the learned structure. \xzlNote{vague, find better rationales from prior work}

\begin{comment}
% below useful...merged 
\xzlNote{Compress the following two paragraphs into a table?}
Following~\cite{dynabert}, we define a shard's weight composition as follows. 
For a \tfm{} layer, 
%it is composed by five key weight matrix $W^Q, W^K, W^V, W^O$ and $FFN$, where
let $d$ denote the hidden state size, $M$ be the total number of attention heads (e.g. $M = 12$), $d_{ff}$ be the number of FFN neurons.
The size of each attention head $d_h$ is given by $d/{M}$, and the neurons of a shard $d_{ff'}$ is given by $d_{ff}/M$.
By equally partitioning the layer, we obtain $M$ vertical slices as model shards, indexed by $[0, M-1]$ from left to right.

The $j$-th shard is hence parameterized by six submatrix: $\{ W_{j}^Q, W_{j}^K, W_{j}^{V}, W_{j}^{O} \} \in \mathbb{R}^{d\times d_h}$ from an attention head, and two from FFN $W_{j}^{FFN1} \in \mathbb{R}^{d_{ff'}\times d},
	 W_{j}^{FFN2} \in \mathbb{R}^{d \times d_{ff'}}$.
The sub-matrix $W_{j}$ are selected by the $j$-th portion from respective $W$ along the non-feature dimension.
For instance, $W_{j}^{Q} = W_{:, j\cdot d_h:j\cdot(d_h+1)}^{Q}$.
Note that the index $j$ explicitly assigns the $j$-th slice of the weight matrix $W$ w.r.t. each shard in an non-overlapping manner.
\end{comment}



%To execute a \tfm{} model using shards, \sys{} first decides a \textit{submodel} of $n$ layers; %$\times$ $m$ shards per layer.
%mandated by the \tfm{} architecture~\cite{transformer}, each layer must have the same width (i.e. number of shards $m$) for an aligned number of output features.
%Although it is possible for a shard to use 0s as placeholder weights, \sys{} expects all $m$ shards to have concrete weights for a good accuracy.
%With $m$ shards, \sys{} computes the attention and FFN output of individual shards using the weight composition in Table~\ref{tab:vertical_slice}, concatenates their outputs, and proceeds to next layer.
%The process therefore preserves the attention mechanism for producing meaningful results.
%For more detailed mathematic formulation, an interested reader may refer to~\cite{16heads,dynabert}.




%The $j$-th model shard at $i$-th layer, $S(i,j)$, is parameterized by:
%%\Note{use a figure}
%
%\begin{equation}
%S(i,j) = \{W_{d_h}^{Q_i}, W_{d_h}^{K}, W_{d_h}^{V}, W_{d_h}^{O}\}\cup\{FFN_{d_h'}\}
%\end{equation}

%\xzlNote{clarify: which subset of a model shards are composable? why partial execution can still give meaningful inference result?}

%\xzlNote{where do we say that in a submodel, each layer must have the same number of shards, and why}

%\xzlNote{much of the following (until the end of S4.3) can go to impl. Important things to mention: what is done at a high level; (typically) how many versions per shard; how are they stored on disk and how large (compression ratio); potential accuracy loss; model accuracy has different sensitivities to individual shards and their bitwidth; mixed precision: shards of different bitwidths can be combined in the same submodel; compute cost of compression/decompression..}
%\Note{this is our novelty. highlight what is ours and what is theirs..}

%We next describe in detail how to quantize them into different precisions (bits).

%gives different fidelity per shard importance for maximizing resource utilization on different devices with diverse IO/compute capabilities. 
%\xzlNote{... and to give different fidelity (compression ratio) per shard importance...}

%of  : fidelity versions reduce their IO by a few $\times$, which can overlap with compute with small bubbles while adapting to .
%The goal is to facilitate elastic IO and amortize IO/compute skewness for maximizing resource utilization: fidelity versions reduce their IO by a few $\times$, which can overlap with compute with small bubbles while adapting to diverse IO/compute capability of different devices.


%The compression is feasible due to high parameter redundancy of \tfm{}, allowing accurate approximation via Gaussian distributions~\cite{tenarybert,gobo}.
%\Note{high level}

%It exploits the Gaussian distribution of \tfm{} weights. 


%\Note{property1: can have high compression ratio, minimum accuracy loss. greatly reduces IO... (no more skewness)}
%how many versions per shard; how are they stored on disk and how large (compression ratio); potential accuracy loss;

\begin{comment}
\Note{may hurt us -- making our design point insignificant}
\textit{Property I: high compression ratios, low accuracy loss.} 
For a K-bit version, the approach compresses a shard by 32/K, as 99.9\% of 32-bit weight are replaced by K-bit dictionary indexes.
For instance, at the lowest bitwidth we target (K=2), the shard is compressed by 16$\times$, whose file size is less than 200KB.
The high compression ratios correct IO/compute skewness and make storing all K versions cheap, e.g. for typically five versions, K=$2\dots6$, it adds only a few hundred MBs. %and is tunable to cater capabilities of diverse devices. 
Meanwhile, the accuracy loss is minimum, incurring less than 1\% accuracy degradation when K=6.
At lower K=2, the accuracy loss may be high, e.g. 10\%, but it can be remedied by \sys{}'s mechanism to load higher-bitwidths shards, which we will describe and evaluate later.
\end{comment}

%\Note{property2: resembles lossy compression. Work smoothly across different fidelity versions}
%model accuracy has different sensitivities to individual shards and their bitwidth;
%mixed precision: shards of different bitwidths can be combined in the same submodel

%\textit{Property II: good compatibility between shard versions.}
%The dictionary compression resembles lossy compression.
 % it satisfies following properties which we seek: 

%1) Its lossy compression nature provides good compatibility between shards of different bitwidths;
%it allows \sys{} to tune the bitwidths of individual shards per their importance and to assemble a submodel with \textit{mixed-bitwidths}.
%allows shards of different versions to work seamlessly with each other, assembling a submodel with \textit{mixed bitwidths}.

%2) It has wide applicability without the need to fine-tune a model or additional hardware support.

%which mixes floating point operations with integer operations~\cite{mixed-precision-cnn-iclr18};

%More importantly, the good compatibility enables \sys{} to tune the bitwidths of individual shards per their importance. 
%\sys{} prioritize important shards which have large impacts on accuracy and allocate higher bitwidths for them, s.t. they may recover the original weight distribution as precisely as possible.
%For less important ones, \sys{} uses lower bitwidths as they do not affect accuracy much.

%\xzlNote{as opposed to XXX techniques. By doing so we avoid tedious per-model retraining as opposed to XXX (is this right?) and ensure to generate adequate compute workloads for high accuracy}
 %(i.e. centroids and outliers).
%To do so, it mass substitutes dictionary indexes with centroids (i.e. floating point numbers) and computes on restored FP32 weights.
%Fortunately, decompression is fast, less than 20ms per layer and can be further alleviated by using a designated accelerator~\cite{gobo}.

%\Note{property3: does not need fine tuning and hardware support}
%\textit{Property III: no fine-tuning nor hardware support required.}
%The quantization approximates the weight distribution of the pretrained model and is oblivious to 
%
%To use, the engine decompresses the shards by simply mass substituting dictionary indexes with centroids (i.e. floating point numbers) and computes on restored FP32 weights;
%the decompression is efficient on a commodity SoC, less than 20ms for one layer.
%%the inference only have floating point operations;
%This differs from a traditional \textit{mixed-precision} network, which mixes floating point operations with integer operations~\Note{cite}.


%We choose it because it incurs little accuracy loss (<1\%) even at $10\times$ compression ratio by accurately approximating \tfm{} weights which follow a Gaussian distribution~\cite{gobo,tenarybert}, and that it is dictionary compression (i.e. simulated), which does not require fine-tuning.
%%We donot use fixed-point quantization~\cite{binarybert,q8bert} because it is less elastic (e.g. fixed 8/4/2bit versions), needs DSP extension which is only seen on microcontrollers (e.g. Cortex-M4~\cite{m4-dsp}), and requires fine-tuning. 
%We donot use fixed-point quantization~\cite{binarybert,q8bert} because it is less elastic (e.g. fixed 8/4/2bit versions), needs DSP extension which is only available on microcontrollers (e.g. Cortex-M4~\cite{m4-dsp}), and requires fine-tuning. 
%Alternatively, a model may be compressed by knowledge distillation~\cite{distilbert} or model pruning~\cite{layerdrop,mobilebert}. 
%However, they also require fine-tuning for \textit{each} version, and they likely lead to severe accuracy degradation as they must remove over 90\% of weights to achieve the same compression ratio as ours.



%
%For minimal accuracy loss, \sys{} uses \textit{simulated quantization}, \Note{reasons for not using real quantziation, i.e. integer operation: require fine-tuning for performance, not friendly to hardware}... 
%It quantizes the full-fledged shards into different lower-bit representations, reducing sizes by up to 16 $\times$. %inspired by a Gaussian-outlier-based quantization technique~\cite{quantization-survey};
%%With model shards as the key building block, \sys{} constructs an elastic pipeline whose IO and compute time is dependent on number of shards and their respective precisions. 
%\Note{Our novelty comp. w/ prior mixed-precision transformer and dynamic transformer:} the first to combine them to achieve elasticity; our goal is not to find a supernet or an optimal mixed-precision net, but to find building blocks. 




%\xzlNote{clarify: impact on IO and compute. why compute remains unaffected. also compare to other compression techniques that reduce both IO and compute (like distillation, transfer learning. why aren't those desirable)}
%Since the vast majority ($99.9\%$) of 32-bit weights are substituted by $b$-bit indexes to centroids, simulated quantization reduces IO by $\lfloor 32/b \rfloor \times$.
%It, however, does not reduce computation delays because the model maintains the same GFLOPS by computing on floating point centroids and outliers. 
\begin{comment}
% --- old, can merge ---
For each layer, the system fits all its weights into a Gaussian distribution, based on which it divides weights into two groups, an outlier group and a Gaussian group;
it preserves the former in full 32-bit fidelity and represents the latter with $2^b$ centroids, which are 32-bit floating point numbers.
%for the latter, it represents them with $2^b$ centroids. 
A weight is deemed as an outlier if the probability of it belongs to the Gaussian distribution is below a configurable threshold;
the larger the threshold, the more full-fidelity outliers, hence the lower compression ratio.  

Following the same practice in~\cite{gobo}, we use $-4$ which is sufficient in maintaining accuracy while maximizing compression ratio;
under the threshold, the outlier group constitute less than $0.1\%$ of total weights. %which is preserved in full precision (i.e. 32-bit). %and incurring only 1\% accuracy degradation. 
For the Gaussian group which constitute the rest $99.9\%$, the system sorts and splits its weights into $2^b$ clusters with equal population;
each cluster has \textit{one} centroid to represent \textit{all} values within it. 
%It then represents \textit{all} values in each cluster with \textit{one} centroid, which is indexed by a $b$-bit integer.
%It then represents \textit{all} values in each cluster with \textit{one} cluster centroid by substituting them with a $b$-bit index to the centroid.
Doing so caters to the weight distribution: weight-concentrated regions deserve higher resolutions, hence having more clusters and centroids.
%the vast majority ($99.9\%$) of original 32-bit weights are represented by $b$-bit integers, reducing model size by $\lfloor 32/b \rfloor \times$.
To decide cluster centroids, prior work adopt K-means based approaches~\cite{deep-compression, zhaoImprovingNeuralNetwork}, which are time-consuming, e.g. it takes a few hours to converge on our server.
Differently, we have found the arithmetic mean of cluster weights suffices -- a 2-bit version takes a few minutes to converge and incurs only 7\% accuracy degradation compared with the full model. 
We will present more results in \sect{eval}.  
%It uses the Gaussian model to find out a group of ``outliers'' parameters and preserve them in full precision.
%For the rest, the system quantizes them into $n$-bit integers (e.g. typically 2 to 4) using \textit{simulated quantization}~\cite{quantization-survey}, where each integer points to a full-precision FP32 value called a centroid, representing a group of original weights.
%The system decides the centroids by dividing the non-outlier parameters into $2^n$ groups and calculating their arithmetic means.

%The rationale is ....
%\Note{quantization rationale..}
%Second, attention head weights are heavily redundant~\cite{16heads}.
%%Most need only a few bits~\cite{ibert,binarybert} while only outliers need high-precision.
%Preserving the few outliers (e.g. 0.01\%~\cite{gobo}) while representing the most others with a small number of values ensures performance.
\end{comment}

%The system repeats the process for each fidelity version and generates a dictionary as the compression metadata, which specifies the centroids and the outlier mapping of full-fidelity weights.

%\Note{how are they stored..}
%\Note{compute cost of compression/decompression..}

%After partitioning, a shard contains $1/M$ of a layer's total parameters, each is a $b$-bit centroid index.

%For instance, (0,0,2) refers to the shard partitioned from the first layer and first slice 
 

%Storing compressed shards is cheap, taking less than 300MB of disk space.

%For a K-bit version, the approach compresses a shard by 32/K, as 99.9\% of 32-bit weight are replaced by  dictionary indexes.
%To generate shards, the system compresses the vertical slices using the dictionaries produced by simulated quantization: 
%for \textit{all} 32-bit parameter, the system looks up the dictionary and uniformly substitutes them with $b$-bit integers, each pointing to one of the $2^b$ centroids.
%It does not preserve the 32-bit outliers in the newly compressed weight matrix to avoid destroying the $b$-bit data alignment.
%It stores the compressed weights as the data and dictionaries (centroids, outliers) as the metadata of model shards on disk.
%This is shown in Figure~\ref{fig:design:shards}. %\xzlNote{Fig 4 needs update, showing the workflow}


%The quantization approximates the weight distribution of the pretrained model using a dictionary and is not specific to network internals. 
%This is because they only change the representations of model parameters but not their amount.
%For instance, by substituting 99.9\% of 32-bit weights with $b$-bit centroid indexes, a shard reduces IO by $\lfloor 32/b \rfloor \times$.
%At inference time, the model retains GFLOPS by computing on the same amount of floating points decompressed from centroids and outliers;
%while being inevitable, the decompression is efficient (10-20ms per layer) and can be further alleviated by designated hardware accelerator~\cite{gobo}.

%In uncompressed, full-fidelity form, their sizes are $1/M$ of a layer (e.g. a few MBs), taking tens of ms to load; 
%in lower fidelities, their IOs are even smaller and elastic w.r.t. bit fidelity. 
%%Hence a model shard equally slices the $j$-th layer it belongs to.
%Note: when in lower fidelities, shards cannot be used directly -- the weights are only indexes. 
%They cannot be used interchangeably, e.g. a 1 in 2-bit and 6-bit shard points to different centroids.  
%For instance, for the 1st layer with 3 shards,  


%Since the vast majority ($99.9\%$) of 32-bit weights can map to centroids, which are indexed by $b$-bit integers, the model size is reduced by $\lfloor 32/b \rfloor \times$.

%Following~\cite{dynabert}, the attention score and output of a layer can be defined as:
%
%\begin{equation}
%	\label{eq:out}
%\end{equation}
%
%Therefore as listed in equation~\ref{eq:out}, the output of a \tfm{} layer can be regarded as the sum of independent model shards, allowing partial execution of the model.

%\paragraph{Storing model shards}
%The system stores all versions of shards and their corresponding centroids on disk. %and pick selectively at run time. 
%Unused ones (e.g. for other tasks) can be further compressed via lossless compression (e.g. Zip). 
%This is possible because of low entropy.
%%Will evaluate its size (smaller than a HD movie) and compression efficiency (>90\%). 
%\Note{why not only store 6bit and derive the others?} 
%Doing so requires to \textit{always} load 6-bit shard IO delays.
%Not elastic, may miss deadline.

%\xzlNote{need cost analysis? }
%At least mention prior work on hardware accelerator


 



==> design.tex <==
% !TeX root = main.tex

%\section{Hypothesis}
%\section{Design overview}

%In this section, we describe in detail the three pillars of \sys{}: word embedding cache, progressive BERT, customized kernel memory management. 

\input{design-overview}
%\input{design-sharding}
%\input{desing-planning}
%\input{design-mm}
%\input{design-embedding}
%\input{design-model}

%\input{design-bert}
%
%\input{design-embedding}
%
%\input{design-mm}


==> desing-planning.tex <==
% !TeX root = main.tex

%\section{The \sys{} engine}
\section{Pipeline planning}

\label{sec:design:planning}
\label{sec:planning}

%\input{fig-planning}


\input{planner-formulation}

\input{planner-engine}

\input{planner-misc}






==> eval-method.tex <==
% !TeX root = main.tex

\subsection{Methodology}
\label{sec:eval:method}

\paragraph{Setup and metrics}
Table~\ref{tab:platform} summarizes our test platforms, which are commodity SoCs.
We choose them to evaluate \sys{} on both CPU and GPU.
%Based on their computation capability (\S\ref{sec:design:planning:compute}), we set up the minimum $T$s for each platform respectively and extend them to cover a practical range usage scenarios.
Based on user satisfaction of NLP inference delays on mobile devices~\cite{nlp-delay-study}, we set T=150, 200, and 400ms. 
Prior work reported that beyond 400ms user satisfaction greatly drops~\cite{nlp-delay-study}.
%On our test hardware (Table~\ref{tab:platform}), \sys{} supports target latencies ranging from 150 ms to several hundred ms, a range known for high user satisfaction~\cite{nlp-delay-study}. 
With T under 100ms, all comparisons including \sys{} show low accuracy -- there is not enough compute bandwidth. 
This is a limit in our test hardware, which shall mitigate on faster CPU/GPU. 

%We set the preload buffer to contain exactly the first layer of shards in 6-bit. \Note{XXX}
%we decide their minimum $T$ .
%\paragraph{Benchmarks}
Table~\ref{tab:benchmarks} summarizes our benchmarks and metrics. 
We diversify them to include each category of GLUE benchmarks~\cite{glue-benchmark}, which span a broad range of NLP use cases on mobile devices. 

\input{tab_benchmarks}

\paragraph{Comparisons} 
We consider two NLP models. 
(1) DistilBERT~\cite{distilbert}, the outcome of knowledge distillation from BERT. 
Due to its high popularity on mobile, we use its accuracy as our references and call it \textit{gold accuracy}.
Yet, DistilBERT has fixed depths/widths (6 layers x 12 heads) and thus cannot adapt to different target latencies. 
(2) DynaBERT~\cite{dynabert}, which is derived from BERT (12 layers x 12 heads), allowing execution of a submodel to meet the target latency. 

Based on DynaBERT, we design the following competitive baselines as summarized in Table~\ref{tab:baselines}. 
%Our main focus is the latter, which has same accuracy as BERT~\cite{bert} but has adaptive widths/depths; 
%it allows us to apply \sys{} compute planning to it for configuring the largest submodel under $T$.
%To make baselines more competitive, we further quantize DynaBERT to reduce its IO.
%\Note{``gold'' accuracy of distilbert is confusing... should we compare with it at all?? it can be done on Jetson within 400ms..}
\input{tab-baselines}

%We consider execution paradigms in \S\ref{sec:motiv:char}. %as baselines . 

\begin{myitemize}
	\item \textit{Load\&Exec}: 
%	the default approach of many inference engines. 
	It loads model as a whole and executes it.	
	% so the total execution time is closest to the target latency. 
	It chooses the best submodel so the sum of IO and execution delays is closest to the target latency, using the algorithm described in Section~\ref{sec:design:planning:compute}. 
	Model parameters are not quantized (32 bits). 

%	The engine can only start execution until the whole model is loaded. %then executes it. 
	
	\item \textit{Standard pipelining (StdPL-X)}: 
	It executes a layerwise pipeline, overlapping IO and computation. 
	It chooses the best submodel so that the total pipeline delay stays under the target latency. 
	We further augment it with quantization. 
%	\textit{X} refers to the parameter bitwidth: full (no quantization, 32 bit), 2bit, 6bit. 
	All parameters in a model have the same \bt{} X.
	
	
	\item \textit{PreloadModel-X}: 
%	it eliminates IO completely by keeping the model of \textit{X} fidelity always in memory.
%	The engine hence starts execution as soon as possible without any delay.
%	Similarly, we also use \textit{X} to denote the model fidelity.
	The whole model is already in memory and no IO is required. 
	It chooses the best submodel so that the total computation delay stays under the target latency. 
	We augment it with quantization;
	all parameters have the same \bt{} X.
%	Similarly, \textit{X} refers to parameter bitwidth.
\end{myitemize}


We choose X=6 as the highest quantization \bt{}, as further increasing the \bt{} has little accuracy improvement. % but stalls the baseline pipelines.
%
%\xzlNote{explain baseline names...}
%
%\xzlNote{SOTA accuracies ... gold accuracies ... diff?}
%
%\xzlNote{Why do we consider DistilBERT accuracy gold?}

\begin{comment}
% merged
\begin{myitemize}
	\item 
	\textbf{Setup:}
	\begin{itemize}
		\item 
		Framework: PyTorch
		\item 
		Dev: Odroid 
		\item 
		Models: DynaBert \xzlNote{careful. possible q: why not bert, why not distilbert}
		\item
		Benchmarks: GLEU
	\end{itemize}
	
	% 	\item
	% 	\textbf{Research questions:}
	% 	\begin{itemize}
	% 		\item 
	% 		Deadline to accuracy (Cold start scenario). Fix deadline for each figure, show different benchmarks in one figure.
	
	% 		\item 
	% 		Vary M, fix T. You have some thing in the memory, 20\%, 50\% of model in memory, etc. 
	
	% 		\item 
	% 		Background memory management task, given a memory load, measure next time inference accuracy. 
	
	% 	\end{itemize}
	
	% 	\item
	% 	\textbf{Benchmarks:}
	% 	\begin{itemize}
	% 		\item 
	% 		Major: $T$ to accuracy, $M$ to accuracy. Expected: ours have highest accuracy.
	
	% 		\item
	% 		Implication of embedding cache
	
	% 		\item 
	% 		Minor: cost of operation, e.g. file size, IO throughput.. 
	% 	\end{itemize}
	
	\item 
	\textbf{Comparisons:}
	\begin{itemize}
		\item 
		Vanilla \xzlNote{load before exec, all in mem}: existing model as-is. No dynamism, no pipelining, no compression. Total: 440MB. IO: 3s. Compute: 120ms.
\textbf{		These should not have preload buffer}
			\begin{itemize}
			\item distilbert
			\item dynabert
			\item dynabert + full model quant
			\end{itemize}
			
			with load delay, without load delay (assuming resident in memory)
		
		\item 
		Naive pipelining + adaptive width/depths (NPP): layerwise pipelining. 
		\Note{this is actually a strong baseline}
		\textbf{These should not have preload buffer}
		Sub-versions:
		\begin{itemize}
			\item 
			\textbf{NPP-base}: unquantized, each layer 40MB, total 440MB.
			\item 
			\textbf{NPP-quant}: fixed 2-bit fidelity version for all layers. Each layer 4MB, total 40MB.
			\xzlNote{use whatever quant that fits in given preload buffer}
		\end{itemize}
		
		\item 
		Ours: elastic pipelining. \xzlNote{useful but less important as above}
		Sub-versions:
		\begin{itemize}
			\item 
			\textbf{V1 (optimal)}: depths > widths, importance
		    Have $M$ attached... E.g. Ours-10M
			\item 
			V2: widths > depths, importance
			\item 
			V3: depths > widths, random			
		\end{itemize}
	\end{itemize}
\end{myitemize}

\paragraph{Benchmark design}
\begin{myitemize}
	\item
	\textbf{Major results}: \sys{} accu. compared with others by fixing $T$ and $M$ respectively.
	\begin{itemize}
		\item 
		Accu under different $T=300ms, 600ms, 900ms, 1200ms$, with a fixed $M$, $M=30MB$.
		Expected results:
		\begin{itemize}
			\item 
			\textbf{Vanilla:} no dynamism, cannot be planned.
			Load (400 - $M$) model, then execute. IO takes >2s, failing all deadlines. Optimal accuracy.
			
			\item 
			\textbf{NPP-base:} depths \& widths decided by compute planning dominated by IO, hence smaller depths \& widths as ours under same $T$. \Note{a strong baseline}
			Example: $300ms$ = 6 x 2. (ours would be 6x3).  
			IO overlaps with computation, but computation is starving. 
			Inferior accu. than us.
			
			\item 
			\textbf{NPP-quant:} compute can dominate to decide widths/depths, but leaving IO starving. 
			Same n,d with us under same $T$. 
			Fixed, low-fidelity, worse than ours.
			  
			\item 
			\textbf{Ours-v1:} Can meet ddl with optimal accu.  
			  
			\item 
			\textbf{Ours-v2:} inferior accu. due to wrong heuristics.
			
			\item 
			\textbf{Ours-v3:} inferior than v1 due to wrong heuristics.
			
		\end{itemize}

		
		\item 
		Accu. under different $M=10MB, 20MB, 30MB$, setting deadline to fixed $T=600ms$.
		Expected results:
		\begin{itemize}
			\item 
			\textbf{Vanilla:} Unable to deliver meaningful results.
			
			\item 
			\textbf{NPP-base:} $M$ can hold 1-2 extra layers. Still smaller depths \& widths than us. 
			IO overlaps with computation, but computation is starving. 
			Accuracy unchanged, and is inferior.
			
			
			\item 
			\textbf{NPP-quant:} compute can dominate IO to decide widths/depths, but with larger $M$, IO starves more. 
			Same n,d with us under same $T$. 
			Fixed, low-fidelity, worse than ours.
			Accuracy unchanged, and is inferior.
			
			\item 
			\textbf{Ours-v1:} Can meet ddl with optimal accu. 
			Accuracy increases. 
			
			\item 
			\textbf{Ours-v2:} inferior accu. due to wrong heuristics.
			Accuracy increases subtly...
			
			\item 
			\textbf{Ours-v3:} inferior than v1 due to wrong heuristics.
		\end{itemize}
	\end{itemize}
\end{myitemize}
\end{comment}


==> eval-prelim.tex <==
%\paragraph{\textit{Preliminary results}}
%We have done preliminary experiments on the pretrained model from DynaBERT~\cite{dynabert}. 
%Figure~\ref{fig:prelim:sharding} validates the importance of outliers with SST-2 frrom GLUE benchmark~\cite{glue-benchmark}, a dual-class sentiment classification task. %to evaluate the model performance of the proposed sharding strategy.
%It shows our proposed quantization technique achieve near original model performance (less than 1\% degradation when quantized into 4 bits) while without outliers the quantized model performance drops to 50\% (i.e. random guess).
%Figure~\ref{fig:prelim:others} shows the proposed quantization technique also achieves decent performance in two other tasks (less than 1\% degradation when quantized into 5 bits), STS-B and MNLI in GLUE~\cite{glue-benchmark}.
%Figure~\ref{fig:prelim:heads} shows the attention-head granularity achieves a decent performance and scales with number of heads, as expected.
%
%
%\paragraph{\textit{Preliminary results}}
%Our principle is based on measured per-layer outlier distribution of pretrained DynaBERT model.
%As shown in Figure~\ref{fig:prelim:weight}, top layers have more outliers thus calling for higher precision.
%We have also characterized the IO and Compute time of BERT~\cite{bert} on an Odroid dev board~\cite{odroid-web} as a sample IO/Compute profile, shown in Figure~\ref{fig:prelim:load}.
%We have also profiled the per-component inference latency of BERT on an x86 machine for convenience, shown in Figure~\ref{fig:prelim:breakdown}. 
%These preliminary results suggest a sublinear increase in Compute time as the number of attention heads (i.e. the sharding granularity) increase.
%They will be as a key heuristic in planning the shard pipeline.
%
%\input{fig-prelim-planning}

==> eval.tex <==
% !TeX root = main.tex
\vspace{2em}
\section{Evaluation}
\label{sec:eval}
%We evaluate \sys{} to address the following questions:



%\Note{Wonkyo's. To merge}
%\begin{myitemize}
%	\item Can \sys{} achieve a comparable accuracy given a deadline (T) compared to other models? \xzlNote{same deadline, same/lower mem usage ... higher accuracy ... }(\S\ref{sec:eval:deadline})
%	\item How much accuracy can \sys{} maximize with preloaded model (M)? (\S\ref{sec:eval:memory})
%	\item Does the resident model significantly reduce a latency for the next inference? 
%	\item Does the Planner effectively schedule compute and IO tasks within the deadline?
%	\item Misc. 
%	\begin{itemize}
%	    \item Background memory management task, given a memory load, measure next time inference accuracy.
%	    \item Implication of embedding cache
%	\end{itemize}
%\end{myitemize}



%\input{eval-method}

%\subsection{Accuracy under constrained $T$s}
%\subsection{Accuracy}
%\input{tab-eval-odroid-acc}
%\subsection{End-to-End Results}
\label{sec:eval:deadline}
%\input{fig-major-deadline}

%\Note{high-lvl messages: 1) ours achieves maximum (oracle) accuracy. 2) ours > vanilla. Due to reduced IO (larger submodel) \& higher-fidel shards. 3) ours > NPP-2/6 because it eliminates IO starvation. Odroid has same perf. as NPP-6 because NPP-6 happens to overlap with computation}
%\paragraph{Accuracy}
%.. within target latency ...

%\xzlNote{fig 8 should be discussed before table 4}

%\Note{first impression: gold accuracy with 1/5MB memory.}

%With T=400ms, the average accuracy is  2.12 percentage point (pp) higher (Odroid) and 0.8 pp lower (Jetson) across benchmarks. 

%\Note{compare with two \textbf{categories} of baselines, using average number of all in each category}

%\Note{detailed of view, compare with each baseline}
%Figure~\ref{fig:eval:memory} zooms in the detailed view of accuracy vs memory under T=200ms of SST and QQP benchmarks. %on our platforms. 
41$\times$ smaller memory to achieve the same accuracy.
%Similarly, \sys{} accuracy on Jetson holds 3$\times$ smaller memory than \textit{PreloadModel-6bit} with only 0.6\% less accuracy as shown in Figure~\ref{fig:eval:memory}(b).
%the memory saving is smaller than when T=400ms because \textit{PreloadModel} employs a smaller submodel. 

%\xzlNote{what's the takeaway message?}
%\Note{Comp. w/ average accu. of each baseline of all Ts; highlight comparison w/ StdPL\& load\&exec which overturns the usability, i.e. from not usable to useful}

%\xzlNote{we compare accuracies under a given latency}
%On average, \sys{} (Ours, 1MB/5MB) increases accuracy by 27.15 percent point compared with \textit{Load\&Exec}, 27.15 point than \textit{StdPL-full}, 22 point than \textit{StdPL-2bit}, and 0.2 point than \textit{StdPL-6bit} \Note{across all benchmarks..}; %while maintaining a gold accuracy;
%On average, \sys{} (Ours) increases accuracy by 27.15 percent point compared with \textit{Load\&Exec} and \textit{StdPL-full} which share same small submodel size due to IO skewness. 

%It is 22 points better than \textit{StdPL-2bit}, and 0.2 points better than \textit{StdPL-6bit} \Note{across all benchmarks..}; %while maintaining a gold accuracy;

%or even slightly better accuracy than the gold accuracy.
%Among them, \textit{PreloadModel-full} has the \textit{gold} accuracy because it preloads all shards in full fidelity and has a largest submodel size.
 %having 51\% accu. similar to random guess. 
%With sys{}, the accuracy increases by XXX and inference results become useful.\Note{XXX less than gold??}


%\sys{} has less accuracy improvement than \textit{StdPL-6bit} because as the submodel reaches 6-bit fidelity, the accuracy is close to gold accuracy, e.g. \textit{PreloadModel-full} and \textit{PreloadModel-6bit} accuracies are similar.

%The accuracy is gold because it has all model preloaded in full fidelity.
%For all benchmarks, \sys{} achieves their SOTA accuracies (listed in Table~\ref{tab:benchmarks}) at T=400ms, a highly satisfying delay to the user~\cite{nlp-delay-study};
%on Jetson, it incurs 2\% accuracy loss on QNLI and QQP, which is considered negligible in NLP inference tasks\Note{cite}.
%Given each target T, it achieves the maximum accuracy, i.e. Oracle-Dyna. 
%\xzlNote{mention why such latency and accuracy are usable}

%\xzlNote{Now compare to baselines. Re-organize by take-aways}

%Compared with \textit{Load\&Exec} and \textit{StdPL-full}, our accuracies are \Note{XX} and \Note{YY} percent point better on Odroid and Jetson, respectively. %than vanilla and NPP, both uncompressed. 
%This is because we reduce IO (i.e. via quantization), avoid starving compute, and allow the pipeline to compute on the largest possible submodel.
%avoid compute starvation by shifts the resource from IO to computation, ...

%\xzlNote{this is a minor point}
%Despite running on a GPU, \sys{} on Jetson has an inferior accuracy than on Odroid.
%This is likely due to submodels on Jetson have a shallower submodel, which we will explain shortly. 
%\Note{don't need to compare with ourselves}

%\Note{discuss jetson ... }
%We are better at 2-bit because NPP starves IO (while we consumes all IO for upgrading shards, etc.).
%We are similar at 6-bit because on Odroid, when quantized to 6bits, its IO happen to overlap well with Computation, which does not starve either IO or computation (same as ours).
%\Note{why lots of accu. are the same:} this is because they have same submodel and shard configuration (e.g. full or same fidelity everywhere).
%\Note{CoLa T=600ms} suspect a glitch in the pretrained model...

% obsolete 
%One of our major goals is to reach the maximum accuracy under a given deadline. We conduct accuracy experiments on different versions of \sys{} by setting a deadline from the lowest to the highest considering an average response time of IPA on mobile systems. Figure~\ref{fig:eval:deadline} shows a result for this. \wk{What is the minimum deadline that baseline can be tested?}
%
%The complete version of \sys{} has X\% amount increase of accuracy compared from DynaBERT.

%\subsection{Memory consumptions}
%\label{sec:eval:memory}
%We have conducted an experiment to observe how much preloaded shards affect accuracy. As shown in Figure~\ref{fig:eval:memory}, the small amount of loaded shards shows a low accuracy and the large amount of loaded shards have a sub-optimal accuracy under the fixed deadline.
%
%\paragraph{Compared to other models} We compared ours with recent models Table~\ref{tab:major:memory}.

%\Note{key msg: our sys achieves same lvl of accuracy while using 2 orders of magnitude memory.}

%\Note{high level, directly say} 
%\Note{the message is we don't scale, so highlight the maximum (up to XXX..). And show the linear scaling, e.g. T from 200 to 400, baseline sizes increase by 2X..}

%More importantly, our memory consumption with number of models, unlike baselines which scale with both \textit{number of models} and \textit{T} linearly.
% This is because in order to scale with T at runtime, baselines need to preload the whole 12x12 model in memory.

%as T gets larger, the submodel also gets larger, to fit which they must also scale their memory correspondingly.
%For instance, when from T=150ms to 200ms, model sizes increase by XX$\times$ (Odroid:XX$\times$, Jetson: YY$\times$), from 200ms to 400ms, it increases by XXX.
 % and by exploiting IO/computation parallelism to adapt Ts.
%at minimum, our memory consumption only scales with number of models. 
% With \sys{}, the OS only need in total a few MBs for hosting all models, whereas baselines require a few hundred MBs or even GBs for them. 

%For instance, on Jetson at T=200ms, \textit{PrealodModel-full} and \textit{PreloadModel-6bit} consumes as much as 85MB and 17MB.
%Yet when T=400ms, their memory consumption bumps to 198MB and 40MB. 
%In comparison, OS only allocates 1 and 5MB of memory to \sys{} on Odroid and Jetson respectively throughout Ts.
%at minimum, our memory consumption only scales with number of models. 
%Therefore with \sys{}, the OS only need in total a few MBs for hosting all models, whereas baselines require a few hundred MBs or even GBs for them. 
%scale with 
%achieve the same accuracy while using  lesser memory.
%even for their quantized versions (\textit{PreloadModel-6bit}), we still reduces memory consumption by 8-14$\times$.

%The small preload memory of \sys{} effectively improves accuracy and saves memory.
%Through all benchmarks and target latencies, \sys{} only requires 1MB and 5MB of preload memory on Odroid and Jetson, respectively. \xzlNote{only requires? we said the size is elastic to OS allocation}
%Their sizes are just enough to host 6-bit shards for the first layer; 
%Jetson has larger memory size due to a wider submodel.
%effectively improves accuracy and saves memory.
%Compared with \textit{Load\&Exec.} and \textit{StdPL} which loads model on demand (i.e. zero preload memory), we achieve XX\% better accuracy with only 1.2MB of preload memory on Odroid;
%the improvement is drastic and overturns the usability, e.g. QQP sees the greatest $45.9\to81.3$ improvement under T=200ms on Odroid.
%which is significant in NLP inference tasks.



%The reason for preload buffer being effective at such small size is, it only needs to contains the minimum number of shards of the first layer (i.e. 3-12, each of a few hundred KB) to bootstrap the inference 
%while they must keep all layers in memory.

%\paragraph{Preprocessing costs}
%\xzlNote{can be really brief}
%\Note{storage and energy}

%It effectively reduces IO by 5-16$\times$. 
%reduces the model sizes, making storing all versions cheap. 
 


% ---- useful but verbose --- 
\begin{comment}
Table~\ref{tab:eval:shard-size} shows details of SST-2. %the compression ratios of SST-2 model in different versions;
other models have similar sizes due to their compression ratios close to SST-2's.
Since storage space is getting larger and cheaper\Note{cite}, it is inexpensive to store multiple models, e.g. a few GBs, about the same size of a HD movie.
%pre-processing each version takes only 2-3 minutes on our server. 
%The high compression ratios are due to small number of outliers (i.e. 0.14-0.17\%). 
%other models show similar compression ratios as they also have small number of outliers, i.e. CoLa/RTE has 0.14\% outliers and QQP has 0.17\%.
\end{comment}

%For fair comparison of energy consumption, we consider 

\input{fig-major-memory}

%Compared with baselines, 
%we do not expect \sys{} to incur a major increase in energy consumption under the same accuracy. %despite it maximizes IO/compute utilization. 
%The reasons are twofold.
%First, to achieve same accuracy (on the same platform) we should have similar GFLOPs (i.e. submodel size) hence a comparable active compute time, which is a major energy contributor on mobile SoCs~\Note{cite}.
%Second, IO costs adds only marginally. 
%%Compared with \textit{Load\&Exec} and \textit{StdPL-full}, we have a much smaller IO time. 
%Despite our IO time is larger (i.e. by consuming all AIBs), the impact is likely marginally because when active inference is going on, the devices are all in high power states without power state transitions, which are the least energy efficient process of an IO device~\cite{transkernel}.

%loading on demand (\textit{Load\&Exec}, \textit{StdPL}), we have similar \textit{active} IO and compute time, while their idling time is much longer (e.g. 3.1s as shown in \sect{motiv:char}), which likely costs more total energy than us.   
%Second, compared with \textit{PreloadModel}, we have similar active compute time but extra IO time (i.e. loading shards during execution). 


%\input{tab-shards-size}
%\input{fig-memory-consumption}


%\input{tab-network-confs}


%\subsection{Preprocessing costs}
\label{sec:eval:micro}

%\begin{myitemize}
%	\item 
%	Bits vs accuracy? \Note{bits 4, 5 may start getting strong}
%\end{myitemize}

%\xzlNote{how about using same submodel, but with random choice of shards??}

%\Note{If a single 32-bit shard can improve accu. from 50\% to 70\% why need more?}
%This is only done on a dev set... in actual deployment... may see more inputs which require ... 


%\Note{concise .. talk about submodel size, with baselines present fig9 as a case study...}

% lays the GFLOPs foundation for accuracy.
%\xzlNote{takeaway messages? we can adjust the submodel to target latency? we can compute larger(?) submodels vs. baselines??}
 % which translate to high accuracy. 
 %used in our benchmarks. %after \sys{}'s compute planning (\S\ref{sec:design:planning:compute}), which dynamically adjust them w.r.t. Ts. 
%Under all Ts, our submodels are consistently the largest (i.e. achieving maximum GFLOPs), same as \textit{PreloadModel} which has eliminated IO. 

%\xzlNote{the following complicated. paraphrase?} depending on the proportion of first layer IO in T. 
%Depending on the proportion of first layer IO in T, \textit{NaivePL-2bit} and \textit{NaivePL-6bit} may have similar sizes with us but cannot surpass us, despite quantization reduces their IO.
%On average, ours GFLOPs are XX\% higher than \textit{Load\&Exec} and \textit{NaivePL}, whose execution is still dominated by IO.
%With reduced IO, \textit{NaivePL-2bit} and \textit{NaivePL-6bit} have similar submodel sizes with ours on Odroid.
%\textit{NaivePL-2bit} and \textit{NaivePL-6bit} also have reduced IO and have similar sizes with us.


%Figure~\ref{fig:submodel} shows the actual submodel used by us on Odroid in SST-2 benchmark when T=200ms.
%As can be seen, ours has one extra layer (i.e. 5x3 vs 4x3) and higher fidelity shards, which contribute to nearly 10 percent point higher accuracy. 


% and thus has poor efficiency 

%the data parallelism per \tfm{} layer during a single execution is too small to exploit GPU hardware, which is optimized for throughput.

%Interestingly, all Jetson submodels are wider and shallower compared with Odroid, most having full 12-shard layers. 
%This is because from \sys{}'s profiling (which we also confirm), the GPU execution does not scale w.r.t. total number of shards per layer\xzlNote{lack of proportionality...}.
%For instance, executing a 12-shard layer vs 3-shard layer only differs by less than one second (56.6ms vs 56.2ms).
%As a result, \sys{} always chooses the 12 shards as layer widths and results in rather ``flat'' submodels. 
%We suspect the data parallelism per \tfm{} layer during a single execution is too small to exploit GPU hardware, which is optimized for throughput.
%

%\xzlNote{can be part of results -- test if our system can dynamically pick submodel}
%
%\xzlNote{Define: Gold accuracy}
%
%\xzlNote{have an ex submodel. widthi, depth, bitwidth, which shards are preloaded...}



%The size is around half the size of the pretrained model (418MB) and is much smaller than a HD movie (a few GBs).
%Note that the outliers are the same for each fidelity version because we use the same log probability to detect them. 
%\xzlNote{not useful to highlight efficacy of model compression. useful to state our storage overhead}



\begin{comment}
Compared to on demand model loading
\xzlNote{state: one bitwidth knob for all shards is too rigid -- pipeline bubbles. either compute starvation (StdPL-full) or IO starvation (StdPL...). Q: how about anything between 6b and 32b??}
boosts accuracy by eliminating IO starvation when the submodel has yet to reach the full fidelity. 
Compared with \textit{StdPL-2bit} and \textit{StdPL-6bit}, ours are XX-YY and XX-YY percent point better on Odroid and Jetson respectively.
This is because once they load fixed-precision 2/6-bit layers, their IO sits idle, while \sys{} keeps pulling as many 32-bit shards as possible, consuming up the remaining AIBs and further increasing the fidelity of submodel.
\Note{numbers weak}
\end{comment}

%with reduced IO, ours are \Note{XX-YY} (on average, Odroid:XXX, Jetson: YYY) and \Note{XX-YY} (on average Odroid: XXX, Jetson: YYY) points better than \textit{StdPL-2bit}, \textit{StdPL-6bit} respectively.
%The reason is \sys{} eliminates IO starvation by consuming AIBs (\S\ref{sec:design:planning:io}) to upgrade as many shards as possible, whereas the baselines let 




% improves accuracy \textit{as fast as possible} by ensuring AIBs collected from the elastic pipeline and preload buffer are spent on the most important shards.

%\paragraph{Shard importance-aware selection} improves accuracy \textit{as fast as possible} by ensuring AIBs collected from the elastic pipeline and preload buffer are spent on the most important shards.
%When compute capability out paces IO, the pipeline can only upgrade some but not all shards to a uniformly higher fidelity. 
%Hence it is important to choose judiciously \textit{which} to upgrade to boost the accuracy as much as possible.
%\xzlNote{what do the following two sentences mean}
%\sys{}'s strategy to upgrade shards based on their importance boosts accuracy \textit{as fast as possible} when upgrading the submodel from a lower fidelity to a higher one. %\textit{the shortest path to a higher accuracy}. %between a lower fidelity version and a higher one.
%When the model cannot afford to 
%It helps when compute capability out paces IO, the pipeline can only upgrade some but not all shards to a uniformly higher fidelity. 
%This is because both of our platforms can load full 6-bit submodel during execution, where the benefits of upgrading to 32-bit shards are non-obvious.


%\textbf{Case study: a 5x3 2-bit submodel.}




\begin{comment}
\textbf{Case study: a 5x3 2-bit submodel.}
We demonstrate the efficacy through a differential analysis. 
To validate, we adopt a 5x3 submodel with all 2-bit shards and upgrade them to 6-bit.
This is because both of our platforms can load full 6-bit submodel during execution, where the benefits of upgrading to 32-bit shards are non-obvious.
To do so, we adjust the IO/compute ratio of Odroid s.t. it may only load a 5x3 2-bit submodel during execution and with bonus IO by preload buffer, it may load extra 6-bit shards. %which we control the size.
%\sys{}'s AIBs only supports to upgrade partial shards but not all.
%\Note{we throttle IO s.t. it can only upgrade some shards to 6bits and vary the preload memory size..}
We gradually increase the preload buffer size to let \sys{} select and load more 6-bit shards. %show the resultant accuracies in 
Table~\ref{tab:eval:shard-selection} on each benchmark. %by varying the number of upgraded shards at each time.
%We use it because 
Compared with random shard selection, our results show much faster convergence towards the accuracy of a full 6-bit model;
at each buffer size, ours are better by 1.7-23.1 percent point.
%\xzlNote{No need to mention} Interestingly in RTE, the accuracies of upgrading 5 and 10 shards are even better than the target accuracies when all 15 shards are in 6 bits.
%This is likely caused by a \Note{XXX what} glitch due to quantization. 
\end{comment}

%\input{tab-shard-selection}

%\xzlNote{what are ``upgraded 1 5 10''?}
%\xzlNote{``upgrade''/``downgrade'' undefined}



%\begin{myitemize}
%	\item 
%	Example results shown in Figure~\ref{fig:eval:importance}.
%	Importance parity exists for individual models... 
%	
%	\item 
%	Time: each model 12x12 iterations.. Depending on size of dev set, each iteration takes a tens of seconds to a few minutes, on a GPU server.
%	
%	\item 
%	Accu. results: w/o shard importance (upgrading randomly).. The accuracy cannot achieve maximum... Sometimes hurt accu.
%\end{myitemize}

%\subsection{Effectiveness of resident model for avoiding cold inference}
%\label{sec:eval:cold}
%[Latency vs. loaded resident model]. This is related to managing model memory.
%
%\subsection{Effectiveness of the Planner scheduler?}
%\label{sec:eval:scheduler}



%\begin{table*}[ht!]
%\begin{tabular}{cccccccccc}
%	\hline
%	System &  \textbf{Memory usage} & MNLI-(m/mm) & QQP & QNLI & SST-2 & CoLA & STS-B & MRPC & RTE \\
%	\hline
%	BERT-base~\cite{bert} & 440MB & 80 / 80 & 80 & 80 & 80 & 80 & 80 & 80 & 80 \\
%	DistilBERT~\cite{distilbert}& 100MB? & 80 / 80 & 80 & 80 & 80 & 80 & 80 & 80 & 80 \\
%	DynaBERT~\cite{dynabert} & 440MB & 80 / 80 & 80 & 80 & 80 & 80 & 80 & 80 & 80 \\
%	Ours-v1-10MB & 10MB & 80 / 80 & 80 & 80 & 80 & 80 & 80 & 80 & 80 \\
%	Ours-v1-30MB & 30MB & 80 / 80 & 80 & 80 & 80 & 80 & 80 & 80 & 80 \\
%	\hline
%\end{tabular}
%\caption{\label{tab:major:memory} Comparison with other models}
%\vspace{-0.5cm}
%\end{table*}

\label{sec:eval:sensitivity}
%\sys{}'s mechanism benefits inference accuracy by exploiting available resources T and M, and by eliminating IO/compute starvation. 

%\xzlNote{important but missing: with what T and M our method will lose benefit over baselines??}

%\sys{} shifts the pipeline bottleneck from IO to compute, so T may have the largest submodel and a maximum accuracy.
%Due to the depth-favoring heuristics of \sys{} (\S\ref{sec:design:planning:compute}), the accuracy is largely dependent on the submodel depths.  
%As the target latency grows from XXX ms to XXX ms, \sys{} executes an increasingly deeper submodel, resulting in higher accuracy. 
 %\wk{possible misleading that the more GFLOP the higher acc.}
 %\wk{relation between depth favor and counterproductive depth...}



\begin{comment}
Due to the depth-favoring heuristics of compute planning (\S\ref{sec:design:planning:compute}), our accuracy is largely dependent on the submodel depth, bound by T.
More specifically, our accuracy is more sensitive in a shallower submodel (i.e. with fewer layers) and sees a diminishing return on a deeper one, aligning with prior work~\cite{layerdrop, dynabert}. 
We hence have following observations on the two platforms: 
1) on CPU, \sys{} is the key to a higher accuracy in the lower range T (i.e. 150-200ms), when the submodel has not yet reached 10 layers. %the diminishing returns of accuracy on a more relaxed target latency stresses the importance of .

%For instance, \sys{} accuracy is more sensitive in the lower range of T, e.g. 150-200ms
%in such range our accuracy is much higher than baselines (by XXX$\times$).
%In the range, our accuracy leaps by XXX points, whilst it increases by only YYY points from 200ms to 400ms, the latter having 4$\times$ more time;
In the range, we are better by XXX points compared with baselines. %XXX\% higher than in 200-400ms range.
When T is more relaxed and allows more layers, i.e. T=400ms, \sys{}'s benefits gradually diminishes.
%The diminishing returns on a more relaxed target latencies stresses the importance of \sys{}, which is designed to operate on restrained T. %is likely due to the intrinsic parameter redundancy of \tfm{}s.
%2) In general, a higher T induces a higher accuracy. 
%\xzlNote{isn't this obvious? or, this does not apply to some baselines?}
%This is due to \sys{} shifts pipeline bottleneck from IO to compute and let T bound the submodel size.
%Given more time T, \sys{} achieves greater accuracies (Table~\ref{tab:accu}) on a larger submodel (Table~\ref{tab:network-confs}) which has more GFLOPs.
%2) \sys{} does not need a sufficiently large T (i.e. large enough execute a 12x12 full model) to achieve a gold accuracy.
%When T is sufficient (1200ms on Odroid and 600ms on Jetson), allowing a full 12x12 submodel to be executed, the accuracy achieves a maximum, same as BERT.
%Yet, such high T is not necessary for achieving the maximum accuracy.
%On both platforms, \sys{} achieves accuracies similar to gold (<2\% accuracy loss) when at T=400ms on a 10x3 submodel, which is 4$\times$ smaller than a full model.
%Whereas on Jetson, baselines are still XXX percent point behind the gold accuracy. 
%suggesting a smaller network is sufficient for such tasks.
2) on GPU, \sys{} keep outperforming baselines by XXX percent point throughout the whole 150-400ms range.
This is because GPU lacks compute proportionality\Note{check}, resulting in a ``shallow'' and ``wide'' submodel.
As a consequence, the submodels are still shallow even until T=400ms, e.g. it only has 7 layers. 
%\xzlNote{point 2 seems: our accuracy has a diminishing return on more relaxed target latency (over 200ms). If so, do we still beat baselines on this latency range? does this mean our method is only significant for lower target latencies?}
\end{comment}

%We do not expect future hardware with faster compute to compress the effective range 
%to drastically compress the range, because as NLP models are becoming larger, it is unlikely the data ingestion rate (of the storage technology) can keep up.

%\Note{1. see consistent and noticeable gain on our platform  larger buffer is not helping because ... 
%2. on future platforms (faster compute) it will help more... point out GPU case...}

%\st{Preload memory improves accuracy by adding bonus IO to AIBs, which \sys{} leverages to upgrade shards without stalling.}  \xzlNote{already stated}
%The benefits of preload buffer hinge on two factors: 1) its size, 
%%i.e. how many preloaded shards, 
%%i.e. how much do preloaded shards contribute to AIBs,
%and 2) the relative speeds of compute and IO hardware. 
%i.e. how effective do added AIBs translate to higher-fidelity shards.
%Therefore it is platform-dependent...
%We consider two scenarios. 

%The benefits of preload buffer hinge on two factors: 1) its size, 
%i.e. how many preloaded shards, 
%i.e. how much do preloaded shards contribute to AIBs,

 
%When the platform has slow compute (as ours) and can load full 6-bit submodel during execution, the preload buffer (1-5MB) is useful to increase submodel size (GFLOPs) by eliminating first layer IO, e.g. 150ms-200ms on Odroid, 150-400ms of Jetson. 
%We are XX better because of larger sumodel..
%Figure~\ref{fig:submodel} shows the case .. 
%		E.g. \textit{StdPL-6bit vs ours} which has larger submodel 
%it has less impacts when first layer IO does not impact submodel size because of the diminishing reutrn of high-fidelity shards (6 -> 32 not as pronounced as 2 -> 6).
%Although such size contributed to only one additional 32-bit shard in our case, but we are still seeing noticeable and consistent accuracy increase in our case.

%In this case preload buffer significantly helps accuracy by a few percent points. 
%E.g. Table~\ref{tab:eval:shard-selection} -- upgrading 10 2-bit shards to 6 bits increase accuracy by up to 19.2 percent point.
%At this point it size is usually a few hundred KB, no larger than 2bit * n * m.
%Table~\ref{tab:eval:shard-selection} -- upgrading 10 2-bit shards to 6 bits increase accuracy by up to 19.2 percent point.


%\paragraph{Applicability to future hardware}
%We expect \sys{} to keep benefiting future hardwares.
%Our insight is the compute will keep out pacing IO.
%%that with faster CPU/GPU/NPU
%On one hand, they may shift the range of target latencies which \sys{} are effective to lower but unlikely to compress it due to slow IO.
%On the other hand, faster compute further stresses the importance of preload buffer of \sys{}.

%On one hand, the slow IO lets \sys{} keep
%The reason is as NLP models are becoming larger, it is unlikely the data ingestion rate (of the storage technology) can keep up.



%Given a submodel, the larger the preload memory is, the more shards \sys{} may upgrade to the higher fidelity, hence the better accuracy. \xzlNote{this is obvious, but the key is when do we see diminishing return}
%Empirically, it is most effective when upgrading lower bits, e.g. 2 bits to 6 bits, as exemplified in Table~\ref{tab:eval:shard-selection} -- upgrading 10 2-bit shards to 6 bits increase accuracy by up to 19.2 percent point.
%It is less effective instead of 6 bits to 32 bits.
%The range of memory size can be given by $[0, n*m*s_b]$
%i.e. how much do these shards contribute to AIBs.
%how many high-fidelity shards it can load within AIBs.

%The preload memory is most effective when the device has fast compute, e.g. the initial AIBs only support loading low-fidelity shards.

\begin{comment}
\Note{below old....}

On our platforms, however, the accuracies are similar for all benchmarks as shown in Table~\ref{tab:accu}, when preload memory increases from 0MB to 1MB (Odroid) and 5MB (Jetson). \xzlNote{I would not call it similar. We see some noticeable, consistent accuracy improvement. Be careful: do not downplay the significance of our preload buffer. We spent lots of writing on it}

This is because the IO of both platforms support loading all 6-bit shards within their AIBs \xzlNote{meaning load during execution?}, whose accuracy is already close to gold (i.e. \textit{PreloadModel-full});
the only upgrade option is 32 bits \xzlNote{this is our implementation limit.}. %the bonus IO provided by preload memory.
Yet, the bonus IO provided by the 1MB and 5MB preload memory barely supports upgrading one additional shard to 32 bits.
Therefore under different sizes, they exhibit similar accuracies.
\xzlNote{State: in what situation do we expect the preload buffer size matters more?}

\Note{To incorporate}
\begin{myitemize}
	\item 
	The effectiveness of preload mem is jointly dependent on its size and also the IO/compute ratio (which is platform dependent)...
	
	Reasons:
	
	1) whether the elimination of first layer IO impacts submodel size..
	E.g. 150-200 on Odroid and 150-400 on Jetson, the first layer IO may be significant enough to impact submodel sizes (decided by compute) (see submodel sizes of NaivePL..). and degrade accuracy by XXX.
	 
	2) how effectively it can translate to upgradeable higher-fidelity shards. 
	This is also affected by the diminishing return of higher bitwidths (e.g. 6 -> 32). 
	
	
	\item 
	Some boundary conditions: (assuming IO capability is unchanged..)
	\begin{itemize}
		\item 
		1) if the platform has fast compute. e.g. it cannot load full 6-bit submodel but only a 2-bit one. 
		Preload buffer significantly helps accuracy by a few percent points. 
		At this point it size is usually a few hundred KB, no larger than 2bit * n * m.
		
		\item 
		2) if the platform has slow compute (as ours) and can support full 6-bit submodel during execution, the preload buffer (1-5MB) is useful to increase submodel size (GFLOPs) by eliminating first layer IO, e.g. 150ms-200ms on Odroid, 150-400ms of Jetson. We are XX better because of larger sumodel..
%		E.g. \textit{StdPL-6bit vs ours} which has larger submodel 
		it has less impacts when first layer IO does not impact submodel size because of the diminishing reutrn of high-fidelity shards (6 -> 32 not as pronounced as 2 -> 6).
		
	\end{itemize}

	
	
	
	\item 
	
	
\end{myitemize}
\end{comment}




%due to there are still AIBs after loading all 6-bit shards..
%Reasons for two platforms to demonstrate little impacts: 1) number of upgradable shards small.. Since platform can load all 6bits while still having spare.. The only shards to load is 32-bit (around 4MB each)...The accuracy diminishing. 2) benchmarks have more important shards in top layers (which can overlap well in bottom layers) and do not need upgrade shards in top layers...

%\xzlNote{merge?}
%\paragraph{Resource requirements}  \xzlNote{much can go to the evaluation section}
%%\sys{} benefits mobile NLP inference by exploring the finer-grained tradeoffs between time $T$ and space $M$. 
%\sys{} benefits inference accuracy by eliminating IO/computation starvation under \textit{constrained} resources $T$ and $M$ of a mobile device. 
%%It eliminates resource starvation under $T$.
%%It ensures under a $T$ the inference computes for as long as possible, and on parts as important as possible.
%In other words, as long as $T$ and $M$ are not unbounded, i.e. large enough to ``load \& execute, and host'' the complete full-fidelity model, \sys{} consistently improves accuracy by striving to compute for as long as possible (\S\ref{sec:design:planning:compute}), and to upgrade shards to highest possible fidelities (\S\ref{sec:design:planning:compute}).
%%In other words, as long as $T$ and $M$ are not unbounded, i.e. enough to ``load, execute, and host'' the complete full-fidelity model, \sys{} consistently improves accuracy by striving to compute for as long as possible (\S\ref{sec:design:planning:compute}), and to use shards of highest possible fidelities (\S\ref{sec:design:planning:compute}).
%\sys{} hence does not set a maximum $T$ or $M$. 


%\xzlNote{content of S3 can come here}
%
%On the other hand, for the accuracy to be practical, \sys{} sets the per-device minimum $T$ as the execution delay of a $3 \times 3$ submodel on the device which incurs $\sim 15\%$ accuracy degradation than the full one;
%upon any $T$s below the threshold, \sys{} executes with the minimum $T$ instead. %but proceeds with minimum $T$...
%Meanwhile, it expects $M$ to be large enough to contain the shards at first few layers of the submodel for bootstrapping inference, e.g. 5MB. %allowing IO/computation overlapping to happen at early stages, without stalling the pipeline. %without starving either...
%However due to high memory pressure, OS may adjust a too small $M$ (e.g. a few KBs) or eliminate it completely (i.e. M=0). %to host one layer of shards. 
%On such occasions \sys{} incurs compulsory pipeline stall to load missing shards at the first layer; 
%subsequent layers remain unaffected.


%\sect{eval} will explore more on the finer-grained tradeoffs between time $T$ and space $M$. 




==> fig-MLXe2eGPTMemory.tex <==
% !TeX root = main.tex

\begin{figure}[h]
	\centering
	\includegraphics[width=0.48\textwidth]{figs/mlxe2egptmemory.pdf}
	%\subcaption{Matrix-matrix product with FP32.}
		
	\caption{Memory consumption over time during the pre-training process of GPT2-large on M2 Ultra with MLX framework.}
	\label{fig:finding:mlxe2egptmemory}
%	\vspace{-5mm}
\end{figure}

==> fig-aib.tex <==
% !TeX root = main.tex


\begin{figure}[h]
	%	\centering
	\includegraphics[width=0.48\textwidth]{./figs/aib}
	%	\vspace*{-2em}
	\caption{A mini example of AIB tracking the layerwise IO budgets.}
	%\caption{Hot vs cold start inference latency Breakdown of IO/Compute on different mobile platforms, showing IO dominates the latency and various IO/Compute ratio.
	%	\textbf{TODO:} show BERT -- show hot inference latency for comparison}
	\label{fig:design:aib}
%	\vspace{-2em}
\end{figure}

==> fig-conv.tex <==
% !TeX root = main.tex

\begin{figure}[h]
	\centering
	\includegraphics[width=0.48\textwidth]{figs/conv.pdf}
	%\subcaption{Matrix-matrix product with FP32.}
		
	\caption{Measurements on convolution. Shape A: Batch size=4, Height=Width=32, Input channel=Output channel=64; shape B: Batch size=4, Height=Width=32, Input channel=Output channel=256; shape C: Batch size=16, Height=Width=512, Input channel=Output channel=3; shape D: Batch size=32, Height=Width=1024, Input channel=Output channel=3. All of convolution kernels are in $5\times 5$, with the stride (1,1) and padding (2,2).}
	\label{fig:finding:conv}
%	\vspace{-5mm}
\end{figure}






==> fig-design-explore.tex <==
% !TeX root = main.tex

\begin{figure}[h]
	\centering
	\includegraphics[width=0.48\textwidth]{./figs/overlap}
%	\vspace{-2em}
	\subcaption{Naively layerwise overlap}
	\label{fig:motiv:overlap}
	
	\includegraphics[width=0.48\textwidth]{./figs/compress_overlap}
	\subcaption{Model compression on layers}
	\label{fig:motiv:compress-overlap}
%	\vspace{-5mm}
\end{figure}

==> fig-io-compute.tex <==
% !TeX root = main.tex
\begin{figure}[h]
	\centering
	\includegraphics[width=0.48\textwidth]{./figs/io_compute}
%	\vspace{-2em}
	\caption{IO/Compute latencies under different Compression ratios of DistilBert model}
	\label{fig:motiv:io-compute}
%	\vspace{-5mm}
\end{figure}

==> fig-lat-breakdown.tex <==
% !TeX root = main.tex

\begin{figure}[h]
	\centering
	\includegraphics[width=0.25\textwidth]{./figs/plot/motiv-lat/fig_lat}
%	\vspace*{-2em}
	\caption{Hot vs cold start inference latency of \textbf{Mob}ileBERT, \textbf{Dis}tilBERT, and BERT on Odroid dev board.}
%\caption{Hot vs cold start inference latency Breakdown of IO/Compute on different mobile platforms, showing IO dominates the latency and various IO/Compute ratio.
%	\textbf{TODO:} show BERT -- show hot inference latency for comparison}
	\label{fig:motiv:lat-breakdown}
%	\vspace{-5mm}
\end{figure}

==> fig-major-deadline.tex <==
% !TeX root = main.tex

\begin{figure}[h]
	\begin{minipage}[t]{0.15\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/major-deadline/fig_major_deadline}
		\subcaption{SST-2}	\label{fig:eval:deadline:sst2}			
	\end{minipage}\hfill
	\begin{minipage}[t]{0.15\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/major-deadline/fig_major_deadline}
		\subcaption{SST-2}	
	\end{minipage}\hfill
	\begin{minipage}[t]{0.15\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/major-deadline/fig_major_deadline}
		\subcaption{SST-2}	
	\end{minipage}\hfill
	%	\vspace*{-2em}
	\caption{\sys{} accuracy on GLUE benchmark. Each deadline variable is set by the system configuration. We assume that 1.5s is the upper limit for IRA. (need to confirm or cite)}
	\label{fig:eval:deadline}
	%	\vspace{-5mm}
\end{figure}

==> fig-major-memory.tex <==
% !TeX root = main.tex
%\begin{figure}[h]
%	\centering
%	\includegraphics[width=0.48\textwidth{}]{./figs/plot/major-memory/fig}
%	%	\vspace{-2em}
%	\caption{
%	\sys{}'s accuracy is significantly higher than \textit{Load\&Exec} and \textit{StdPL}, and is similar/higher compared to \textit{PreloadModel} albeit using an order of magnitude smaller memory. 
%	T=200ms. 
%	Full data and more benchmarks in Table~\ref{tab:accu}.
%	XXXX color code can be problematic}
%	\label{fig:eval:memory}
%	%	\vspace{-2em}
%\end{figure}



\begin{figure}[t]
	\begin{minipage}[t]{0.48\textwidth}
		\centering
		\includegraphics[width=0.48\textwidth]{./figs/plot/major-memory/fig_sst-2_200-anno}
		\includegraphics[width=0.48\textwidth]{./figs/plot/major-memory/fig_qqp_200}
		\subcaption{Odroid}	
%		\label{fig:eval:sst2:200}			
	\end{minipage}\hfill
	\begin{minipage}[t]{0.48\textwidth}
	\centering
	\includegraphics[width=0.48\textwidth]{./figs/plot/major-memory/fig_sst-2_200_jetson}
	\includegraphics[width=0.48\textwidth]{./figs/plot/major-memory/fig_qqp_200_jetson}
	\subcaption{Jetson}
	\label{fig:eval:memory:jetson}
%	\label{fig:eval:rte:300}			
	\end{minipage}\hfill
	\caption{
	\sys{}'s accuracy is significantly higher than \textit{Load\&Exec} and \textit{StdPL}, and is similar/higher compared to \textit{PreloadModel} albeit using 1-2 orders of magnitude smaller memory. 
	T=200ms. 
	Full data and benchmarks in Table~\ref{tab:accu}.}
	\label{fig:eval:memory}
	%	\vspace{-5mm}
\end{figure}

==> fig-memory-consumption.tex <==
% !TeX root = main.tex

\begin{figure}[h]
    \centering
	\begin{minipage}[t]{0.22\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/preloaded-memory/fig_preloaded_odroid}
		\subcaption{Odroid}	\label{fig:eval:preloaded:odroid}			
	\end{minipage}
	\begin{minipage}[t]{0.225\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/preloaded-memory/fig_preloaded_jetson}
		\subcaption{Jetson}	\label{fig:eval:preloaded:jetson}			
	\end{minipage}\hfill
	%	\vspace*{-2em}
	\caption{PreloadedModel vs. Ours of preloaded memory size at different latencies. Lower is better.}
	\label{fig:eval:memory-consumption}
	%	\vspace{-5mm}
\end{figure}

==> fig-memoryNearCapacity.tex <==
% !TeX root = main.tex

\begin{figure}[h]
	\centering
	\includegraphics[width=0.48\textwidth]{figs/memoryNearCapacity.pdf}
	%\subcaption{Matrix-matrix product with FP32.}
		
	\caption{Memory consumption over time when near the capacity of training of Whisper.medium. }
	%\xzlNote{Dec 5: blue? orange?}}
	\label{fig:finding:memorynearcapacity}
%	\vspace{-5mm}
\end{figure}

==> fig-memorySc1.tex <==
% !TeX root = main.tex

\begin{figure}[h]
	\centering
	\includegraphics[width=0.48\textwidth]{figs/memorySc1.pdf}
	%\subcaption{Matrix-matrix product with FP32.}
		
	\caption{Memory consumption over time during the training process of Whisper-medium.}
	\label{fig:finding:memorysc1}
%	\vspace{-5mm}
\end{figure}

==> fig-nearCapacityTimeWhisperLarge.tex <==
% !TeX root = main.tex


\begin{figure}[h]
	%	\centering
	\includegraphics[width=0.48\textwidth]{figs/nearCapacityTimeWhisperLarge.pdf}
	%	\vspace*{-2em}
	\caption{The time required in each pass during near-capacity training of Whisper-large on M2 MAX. \textbf{Jan 2 - has to compare its average to CUDA?}(Done in writing)}
	%\caption{Hot vs cold start inference latency Breakdown of IO/Compute on different mobile platforms, showing IO dominates the latency and various IO/Compute ratio.
	%	\textbf{TODO:} show BERT -- show hot inference latency for comparison}
	\label{fig:finding:nearcapacitytimewhisperlarge}
%	\vspace{-2em}
\end{figure}

==> fig-overview-timeline.tex <==
% !TeX root = main.tex

\begin{figure}[h]
%	\centering
	\includegraphics[width=0.48\textwidth]{./figs/overview-timeline}
%	\vspace*{-2em}
	\caption{Comparison of model execution methods. Our method achieves high accuracy at low memory cost. T: target latency. M: model memory for Transformer weights.}
%\caption{Hot vs cold start inference latency Breakdown of IO/Compute on different mobile platforms, showing IO dominates the latency and various IO/Compute ratio.
%	\textbf{TODO:} show BERT -- show hot inference latency for comparison}
	\label{fig:overview-timeline}
%	\vspace{-5mm}
\end{figure}

==> fig-overview.tex <==
% !TeX root = main.tex

\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth]{./figs/overview}
%		\includegraphics[width=0.98\textwidth]{./figs/overview-large}
%	\vspace*{-2em}
	\caption{System architecture of \textbf{S}peedy \textbf{T}ransformer \textbf{I}nference (\sys{}) and workflow.}
		%XXX: no need to cover the pipeline details etc which are covered in later figures. only show high level sys components (esp buffers.}
%\caption{Hot vs cold start inference latency Breakdown of IO/Compute on different mobile platforms, showing IO dominates the latency and various IO/Compute ratio.
%	\textbf{TODO:} show BERT -- show hot inference latency for comparison}
	\label{fig:design:overview}
%	\vspace{-5mm}
\end{figure}

==> fig-pagefault.tex <==
% !TeX root = main.tex

\begin{figure}[h]
	\centering
	\includegraphics[width=0.48\textwidth]{figs/pagefault.pdf}
	%\subcaption{Matrix-matrix product with FP32.}
		
	\caption{The number of page fault triggered during the training process when the memory is sufficient enough. \xzm{describe it in text and remove this figure}}
	\label{fig:finding:pagefault}
%	\vspace{-5mm}
\end{figure}

==> fig-pagefaultNearCapacity.tex <==
% !TeX root = main.tex

\begin{figure}[h]
	\centering
	\includegraphics[width=0.48\textwidth]{figs/pagefaultNearCapacity.pdf}
	%\subcaption{Matrix-matrix product with FP32.}
		
	\caption{The number of page fault triggered during the near-capacity training. }%\xzlNote{Dec 5: better show throughput, Ops/sec}
	\label{fig:finding:pagefaultnearcapacity}
%	\vspace{-5mm}
\end{figure}

==> fig-planning.tex <==
% !TeX root = main.tex
\begin{figure*}
%	\begin{figure}{r}{0.5\textwidth}
	\centering
	\includegraphics[width=1\textwidth]{./figs/planning}
%	\vspace*{-2em}
	\caption{The proposed planning strategy. XXX:update}
%\caption{Hot vs cold start inference latency Breakdown of IO/Compute on different mobile platforms, showing IO dominates the latency and various IO/Compute ratio.
%	\textbf{TODO:} show BERT -- show hot inference latency for comparison}
	\label{fig:design:planning}
%	\vspace{-5mm}
\end{figure*}

==> fig-prelim-planning.tex <==
% !TeX root = main.tex

\begin{figure}[h]
%\begin{figure}{r}{0.3\textwidth}
%	\centering
	\begin{minipage}[t]{0.15\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/planning-weight/fig_weight}
		\subcaption{The outlier percentage of each layer in DynaBERT~\cite{dynabert} model. 
		Our planning strategy fits the outlier distribution.}
		\label{fig:prelim:weight}
	\end{minipage}\hfill
	\begin{minipage}[t]{0.15\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/planning-load/fig_load}
		\subcaption{Cold start inference latency of MobileBERT, DistilBERT, and BERT on Tensorflow and PyTorch.}	
		\label{fig:prelim:load}			
	\end{minipage}\hfill
	\begin{minipage}[t]{0.15\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/planning-breakdown/fig_breakdown}
		\subcaption{Per-component latency breakdown of a BERT layer with different number of attention heads on an x86 machine.}
		\label{fig:prelim:breakdown}
	\end{minipage}
	\caption{Preliminary results back up our proposed planning strategy.}
\end{figure}


==> fig-prelim-sharding.tex <==
% !TeX root = main.tex
\begin{figure}[h]
%\begin{figure}{r}{0.3\textwidth}
%	\centering
	\begin{minipage}[t]{0.15\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/shard-outlier/fig_sharding}
		\subcaption{SST-2~\cite{glue-benchmark} accuracy with our proposed quantization technique.}	\label{fig:prelim:sharding}			
	\end{minipage}\hfill
	\begin{minipage}[t]{0.15\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/shard-others/fig_others}
		\subcaption{Our propsoed quantization technique also works with MNLI and STS-B~\cite{glue-benchmark}.}
		\label{fig:prelim:others}
	\end{minipage}\hfill
	\begin{minipage}[t]{0.15\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/shard-heads/fig_heads}
		\subcaption{SST-2 accuracy increases as number of attention heads, the proposed sharding granulairty.}
		\label{fig:prelim:heads}
	\end{minipage}
	\caption{Preliminary results on our proposed sharding strategy on DynaBERT~\cite{dynabert}.}
\end{figure}


==> fig-res-model.tex <==
% !TeX root = main.tex

\begin{figure}[h]
%	\centering
	\includegraphics[width=0.45\textwidth]{./figs/pipeline}
%	\vspace*{-2em}
	\caption{IO/Compute pipeline execution... XXX need discussion}
%\caption{Hot vs cold start inference latency Breakdown of IO/Compute on different mobile platforms, showing IO dominates the latency and various IO/Compute ratio.
%	\textbf{TODO:} show BERT -- show hot inference latency for comparison}
	\label{fig:design:pipeline}
%	\vspace{-5mm}
\end{figure}

==> fig-sc1memgpt2.tex <==
% !TeX root = main.tex

\begin{figure}[h]
	\centering
	\includegraphics[width=0.48\textwidth]{figs/sc1GPT2lorafp32.pdf}
	%\subcaption{Matrix-matrix product with FP32.}
		
	\caption{Memory consumption over time during the training of GPT2-large with LoRA.}
	\label{fig:finding:sc1GPT2lorafp32}
%	\vspace{-5mm}
\end{figure}

==> fig-sc1memgpt2rtx4090.tex <==
% !TeX root = main.tex

\begin{figure}[h]
	\centering
	\includegraphics[width=0.48\textwidth]{figs/sc1GPT2lorafp32rtx4090.pdf}
	%\subcaption{Matrix-matrix product with FP32.}
		
	\caption{Memory consumption over time during the training of GPT2-large on RTX 4090.}
	\label{fig:finding:sc1GPT2lorafp32rtx4090}
%	\vspace{-5mm}
\end{figure}

==> fig-sharding.tex <==
% !TeX root = main.tex

\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{./figs/shards}
%	\vspace*{-2em}
	\caption{Instantiating $N\times M \times K$ model shards on disk. 
	The example shows a 2-bit shard.
	99.9\% of its weights are represented by 2-bit indexes pointing to $2^2$ centroids;
	the rest 0.1\% outliers are preserved as-is.
	}
	%XXX show: all BERT layers (zoom in one layer); a shard; XXXX To simplify: Q/K/V (attention head); outliers. Explain: centroids. which bits represent what centroids. multi versions }
%\caption{Hot vs cold start inference latency Breakdown of IO/Compute on different mobile platforms, showing IO dominates the latency and various IO/Compute ratio.
%	\textbf{TODO:} show BERT -- show hot inference latency for comparison}
	\label{fig:design:shards}
%	\vspace{-5mm}
\end{figure}

==> fig-submodel.tex <==
% !TeX root = main.tex

\begin{figure}[h]
%	\centering
	\includegraphics[width=0.45\textwidth]{./figs/submodel}
%	\vspace*{-2em}
	\caption{A comparison between submodels executed by \textit{Ours} and \textit{StdPL-6bit}. Benchmark: SST-2 on Odroid. T=200ms.
	\textit{Ours} runs a larger submodel and higher FLOPs, resulting in 9.2 pp higher accuracy.}
%	\textbf{TODO:} show BERT -- show hot inference latency for comparison}
	\label{fig:submodel}
%	\vspace{-5mm}
\end{figure}

==> fig-thesis-overview.tex <==
% !TeX root = proposal_memo.tex
\begin{figure}[h]
	\centering
	\includegraphics[width=0.6\textwidth]{./figs/thesis_overview}
	\caption{My thesis comprises a series of systems design towards a more efficient and secure heterogeneous edge platform; the figure shows their corresponding positions in the software/hardware stack.
	\protect\circled{1}~: Psbox (\S\ref{sec:thesis:psbox}), \protect\circled{2}~: Transkernel (\S\ref{sec:thesis:dbt}), \protect\circled{3}~: Enigma (\S\ref{sec:thesis:enigma}), \protect\circled{4}~: Driverlet (\S\ref{sec:thesis:driverlet}), \protect\circled{5}~: STI (\S\ref{sec:thesis:sti})}
	\label{fig:thesis}
\end{figure}

==> fig-timeNearCapacity.tex <==
% !TeX root = main.tex


\begin{figure}[h]
	%	\centering
	\includegraphics[width=0.48\textwidth]{figs/timeNearCapacity.pdf}
	%	\vspace*{-2em}
	\caption{The time required in each pass during near-capacity training of Whisper.medium.}
	%\caption{Hot vs cold start inference latency Breakdown of IO/Compute on different mobile platforms, showing IO dominates the latency and various IO/Compute ratio.
	%	\textbf{TODO:} show BERT -- show hot inference latency for comparison}
	\label{fig:finding:timenearcapacity}
%	\vspace{-2em}
\end{figure}

==> fig-trainingSc1.tex <==
% !TeX root = main.tex


\begin{figure}[h]
	%	\centering
	\includegraphics[width=0.48\textwidth]{figs/trainingSc1.pdf}
	%	\vspace*{-2em}
	\caption{The forward time, backward time on different devices on the two workloads. \xzlNote{Jan 10: needs revision; not quite readable}}
	\label{fig:finding:trainingSc1}
%	\vspace{-2em}
\end{figure}

==> fig-trainingSc2.tex <==
% !TeX root = main.tex


\begin{figure}[h]
	%	\centering
	\includegraphics[width=0.48\textwidth]{figs/trainingSc2.pdf}
	%	\vspace*{-2em}
	\caption{The forward time, backward time on different devices during training on the two workloads, when CUDA devices are applied with Zero-Offload. }
	\label{fig:finding:trainingSc2}
%	\vspace{-2em}
\end{figure}

==> fig-trainingTIme.tex <==
% !TeX root = main.tex


\begin{figure*}[h]
	%	\centering
	\includegraphics[width=0.48\textwidth]{figs/trainingTime.pdf}
	%	\vspace*{-2em}
	\caption{The forward time, backward time on different devices on the two workloads. }
	\label{fig:finding:trainingtime}
%	\vspace{-2em}
\end{figure*}

==> fig-transformer.tex <==
% !TeX root = main.tex

\begin{figure}[t]
	\vspace{1em}
	\centering
	\includegraphics[width=0.38\textwidth]{./figs/transformer}

	\caption{(Left) The BERT model comprising transformer layers and (Right) the number of 32-bit floating point parameters within a layer~\cite{transformer}.}
%\caption{Hot vs cold start inference latency Breakdown of IO/Compute on different mobile platforms, showing IO dominates the latency and various IO/Compute ratio.
%	\textbf{TODO:} show BERT -- show hot inference latency for comparison}
	\label{fig:motiv:transformer}
%	\vspace{-5mm}
\end{figure}

==> fig_shard_importance.tex <==
% !TeX root = main.tex
\begin{figure}[t]
	\begin{minipage}[t]{0.23\textwidth}
	\centering
	\includegraphics[width=1\textwidth]{./figs/plot/shard-importance/sst-2_prof_map}
	\subcaption{SST-2}	\label{fig:eval:importance:sst}			
\end{minipage}\hfill
\begin{minipage}[t]{0.23\textwidth}
	\centering
	\includegraphics[width=1\textwidth]{./figs/plot/shard-importance/rte_prof_map}
	\subcaption{RTE}	\label{fig:eval:importance:rte}			
\end{minipage}\hfill
	\caption{Example shard profiles on SST-2 and RTE show distinct importance distribution.
	Each cell at (x, y) marks a shard; the lighter its color is, the more important the shard is (i.e. the higher accuracy during profiling).
	Y-axis: \tfm{} layer index, X-axis: vertical slice index.  }
	\label{fig:eval:importance}
\end{figure}

==> impl.tex <==
% !TeX root = main.tex
%\vspace{2cm}
\section{Implementation}
\label{sec:impl}



 %have good community support and documentation.






%We also preload the embedding table as we target model execution. 

%\subsection{Handling miscellaneous parameters}
%%These are much smaller compared with \tfm{} model shards, they include poolers, add \& norm layers, as well as classification heads used in downstream tasks. 
%%
%%For them, we quantize them uniformly to 6 bits. 
%\Note{Not realted to key ideas. may move to impl. }
%\textbf{Key idea:} small enough for fixed-precision quantization (potentially low-precision) and can be loaded along side the shards. 
%
%There are miscellaneous parameters to a \tfm{} model, which are not counted towards a model shard. 
%They include layer normalization (layernorm) in the encoder layers, a pooler layer for pooling encoder outputs of hidden states, and a classifier for downstream tasks.
%
%Compared with shards, they are much smaller and do not deserve an elastic IO.
%For instance, of a \tfm{} layer, there are only two layernorms, each having only 768 parameters; 
%after all encoder layers, the pooler is a 768x768 dense layer which pools encoder outputs of hidden states;
%for the last classifier layer, its size is only 768 x 2 for a bi-class classification task (e.g. sentiment analysis).
%
%Hence \sys{} quantized them into a fixed 6-bit precision, and the planner schedules their IO among shards and ensures the data dependency.

%specified and measures the average delay of decompression and \tfm{} computation...
%To measure shard importance, we run the ablation study on test sets of GLUE tasks...
%As our target is balance computation and IO of \tfm{} layers, we cache the embedding layer.. 

%We preprocess pretrained, fine-tuned models from DynaBERT for model shards..
%To compress them, we fit the parameters using Guassian mixture ... to detect outliers with threshold -4... 
%We use arithmetic mean to decide cluster centroids, which achieves competitive accuracy with SOTA~\cite{gobo} but is XXX faster.
%We compress 2-6 in total 5 versions...
%%We cache the embedding layer...
%Then we load shards of each version to measure their average delay.
%To measure the computation delay, we fix input length =128, and operating frequency to the peak.

%One may use complementary techniques to reduce embedding size, e.g.~\cite{flashembedding, embedding-cache}..
%
%
%\Note{moved.}
%To compress, the system fits layerwise weights into a Gaussian distribution and detects outliers if the log probabilities of them belong to the distribution are below a threshold, for which we use -4 following~\cite{gobo}.
%%it divides weights into two groups, an outlier group and a Gaussian group;
%%deems a parameter as an outlier the Gaussian
%To decide centroids, the system sorts non-outliers, puts them in $2^b$ equally populated clusters, and calculates the mean of each cluster.
%For each layer of every fidelity version, the system generates a dictionary, mapping a weight to a centroid or an outlier.
%The process is done ahead of time and efficient, which only takes a few minutes per version on our X86 server.
%
%\Note{moved}
%The system generates $N \times M\times K$ such shards and stores them on disk by their identities using a three-tuple $S=(n, m, b)$, where $n$, $m$ are the indexes of the layer and vertical slice respectively, $b$ is the fidelity.
%It co-locates their disk blocks for access locality.
%
%\Note{moved}
%Following the same practice in~\cite{gobo}, we use $-4$ which is sufficient in maintaining accuracy while maximizing compression ratio;
%under the threshold, the outlier group constitute less than $0.1\%$ of total weights. %which is preserved in full precision (i.e. 32-bit). %and incurring only 1\% accuracy degradation. 
%For the Gaussian group which constitute the rest $99.9\%$, the system sorts and splits its weights into $2^b$ clusters with equal population;
%each cluster has \textit{one} centroid to represent \textit{all} values within it. 
%%It then represents \textit{all} values in each cluster with \textit{one} centroid, which is indexed by a $b$-bit integer.
%%It then represents \textit{all} values in each cluster with \textit{one} cluster centroid by substituting them with a $b$-bit index to the centroid.
%Doing so caters to the weight distribution: weight-concentrated regions deserve higher resolutions, hence having more clusters and centroids.
%%the vast majority ($99.9\%$) of original 32-bit weights are represented by $b$-bit integers, reducing model size by $\lfloor 32/b \rfloor \times$.
%To decide cluster centroids, prior work adopt K-means based approaches~\cite{deep-compression, zhaoImprovingNeuralNetwork}, which are time-consuming, e.g. it takes a few hours to converge on our server.
%Differently, we have found the arithmetic mean of cluster weights suffices -- a 2-bit version takes a few minutes to converge and incurs only 7\% accuracy degradation compared with the full model. 
%We will present more results in \sect{eval}.  
%It uses the Gaussian model to find out a group of ``outliers'' parameters and preserve them in full precision.
%For the rest, the system quantizes them into $n$-bit integers (e.g. typically 2 to 4) using \textit{simulated quantization}~\cite{quantization-survey}, where each integer points to a full-precision FP32 value called a centroid, representing a group of original weights.
%The system decides the centroids by dividing the non-outlier parameters into $2^n$ groups and calculating their arithmetic means.

%Instead, it stores the outlier mapping separately to the compressed weights, which specifies 

%\input{tab-platform}

==> intro-xzl-comment.tex <==
% !TeX root = main.tex

\xzlNote{---------- begin xzl ------------}: 


\begin{itemize}
\item 
upon user request (impromptu), model has to be loaded and executed; 
(upon request -- maximum inference accuracy under a deadline) load and execute  model; compute/IO pipelining (with high parallelism); 

\item 
in the background: opportunistically load  and unload (a fraction of model). 
(background -- responding to changes in available memory) 
OS could opportunistically preload/evict model parts subject to available memory (policy -- Not this paper's focus)
\end{itemize}


\textbf{Current:} 
% model and OS are designed in isolation; oblivious to each other. 
rigid resource management in isolation. 
Techniques (knobs...hyperparameters...) exist to adjust individual resources 
(compute: model compression -- NestDNN, DynaBERT; 
memory/IO: quantization ...)
But the OS lacks mechanisms to manage the resources in a joint fashion towards the aforementioned goal. 

As a result ... Model load and execution: layer-wise execution; no or limited pipelining. 
Reason: skewed compute/IO ratio. Compute starvation. 
Most notable example is cold inference: ...

Model memory management: page in/out (monolithic -- Android; prior research: by layers). Result: model weights are swapped regardless of their impact on accuracy. 

\xzlNote{---------- end xzl ------------}: 

==> memo_sti_motiv.tex <==
% !TeX root = proposal_memo.tex

\section{Supplementary materials for \textit{S}peedy \textit{T}ransformer \textit{I}nference (\sys{})}
\label{sec:thesis:sti}

\subsection{How does \sys{} fit into the thesis?}
\sys{} addresses the first challenge (i.e. poor energy efficiency) as stated in \sect{thesis:challenge}. 
Specifically, it eliminates the CPU idle due to waiting for model load, by forming a IO/compute pipeline with elastic IO shards. 
Doing so reduces the cold inference latency significantly and improves energy efficiency;
targeting user software, it complements the accomplished work, which is done in kernel software. 

\subsection{\sys{} motivations}

\paragraph{Motivating scenario.}
\sys{} targets an interactive NLP scenario with intelligent personal assistant (IPA) on a multi-tenant mobile device.
In the scenario, a user typically interacts with the IPA for querying weather/personal emails/medical records~\cite{ipa-survey}, managing tasks~\cite{myersIntelligentPersonalAssistant2007} etc.
A typical interaction takes 2-3 turns and lasts for a few seconds~\cite{ipa-study-denmark};
during the interaction, the length of each utterance is often 10-20 words~\cite{tsaiFasterResponsesAre2019}. 

Under the hood, the IPA may run the pretrained Transformer language model to directly generate responses by running downstream tasks such as question answering~\cite{dynabert}, and dialog generation~\cite{dialogpt}.
Alternatively, it may generate responses from templates. 
It does so by filling the blanks in the templates~\cite{mdfn-aaai21} or selecting existing answers from its knowledge base, based on intent classification~\cite{dbpedia-chatbot} and sentiment analysis~\cite{yasudaDesigningChatbotSystem2021} results of the Transformer model.

\input{fig-lat-breakdown}

\paragraph{Why cold inference matters?}
Mobile app interactions are brief, for less than a minute~\cite{livelab};
interactions with IPAs are even shorter, for only a few seconds~\cite{ipa-study-denmark,tsaiFasterResponsesAre2019}.
During such a short period, human attention is a scarce resource~\cite{proj-aura}.
It is vital that the system be responsive and rapid upon invocations, for a smooth user experience~\cite{falcon-mobisys12}. 

Existing cold inference latency of \tfm{} inference, however, is far from ideal.
As shown in Figure~\ref{fig:motiv:lat-breakdown}, on a commodity embedded SoC the cold inference is as high as 4 seconds, which has already exceeded the typical duration of interactions with IPAs.
This is unacceptable to user experience.

Hence for the interactive NLP tasks we target, \sys{} aims to reduce its cold inference latency to the same level as \textbf{human interactions}.
That is, the latency (i.e. set by the deadline) is only a few hundred milliseconds~\cite{human-latency-study}, with hundred-milliseconds breaks between utterances.



\paragraph{Existing techniques are inadequate.}
We consider two common approaches to reducing cold inference latency as follows.
\begin{myenumerate}
	\item 
	\textit{How about pinning the model files in memory for good?}
	The approach conceptually eliminates cold inference, as the model files are always in memory.
	Yet, it eschews the IO time waiting for storage at the cost of high memory pressure, and is undesirable. 
	This is because:
	1) transformer model files are as large as a few hundred MBs, which take a significant portion of memory space of commodity mobile devices (e.g. a few GBs~\cite{iphone13});
	2) in the constrained memory space, the OS of the device must accommodate multiple tenant apps~\cite{acclaim-atc20} and ensure fairness of responsiveness~\cite{asap-atc21}, too;
	it shall not sacrifice the user experience of other apps.
	As a result of resource contention, cold inference happens frequently on today's mobile devices, causes ``latency variability''~\cite{dnn-mobile-lat-var}, and degrades user experience.
	
	\item 
	\textit{How about compressing the models?}
	Alternatively, one may compress a \tfm{} model to reduce the number/precision of parameters, hence the file size. 
	Common techniques include \ul{structured pruning} which reduces the width and/or depths of a \tfm{}~\cite{distilbert,mobilebert,dynabert,layerdrop},
	\ul{weight sharing} which makes \tfm{} layers to share same set of parameters~\cite{albert, universal-transformer},
	and \ul{quantization} which reduces the full precision of parameters (often in 32 bits) to low-bit representations or integers~\cite{binarybert,bibert}.
	However, these approaches share a key inadequacy -- still, the (cold) inference can only start as soon as the model is loaded.
	They hence face a dilemma between latency and accuracy: a low compression ratio (e.g. DistilBERT~\cite{distilbert} is 2$\times$ smaller than BERT~\cite{bert}) cannot meet the latency goal (e.g. a few hundred milliseconds) because it still takes seconds to load the model;
	a high compression ratio (e.g. BinaryBERT~\cite{binarybert} is 24$\times$ smaller) meets the latency goal while suffering from inferior accuracy, e.g. a few full GLUE scores lower, which is deemed significant in NLP literature~\cite{bibert,binarybert}.

\end{myenumerate}

\subsection{Clarifications from Q\&A}

\paragraph{What are key innovations?}
The key contribution of \sys{} is: 
1) it identifies the model shards which have elastic IO time, as the proper building block for the IO/compute pipeline of transformer inference;
2) based on model shards, it proposes a novel planning algorithm that maximizes the inference accuracy while meeting a user-set deadline on different devices.

We do not claim: 1) quantization techniques used to generate shards, and 2) IO/compute pipeline as our contribution since these techniques are well-known. 

\paragraph{How does the IO/compute pipeline work with shards?}
The number of shards per layer can be regarded as the ``width'' of the \tfm{} model during an inference;
it is the same across all layers during one inference.
Prior to each inference, \sys{} decides how many shards and the bitwidth of each shard to be used, depending on the deadline and device-specific IO/compute capability. 
For one inference, \sys{} constructs the IO/compute pipeline in the following way: it first loads the initial set of shards for layer 1; it then begins computing on shards of layer 1, while overlapping shard loading for layer 2, and so on and so forth.

\paragraph{Why do partial model composed of shards give meaningful results?}
Because of the parameter redundancy of \tfm{} models: 
a \tfm{} model may still give meaningful results even if attention heads are reduced from full sixteen to a few~\cite{16heads}, or layers share the same set of parameters~\cite{albert}. 
In \sys{}, one shard is a vertical slice of the transformer layer, comprising one attention head plus a set of FFN neurons; 
it preserves the structure on which the model is trained and the learned features. 
By stacking them in layers, the resultant model resembles a partial model with a smaller width~\cite{dynabert, liDynamicSlimmableNetwork2021}, hence still giving meaningful results.



\paragraph{\sys{} seems a generic model compression technique, why target cold inference only?}
To clarify: the model compression technique used by \sys{} is not new~\cite{gobo};
it acts only as an enabling tool for \sys{} to generate shards as the IO/compute pipeline building block.

\sys{}'s key ideas are tailored to cold inference due to the deadline constraint, where IO is the bottleneck.
The compression, however, does not affect compute time w.r.t. a full-precision model.
It hence has little benefits in a hot inference scenario, i.e. same latency but inferior accuracy than a full-precision model.

\paragraph{Can a GPU help reduce cold inference latency?}
No. 
This is because during cold inference, IO is the bottleneck, dominating over 90\% of the latency.
By simply offloading the compute to GPU, the IO keeps blocking compute and still results in high cold inference latency.

\paragraph{Why not offload to cloud?}
First, on-device inference ensures better privacy. 
The query as well as content being queried (e.g. medical records) do not have to be exposed to cloud.
Second, it is more reliable where spotty network connections are common on mobile devices~\cite{livelab,backgnd-in-wild2}.
Third, cloud offloading is a complementary approach, e.g. for other non-private queries, the user can always offload to cloud.

\paragraph{Can we leverage idle intervals between IPA interactions to load model?}
This is an orthogonal approach.
The idea is to prefetch the model file prior to inference.
Its challenge is twofold: 1) it is unclear how well IPA invocations can be predicted, while misprediction leads to excessive memory usage and poor user experience.
2) coordinating with other apps which compete for memory may be challenging, e.g. the already prefetched model file may be swapped out due to contention.


\paragraph{Why sacrifice accuracy for latency?}
Because in the scenario we target, reducing the latency from seconds to milliseconds significantly improves user experience.
Meanwhile, the accuracy loss is only 1\%, which is considered negligible in NLP literature~\cite{albert,nagarajanOptimizingTransformersApproximate}.
Prior study on IPAs~\cite{tsaiFasterResponsesAre2019} support our design, advocating ``faster responses are better responses''. 





==> memo_stmt.tex <==
% !TeX root = proposal_memo.tex

\section{Thesis statement}
\label{sec:thesis}

Emerging edge platforms are equipped with increasingly abundant and heterogeneous computing resources.
Yet, its existing systems software is inadequate in fully utilizing them.
To this end, my thesis features a series of novel systems designs that help these edge platforms run more efficiently and securely.

\subsection{Background: heterogeneous edge platforms}

Emerging edge platforms\footnote{We use ``edge'' to refer to embedded/mobile Arm SoCs by convention} are armed with abundant, heterogeneous computing resources:
for energy efficiency, in addition to Arm CPUs they have microcontroller-like peripheral cores which run a few $\times$ slower than the CPU but are 100 $\times$ more efficient;
they are equipped with diverse IO devices and accelerators, including DSPs, GPUs, DMAs; 
for security, they are guarded by Arm TrustZone Trusted Execution Environment (TEE) which partitions the SoCs into secure/normal world and isolates security-sensitive execution from the normal world OS (e.g. Linux). 
Figure~\ref{fig:thesis} shows a typical software/hardware stack of the heterogeneous edge platform.

\input{fig-thesis-overview}

\subsection{Challenges to systems software (OS and Runtime)}
\label{sec:thesis:challenge}

Despite the rich hardware computing resources, existing systems software on edge platforms fails to fully utilizes them and faces two key inadequacies as follows.

\paragraph{First, poor energy efficiency.}
As edge platforms are often battery-powered, energy efficiency is crucial to them. 
However, as demonstrated by prior work~\cite{livelab,mobisys16-wear,central-pm-asplos}, they often suffer from energy drain and have poor energy efficiency. 
We discover two key bottlenecks: 
\begin{myitemize}
	\item 
	\textbf{Lack of system support for energy accounting.} 
	Existing systems provide no reliable, accurate energy accounting facilities. 
	As a result, there is no means for apps running on the edge platform to tell their actual power consumption and adapt towards better efficiency, which is a long desired goal~\cite{odyssey}. 
	
	\item
	\textbf{Large CPU idle epochs.} 
	CPU execution is not efficient, either.
	In many driver workloads, there exist small, yet accumulatively large CPU idle epochs~\cite{zhai17hotmobile};
	in ML inference, which is an increasingly important use case for edge platforms, a CPU also has to idle for long, waiting for IO~\cite{dnn-mobile-imc}.
	While the idle epochs being necessary, the edge platform wastes energy on doing nothing. 
	
\end{myitemize}

\paragraph{Second, compromised security goals.}
As an isolated execution environment, TrustZone TEE and its runtime kernel (e.g. OPTEE-OS~\cite{optee}) lacks filesystems and device driver support.
As a result, apps of TEE (i.e. trustlets) must forward the file calls, IO job requests to OS and rely on its software stack in the normal world for execution.
This creates two security risks which break the data integrity and confidentiality goal of TrustZone TEE:

\begin{myitemize}
	\item 
	\textbf{External IO as a side channel.}
	As forwarding must send the arguments of a request in the clear (e.g. file offsets), they can be used to infer the input data of the trustlet, creating a side channel.
	For instance, by inferring the accessed file offsets of a SQLite query, the attacker learns the query content~\cite{obliviate}.
	
	\item 
	\textbf{Possible data leak and tampering.}
	During execution of forwarded requests, the data passes through the OS. 
	For devices without end-to-end encryption, this leads to possible data leak and tampering: a malicious OS (including its drivers) may peek into the data content, tamper with it, and feed the trustlets with tampered data.
\end{myitemize} 

The above challenges are exacerbated by the ``ossification'' of existing systems software.
That is, the edge platforms run commodity Linux kernels and it is unlikely to see a full swap of the software stack.


\subsection{Accomplished work}

My thesis, comprising four accomplished pieces have addressed the above challenges from the angle of ``ossified'' kernel software, in a holistic manner -- they leverage the existing, mature interfaces between software/hardware, perform surgical modifications to kernel subsystems, and can easily integrate with Linux kernel.
In the remainder of the section, I will describe briefly each piece by answering the following questions:
\begin{itemize}
	\item 
	Why does it matter? 
	
	\item 
	What are the key innovations \& results? 
	
	\item 
	What are the contributions to the field?
\end{itemize} 

\subsubsection{Redefining power awareness (Eurosys'18~\cite{psbox})}
\label{sec:thesis:psbox}

\paragraph{Why important?}
Power awareness is desired by apps for long; 
by knowing its own power consumption, an app can dynamically adjust its runtime behavior (e.g. throttle data transmission bandwidth, vary streaming fidelity), thus achieving better energy efficiency.
However, in the existing approach an OS often meters system power and divides it among apps. 
Since the impacts of concurrent apps on system power are entangled, this approach not only makes it difficult to reason about power and but also results in power side channels, a serious vulnerability.

\paragraph{Key innovations.}
We contribute a novel kernel OS principal called \psb{} (psbox, \circled{1}), provided to apps.
A psbox enables one app to observe the fine-grained power consumption of itself running in its vertical slice of the hardware/software stack. 
The observed power is insulated from the impacts of other apps.
We support the psbox through two new kernel extensions: resource ballooning and power state virtualization. 
The former grants a psbox exclusive use of resource partitions at fine spatial or temporal granularities; it meters and reports the power of resource balloons. 
The latter virtualizes hardware power states for every single psbox upon exit and re-entry, eliminating power side channel.

\paragraph{Key results.}
We implement psbox for a variety of major hardware components, including CPU, GPU, DSP, and WiFi interface on two embedded platforms.
Psbox keeps an app's power observations highly consistent even when the app co-runs with other different apps. 
Across these runs, the app’s energy, as observed by the app itself, differs by less than 5\%; 
by contrast, energy shares reported by a prior approach differ by up to 60\%.

\paragraph{What matters to the field?}
Power sandbox is the first work that recognizes the power entanglement problem, which makes prior energy accounting approaches inadequate;
it is the first kernel mechanism to address the problem and empowers apps with their power consumption.

\subsubsection{Bridging monolithic kernels to peripheral cores (USENIX ATC'19~\cite{transkernel})}
\label{sec:thesis:dbt}

\paragraph{Why important?}
A major energy drain of smart devices is ephemeral tasks driven by background activities. 
To execute such a task, the OS kernel wakes up the platform beforehand and puts it back to sleep afterward. 
Such kernel executions are inefficient as they mismatch typical CPU hardware. 
They are better off running on a low-power, microcontroller-like core, i.e., peripheral core, relieving CPU from the inefficiency.

\paragraph{Key innovations.}
We contribute a new OS structure, in which a lightweight virtual executor called \dbt{} (\circled{2}) offloads specific phases from a monolithic kernel. 
The OS has a set of novel designs. It translates stateful kernel execution through cross-ISA, dynamic binary translation (DBT); it emulates a small set of stateless kernel services behind a narrow, stable binary interface; it specializes for hot paths; it exploits ISA similarities for lowering DBT cost.

\paragraph{Key results.}
In 10K SLoC, we implemented a transkernel prototype called ARK atop an ARM SoC.
ARK offers complete support for device suspend/resume in Linux, capable of executing diverse drivers that implement rich functionalities (e.g., DMA and firmware loading) and invoke sophisticated kernel services (e.g., scheduling and IRQ handling).
As compared to native kernel execution, transkernel only incurs 2.7× overhead, 5.2×
lower than a baseline of off-the-shelf DBT. 
It reduces system energy by 34\% under real-world usage.

\paragraph{What matters to the field?}
The transkernel represents a new OS design point for harnessing heterogeneous SoCs. 
It contributes a key insight: while cross-ISA DBT is typically used under the assumption of efficiency loss, it can enable efficiency gain, even on off-the-shelf hardware.

\subsubsection{Enabling private file services for TrustZone via deception (Under review)}
\label{sec:thesis:enigma}

\paragraph{Why important?}
As TrustZone TEE lacks filesystem implementations, the in-TEE apps (trustlets) often invoke external filesystems of a normal world OS for file services (e.g. persist the collected sensor data, access user credentials).
While filedata can be encrypted, the file activities, including file operation types (e.g. read/write), sizes/offsets, and access occurrence (e.g. “the trustlet just created a file”) must be sent in the clear.
From the received file activities, the OS can infer a truslet's secrets such as input data, compromising the trustlet's privacy. 

\paragraph{Key innovations.}
We propose Enigma (\circled{3}), a deception-based defense injecting sybil file activities as the cover of actual file activities.
Enigma contributes three new designs. 
(1) To make the deception credible, the TEE generates sybil calls by replaying file calls from the TEE code under protection. 
(2) To make sybil activities cheap, the TEE requests the OS to run K filesystem images simultaneously. Concealing the disk, the TEE backs only one image with the actual disk while backing other images by only storing their metadata. 
(3) To protect filesystem image identities, the TEE shuffles the images frequently, preventing the OS from observing any image for long.

\paragraph{Key results.}
We build Enigma on Raspberry Pi 3, which works with unmodified EXT4 and F2FS shipped with Linux. 
We show that Enigma can concurrently run as many as 50 filesystem images
with 37\% disk overhead (less than 1\% of disk overhead per image). 
Compared to common obfuscation for hiding addresses in a flat space, Enigma hides file activities with richer semantics. 
Its cost is lower by one order of magnitude while achieving the same level of probabilistic security guarantees.

\paragraph{What matters to the field?}
Enigma is the first system to guard the external IO of TrustZone.
Its deception approach opens the door for a TEE to external untrusted OS services.

\subsubsection{Enabling TrustZone secure IO via minimum viable device drivers (Eurosys'22~\cite{driverlet})}
\label{sec:thesis:driverlet}

\paragraph{Why important?}
Designed for IO-rich client devices, TrustZone features secure IO, allowing TrustZone apps (trustlets) to access IO devices without being known or tampered by the OS.
However, Secure IO remains largely untapped today due to the difficulty in implementing device drivers for TrustZone.

\paragraph{Key innovations.}
We present a new model called the driverlet (\circled{4}) for deriving device drivers for TrustZone.
It contributes a key insight: instead of reusing drivers \textit{code}, we may reuse driver/device \textit{interactions} from mature Linux driver via record and replay. 
Ahead of time, developers exercise a full driver and record the driver/device interactions; 
the processed recordings, called interaction templates, are replayed in the TEE at run time to access IO devices.
The interaction template ensures faithful reproduction of recorded IO jobs (albeit on new IO data);
it accepts dynamic input values; it tolerates nondeterministic device behaviors

\paragraph{Key results.}
We build driverlets for three devices MMC, USB Mass, and a CSI Camera on RaspberryPi 3.
We show driverlets are easy to build and have sufficient performance to trustlets: 
it only takes a few days to build a driverlet while porting/implementing a driver takes at least months;
with driverlets, trustlets can execute over 100 SQLite queries per second (1.4$\times$ slower than a full-fledged native driver) and
capture images at 2.1 FPS from a CSI camera (2.7$\times$ slower).

\paragraph{What matters to the field?}
Driverlets fix the key missing link for secure IO, and for the first time open a door for trustlets to access complex yet essential devices.




%6\subsection{Common principles}

==> method__Feng_Dahua_____________________2025-01-08_.tex <==
% !TeX root = main.tex

%\section{A case for elastic model management}
%\section{A case for managing \tfm{} in full elasticity}
\section{Method}
%\section{Motivations: high cold start inference latency of Transformers}
\label{sec:method}

\subsection{Choices of hardware}
We use several servers and devices to conduct our experiments. We mainly focus on the devices with comparable costs that can be afforded by regular research groups and institutions.

For Nvidia devices, we conduct experiments on servers with four distinct models of middle to high end consumer and professional GPUs. Specificaly, our setup consists of: 1) Quadro RTX 4000 with 8 GB of VRAM; 2) GeForce RTX 2080Ti with 11 GB of VRAM; 3) GeForce RTX 4090 with 24 GB of VRAM; 4) RTX A6000 with 48 GB of VRAM. We do not include RTX A100 or similar products popular in data centers because their limited availability, especially when ordered in smaller quantities, and prohibitively high prices.

For Apple Silicon devices, we conduct experiments on three M2 series models: 1) Mac Pro with M2 Ultra chip of 192 GB unified memory; 2) Mac Pro with M2 Max chip of 64 GB unified memory; 3) Macbook Pro with M2 Pro chip of 32 GB unified memory. \xzm{Add Macbook to} Table \ref{tab:deviceinfo}.

% Since we mainly consider the devices with a comparable device, so some of delicated GPU devices, such as A100, will not be in the scope of our discussion.

% \textbf{justify the selection of these devices.}

% -- similar price??? similar year??
% \xzlNote{fix this}

% Also: need to include not only Mac studios, but also macbook pros. 

%would have to say: no way Mac can compare to A100. 
%\xzlNote{Dec 5: justify this: that we dont consider A100}


% \xzlNote{Dec 5: M2/M3 pro possible?}

% \xzm{I have tried running GPT-2 large on M2 Pro with 32 GB memory, and it is working. However, I do not think we need to report it as a major result. Our setting is more workstation-focused where Max and Ultra chips are more common.}

% \xzlNote{Dec 15: still think it would be nice to do "Pro" -- a popular choice of Macbook. Btw, I think Macbook has far more sales than Mac studios}

Table~\ref{tab:deviceinfo} shows the single-precision compute power and the price of each devices \cite{applem2pro,applem2ultra,gpuprice}.
% \xzlNote{need citations}

\input{tab-deviceinfo}

%\xzlNote{Dec 5: list numbers of cores (note apple and NV's core def are different; can use extra words in table)}


\subsection{Workloads}
\paragraph{Pretraining and finetuning large models}
In our experiment, we mainly select a representative set of the most widely used workloads in the training and fine-tuning of large models. Specifically, we conduct experiments on two modalities of data, i.e., speech and text.

For speech, we finetune Whisper, a pre-trained automatic speech recognition model designed to transcribe spoken words into text with high accuracy for multiple languages and dialects~\cite{radford2022robust}. Based on the Transformer architecture~\cite{vaswani2017attention}, Whisper is computationally intensive, requiring a lot of memory and processing resources to manage its large number of parameters and operate efficiently on complex audio data. We use the medium and large variations of Whisper.

For text, we both pretrain and finetune GPT-2~\cite{radford2019language}, a classic large language model that precedes Whisper but is built on the same Transformer architecture. The computational complexity and memory footprint of GPT-2 is slightly less than that of Whisper, making it a great example of examining whether less computationally capable Apple Silicon devices can be used in pretraining rather than merely fine-tuning. We use the large and XL variations of GPT-2.

\xzlNote{how about convolution etc} \xzm{we will run conv in the BLAS section, we can cite that conv models are smaller and comparably less demanding, and omit its discussion here.}

% \xzlNote{need to run more models} \xzm{updated}
We evaluated the model pre-training and fine-tuning under different settings. When all of the large model is stored in VRAM or memory, the training process become memory-constrained. If the memory is not sufficient to hold both the model and the training data, zero-offload~\cite{ren2021zero}, which can offload part of the model to the CPU or DRAM etc., needs to be applied to ensure the training can be processed smoothly. We list the total parameters and theoretical memory consumption of each model in \autoref{tab:workload}. In practice, the runtime memory footprint is slightly larger since there are other background processes running at the same time. Depending on the total available memory on the device we evaluate, these workflows fall under different scenarios as introduced in \autoref{fig:finding:scenariobar}. We outline the corresponding memory scenario for each device and workload combination in \autoref{tab:scenarioconfig}.
\xzlNote{connect to figure 2} \xzm{updated, to be updated again with all results}

%There are five configurations of Whisper checkpoints, with varying model sizes. 
%The size we select, the medium size, contains 24 layers with the width of 1024, and 16 attention heads. The total number of parameters it contains reaches 769M.

We select the time required for a single pass during training and the memory footprint during training as the metrics for our experiments. In particular, for Apple Silicon, we also observe the number of page faults that occurred during training to try to explain the training performance of Apple Silicon. In addition, we were also concerned about the thermal and power issues during training.

\paragraph{System-level measurement} macOS maintains a dynamic swap that serves as an extension to the SoC memory when the latter runs out of space. This allows for a memory-intensive application to run without issues. However, the additional swap is not free to use since its bandwith and read-write speed are much lower than the memory itself. Therefore, we measure the number of page faults, one of the most common and costly system calls, over the time of the workload when our workload reaches the SoC memory limit. It can help us understand the memory access pattern, and how it may introduce overheads on the operating system, and potentially undermine the benefit brought by the unified memory.

\paragraph{Micro benchmarks} During the whole process of LLM training, the operators mainly contain matrix-matrix product, matrix-vector product and vector-Jacobian product, so we conduct experiments on a curated set of operators with various tensor shapes respectively. We perform these experiments on CUDA and MPS of Pytorch and MLX to make comparisons of their performance. At this point we are concerned with the total time required to complete the whole operation, the time taken for the calculation process, and the time required to launch the kernel.

\paragraph{ZeRO-Offload} When the 


% Training startegy... in the face of memory constriant. 

% all in memory... 

% zero offload, etc. 





==> motiv-char.tex <==
% !TeX root = main.tex

\subsection{subsection}
%\subsection{\Tfm{}s challenge existing execution paradigms}
\label{sec:motiv:char}

%Next, we explain why existing techniques are inadequate to overcome these challenges. 

%\paragraph{What matters to inference on a mobile device?}
%\paragraph{\Tfm{} challenges to a mobile device}
%For instance, DistilBERT~\cite{distilbert} is designed for mobile devices as a smaller variant of BERT~\cite{bert}, and is over 200MB, two orders of magnitude larger than mobile vision networks~\cite{}.
%It hence challenges the capability of existing execution paradigms in managing $T$ and $M$. 

%Despite many being highly redundant~\cite{head-prune-acl19}, a typical pretrained model is of a few hundred MBs (e.g. BERT~\cite{bert} model size is over 400MB). 
%This contrasts with CV models, which are much smaller with less redundant parameters. 
%a known big Convolutional Neural Network (CNN). 
%to inference latency $T$ and memory consumption $M$ on a mobile device. 

%\paragraph{What do mobile devices care?}
%In executing an inference task, a mobile device cares about the execution latency $T$ and memory consumption $M$. 
%On one hand, a mobile device is latency-sensitive, as it is used by an end user who expects a rapid response upon invocations, e.g. by meeting a target latency $T$.
%%For a smooth user experience~\cite{falcon-mobisys12}, it is vital that the system be responsive and rapid upon invocations, e.g. by meeting a target latency $T$. 
%However, given the medium to low storage throughput of a mobile device (e.g. 80MB/s), it takes a few seconds to load a (large) \tfm{} model, which is unacceptable to user experience. %given the medium to low storage throughput of a mobile device, e.g. 80MB/s;
%%mobile app interactions are brief, for less than a minute~\cite{livelab};
%%interactions with IPAs are even shorter, for only a few seconds~\cite{ipa-study-denmark,tsaiFasterResponsesAre2019}.
%%During such a short period, human attention is a scarce resource~\cite{proj-aura}.
%%It is vital that the system be responsive and rapid upon invocations by meeting a target latency $T$, for a smooth user experience~\cite{falcon-mobisys12}. 
%On the other hand, a mobile device is memory constrained, with only a few GBs of memory~\cite{marvin-atc20}. 
%Yet, such a space is crowded with many co-located mobile apps.
%%Mobile devices are resource-constrained...
%Their sporadic usage patterns~\cite{livelab} further render hosting large models always in memory non-economic.




%Given aggressive memory management of mobile OSes \xzlNote{cite}, 
%such an app with abnormally large memory footprint is likely to be quickly killed by the OS as the system memory pressure increases. 


%Yet, the approach trades IO for a huge $M$, a noticeable proportion of the total system memory.
%It is undesirable for the following reasons: 
%%1) it is unfair to other co-existing apps by reserving a few hundred MBs, which is a few $\times$ more than what an app normally needs~\cite{marvin-atc20};
%1) it breaks the unspoken fairness contract between OS and tenant apps by reserving a few hundred MBs, which is already a few $\times$ more than what an app normally uses~\cite{marvin-atc20};
%2) as mobile apps often exhibit sporadic and ad hoc usage patterns~\cite{livelab,mobile-study-chi15}, it is not economic to pin large $M$ just to cater such pattern;
%%further create difficulty in mobile memory management~\cite{marvin-atc20}. %render hosting large models always in memory non-economic.
%3) the a few hundred MBs are only for \textit{a single model}, whereas it is common for multiple NLP tasks to co-exist. 
%%2) in the constrained memory space, the OS of the device must accommodate multiple tenant apps~\cite{acclaim-atc20} and ensure fairness of responsiveness~\cite{asap-atc21}, too;
%%it shall not sacrifice the user experience of other apps.




%It fully offloads the memory management responsibility to OS via file-backed abstraction, which leads to an ``all or nothing'' dichotomy in memory.


%The two steps are sequential -- the inference execution must wait for the completion of model loading to begin.
%This approach exposes the model loading IO to the user-perceived delay, increasing it to as high as a few seconds. 

%Given the medium to low storage throughput of a mobile device (e.g. 80MB/s), it takes a few seconds to load a (large) \tfm{} model, %given the medium to low storage throughput of a mobile device, e.g. 80MB/s;

%\xzlNote{note one paper is for cloud based inference only}

% \paragraph{\textit{Third, naive pipelining.}}

%\xzlNote{(for inference): cite Hongyu's and others}

% e.g. loading a layer of DistilBERT can take several hundred ms while executing it takes less than 100 ms. 
%e.g. 3.1 seconds  of IO vs 0.4s of compute. %IO delay is 10X larger than that of computation.

% be tens of of MB/sec.
%which limits how fast \textit{streaming} ML parameters can be streamed from storage. 
% which is not suitable for \textit{streaming} ML parameters with low delays. 
%This is caused by the large model size plus a medium to low storage throughput (e.g. 80 MB/s on Odroid) of a mobile device.
%		To make matters worse, the large NLP model composition (hundreds of MBs) plus a medium to low storage throughput (tens of MB/s) of mobile SoCs further causes .
%The high skewness renders the naive pipelining strategy futile, because IO and computation can hardly overlap.
%For example, loading a layer takes nearly 400ms while computing on one takes only 100ms; 
%e.g. overlap layerwise load and computation. 
%This is because IO is the bottleneck of the pipeline: loading a layer takes 500ms while computing on one takes only 50ms; 
%The result is a pipeline bottlenecked by IO with large bubbles, which stalls on loading at each layer;

%its end execution delay is not much different from \textit{load \& execute}.

%comparing with each paradigm in 

\begin{comment}
A case study of cold start. Compare BERT \& DistilBERT with no pipelining (existing) V.S. layerwise pipelining (naive). Long delays regardless, unacceptable to UX.
minor: low energy efficiency (CPU idle). 

\textbf{An outline for the section}
\Note{to udpate based on intro}
\begin{myitemize}
	
	\item 
	\S2.2 NLP inference at the edge. 
	
	\textbf{Context:}
	\begin{myitemize}
		\item 
		Scenario: on-demand \& bursty pattern (IPA as a mobile app), in short intervals/sessions (<1min) -- latency-sensitive.
		\item 
		Platform: small memory (a few GBs), storage throughput limited, a few cores -- resource constrained.
	\end{myitemize}
	
	\textbf{Problem: rigid resource management}
	
	We study three popular inference engines: Torch, TF, NCNN (?) and find...
	
	Existing engines are designed mainly for execution with a focus on programmability (simple inference APIs) and computation efficiency (SIMD insns, memory layout optimization, etc.).
	
	Assuming model as a rigid binary file (i.e. it is OSes' responsibility to manage the file), they often omit or oversimplify model management.  
	It may not be a problem for cloud, i.e. ML serving, large RAM, throughput-sensitive;
	the paradigm misfits a mobile SoC, i.e. bursty, resource-constrained, latency-sensitive. 
	
	
\paragraph{Inadequacies}	
	We find following two key design inefficacies:
	\begin{myitemize}
		\item 
		%		\textit{1. Huge, rigid model file creates memory management inefficiencies}. 
		\textit{1. Huge, rigid model file contrasts fluctuating, dynamic memory pressures.}
		
		It fully offloads the memory management responsibility to OS via file-backed abstraction, which leads to an ``all or nothing'' dichotomy in memory.
		Examples: Pytorch (XXX API), TensorFlow (XXX API), NCNN (XXX API) -- all file-backed; interact with OS via simple file IO. 
		\Note{can we find any data/tangible problem like cold start?} 
		
		The dichotomy is rigid and unfit for the mobile SoC with scarce memory.
		Reasons are:
		\begin{myitemize}
			\item 
			1) under high memory pressure (e.g. less than 100MB available), OS needs to evict pages of many other (XXX how many, average memory consumption of mobile app=?) apps to make room for the large model, which is unfair to others. 
			
			\item 
			2) vice versa, OS tends to reclaim the large space occupied by the model, which likely leads to thrashing when apps are constantly and frequently used then shut down in a bursty pattern~\cite{mobile-usage-chi16,mobile-usage-sigir20}.
			Furthermore, it is not economic to always keep such a large, full-fledged model.
		\end{myitemize} 
		
		\item 
		\textit{2. Lack of IO/computation parallelism causes long inference delay.}
		
		The engine modularizes the model loading and inference design, manages them in rigid isolation, and misses the opportunity of overlapping IO with computation.
		The result is IO blocks inference: inference can only start after the full model has been loaded from disk to memory.
		%		Model loading designed in isolation with inference computation
		For instance, all APIs invocations of Torch,TF, etc. follow the such same paradigm: first call XXX (synchronous API) to load model, then call YYY to start inference.
		
		Such a design may be tolerated by cloud deployment, as it is throughput-oriented, whose (blocking) IO overhead is amortized among many subsequent inference calls. 
		Yet, on mobile platforms, it may cause long, user-perceivable delays (a few seconds), which is unacceptable to user experience.
		\textbf{Case study} 
		The problem is known as \textit{cold start}, a tangible bad fruit borne by the lack of above inefficacies.	
		
		\begin{itemize}
			\item 
			We profile cold start inference on 3 engines (torch, tf, ncnn -- no tfm?) on a dev board, breaking down the IO delay vs compute delay. 
			
			\item
			We further characterize the delays by layers, reporting their respective delays. 
		\end{itemize}
		
		As the case study shows, there exists a high skewness in IO v.s. computation delay, e.g. IO delay is 10X larger than that of computation.
		This is caused by the large NLP model composition (hundreds of MBs) plus a medium to low storage throughput (tens of MB/s) of mobile SoCs.
		%		To make matters worse, the large NLP model composition (hundreds of MBs) plus a medium to low storage throughput (tens of MB/s) of mobile SoCs further causes .
		The high skewness renders naive pipelining strategy futile, e.g. overlap layerwise load and computation. 
		This is because IO is the bottleneck of the pipeline: loading a layer takes 500ms while computing on one takes only 50ms; 
		the pipeline has large bubbles (i.e. 450ms) and stalls on every loading, whose end delay is not much different from the baseline (<10\% improvement). 
		
	\end{myitemize}
	
	\textbf{Summary \& design goals}
	To make mobile NLP inference more efficient, we advocate for a more ``responsible'' engine which manages system resource in elasticity.
	
	Specifically, two types of coordination are needed: 
	1) OS-engine memory management. 
	Engine needs to takes the initiative to manage model memory.
	2) IO/computation for exploiting parallelism. 
	Needs to construct an elastic pipeline to offset the high IO/Computation delay skewness.
	
	Achieving the two coordination requires three dimensions of resource need elasticity: IO/Computation/Memory. 
	
	\textbf{Goals} We target:
	\begin{myitemize}
		\item 
		Deadline-driven inference, i.e. for consistent delay, no long delay due to cold start, while achieving maximum accuracy. 
		
		\item 
		Fine-grained/elastic adaptation to OS memory pressure. May preload (inflate the model or increase fidelity) and unload (deflate the model or downgrade fidelity)
	\end{myitemize}
	
	We next describe why existing techniques are inadequate: which coordination and elasticity is not yet achieved, and bars us from achieving the goals.  
	
\end{myitemize}

%\input{fig-lat-breakdown}

\end{comment}


%\subsection{To update: --- --- Case study: cold start inference}






==> motiv-memo.tex <==
% !TeX root = main.tex

\subsection{\sys{} motivations}


==> motiv-prior.tex <==
% !TeX root = main.tex

\subsection{subsection}

% To reduce $T$ and/or $M$, 

%dy distilling knowledge~\cite{knowledge-distillation} from BERT, 
 % while retaining 97\% of the accuracy.

 
%The result is a heavy tension between compression ratios and accuracy. As we will show in \sect{eval}, for $T$ and $M$ to be small enough, the \tfm{} has to be aggressively compressed (e.g. to have a very small widths/depths), leading to inferior accuracy. 



%because they do not 
%First, a fixed compression strategy such as DistilBERT does not to accommodate diverse hardware capabilities of mobile devices. 
%Albeit one compressed model may enable IO/computation overlapping on a device and facilitate naive pipelining, it is unlikely to work with other devices, as they are increasingly heterogeneous~\cite{transkernel}.
%More importantly, model compression only scales the model size without changing the landscape of execution paradigm which is bottlenecked by IO.

%It does not eliminate 



\begin{comment}
\textit{How about compressing the models?}
Alternatively, one may compress a \tfm{} model to reduce the number/precision of parameters, hence the file size. 
Common techniques include \ul{structured pruning} which reduces the width and/or depths of a \tfm{}~\cite{distilbert,mobilebert,dynabert,layerdrop},
\ul{weight sharing} which makes \tfm{} layers to share same set of parameters~\cite{albert, universal-transformer},
and \ul{quantization} which reduces the full precision of parameters (often in 32 bits) to low-bit representations or integers~\cite{binarybert,bibert}.
However, these approaches share a key inadequacy -- still, the (cold) inference can only start as soon as the model is loaded.
They hence face a dilemma between latency and accuracy: a low compression ratio (e.g. DistilBERT~\cite{distilbert} is 2$\times$ smaller than BERT~\cite{bert}) cannot meet the latency goal (e.g. a few hundred milliseconds) because it still takes seconds to load the model;
a high compression ratio (e.g. BinaryBERT~\cite{binarybert} is 24$\times$ smaller) meets the latency goal while suffering from inferior accuracy, e.g. a few full GLUE scores lower, which is deemed significant in NLP literature~\cite{bibert,binarybert}.



\xzlNote{compress to 1/4 page}
\paragraph{Existing techniques are inadequate.}
We consider two common approaches to reducing cold inference latency as follows.
\begin{myenumerate}
	\item 
	\textit{How about pinning the model files in memory for good?}
	The approach conceptually eliminates cold inference, as the model files are always in memory.
	Yet, it eschews the IO time waiting for storage at the cost of high memory pressure, and is undesirable. 
	This is because:
	1) transformer model files are as large as a few hundred MBs, which take a significant portion of memory space of commodity mobile devices (e.g. a few GBs~\cite{iphone13});
	2) in the constrained memory space, the OS of the device must accommodate multiple tenant apps~\cite{acclaim-atc20} and ensure fairness of responsiveness~\cite{asap-atc21}, too;
	it shall not sacrifice the user experience of other apps.
	As a result of resource contention, cold inference happens frequently on today's mobile devices, causes ``latency variability''~\cite{dnn-mobile-lat-var}, and degrades user experience.
	
	\item 
	\textit{How about compressing the models?}
	Alternatively, one may compress a \tfm{} model to reduce the number/precision of parameters, hence the file size. 
	Common techniques include \ul{structured pruning} which reduces the width and/or depths of a \tfm{}~\cite{distilbert,mobilebert,dynabert,layerdrop},
	\ul{weight sharing} which makes \tfm{} layers to share same set of parameters~\cite{albert, universal-transformer},
	and \ul{quantization} which reduces the full precision of parameters (often in 32 bits) to low-bit representations or integers~\cite{binarybert,bibert}.
	However, these approaches share a key inadequacy -- still, the (cold) inference can only start as soon as the model is loaded.
	They hence face a dilemma between latency and accuracy: a low compression ratio (e.g. DistilBERT~\cite{distilbert} is 2$\times$ smaller than BERT~\cite{bert}) cannot meet the latency goal (e.g. a few hundred milliseconds) because it still takes seconds to load the model;
	a high compression ratio (e.g. BinaryBERT~\cite{binarybert} is 24$\times$ smaller) meets the latency goal while suffering from inferior accuracy, e.g. a few full GLUE scores lower, which is deemed significant in NLP literature~\cite{bibert,binarybert}.
	
\end{myenumerate}


Model compression is widely used to reduce both IO and Compute time by reducing the total number of parameters or the complexity of math operations. 

\textbf{Motivate the use of finer-grained units}
\Note{How about loseless compress quantized layer and load it?}
The rational is quantized weights have lower entropy. 
We can load them, and decompress in memory; 
the total latency count towards as new IO.

\textbf{We can but the additional decompression costs is still unacceptable.}  
Quantizing a layer -- 55M raw file, in 3-bit. 
After compression, 90\% of size is reduced, i.e. to only 2-5MB.
bzip has highest compression ratio, can reduce it to 2.6MB. 
gzip has lower compressino ratio, with 4.6MB.

Decompression takes 150ms for gzip, and 1.1s for bzip;
both decompression processes are parallelized. 
Even for faster decompression such as gzip, it cannot meet deadline, e.g. 500ms.

This motivates a finer grained partitioning strategy.

\Note{useful but very subtle}
\textbf{Can we compress the shards?}
If we do so, each shard is around 5MB in ``restored'' quantized from (1M parameters in 32-bit precision floating point numbers which are restored from centroids)

After gzip compression, the shard gets 90\% smaller, which becomes only 440KB. 
The new IO time hence becomes load the compressed + decompress in-memory.	
The time is around 5$\sim$10 ms (disk load) \& 40ms decompress, in total around 50ms. 
The time is roughly same as load an uncompressed shard.
\end{comment}

\begin{comment}
%%  not useful
\Note{shard upgrading??}

\Note{It seems quantized shards can be switched efficiently without significant reloading costs:}

It can be done in the following way: 

\begin{itemize}
\item High to low: can be done by directly converting high bits to low bits. 
E.g. A value 7 (0b111) in 3-bit shard can be converted to a value 3 (0b11) in 2-bit shard. 
A value 0 (0b000) in 3-bit shard can be converted to a value 0 (0b00) in 2-bit. 
Some values are in the middle, can be rounded up or down. 
This is doable because how we calculate the centroids -- by sorting \& binning \& calculate arithmetic mean. 
\textbf{This can be done without reloading and has 0 precision loss.}
\Note{what's the usecase??}

\item Low to high: 
Must reload for accurate reconstruction of values -- the loss of precision must be compensated. 
An efficient way to switch may be loading a \textbf{delta encoding} from low to high bits. 
Since there are only a few values, it shall have low entropy and highly compressible. 
\end{itemize}
\end{comment}


==> motiv-scenario.tex <==
% !TeX root = main.tex
\paragraph{Motivating scenario.}
\sys{} targets an interactive NLP scenario with intelligent personal assistant (IPA) on a multi-tenant mobile device.
In the scenario, a user typically interacts with the IPA for querying weather/personal emails/medical records~\cite{ipa-survey}, managing tasks~\cite{myersIntelligentPersonalAssistant2007} etc.
A typical interaction takes 2-3 turns and lasts for a few seconds~\cite{ipa-study-denmark};
during the interaction, the length of each utterance is often 10-20 words~\cite{tsaiFasterResponsesAre2019}. 

Under the hood, the IPA may run the pretrained Transformer language model to directly generate responses by running downstream tasks such as question answering~\cite{dynabert}, and dialog generation~\cite{dialogpt}.
Alternatively, it may generate responses from templates. 
It does so by filling the blanks in the templates~\cite{mdfn-aaai21} or selecting existing answers from its knowledge base, based on intent classification~\cite{dbpedia-chatbot} and sentiment analysis~\cite{yasudaDesigningChatbotSystem2021} results of the Transformer model.

==> motiv.tex <==
% !TeX root = main.tex

%\section{A case for elastic model management}
%\section{A case for managing \tfm{} in full elasticity}
\section{Motivations}
%\section{Motivations: high cold start inference latency of Transformers}
\label{sec:motiv}


%\begin{myenumerate}
%	\item 
%	Transformer on mobile
%		\begin{myitemize}
%			\item 
%			Tfm primer.. 
%			Large model sizes... 
%			\item
%			Why challenging on mobile? Resource constraints, target latencies, memory consumptions.... Ideal memory footprints...
%		\end{myitemize}
%	\item 
%	Existing execution paradigm... 
%	\begin{myitemize}
%		\item 
%		Load and execute
%		\item 
%		Naive PL
%		\item 
%		All in mem
%	\end{myitemize}
%	\item 
%	Why model compression is inadequate? 
%	\begin{myitemize}
%			\item 
%			Distilbert
%			\item 
%			Dynabert
%	\end{myitemize}
%\end{myenumerate}


\input{motiv-bkgnd}

\input{motiv-char}

%\input{motiv-memo}

\input{motiv-prior}




==> plan.tex <==
% !TeX root = main.tex

\section{Project plan \& timeline}

\paragraph{\textit{Research milestones}}
We have set up the research milestones for the project as follows.
\begin{myitemize}
	\item 
	\textbf{Milestone I.}
	We have done preliminary experiments (\S\ref{sec:design:sharding}), which have shown the promise of the high accuracy of the proposed sharding strategy based on attention heads.
	We plan to further apply the proposed strategy to more pretrained models, such as RoBERTa~\cite{roberta} and DistilBERT~\cite{distilbert}. 
	
	\item 
	\textbf{Milestone II.}
	We plan to conduct more comprehensive experiments on different planning schedules. 
	Current preliminary results in \S\ref{sec:design:planning} have demonstrated feasibility. 
	It is yet to be explored if current strategy is already optimal and whether a better planning exists.
	The outcome is a concrete and detailed planning algorithm. 
\end{myitemize}

We plan to achieve the above milestones by \underline{April 30th, 2022}.


\paragraph{\textit{Implementation \& evaluation plan}}
We plan to implement the proposed system in Python with PyTorch framework~\cite{pytorch-web}, using DynaBERT~\cite{dynabert} as the backbone network.
\ul{For the model sharding task}, we plan to modify the existing modeling utility. 
Specifically, we will first quantize individual attention heads.
We will then introduce shards as a new abstraction and implement the new interface which operate on shards. 
\ul{For the shard planning task}, we will first implement the devised planning algorithm, which accepts the device's IO/Compute profile and a deadline as inputs, and generate an optimal IO/Compute plan. 
Second, we plan to refactor the PyTorch framework.
We will implement the proposed pipeline and integrate it with the planning algorithm. 

\ul{To evaluate,} we will answer two research questions.
1) How much time does the proposed system save for cold start inference? 
We plan to set a fixed accuracy and compare the cold start inference latency of the proposed system with SOTA models~\cite{bert,distilbert,mobilebert}. 
2) What is the tradeoff between accuracy and deadlines of the proposed system? 
First, we plan to evaluate the system with different planning strategies, which give insights into \ul{the accuracy-latency implication} of IO/Compute of attention heads with different bitwidths.
Second, we plan to set a similar deadline for SOTA models and compare the resultant accuracy with the proposed system;
we will consider popular compressed BERT variants such as DistilBERT~\cite{distilbert}, MobileBERT~\cite{mobilebert}, I-BERT~\cite{ibert}, BinaryBERT~\cite{binarybert} as well as EdgeBERT~\cite{edgebert}, a deadline-aware system based on early exits.

We plan to finish the implementation and evaluation by \underline{July 31st, 2022}.

\paragraph{\textit{Project outcome}}
We plan to summarize the project and send the paper to premier systems venues such as ASPLOS'23, Eurosys'23, and MobiSys'23. 
We plan to open source the code artifact to cultivate further research into the cold start inference problem, as well as potential deployment and integration in popular deep learning frameworks.




==> prelim-explore.tex <==
% !TeX root = main.tex
%\subsection{Model compression is inadequate}
\subsubsection{Design space exploration}
\label{sec:motiv:design-explore}
%\textbf{Carefully discuss: can existing models/methods fit into our approach of overlapping IO vs Compute}

\textbf{TODO: review the complete landscape of weight sharing status of supertransformers}

%\textbf{Discuss the IO/Compute task in model compression techniques which reduce latency}

\textbf{Does early exit have a place here?}

Towards reducing cold inference latency of transformer, we set to overlap IO with Compute and take into account the architectural differences of different platforms. 
We explore the following designs. 

\input{fig-design-explore}

\input{fig-io-compute}


\paragraph{Why Post-training Quantization?}

There are two quantization techniques: quantization-aware training (QAT) and post-training quantization (PTQ). 
We set for the latter (PTQ) for two key benefits:
1. faster deployment. 
PTQ does not require to fine-tune the pretrained models on downstream tasks, which is time-consuming, e.g. one epoch takes a few hours on a GTX1080 Ti GPU~\cite{XXX}.
2. better data privacy.
As QAT fine tunes the model, it needs access to the whole training set, which is often not accessible due to privacy and proprietary concerns. 


\paragraph{Can we pipeline transformer layers as-is?}
As described in \sect{motiv:primer}, transformer models are stacked in layers. 
A naive approach is to take a transformer model as-is (e.g. BERT~\cite{bert}) and pipeline the compute of one layer with IO of \textit{next} layer. 

The design is shown in Figure~\ref{fig:motiv:overlap}.
While being intuitive, unfortunately, this approach barely reduces the latency: due to the disproportionate IO vs Compute time of a transformer, e.g. IO time is 6$\times$ larger than Compute on Odroid, pipelining them as-is incurs large pipeline stall, rendering it ineffectively. 
\sect{eval} will present a quantitative evaluation.

\paragraph{How about pipelining compressed layers?}
To mitigate large pipeline stalls, one may want to compress the layers instead of pipelining them as-is, which brings the IO vs Compute time closer.
Figure~\ref{fig:motiv:compress-overlap} shows the idea.

We consider the following compression techniques.
\begin{myitemize}
	\item 
	\textit{width reduction}, which can be either static~\cite{distilbert} or dynamic~\cite{dynabert}.
	However, to fully close the gap between IO vs Compute, both MHA and FFN feature dimensions need to be compressed significantly. 
	For instance, per our measurement on Odroid in Figure~\ref{fig:motiv:io-compute}, they need to be compressed by 4$\times$ -- from 768 to 192, 3172 to 793. 
	Later we show in \sect{eval} that the compression greatly limits the expressiveness of a transformer block and leads to persistent performance degradation (XX\% in SQuad for same number of layers), even for hot inference. 
	
	\item
	Other techniques such as quantization~\cite{q8bert,tenarybert}, low-rank matrix factorization~\cite{groupreduce} share the same drawback: it requires to compress a full layer to close the IO vs Compute gap; 
	the inferior performance is persistent. 
\end{myitemize}

\paragraph{Design implication:}
Coarse-grained layerwise pipelining won't work for either uncompressed or compressed;
persistent performance degradation is undesirable.
\Note{the key is not to do layerwise pipelining -- but finer grained, attention head wise pipelining.}

\begin{comment}
\Note{merge below -- note the idea of overlapping is not introduced yet, whether it is dynamic or static does not matter...}
While \textit{cold inference} receives only scant attention in literature, there are a primary body of work targeting at reducing \textit{inference} latency using model compression: by making the transformer model parameter- and compute-efficient, its IO and Compute time can thus both be reduced.

%\Note{why static vs dynamic matters}
%One may compress a transformer model to make it parameter- and compute-efficient, thus reducing both the IO and Compute time. 

To this end, common compression techniques include reducing model depth~\cite{distilbert} and/or width~\cite{mobilebert}, quantization~\cite{q8bert,tenarybert}, low-rank matrix factorization~\cite{groupreduce}, weight sharing~\cite{albert}.
Compression can also be dynamic and adaptive. 
For instance, each sentence can have a subtransformer/subnet with smaller width and depth~\cite{dynabert,layerdrop}; 
even for individual tokens, they can have different depths~\cite{spatten,ltp}. 

\paragraph{Missed opportunities.}
While being effective, model compression alone is inadequate: 

\textit{Does not overlap IO vs Compute.} 
It still waits for the full model loading completion before continuing. 
Despite the compressed models are a few times smaller than the original, IO is still the key bottleneck.
For instance, Distilbert is 4$\times$ smaller than BERT, but still taking 3 seconds in IO task. 

\textit{Poor performance.} 
Esp. for static model compression -- the performance is consistently low, compared with a full model. 
To make it worse, if one wants to reduce the IO time significantly, he has to make the model 4$\times$ narrower in MHA and includes only 2-3 layers. 
This greatly limits the expressiveness of MHA~\cite{XXX}.


\paragraph{What about \textit{static} model compression?}
One may statically compress BERT, e.g. via simplified structure~\cite{distilbert,mobilebert}, quantization~\cite{q8bert,tenarybert}.
To fit in our scenario, one may compress a layer such that its IO overlaps with Compute. 

This approach faces a key drawback of poor performance.
To overlap, it requires large compression ratio per layer. 
We show the IO/Compute vs transformer layer compression ratio in Figure~\ref{fig:motiv:io-compute}.
To effectively overlap IO with Compute, one needs to compress both dim and hidden dim so that IO may meet compute.
E.g. for Odroid, they need to be compressed by 4$\times$ -- from 768 to 192, 3172 to 793. 
The compression greatly limits the expressiveness of a transformer block and leads to performance degradation (even for hot inference). 
\Note{key argument: at the end, there is only one model in which you can overlap IO/Compute at the cost of bad performance}



\paragraph{What about \textit{dynamic} model pruning?} 
It selects a part of model parameters (subnet) from a supernet at inference time. 
There are two directions along the selection depth and width.
\begin{myitemize}
	\item \textbf{Depth}. 
	\cite{layerdrop,universal-transformer,edgebert} adaptively change the number of layers at runtime.
	
	\item 
	\textbf{Width}. 
	\cite{dynabert,hat} adjusts the width by varying the feature dimensions of attentions and FFNs. 
	%number of attention heads and neurons an FFN layer, i.e. leftmost attention heads and FFN neurons.
%		~\cite{dynabert} adjusts width by varying the number of attention heads and neurons an FFN layer, i.e. leftmost attention heads and FFN neurons.
\end{myitemize} 

The key drawbacks are: 
1) a width/depth is selected at each inference time, forming a subtransformer.
subtransformers are independent and disconnected from each other -- this does not solve cold inference because the model is always loaded fresh.
Some networks have shared weights, e.g. \cite{hat} shares FFN, \cite{dynabert} shares important attention heads and neurons in FFN;
ad hoc optimization helps accelerating loading shared parameters, but the reduction is minor (compared with).
2)\Note{Merge below}
key argument: some dynamic networks exploit the weight sharing opportunities of a supernet and its subnets but not all; the weight sharing decision is ad hoc and is not tied to hardware.
\end{comment}

% Below useful about Dynabert 
\begin{comment}
The implication is one may incrementally load parameters from subnets of the mentioned supernets;
starting from the smallest width and depth, the parameters can be gradually loaded and become the whole model.


Back of envelope calculation, $m_w, m_d$ as width and depth multiplier:

Let $m_w = \frac{1}{12}, m_d=1$. 
The pipelining strategy being load one attention head at a time. 
Load one layer takes $320ms/12 \simeq 30ms$. 
Compute on one head takes roughly same time, i.e. $30ms$, 12 full heads takes $50ms$.
This case the IO and Compute overlaps well. 
W/o considering word embedding, end-to-end latency is $30+30*12=390ms$. 
Doing this for 11 more inferences we can achieve the accuracy of $m_w=1, m_d=1$.
	
On accuracy -- on a 3-head subnet, the SST accuracy seems quite high ($91 \sim 92$), which is higher than all-shared albert. 

A challenge might be: how to choose overlapping strategies for different platforms, where the IO vs Compute is different. 
Odroid (our platform) is an ideal, coincidental case -- we can load one full slice of attention head \& FFN per time.
What if IO is slower? I.e. cannot fully load the slice within the compute boundary. 
Can our system adjust overlapping strategy? 
For instance, load one slice of attention, share its weights with FFN.
\end{comment}

\begin{comment}
\Note{bewlow for completeness, can omit}
\paragraph{Why not offload to cloud?}
This work focuses on \textit{on-device} inference.
We discuss \textit{cloud offloading} as an alternative approach for completeness.
Cloud offloading~\cite{deepcod,edgepipe} trades off the cost of compute and model loading of cold inference for network latency, where the inference is always hot in the cloud. 

%We do not aim to settle the debate which is better.
First, offloading is complementary.
It is valuable when applications need strong results because cloud is more computationally-capable. 
This does not diminish the need for on-device inference. 
Second, on-device inference guarantees (stable?)lower latency (better QoS?). 
Mobile networks are often spotty with fluctuating latencies;
in contrast, on-device NN inference latency is almost stable/deterministic due to the workload nature of matrix multiplications. 
Third, on-device inference offers higher privacy assurance, because data is never uploaded to the cloud. 
It has become increasingly popular\Note{cite}.

%If we do cloud offloading, the latency is largely bound by network roundtrip time (tens of ms), assuming a serving scenario in the cloud (more computationally-capable);
%larger models are deployed in the cloud, as well.
\end{comment}



==> prior.tex <==
% !TeX root = main.tex

\section{Accomplished work from the student}

\textbf{Liwei Guo} is a 6-th year Ph.D. student of the Computer Science Department at University of Virginia (UVA).
He was a direct Ph.D. student of the school of Electrical and Computer Engineering at Purdue University and transferred to UVA from Purdue with his advisor Prof. Felix Xiaozhu Lin in his 5th year. 

He has been focusing on making edge devices more efficient and secure, using a systematic and principled approach. 
To this end, his prior work took the angle of kernel softwares, including redesigning kernel structures~\cite{transkernel,psbox}, refactoring the storage stack~\cite{enigma,overwatch}, and reusing mature drivers via record-and-replay~\cite{driverlet}.
His work has been seen on premier systems venues such as Eurosys~\cite{psbox,driverlet} and USENIX ATC~\cite{transkernel}. 

Complementary to his prior work, the proposed project takes the angle of user software and case studies an important NLP user application, i.e. Transformer.
Together with his prior work, the proposed project completes his thesis (i.e. making edge devices more efficient and secure) in a holistic manner, covering both kernel and user software. 
 

==> recycle-next.tex <==
% !TeX root = main.tex

\subsection{Next steps}

==> recycle-prelim.tex <==
% !TeX root = main.tex

\subsection{Preliminary experiments}
\label{sec:motiv:char}

We have done the following preliminary experiments which support our design choice. 

\input{prelim-char}

\input{prelim-explore}

==> recycle/design-res-model.tex <==
% !TeX root = main.tex

% Not used....

\Note{moved from S4 -- to merge }
\subsection{Hosting the resident model in memory}

%\xzlNote{what is stored on disk; who loads shards to memory. Show the mapping (perhaps in Fig4)}
\Note{may move to overview; resident model -> shard buffer...}
\input{fig-res-model}

Based on model shards, we next present the resident model, which is long lived in memory and serves as an important cushion for hiding bootstrapping IO during inference. 
\paragraph{Formulation}
The resident model $R$ is composed of a set of in-memory, loosely coupled, and independent model shards, defined by $R=\{S(n,m,b) \mid n \leq N, m \leq M, b=2\dots6, 32\}$, where the number of shards $|R| \in [1, n\times m]$. %of the resident model shards  can only have a distinct version $b$, 
%Each shard $S(n, m, b)$ is uniquely identified by $(n, m)$, that is, at one index $(n, m)$ there exists at most one version $b$.
To save memory, at one index $(n, m)$ there exists at most one version $b$.
Figure~\ref{fig:design:res-model} shows an example R = \{S(0,0,2),  S(0,1,3), S(0,2,6), S(1,0,2), S(1,1,6)\}.

%In memory, $N$ layers of $M$ model shards stack upon each other to form a resident model.
%In the $M \times N$ grid, each cell marks a model shard $S(m, n, b)$, defined by its position ($m$-th vertical slice in $n$-th layer) and $b$-bit fidelity.
%Following the convention, we describe a resident model by its widths $M$ -- number of shards per layer, and depths $K$ -- number of such layers. 

%Besides shards, the resident model keeps miscellaneous parameters in full fidelity due to their small sizes (e.g. only 768 dimensions), including layer normalization, pooler, and classification head.

%\paragraph{Tunable knobs}
%A resident model may be adjusted and tuned along three dimensions. 
%\textit{First, width}: by adjusting $M$ per layer.
%It applies to all layers because inference computation must execute on layers with the same $M$.
%\textit{Second, depths}: by adjusting $K$, number of layers. 
%\textit{Third, fidelity}: by adjusting $b$ of individual shards.  
%By tuning the shard configuration, a resident model may be adjusted along three dimensions. 
%\textit{1) Widths and 2) depths} are adjustable through $M$ and $N$, similar to dynamic \tfm{}. 
%\textit{3) Fidelity} can be tuned by specifying the $B$ fidelity of individual shards. 

\paragraph{Operators}
\xzlNote{merge to overview. the content shall be updated}
To tune $R$ for adapting to the changing memory pressure, the system implements two operators: 
\begin{myitemize}
	\item 
	\textit{inflate(n, m, b)} pulls the $b$-bit version shard at $(n, m)$ from disk into memory. 
	When extra memory allows, it is used to append to $R$, as well as replacing an existing one with a new version $b$.
	
	\item 
	\textit{deflate(n, m)} evicts existing shards at $(n, m)$. 
	It is used to reduce resident model size when memory pressure is high.	
\end{myitemize}

%\Note{to merge}
%\xzlNote{move (some) to implementation?}
%\Note{unsure if needed}
\paragraph{Example use case}
\xzlNote{merge to Sec. overview}
The key use case of resident model is to bootstrap the pipelined inference. 
By hosting the shards of the few bottom layers, an inference starts as soon as possible when the shards of the very first layer are decompressed, instead of incurring significant IO for loading them, which takes tens of ms and is a few $\times$ than the former (e.g. 10-20ms).
Figure~\ref{fig:design:res-model} shows an example.

\xzlNote{decompression details should go to Impl.}
To begin, the system gathers shards of the first layer (L1) in the resident model and decompresses them in the working buffer. 
To decompress, the system concurrently substitutes low-bit weights~\Note{consider using "low-bit indices"} with 32-bit centroids and outliers.
The process is fast and takes only a few ms per shard on our 6-core Odroid dev board~\cite{odroid-web};
due to the high parallelizable nature of the workload, further optimization is possible, e.g. by designating a hardware accelerator~\cite{gobo}.
\xzlNote{contents below should be updated}
In the mean time, the system \textit{inflate} the resident model by loading more shards: it \textit{inflate} (1,2,2) for completing the width of L2, \textit{inflate} (1,1,3), (0,0,6) and (0,1,6) for upgrading the resident model fidelity.
After inference, the resident model is updated with newly loaded shards, i.e. (0,0,6), (0,1,6), (1,0,3), and (0,2,2) as highlighted in Figure~\ref{fig:design:res-model}. 

==> recycle/design-sharding-recycle2.tex <==
% !TeX root = main.tex

\section{Managing the model in elastic shards}
%\section{Managing \Tfm{}s in fine elasticity}
%\section{Building an elastic IO/compute pipeline}
\label{sec:design:sharding}


\xzlNote{quantization rationale, moved from intro, to merge}



For minimal accuracy loss, \sys{} uses \textit{simulated quantization}, \Note{reasons for not using real quantziation, i.e. integer operation: require fine-tuning for performance, not friendly to hardware}... 
It quantizes the full-fledged shards into different lower-bit representations, reducing sizes by up to 16 $\times$. %inspired by a Gaussian-outlier-based quantization technique~\cite{quantization-survey};
%With model shards as the key building block, \sys{} constructs an elastic pipeline whose IO and compute time is dependent on number of shards and their respective precisions. 
\Note{Our novelty comp. w/ prior mixed-precision transformer and dynamic transformer:} the first to combine them to achieve elasticity; our goal is not to find a supernet or an optimal mixed-precision net, but to find building blocks. 



%\textbf{Key points (structured around resident model):}1
%\begin{itemize}
%	\item 
%	Challenge: how to properly select a model shard? Must meet a list of criteria..
%	
%	\item
%	Model shards. Two things: partition by vertical slice (insights, formal definition), quantization technique (rationale, operation)
%	
%	\item
%	Resident model structure: in-memory representation, how to use, 
%	misc: activations (fixed high bits due to small, negligible).
%\end{itemize}



\subsection{Key challenges}
%\Note{merge challenges to below}
%We solve a key challenge in constructing a resident model: how to choose the proper parameter composition of a shard? %(as a smallest tunable unit for resident model)? 
%We solve a key challenge in constructing a resident model: how to instantiate a model shard? %(as a smallest tunable unit for resident model)? 
We solve a key challenge: how to instantiate an elastic shard? %(as a smallest tunable unit for resident model)? 
%As they are set to enable the engine to manage resident model in fine-granularity: depths, width, and fidelity. \Note{why use multiple fidelity has to be motivated early on}
%As they are 
Set to enable the elasticity of a model (i.e. depths, widths, fidelity) and management (i.e. IO/computation/memory), they must meet the following criteria: 
\begin{myitemize}	
	\item 
	Can execute partially (with existing shards) and incrementally (with newly loaded shards). %Independent, compatible with each other 
	
	\item
	IO delay must not starve computation. 
	This is to counter skewed IO delays. 
	\xzlNote{IO delays must be tunable -- accommodate different hardware}
	
	\item 
	Support variable compression ratio, no re-finetuning, minimum accuracy loss. 
	\xzlNote{overlap with point 2? I can see the point of shard importance}
\end{myitemize}

%To exploit the pipeline parallelism and construct the io/compute pipeline, we face the following two challenges.
%\Note{skewed io/compute: within a model; across diff. devices...}

% obsolete 
%\textit{First, pipelining at what granularity?}
%The key requirement is to allow for partial model execution.
%I.e. the inference may start as soon as the small part of the model is loaded.
%In hindsight, one may partition and pipeline the model by layers. 
%Yet, due to large model size, the \tfm{} models have a highly \textit{skewed} io/compute time\Note{TODO: there are more fundamental reasons for this}.
%For instance, io and compute latency of a layer differs by over 10$\times$ as demonstrated in~\S\ref{sec:motiv:char}.
%The naive layerwise partitioning leads to excessive, large pipeline bubbles and starves the CPU;
%as a result, the pipeline is no different from serial execution, failing the deadline..
%This is demonstrated in Figure \Note{XXX}.

%\textit{Second, how to handle device heterogeneity?}
%\Note{Do not need much exposure...}
%Not only the model itself are skewed in io/compute, edge devices are also known to have diverse hardware\Note{cite}. 
%Due to their different io/compute capability, there is no silver-bullet partitioning strategy given a deadline.
%As shown in \sect{motiv:char}, Rpi3 has much slower io compared with Odroid -- one partitioning strategy may have small pipeline bubbles on the latter but much larger bubbles on the former, starving CPUs.

%The \underline{second} research question is how to compress the shards?
%Broadly, three techniques can be used to compress the shards:
%shards may be pruned and discarded~\cite{cnn-entropy-filter-pruning, cnn-prune-nvidia}; 

%We set to shard \textit{pretrained} language models (e.g. BERT) without retraining. 
%The \underline{first} research question is at 
%To do so, there are two design choices. 
%One is \textit{unstructured} sharding~\cite{gordonCompressingBERTStudying2020,ladabert}, that is, viewing the whole (over 100 million) parameters as a large flat data array and splitting it in trunks. % which is common in network pruning

%they may share weights with each other~\cite{transformer-attention-share,nn-weight-share};
%they may be quantized into a lower bitwidth~\cite{binarybert,ibert,bibert}.
%%Our system must navigate through the compression techniques to ensure that shards 
%Our system must shard a model cautiously, navigate through the compression techniques, and ensure a decent model performance. %shards should work well with each other



\subsection{Instantiating model shards}
\label{sec:design:sharding:shard}
%For pretrained \tfm{} models, we propose a retraining-free sharding approach, which is a novel combination of width-adaptive \tfm{} and outlier-aware quantization.
%\textbf{structured}, \textbf{outlier-aware quantization} approach for sharding the pretrained \tfm{} model. 
%Our key idea is to shard the model by layers, and by their attention heads.
%\Note{Our key construct is ...}
%In response, our key construct is \textit{model shards}, where we partition the transformer layers into mixed-precision, finer grained pieces.
To address the challenges, our key insight is to integrate a novel combination of two techniques: dynamic \tfm{} and outlier-aware quantization. 
%compress a dynamic \tfm{} (e.g. DynaBERT~\cite{dynabert}, HAT~\cite{hat}) with Gaussian-outlier-aware simulated quantization~\cite{quantization-survey}.
%To address the challenges, our key insight is to leverage a dynamic \tfm{} with adaptive widths and depths (e.g. DynaBERT~\cite{dynabert}, HAT~\cite{hat}), with Gaussian-outlier-aware simulated quantization~\cite{gobo}.
%Our rationale is dynamic \tfm{} enables partial and incremental model execution because sub\Tfm{}s (\xzlNote{??}) share weights with the super\Tfm{}; 
%Gaussian-based simulated quantization works with pretrained models and incurs little accuracy degradation by accurately approximating parameter distribution~\cite{gobo,deep-compression}.
%We next describe the details.
%\Note{rationale, merge}
%The former enables partial and incremental model execution because sub\Tfm{}s share weights with the super\Tfm{}; 
%the latter works with pretrained models and incurs little accuracy degradation by exploiting parameter redundancy (\S\ref{sec:motiv:primer}).
%\Note{rationale merge}
%We do so because the parameter distribution of a \tfm{} layer is known to resemble Gaussian distribution~\cite{gobo};
%hence we can approximate the majority of values with a few representatives called centroids, while preserving the rest outliers (i.e. outside the Gaussian distribution). 
%The whole process resembles lossy compression and does not require fine tuning..

%We then partition each version into vertical slices by layers, which are model shards. 
%To address the challenges, our key insight is to leverage a dynamic \tfm{} with adaptive widths and depths (e.g. DynaBERT~\cite{dynabert}, HAT~\cite{hat}), and compress it into different fidelity versions using Gaussian-outlier-aware simulated quantization;
%we then partition each version into vertical slices by layers, which are model shards.

%Our rationale are as follows. 
%Dynamic \tfm{} allows for partial model execution;
%the parameter distribution of a \tfm{} layer 
%by approximating it with Gaussian distribution while preserving outliers resembles lossy compression which incurs little accuracy degradation. 

%integrating a novel combination of two known techniques: structured pruning \& outlier-aware quantization. 

%Compared with partitioning by layers, model shards bridges the gap between the skewed io vs compute (XXX vs XXX), allowing for efficient pipeline execution with small bubbles;
%their variable fidelity further enables elastic IO time.  %adapting to various deadlines on heterogeneous devices.
%\Note{merge below}
%% obsolete 
%\paragraph{\textit{Benefits}} are as follows.
%\begin{myitemize}
%	\item 
%	\textit{Partial model execution.}
%	First (cold) inference may start execution on only a few (e.g. 3) shards per layer, while subsequent inferences may incrementally load more.
%	
%	%Our rationale is as follows.
%	%First, an attention head is an atomic structure of the MHA mechanism~\cite{transformer}, which is learned at training time;
%	%shards conforming to the structure preserves the same mechanism.
%	%%shards can work seamlessly with each other. 
%	
%	\item 
%	\textit{Close and elastic IO/compute.}
%	A typical shard contains only one twelve-th parameter as a layer, thus having the same small portion of its IO (e.g. 40ms), approximating the compute time on a shard per layer (e.g. 30ms).
%	Mixed-precisions allow for multiple other devices..
%	
%\end{myitemize}

\input{fig-sharding}

\xzlNote{each techniques below shall map back to challenges.}

\paragraph{First, simulated quantization.}
\label{sec:design:sharding:quantize}
%We next describe in detail how to quantize them into different precisions (bits).

\xzlNote{clarify: what comes from prior work (therefore brief/high-level/layman description) and what is ours}

Ahead of time, we use Gaussian-outlier-aware simulated quantization to compress the pretrained \tfm{} model into different, $b$-bit fidelities, e.g. $b=2\dots 6$. 

For each layer, the system fits all its weights into a Gaussian distribution, based on which it divides weights into two groups, an outlier group and a Gaussian group;
it preserves the former in full 32-bit fidelity and represents the latter with $2^b$ centroids, which are 32-bit floating point numbers.
%for the latter, it represents them with $2^b$ centroids. 
A weight is deemed as an outlier if the probability of it belongs to the Gaussian distribution is below a configurable threshold;
the larger the threshold, the more full-fidelity outliers, hence the lower compression ratio.  

Following the same practice in~\cite{gobo}, we use $-4$ which is sufficient in maintaining accuracy while maximizing compression ratio;
under the threshold, the outlier group constitute less than $0.1\%$ of total weights. %which is preserved in full precision (i.e. 32-bit). %and incurring only 1\% accuracy degradation. 
For the Gaussian group which constitute the rest $99.9\%$, the system sorts and splits its weights into $2^b$ clusters with equal population;
each cluster has \textit{one} centroid to represent \textit{all} values within it. 
%It then represents \textit{all} values in each cluster with \textit{one} centroid, which is indexed by a $b$-bit integer.
%It then represents \textit{all} values in each cluster with \textit{one} cluster centroid by substituting them with a $b$-bit index to the centroid.
Doing so caters to the weight distribution: weight-concentrated regions deserve higher resolutions, hence having more clusters and centroids.
%the vast majority ($99.9\%$) of original 32-bit weights are represented by $b$-bit integers, reducing model size by $\lfloor 32/b \rfloor \times$.
To decide cluster centroids, prior work adopt K-means based approaches~\cite{deep-compression, zhaoImprovingNeuralNetwork}, which are time-consuming, e.g. it takes a few hours to converge on our server.
Differently, we have found the arithmetic mean of cluster weights suffices -- a 2-bit version takes a few minutes to converge and incurs only 7\% accuracy degradation compared with the full model. 
We will present more results in \sect{eval}.  
%It uses the Gaussian model to find out a group of ``outliers'' parameters and preserve them in full precision.
%For the rest, the system quantizes them into $n$-bit integers (e.g. typically 2 to 4) using \textit{simulated quantization}~\cite{quantization-survey}, where each integer points to a full-precision FP32 value called a centroid, representing a group of original weights.
%The system decides the centroids by dividing the non-outlier parameters into $2^n$ groups and calculating their arithmetic means.

%The rationale is ....
%\Note{quantization rationale..}
%Second, attention head weights are heavily redundant~\cite{16heads}.
%%Most need only a few bits~\cite{ibert,binarybert} while only outliers need high-precision.
%Preserving the few outliers (e.g. 0.01\%~\cite{gobo}) while representing the most others with a small number of values ensures performance.

The system repeats the process for each fidelity version and generates a dictionary as the compression metadata, which specifies the centroids and the outlier mapping of full-fidelity weights.

\xzlNote{clarify: impact on IO and compute. why compute remains unaffected. also compare to other compression techniques that reduce both IO and compute (like distillation, transfer learning. why aren't those desirable)}

%\Note{update Figure 5}
\paragraph{Second, vertical partitioning.}
\xzlNote{This this should go before quantization}

%The system then partitions each of $B$ fidelity versions into $M$ vertical slices by $K$ layers (in total $b\times m \times k$ such slices). 
The system then partitions the full-fledged pretrained model into $M$ vertical slices by $N$ layers.
Each vertical slice constitutes one attention head plus $1/M$ FFN neurons.
%A slice/shard $S$ can be uniquely identified by a three-tuple $S=(m,k,b)$, where $m, k$ are the indexes for the slice and layer respectively, and $b$ is its fidelity.
Doing so preserves the language features in the learned structure. \xzlNote{vague, find better rationales from prior work}

Formally, we define shards as follows. 
For a \tfm{} layer, 
%it is composed by five key weight matrix $W^Q, W^K, W^V, W^O$ and $FFN$, where
$d$ is the hidden state size (e.g. $d=782$), $d_{ff}$ is the number of neurons in FFN, $M$ is the total number of attention heads (e.g. $M = 12$), and the size of each attention head $d_h$ is $d/{M}$, and the number of connected neurons $d_h'$ is $d_{ff}/{M}$.
A model shard $W_S$ is hence parameterized by:
%\Note{use a figure}

\begin{equation}
	W_S = \{W_{d_h}^{Q}, W_{d_h}^{K}, W_{d_h}^{V}, W_{d_h}^{O}\}\cup\{FFN_{d_h'}\}
\end{equation}

\xzlNote{clarify: which subset of a model shards are composable? why partial execution can still give meaningful inference result?}

\paragraph{Third, generating shards.}
%After partitioning, a shard contains $1/M$ of a layer's total parameters, each is a $b$-bit centroid index.
To generate shards, the system compresses the vertical slices using the dictionaries produced by simulated quantization: 
for \textit{all} 32-bit parameter, the system looks up the dictionary and uniformly substitutes them with $b$-bit integers, each pointing to one of the $2^b$ centroids.
It does not preserve the 32-bit outliers in the newly compressed weight matrix to avoid destroying the $b$-bit data alignment.
It stores the compressed weights as the data and dictionaries (centroids, outliers) as the metadata of model shards on disk.
This is shown in Figure~\Note{XXX}. \xzlNote{Fig 4 needs update, showing the workflow}
Since the vast majority ($99.9\%$) of original 32-bit weights are represented by $b$-bit integers, model size is reduced by $\lfloor 32/b \rfloor \times$.
The system generates and stores $N \times M\times B$ such shards on disk and co-locates their disk blocks for access locality.
%Instead, it stores the outlier mapping separately to the compressed weights, which specifies 

%In uncompressed, full-fidelity form, their sizes are $1/M$ of a layer (e.g. a few MBs), taking tens of ms to load; 
%in lower fidelities, their IOs are even smaller and elastic w.r.t. bit fidelity. 
%%Hence a model shard equally slices the $j$-th layer it belongs to.
%Note: when in lower fidelities, shards cannot be used directly -- the weights are only indexes. 
%They cannot be used interchangeably, e.g. a 1 in 2-bit and 6-bit shard points to different centroids.  
%For instance, for the 1st layer with 3 shards,  


%Since the vast majority ($99.9\%$) of 32-bit weights can map to centroids, which are indexed by $b$-bit integers, the model size is reduced by $\lfloor 32/b \rfloor \times$.

%Following~\cite{dynabert}, the attention score and output of a layer can be defined as:
%
%\begin{equation}
%	\label{eq:out}
%\end{equation}
%
%Therefore as listed in equation~\ref{eq:out}, the output of a \tfm{} layer can be regarded as the sum of independent model shards, allowing partial execution of the model.

%\paragraph{Storing model shards}
%The system stores all versions of shards and their corresponding centroids on disk. %and pick selectively at run time. 
%Unused ones (e.g. for other tasks) can be further compressed via lossless compression (e.g. Zip). 
%This is possible because of low entropy.
%%Will evaluate its size (smaller than a HD movie) and compression efficiency (>90\%). 
%\Note{why not only store 6bit and derive the others?} 
%Doing so requires to \textit{always} load 6-bit shard IO delays.
%Not elastic, may miss deadline.

\xzlNote{need cost analysis? }
At least mention prior work on hardware accelerator

\subsection{Resident model}

\xzlNote{what is stored on disk; who loads shards to memory. Show the mapping (perhaps in Fig4)}

\paragraph{Formulation}
In memory, $N$ layers of $M$ model shards stack upon each other to form a resident model.
In the $M \times N$ grid, each cell marks a model shard $S(m, n, b)$, defined by its position ($m$-th vertical slice in $n$-th layer) and $b$-bit fidelity.
%Following the convention, we describe a resident model by its widths $M$ -- number of shards per layer, and depths $K$ -- number of such layers. 
A resident model $R$ is thus configured by the set of shards: $R=\{S(m,n,b) \mid m \leq M, n \leq N, b=2\dots6, 32\}$.
Besides shards, the resident model keeps miscellaneous parameters in full fidelity due to their small sizes (e.g. only 768 dimensions), including layer normalization, pooler, and classification head.


\paragraph{Tunable knobs}
%A resident model may be adjusted and tuned along three dimensions. 
%\textit{First, width}: by adjusting $M$ per layer.
%It applies to all layers because inference computation must execute on layers with the same $M$.
%\textit{Second, depths}: by adjusting $K$, number of layers. 
%\textit{Third, fidelity}: by adjusting $b$ of individual shards.  
By tuning the shard configuration, a resident model may be adjusted along three dimensions. 
\textit{1) Widths and 2) depths} are adjustable through $M$ and $N$, similar to dynamic \tfm{}. 
\textit{3) Fidelity} can be tuned by specifying the $B$ fidelity of individual shards. 

To tune the shard configuration, the system implements two operators: \textit{load(m, n, b)} and \textit{unload(m, n)}. 
The former pulls corresponding model shard version from disk into memory and is used when extra shards are needed to increase widths and/or depths, as well as replacing the existing one with a new fidelity.
The latter evicts existing shards, i.e. to decrease widths and/or depths.

\paragraph{How to use}
\xzlNote{move (some) to implementation?}
The system decompresses the resident model $R$ into the working buffer for inference, as model shards are quantized w.r.t. different fidelities, whose weights are centroid indexes. 

Prior to inference, the system allocates a working buffer which is large enough to host a layer of $M$ full-fidelity shards.
It decompresses each shard $S(m,n,b)$ in $R$ by projecting centroids onto the weight matrix of the shard, replacing the $b$-bit integers with 32-bit floating points. 
It then restores the outliers by patching respective indexes of the matrix. 
The process is efficient and takes a few ms on a 6-core dev board per shard.
%The process is efficient and takes $10\sim20$ ms on a 6-core dev board per 12-shard layer.

During inference, the system executes normally based on the 32-bit weights restored from centroids and outliers in the working buffer, whose execution time is dependent on sentence input lengths, number of shards per layer, and the number of layer. 

After inference, the system deallocates the working buffer while keeping the resident model in memory.

%Model shards breaks down a large model into fine-grained $K \times M$ grids, where each cell 
%Hence a resident model $R$ is defined as a set of shards: $R=\{S(i,j,b) | \}$


%
%\Note{key difference with prior work:}
%
%The key difference to prior work: 
%1) finer-grained, vertical slice. Others -- horizontal slice, e.g. quantization by layer, by component (weight matrix); 
%2) quantization is not ``done deal''. 
%All quantization versions of are stored but only some will be picked and selected at run time.\Note{can be optimized?} 

%% obsolete 
%\begin{myitemize}
%	\item 
%	During one inference, \# of shards is the same across all layers
%	
%	\item 
%	Overlap what? IO of \textit{next} layer and compute of \textit{current} layer
%	
%	\item 
%	What is being computed on? Restored, full-precision weights. 
%	After quantization, shard stores the index to centroids (FP32).
%	\sys{} restore them (with minimal cost).
%	
%%	is our system does not quantize the attention heads uniformly into $n$-bit. 
%%	Instead, each shard may be quantized into different bitwidths; 
%%	the eventual model comprises shards with different precisions.
%
%\end{myitemize}
 



==> recycle/design-sharding-recycle3.tex <==
% !TeX root = main.tex

\section{Elastic model sharding}
%\section{Managing the model in elastic shards}
%\section{Managing \Tfm{}s in fine elasticity}
%\section{Building an elastic IO/compute pipeline}
\label{sec:design:sharding}


%\textbf{Key points (structured around resident model):}1
%\begin{itemize}
%	\item 
%	Challenge: how to properly select a model shard? Must meet a list of criteria..
%	
%	\item
%	Model shards. Two things: partition by vertical slice (insights, formal definition), quantization technique (rationale, operation)
%	
%	\item
%	Resident model structure: in-memory representation, how to use, 
%	misc: activations (fixed high bits due to small, negligible).
%\end{itemize}


\xzlNote{moved here, to merge}
where each shard spans one Transformer attention head and $1/M$ FFN neurons of this layer. 
For each shard, it creates $K$ fidelity versions, which are lower-bit representations of this shard's weights. 
For instance, a full-fidelity version that represents each weight with 32 bits, a two-bit version that does so with 2 bits. 
We therefore store $NxMxK$ shard versions on disk. 
The preprocessing is a one-time effort per model; being light transformation of an existing model without pre-training, it can be done on device at the model installation time. 



%The preprocessing is a one-time effort per model; 
%lightweight and requiring no model re-retraining, it can be done on mobile devices. 


\Note{Model shards trade inexpensive disk storage for expensive, scarce memory... }


\subsection{Key challenges}
%\Note{merge challenges to below}
%We solve a key challenge in constructing a resident model: how to choose the proper parameter composition of a shard? %(as a smallest tunable unit for resident model)? 
%We solve a key challenge in constructing a resident model: how to instantiate a model shard? %(as a smallest tunable unit for resident model)? 
%We solve a key challenge: how to instantiate an elastic shard? %(as a smallest tunable unit for resident model)? 
We solve a key challenge: how to partition the model into individual shards? %(as a smallest tunable unit for resident model)? 
%As they are set to enable the engine to manage resident model in fine-granularity: depths, width, and fidelity. \Note{why use multiple fidelity has to be motivated early on}
%As they are 
%Set to enable the elasticity of a model (i.e. depths, widths, fidelity) and management (i.e. IO/computation/memory), they must meet the following criteria: 
Set to enable the resource elasticity of a model (i.e. depths/widths/fidelity), the shards must meet the following criteria: 
\begin{myitemize}	
	\item 
	\textit{Elastic execution.}
	Shards must preserve the same expressiveness of the attention mechanism and can execute partially. 
%	Can execute partially (with existing shards) and incrementally (with newly loaded shards). %Independent, compatible with each other 
	
	\item
	\textit{Tunable IO.} 
	IO compression ratios must be tunable to accommodate IO/computation capability of different hardware (e.g. due to diverse CPU/GPUs and DVFS). 
	Compression should not require further fine-tuning for fast deployment.
%	must not starve computation. 
%	This is to counter skewed IO delays. 
%	\xzlNote{IO delays must be tunable -- accommodate different hardware}
	
%	\item 
%	Support variable compression ratio, no re-finetuning, minimum accuracy loss. 
%	\xzlNote{overlap with point 2? I can see the point of shard importance}
\end{myitemize}

%To exploit the pipeline parallelism and construct the io/compute pipeline, we face the following two challenges.
%\Note{skewed io/compute: within a model; across diff. devices...}

% obsolete 
%\textit{First, pipelining at what granularity?}
%The key requirement is to allow for partial model execution.
%I.e. the inference may start as soon as the small part of the model is loaded.
%In hindsight, one may partition and pipeline the model by layers. 
%Yet, due to large model size, the \tfm{} models have a highly \textit{skewed} io/compute time\Note{TODO: there are more fundamental reasons for this}.
%For instance, io and compute latency of a layer differs by over 10$\times$ as demonstrated in~\S\ref{sec:motiv:char}.
%The naive layerwise partitioning leads to excessive, large pipeline bubbles and starves the CPU;
%as a result, the pipeline is no different from serial execution, failing the deadline..
%This is demonstrated in Figure \Note{XXX}.

%\textit{Second, how to handle device heterogeneity?}
%\Note{Do not need much exposure...}
%Not only the model itself are skewed in io/compute, edge devices are also known to have diverse hardware\Note{cite}. 
%Due to their different io/compute capability, there is no silver-bullet partitioning strategy given a deadline.
%As shown in \sect{motiv:char}, Rpi3 has much slower io compared with Odroid -- one partitioning strategy may have small pipeline bubbles on the latter but much larger bubbles on the former, starving CPUs.

%The \underline{second} research question is how to compress the shards?
%Broadly, three techniques can be used to compress the shards:
%shards may be pruned and discarded~\cite{cnn-entropy-filter-pruning, cnn-prune-nvidia}; 

%We set to shard \textit{pretrained} language models (e.g. BERT) without retraining. 
%The \underline{first} research question is at 
%To do so, there are two design choices. 
%One is \textit{unstructured} sharding~\cite{gordonCompressingBERTStudying2020,ladabert}, that is, viewing the whole (over 100 million) parameters as a large flat data array and splitting it in trunks. % which is common in network pruning

%they may share weights with each other~\cite{transformer-attention-share,nn-weight-share};
%they may be quantized into a lower bitwidth~\cite{binarybert,ibert,bibert}.
%%Our system must navigate through the compression techniques to ensure that shards 
%Our system must shard a model cautiously, navigate through the compression techniques, and ensure a decent model performance. %shards should work well with each other



\subsection{Instantiating model shards on disk}
\label{sec:design:sharding:shard}
%For pretrained \tfm{} models, we propose a retraining-free sharding approach, which is a novel combination of width-adaptive \tfm{} and outlier-aware quantization.
%\textbf{structured}, \textbf{outlier-aware quantization} approach for sharding the pretrained \tfm{} model. 
%Our key idea is to shard the model by layers, and by their attention heads.
%\Note{Our key construct is ...}
%In response, our key construct is \textit{model shards}, where we partition the transformer layers into mixed-precision, finer grained pieces.
To address the challenges, our key idea is to combine two machine learning techniques -- dynamic \tfm{}~\cite{dynabert,hat} and dictionary-based quantization~\cite{deep-compression}, in a novel way.
%To address the challenges, our key idea is to leverage a novel combination of two techniques: dynamic \tfm{}~\cite{dynabert,hat} and dictionary-based quantization~\cite{deep-compression}. 
We next describe details.
%compress a dynamic \tfm{} (e.g. DynaBERT~\cite{dynabert}, HAT~\cite{hat}) with Gaussian-outlier-aware simulated quantization~\cite{quantization-survey}.
%To address the challenges, our key insight is to leverage a dynamic \tfm{} with adaptive widths and depths (e.g. DynaBERT~\cite{dynabert}, HAT~\cite{hat}), with Gaussian-outlier-aware simulated quantization~\cite{gobo}.
%Our rationale is dynamic \tfm{} enables partial and incremental model execution because sub\Tfm{}s (\xzlNote{??}) share weights with the super\Tfm{}; 
%Gaussian-based simulated quantization works with pretrained models and incurs little accuracy degradation by accurately approximating parameter distribution~\cite{gobo,deep-compression}.
%We next describe the details.
%\Note{rationale, merge}
%The former enables partial and incremental model execution because sub\Tfm{}s share weights with the super\Tfm{}; 
%the latter works with pretrained models and incurs little accuracy degradation by exploiting parameter redundancy (\S\ref{sec:motiv:primer}).
%\Note{rationale merge}
%We do so because the parameter distribution of a \tfm{} layer is known to resemble Gaussian distribution~\cite{gobo};
%hence we can approximate the majority of values with a few representatives called centroids, while preserving the rest outliers (i.e. outside the Gaussian distribution). 
%The whole process resembles lossy compression and does not require fine tuning..

%We then partition each version into vertical slices by layers, which are model shards. 
%To address the challenges, our key insight is to leverage a dynamic \tfm{} with adaptive widths and depths (e.g. DynaBERT~\cite{dynabert}, HAT~\cite{hat}), and compress it into different fidelity versions using Gaussian-outlier-aware simulated quantization;
%we then partition each version into vertical slices by layers, which are model shards.

%Our rationale are as follows. 
%Dynamic \tfm{} allows for partial model execution;
%the parameter distribution of a \tfm{} layer 
%by approximating it with Gaussian distribution while preserving outliers resembles lossy compression which incurs little accuracy degradation. 

%integrating a novel combination of two known techniques: structured pruning \& outlier-aware quantization. 

%Compared with partitioning by layers, model shards bridges the gap between the skewed io vs compute (XXX vs XXX), allowing for efficient pipeline execution with small bubbles;
%their variable fidelity further enables elastic IO time.  %adapting to various deadlines on heterogeneous devices.
%\Note{merge below}
%% obsolete 
%\paragraph{\textit{Benefits}} are as follows.
%\begin{myitemize}
%	\item 
%	\textit{Partial model execution.}
%	First (cold) inference may start execution on only a few (e.g. 3) shards per layer, while subsequent inferences may incrementally load more.
%	
%	%Our rationale is as follows.
%	%First, an attention head is an atomic structure of the MHA mechanism~\cite{transformer}, which is learned at training time;
%	%shards conforming to the structure preserves the same mechanism.
%	%%shards can work seamlessly with each other. 
%	
%	\item 
%	\textit{Close and elastic IO/compute.}
%	A typical shard contains only one twelve-th parameter as a layer, thus having the same small portion of its IO (e.g. 40ms), approximating the compute time on a shard per layer (e.g. 30ms).
%	Mixed-precisions allow for multiple other devices..
%	
%\end{myitemize}

\input{fig-sharding}

%\xzlNote{each techniques below shall map back to challenges.}


%\Note{update Figure 5}
\paragraph{First, vertical partitioning per layer}
%\xzlNote{This this should go before quantization}
%The system then partitions each of $B$ fidelity versions into $M$ vertical slices by $K$ layers (in total $b\times m \times k$ such slices). 
The system adopts a pretrained \tfm{} model, which has already been fine-tuned on a downstream task. %(e.g. models from Huggingface~\cite{huggingface)}.
%such models they may be publicly accessible  
The model must have adaptive widths and depths, that is, at run time it may decide differently how many parameters of a layer to use (i.e. widths), as well as the number of layers (i.e. depths).
%The model must have adaptive widths and depths, that is, at run time it may decide differently how many number of attention heads and FFN neurons of a layer (i.e. widths), as well as the number of layers (i.e. depths) to use.
%The system adopts a pretrained dynamic \tfm{} model as the backbone network,  which is already fine-tuned on a downstream task (e.g. sentiment analysis) to have adaptive widths and depths. 
%That is, it can vary the number of attention heads and FFN neurons of a layer, as well as the number of layers.

For each of the $N$ layers, the system partitions it into $M$ vertical slices. %by total $N$ layers.
By construction, each vertical slice is independent, constituting one attention head plus $1/M$ of FFN neurons of the layer. %whose parameters compose a shard.
Table~\ref{tab:vertical_slice} shows the weight compositions of a vertical slice.
Each cell of the table describes the dimension of the weight matrix, where $d$ is hidden state size, $M$ is the number of attention heads, and $d_{ff}$ is the number of FFN neurons;
a shard is therefore one of the $M$ equal slices. 
%as can be seen, the partitioning equally slices the layer 
Doing so warrants model shards elasticity and the same capability to extract linguistic features from inputs, as done by the attention mechanism: 
%Doing so warrants model shards attending to linguistic features of input tokens: 
%Doing so warrants model shards with same attention mechanism linguistic features : 
of an individual shard, its attention head obtains one independent representation of input tokens, which is projected into a higher feature dimension by FFN neurons~\cite{attention-head-acl19,bert-acl19};
jointly, multiple shards attend to information from different representation subspace at different positions~\cite{transformer}.
%jointly, multiple shards recover full semantic features of inputs.
%A slice/shard $S$ can be uniquely identified by a three-tuple $S=(m,k,b)$, where $m, k$ are the indexes for the slice and layer respectively, and $b$ is its fidelity.
Therefore, an arbitrary subset of shards of a layer can be executed to produce meaningful results. % and their results can be combined to produce meaningful output.

%Doing so preserves the language features in the learned structure. \xzlNote{vague, find better rationales from prior work}

\begin{comment}
% below useful...merged 
\xzlNote{Compress the following two paragraphs into a table?}
Following~\cite{dynabert}, we define a shard's weight composition as follows. 
For a \tfm{} layer, 
%it is composed by five key weight matrix $W^Q, W^K, W^V, W^O$ and $FFN$, where
let $d$ denote the hidden state size, $M$ be the total number of attention heads (e.g. $M = 12$), $d_{ff}$ be the number of FFN neurons.
The size of each attention head $d_h$ is given by $d/{M}$, and the neurons of a shard $d_{ff'}$ is given by $d_{ff}/M$.
By equally partitioning the layer, we obtain $M$ vertical slices as model shards, indexed by $[0, M-1]$ from left to right.

The $j$-th shard is hence parameterized by six submatrix: $\{ W_{j}^Q, W_{j}^K, W_{j}^{V}, W_{j}^{O} \} \in \mathbb{R}^{d\times d_h}$ from an attention head, and two from FFN $W_{j}^{FFN1} \in \mathbb{R}^{d_{ff'}\times d},
	 W_{j}^{FFN2} \in \mathbb{R}^{d \times d_{ff'}}$.
The sub-matrix $W_{j}$ are selected by the $j$-th portion from respective $W$ along the non-feature dimension.
For instance, $W_{j}^{Q} = W_{:, j\cdot d_h:j\cdot(d_h+1)}^{Q}$.
Note that the index $j$ explicitly assigns the $j$-th slice of the weight matrix $W$ w.r.t. each shard in an non-overlapping manner.
\end{comment}


\sys{} uses the \textit{submodel} to describe the \tfm{} model on shards, e.g. a  $n \times m$ submodel comprises n layers, each layer having m shards.
The number m is the same across all layers, as mandated by the \tfm{} architecture~\cite{transformer}, which specifies each layer must have the same width (i.e. number of shards m) for aligning input/output features between layers.
Although it is possible for a shard to use 0s as placeholder weights, \sys{} expects all m shards to have concrete weights for a good accuracy.
%To execute a \tfm{} model using shards, \sys{} first decides a \textit{submodel} of $n$ layers; %$\times$ $m$ shards per layer.
%mandated by the \tfm{} architecture~\cite{transformer}, each layer must have the same width (i.e. number of shards $m$) for an aligned number of output features.
%Although it is possible for a shard to use 0s as placeholder weights, \sys{} expects all $m$ shards to have concrete weights for a good accuracy.
%With $m$ shards, \sys{} computes the attention and FFN output of individual shards using the weight composition in Table~\ref{tab:vertical_slice}, concatenates their outputs, and proceeds to next layer.
%The process therefore preserves the attention mechanism for producing meaningful results.
%For more detailed mathematic formulation, an interested reader may refer to~\cite{16heads,dynabert}.


\input{tab-shard-param}

%The $j$-th model shard at $i$-th layer, $S(i,j)$, is parameterized by:
%%\Note{use a figure}
%
%\begin{equation}
%S(i,j) = \{W_{d_h}^{Q_i}, W_{d_h}^{K}, W_{d_h}^{V}, W_{d_h}^{O}\}\cup\{FFN_{d_h'}\}
%\end{equation}

%\xzlNote{clarify: which subset of a model shards are composable? why partial execution can still give meaningful inference result?}

%\xzlNote{where do we say that in a submodel, each layer must have the same number of shards, and why}

%\xzlNote{much of the following (until the end of S4.3) can go to impl. Important things to mention: what is done at a high level; (typically) how many versions per shard; how are they stored on disk and how large (compression ratio); potential accuracy loss; model accuracy has different sensitivities to individual shards and their bitwidth; mixed precision: shards of different bitwidths can be combined in the same submodel; compute cost of compression/decompression..}
\Note{this is our novelty. highlight what is ours and what is theirs..}
\paragraph{Second, quantization per shard}
\label{sec:design:sharding:quantize}
%We next describe in detail how to quantize them into different precisions (bits).
The system compresses the each of the $N \times M$ shards into $K$ fidelity versions (e.g. 5 versions, $b=2\dots 6$). %each of which reduces the model size by a few $\times$.
We are the first to bring quantization to \textit{shard} granularity, whereas prior work only explores layer granularity~\cite{mixed-quantization-energy,hawq,haq}.
Doing so reduces IO/compute skewness and facilitates elastic IO, allowing \sys{} to  allocate IO resources at a finer granularity to more important shards.

%gives different fidelity per shard importance for maximizing resource utilization on different devices with diverse IO/compute capabilities. 
%\xzlNote{... and to give different fidelity (compression ratio) per shard importance...}

%of  : fidelity versions reduce their IO by a few $\times$, which can overlap with compute with small bubbles while adapting to .
%The goal is to facilitate elastic IO and amortize IO/compute skewness for maximizing resource utilization: fidelity versions reduce their IO by a few $\times$, which can overlap with compute with small bubbles while adapting to diverse IO/compute capability of different devices.


%The compression is feasible due to high parameter redundancy of \tfm{}, allowing accurate approximation via Gaussian distributions~\cite{tenarybert,gobo}.
%\Note{high level}
To compress, we use Gaussian outlier-aware quantization~\cite{gobo}.
%It exploits the Gaussian distribution of \tfm{} weights. 
The key idea is to replace the vast majority (i.e. 99.9\%) of weights which follow a Gaussin distribution with a $k$-bit indice pointing to one of the $2^k$ floating point numbers called \textit{centroids}, and preserve the very few \textit{outliers} (i.e. 0.01\%) as-is.
The process is shown in Figure~\ref{fig:design:shards} (2).


%\Note{property1: can have high compression ratio, minimum accuracy loss. greatly reduces IO... (no more skewness)}
%how many versions per shard; how are they stored on disk and how large (compression ratio); potential accuracy loss;

\begin{comment}
\Note{may hurt us -- making our design point insignificant}
\textit{Property I: high compression ratios, low accuracy loss.} 
For a K-bit version, the approach compresses a shard by 32/K, as 99.9\% of 32-bit weight are replaced by K-bit dictionary indexes.
For instance, at the lowest bitwidth we target (K=2), the shard is compressed by 16$\times$, whose file size is less than 200KB.
The high compression ratios correct IO/compute skewness and make storing all K versions cheap, e.g. for typically five versions, K=$2\dots6$, it adds only a few hundred MBs. %and is tunable to cater capabilities of diverse devices. 
Meanwhile, the accuracy loss is minimum, incurring less than 1\% accuracy degradation when K=6.
At lower K=2, the accuracy loss may be high, e.g. 10\%, but it can be remedied by \sys{}'s mechanism to load higher-bitwidths shards, which we will describe and evaluate later.
\end{comment}

%\Note{property2: resembles lossy compression. Work smoothly across different fidelity versions}
%model accuracy has different sensitivities to individual shards and their bitwidth;
%mixed precision: shards of different bitwidths can be combined in the same submodel

%\textit{Property II: good compatibility between shard versions.}
%The dictionary compression resembles lossy compression.
We choose it for mainly for two reasons. % it satisfies following properties which we seek: 
1) its lossy compression nature provides good compatibility between shards of different versions, allowing them to assemble a submodel with \textit{mixed-bitwidths}.
%allows shards of different versions to work seamlessly with each other, assembling a submodel with \textit{mixed bitwidths}.
This is because shards still preserve the original distribution of layer weights, albeit in different fidelities. 
More importantly, the good compatibility enables \sys{} to tune the bitwidths of individual shards per their importance. 
%\sys{} prioritize important shards which have large impacts on accuracy and allocate higher bitwidths for them, s.t. they may recover the original weight distribution as precisely as possible.
%For less important ones, \sys{} uses lower bitwidths as they do not affect accuracy much.

%\Note{property3: does not need fine tuning and hardware support}
\textit{Property III: no fine-tuning nor hardware support required.}
The quantization approximates the weight distribution of the pretrained model and is oblivious to 


To use, the engine decompresses the shards by simply mass substituting dictionary indexes with centroids (i.e. floating point numbers) and computes on restored FP32 weights;
the decompression is efficient on a commodity SoC, less than 20ms for one layer.
%the inference only have floating point operations;
This differs from a traditional \textit{mixed-precision} network, which mixes floating point operations with integer operations~\Note{cite}.


We choose it because it incurs little accuracy loss (<1\%) even at $10\times$ compression ratio by accurately approximating \tfm{} weights which follow a Gaussian distribution~\cite{gobo,tenarybert}, and that it is dictionary compression (i.e. simulated), which does not require fine-tuning.
%We donot use fixed-point quantization~\cite{binarybert,q8bert} because it is less elastic (e.g. fixed 8/4/2bit versions), needs DSP extension which is only seen on microcontrollers (e.g. Cortex-M4~\cite{m4-dsp}), and requires fine-tuning. 
We donot use fixed-point quantization~\cite{binarybert,q8bert} because it is less elastic (e.g. fixed 8/4/2bit versions), needs DSP extension which is only available on microcontrollers (e.g. Cortex-M4~\cite{m4-dsp}), and requires fine-tuning. 
Alternatively, a model may be compressed by knowledge distillation~\cite{distilbert} or model pruning~\cite{layerdrop,mobilebert}. 
However, they also require fine-tuning for \textit{each} version, and they likely lead to severe accuracy degradation as they must remove over 90\% of weights to achieve the same compression ratio as ours.



%
%For minimal accuracy loss, \sys{} uses \textit{simulated quantization}, \Note{reasons for not using real quantziation, i.e. integer operation: require fine-tuning for performance, not friendly to hardware}... 
%It quantizes the full-fledged shards into different lower-bit representations, reducing sizes by up to 16 $\times$. %inspired by a Gaussian-outlier-based quantization technique~\cite{quantization-survey};
%%With model shards as the key building block, \sys{} constructs an elastic pipeline whose IO and compute time is dependent on number of shards and their respective precisions. 
%\Note{Our novelty comp. w/ prior mixed-precision transformer and dynamic transformer:} the first to combine them to achieve elasticity; our goal is not to find a supernet or an optimal mixed-precision net, but to find building blocks. 




%\xzlNote{clarify: impact on IO and compute. why compute remains unaffected. also compare to other compression techniques that reduce both IO and compute (like distillation, transfer learning. why aren't those desirable)}
%Since the vast majority ($99.9\%$) of 32-bit weights are substituted by $b$-bit indexes to centroids, simulated quantization reduces IO by $\lfloor 32/b \rfloor \times$.
%It, however, does not reduce computation delays because the model maintains the same GFLOPS by computing on floating point centroids and outliers. 
\begin{comment}
% --- old, can merge ---
For each layer, the system fits all its weights into a Gaussian distribution, based on which it divides weights into two groups, an outlier group and a Gaussian group;
it preserves the former in full 32-bit fidelity and represents the latter with $2^b$ centroids, which are 32-bit floating point numbers.
%for the latter, it represents them with $2^b$ centroids. 
A weight is deemed as an outlier if the probability of it belongs to the Gaussian distribution is below a configurable threshold;
the larger the threshold, the more full-fidelity outliers, hence the lower compression ratio.  

Following the same practice in~\cite{gobo}, we use $-4$ which is sufficient in maintaining accuracy while maximizing compression ratio;
under the threshold, the outlier group constitute less than $0.1\%$ of total weights. %which is preserved in full precision (i.e. 32-bit). %and incurring only 1\% accuracy degradation. 
For the Gaussian group which constitute the rest $99.9\%$, the system sorts and splits its weights into $2^b$ clusters with equal population;
each cluster has \textit{one} centroid to represent \textit{all} values within it. 
%It then represents \textit{all} values in each cluster with \textit{one} centroid, which is indexed by a $b$-bit integer.
%It then represents \textit{all} values in each cluster with \textit{one} cluster centroid by substituting them with a $b$-bit index to the centroid.
Doing so caters to the weight distribution: weight-concentrated regions deserve higher resolutions, hence having more clusters and centroids.
%the vast majority ($99.9\%$) of original 32-bit weights are represented by $b$-bit integers, reducing model size by $\lfloor 32/b \rfloor \times$.
To decide cluster centroids, prior work adopt K-means based approaches~\cite{deep-compression, zhaoImprovingNeuralNetwork}, which are time-consuming, e.g. it takes a few hours to converge on our server.
Differently, we have found the arithmetic mean of cluster weights suffices -- a 2-bit version takes a few minutes to converge and incurs only 7\% accuracy degradation compared with the full model. 
We will present more results in \sect{eval}.  
%It uses the Gaussian model to find out a group of ``outliers'' parameters and preserve them in full precision.
%For the rest, the system quantizes them into $n$-bit integers (e.g. typically 2 to 4) using \textit{simulated quantization}~\cite{quantization-survey}, where each integer points to a full-precision FP32 value called a centroid, representing a group of original weights.
%The system decides the centroids by dividing the non-outlier parameters into $2^n$ groups and calculating their arithmetic means.

%The rationale is ....
%\Note{quantization rationale..}
%Second, attention head weights are heavily redundant~\cite{16heads}.
%%Most need only a few bits~\cite{ibert,binarybert} while only outliers need high-precision.
%Preserving the few outliers (e.g. 0.01\%~\cite{gobo}) while representing the most others with a small number of values ensures performance.
\end{comment}

%The system repeats the process for each fidelity version and generates a dictionary as the compression metadata, which specifies the centroids and the outlier mapping of full-fidelity weights.

\Note{how are they stored..}
\Note{compute cost of compression/decompression..}
\paragraph{Third, generating shards per version}
%After partitioning, a shard contains $1/M$ of a layer's total parameters, each is a $b$-bit centroid index.
To generate shards, the system compresses the vertical slices using the dictionaries produced by simulated quantization: 
for \textit{all} 32-bit parameter, the system looks up the dictionary and uniformly substitutes them with $b$-bit integers, each pointing to one of the $2^b$ centroids.
It does not preserve the 32-bit outliers in the newly compressed weight matrix to avoid destroying the $b$-bit data alignment.
It stores the compressed weights as the data and dictionaries (centroids, outliers) as the metadata of model shards on disk.
This is shown in Figure~\ref{fig:design:shards}. %\xzlNote{Fig 4 needs update, showing the workflow}
The system generates $N \times M\times K$ such shards and stores them on disk by their identities using a three-tuple $S=(n, m, b)$, where $n$, $m$ are the indexes of the layer and vertical slice respectively, $b$ is the fidelity.
It co-locates their disk blocks for access locality.
%Instead, it stores the outlier mapping separately to the compressed weights, which specifies 

Note that model shards \xzlNote{quantization} reduces IO but not computation (GFLOPs). \xzlNote{as opposed to XXX techniques. By doing so we avoid tedious per-model retraining as opposed to XXX (is this right?) and ensure to generate adequate compute workloads for high accuracy}
This is because they only change the representations of model parameters but not their amount.
For instance, by substituting 99.9\% of 32-bit weights with $b$-bit centroid indexes, a shard reduces IO by $\lfloor 32/b \rfloor \times$.
At inference time, the model retains GFLOPS by computing on the same amount of floating points decompressed from centroids and outliers;
while being inevitable, the decompression is efficient (10-20ms per layer) and can be further alleviated by designated hardware accelerator~\cite{gobo}.

%In uncompressed, full-fidelity form, their sizes are $1/M$ of a layer (e.g. a few MBs), taking tens of ms to load; 
%in lower fidelities, their IOs are even smaller and elastic w.r.t. bit fidelity. 
%%Hence a model shard equally slices the $j$-th layer it belongs to.
%Note: when in lower fidelities, shards cannot be used directly -- the weights are only indexes. 
%They cannot be used interchangeably, e.g. a 1 in 2-bit and 6-bit shard points to different centroids.  
%For instance, for the 1st layer with 3 shards,  


%Since the vast majority ($99.9\%$) of 32-bit weights can map to centroids, which are indexed by $b$-bit integers, the model size is reduced by $\lfloor 32/b \rfloor \times$.

%Following~\cite{dynabert}, the attention score and output of a layer can be defined as:
%
%\begin{equation}
%	\label{eq:out}
%\end{equation}
%
%Therefore as listed in equation~\ref{eq:out}, the output of a \tfm{} layer can be regarded as the sum of independent model shards, allowing partial execution of the model.

%\paragraph{Storing model shards}
%The system stores all versions of shards and their corresponding centroids on disk. %and pick selectively at run time. 
%Unused ones (e.g. for other tasks) can be further compressed via lossless compression (e.g. Zip). 
%This is possible because of low entropy.
%%Will evaluate its size (smaller than a HD movie) and compression efficiency (>90\%). 
%\Note{why not only store 6bit and derive the others?} 
%Doing so requires to \textit{always} load 6-bit shard IO delays.
%Not elastic, may miss deadline.

%\xzlNote{need cost analysis? }
%At least mention prior work on hardware accelerator


 



==> recycle/intro-0624.tex <==
% !TeX root = main.tex

\section{Introduction}
\label{sec:intro}

%\Note{Fig1: mark the resource elasticity, prior work vs our work}

\input{fig-overview-timeline}

%\footnote{\textbf{XXX why need this?} Specifically, we target Arm devices with CPUs capable of floating point operations, e.g. Cortex-A73}~\cite{mengwei19www}. 

Natural Language Processing (NLP) is seeing adoption by many mobile applications~\cite{ipa-survey}. % \xzlNote{cite}
%A well-known application is Intelligent Personal Assistant (IPA): users verbally query information such as traffic~\cite{ipa-survey} and dictate tasks such as navigation~\cite{myersIntelligentPersonalAssistant2007}.
%For instance, users verbally query information such as traffic~\cite{ipa-survey} and dictate tasks such as navigation~\cite{myersIntelligentPersonalAssistant2007}.
For instance, a note-taking app allows users to verbally query for old notes and dictate new notes. 
Under the hood, the application invokes modern language models in order to make inference on user input. % and generate response. 
As modern NLP models are pretrained and then fine-tuned \xzlNote{cite}, 
different applications run NLP models tuned for their respective NLP tasks, e.g. one for sentiment classification and one for sequence tagging. 


IPA exemplifies the typical usage of mobile NLP: 
user engagements are impromptu; 
%just as other mobile tasks~\cite{falakiDiversitySmartphoneUsage,mobile-usage-imc15,mobile-usage-sigir20,mobile-usage-chi16}; 
each engagement is as brief as a few seconds~\cite{ipa-study-denmark}; 
%each utterance often has 10-20 words~\cite{tsaiFasterResponsesAre2019}. 
% To gain adoption, interactive NLP shall deliver latency lower than \xzlNote{XXX} ms, often mandated as a deadline~\cite{edgebert}. 
users expect short delays (lower than \xzlNote{XXX} ms), often mandated as target latencies of NLP tasks~\cite{edgebert}. 

This paper focuses on maximizing NLP inference accuracy towards a target latency $T$. 
We consider \textit{on-device} NLP inference. 
To mobile users, 
on-device execution crucially preserves privacy and eliminates network trips to the cloud. \xzlNote{cite}
We focus on Transformer-based models such as BERT, which are the norm for modern NLP. \xzlNote{cite}: 
such a model comprises a sequence of layers (e.g. 6 or 12) to be executed in order. 

 
A key challenge of on-device NLP is the large model size: 
numerous parameters of a model must be loaded from flash storage to memory for execution. 
% As their defining characteristic, 
Towards generalization and accuracy, NLP models are designed to be over-parameterized \xzlNote{cite}. 
It is common that an NLP model has a few hundred MBs each \xzlNote{cite}, much larger than other ML models such as vision which is often XX--XX MBs each \xzlNote{cite}.
Loading such a model often takes longer than the actual model execution. 
As we will show,  DistilBERT, a popular NLP model for mobile, takes XXX seconds to load from embedded flash,  much longer than the computation (XXX ms) and 
what a user would desire (a few hundred ms). 


%Therefore, a model's parameters are likely to be out of memory in part or in full as an execution starts, requiring the model parameters to be loaded as the execution goes on. 
%As it is impractical to pin NLP models in memory permanently
%While it may be possible to satisfy the memory demand \textit{temporarily} at the execution time (to store both parameters and activations), 
%it is impractical to pin these NLP models in memory permanently for future executions. 
%As a model is unlikely to be fully in memory as an execution starts, the model weights shall be loaded during the execution. 
%Given the fragmented smartphone memory \xzlNote{cite}, a likely case is cold start, where execution starts with no weights in memory. 
% IO for model loading will be an integral part of model execution. 
%Ideally, IO and computation should enjoy high pipeline parallelism, and IO should not starve the computation. 
% As we will show, IO is often the bottleneck, starving the computation. 

How to load and execute NLP models timely? There are a few common approaches (Figure XXX).
(1) Preload model in memory: 
%this includes loading the model upon a model is loaded upon users request, as done in many ML frameworks
%This adds model loading IO (as long as XXX seconds) to user perceived delays, far exceeding ideal delays of XXX ms. 
loading a model speculatively before user engagement (invoking NLP models) 
or keep the model linger in memory after executing with it. 
The efficacy is limited for multiple reasons. 
An NLP model in memory increases one app's memory footprint (often XX MBs \xzlNote{cite}) by several times, making the app much more likely to be killed by the OS. 
Since user engagements are impromptu, precisely predicting timing is challenging. \xzlNote{cite}
As each engagement consists of as few as 2-3 turns (executions)~\cite{ipa-study-denmark}, the benefit of a lingering model is limited. 

%the first execution always suffers from 

%Predicting how long the model will be needed is difficult, as 
% as an engagement starts, NLP models are likely to have been evicted since the last engagement; 

%(2) Load during execution: 
(2) Pipelined load and execution: 
load a model layer prior to its execution and discard it afterward; 
meanwhile, overlap computation and IO: executing layer $k$ while loading layer $k+1$.
%While such a compute/IO pipeline can hide IO delays for some ML models \xzlNote{cite}, 
While overlapping compute and IO can hide IO delays for some ML models \xzlNote{cite}, 
doing so for common NLP models is ineffective:
the core parts of NLP models such as attention has low arithmetic intensity \xzlNote{cite}, 
and therefore %demanding intense data move while low computation. 
highly skewed IO/compute time (XXX seconds vs. XXX seconds per layer, see XXX for details). 
As a result, for XXX\% of the time the pipeline blocks on IO and computation stalls. 

%Section XXX further discusses related ML techniques such as model compression.

These existing approaches miss two opportunities.
%These approaches suffer from two common flaws.
%NLP execution under commodity frameworks lacks resource elasticity. 
%(2) IO and computation lack parallelism.
% (2) Low compute utilization. \xzlNote{pipeline stall...}
First, key resources -- the preload buffer, IO, and computation -- are managed in isolation and lack coordination. 
Hence, the preload buffer holds parameters that could have been loaded during execution; IO loads excessive parameters that the computation cannot consume within the target latency.
This results in memory waste, frequent pipeline stalls, and inferior model accuracy. 
Second, 
%while NLP model parameters are known redundant \xzlNote{cite}, 
% the pipeline is oblivious to the importance of model parameters: 
%the system loads and consumes parameters without prioritizing ones with higher impact on the inference accuracy (termed as \textit{parameter importance}). 
the system loads and consumes parameters while being oblivious to their importance, i.e. which parameters have higher impact on model accuracy. 

%\paragraph{Our principles...} We identify two principles. 


\paragraph{Our key idea}
%(1) \textit{maximize utilization of multiple resources}. 
% The key idea is to manage a language model as fine-grained, individually tunable shards for resource-elastic execution.
%We build our system on resource-elastic NLP models. 
We co-design NLP models and its execution pipeline. 

\textit{(1) Model as elastic shards}
We make NLP models resource-elastic by splitting a model as small \textit{shards}. 
By selecting shards and tuning their fidelity for execution, the engine can fine control the resource of the whole model as well as of individual shards: dynamically varying the model's  execution time, allocating IO bandwidth among shards, and adjusting compute/IO ratio per shard. 
%from which a subset can be dynamically composed and executed to fit time constraints. 
%To fit resource constraints, 
%the system dynamically composes a subset of the shards and schedules an execution pipeline. 


%\paragraph{Model as elastic shards}
\paragraph{(1) Model as composable shards}
\xzlNote{k-version sharding... a good term??}
Given a model of N layers, \sys{} preprocesses it by partitioning each layer into $M$ shards; 
%for each shard, it creates $K$ fidelity versions, 
it compresses each shard as $K$ fidelity versions, 
each version with a different bitwidth to represent the shard's weights. 
\sys{} therefore stores the $NxMxK$ shard versions on flash. 
%Model shards gives the engine high flexibility of executing a fraction of the model: 
With sharding, the engine can execute a selective \textit{submodel}:
select a subset of $n$ layers ($n<=N$); 
for each selected layer, select $m$ shards ($m<=M$); 
for each selected shard, select a fidelity version. 
\textit{Any such combination of shards \xzlNote{? submodel??} will generate meaningful inference results}, albeit with different accuracies and resource costs. 
Modeling sharding is a new combination of existing ML techniques -- dynamic Transformers \cite{dynabert} and Transformer quantization \xzlNote{cite}.

%By selecting and assembling individual model shards, the engine tunes a resident model via three knobs: 
%1) \textit{widths}. 
%The engine adjusts the number of shards within a resident model layer.
%2) \textit{depths}.
%It stacks/unstacks resident model layers by adding/removing respective shards in their layers.
%3) \textit{fidelity}.
%For every single shard of the resident model, the engine may adjust its fidelity independently.  




\xzlNote{to merge...}
The engine jointly manages preloaded shards and its execution pipeline. 
\sys{} preloads a set of shards in memory, dynamically adjusting the set size to fit in the memory budget set by the OS. 
Spanning a model's bottom layers (closer to input), 
preloaded shards allow execution of these layers to start with much of their parameters already in memory, which otherwise would have to stall for IO. 
Through selecting fidelity of individual shards, 
the engine adjusts IO delays to computation delays,
keeps the pipeline non-stalling: 
%hence never stalling computation in the pipeline. 
IO for layers $1..k$ always completes prior to the execution with layer $k$, 
The engine selects higher fidelity for more important shards, hence allocating more IO bandwidth to shards that would result in higher accuracy gain. 
%Overall, the engine achieves high utilizations of compute and IO, executing the most important shards that maximize the accuracy. 

Based on the shards, 
the engine co-plans a preload buffer and a pipeline of computation/IO. 
In the background, it maintains a set of shards in memory (\textit{preloaded shards}); 
in response to user request, the engine bootstraps the pipeline with the preloaded shards and loads/executes additional shards of its choice. 
As a result, 
% the pipeline enjoys high computation/IO parallelism; 
computation and IO are utilized with high parallelism; 
important shards are loaded and consumed with priority; 
the results enjoy high accuracy. 



%(2) that the inference engine judiciously assembles and tunes shards in order to orchestrate the demands for multiple resources. 
% (2) for each execution, the inference engine judiciously assembles and tunes shards according to available resources. 


%We instantiate the idea as an inference engine called \sys{}. 




\xzlNote{shard importance -- ranking}



\paragraph{(2) The planner}
The engine's planner selects shards to preload and to execute. 
The challenge is to come up with a submodel from the huge configuration space that can be executed within the deadline, minimum pipeline stalling, and maximum accuracy. 
To this end, the key is to track fine-grained IO budgets: 
the spare IO for loading a shard $S$ is the time between loading all shards prior to $S$ and the time the computation with $S$ starts; 
for a non-stalling pipeline, no shard (or layer) should have deficient IO budgets. 
%To this end, the key insight is to set accumulative IO budgets across layers and then allocate IO budgets among shards by considering their importance.  

With this insight, \sys{} first plans a maximum submodel (with maximum width and depth) that can be computed within T (it favors a deeper model over a wider one). 
The engine sets \textit{accumulated IO budgets} at each layer as the computation delays of all prior layers. 
With the budgets, the engine iterates over all shards in the descending order of their importance, setting higher (bitwidth) for more important shards and accordingly debit the accumulated IO budgets of all subsequent layers; 
when no shards can use higher fidelity without any AIB deficiency, 
the engine concludes planning. 
The engine then preloads the first $k$ shards in the layer order (pipeline/consumption execution order) that maximizes usage of given free memory $M$ but not exceeding $M$. 

\xzlNote{old}

The plan ensures high pipeline parallelism: each shard's IO must complete before the shard's computation starts, and the total IO times max out the budget T. 
The plan maximizes model accuracy with empirical heuristics: the engine prioritizes loading nonresident shards in low fidelity over upgrading resident shards to higher fidelity; 
to pick shards for loading or upgrading, it prioritizes shards with higher impact on accuracy, for which it profiles ahead of time. 
% it prioritizes shards at top model layers over shards at bottom layers. 



By adjusting $n$ and $m$, the engine scales the required computation close to the deadline; 
by setting fidelity versions 
%$\{k_i\},i=1..m \times n$ 
$\{k_{i=1..m \times n}\}$, the engine scales per shard IO delays (without affecting computation much), corrects the skewed IO/compute ratio, and therefore enjoy high IO/compute parallelism. 
Tuning these knobs jointly, the engine adjusts the memory footprint of the resident model in response to the system memory pressure. 


The engine also provides background model preload/unload, for which the engine inflates or deflates the resident model to a given memory budget $M$. 
It does so by tuning individual shards, including preloading new shards or unloading existing ones, as well as upgrading/downgrading their fidelities.


\paragraph{Results}
As a result, we implement \sys{} on XXX dev board with Pytorch in XXX SLOC.
We conduct comprehensive benchmarks on GLUE benchmark...


With all these, timely NLP inference (?? accuracy loss) is possible with low memory cost (XXX\% a small fraction) of the total model size. 


%exploits IO/compute parallelism to upgrade the model while executing inference on the fly;

%instructed by the OS and user, it manages the resident model in full elasticity: depending on available IO/compute/memory resources, it may not only in/deflate its depths and widths, but also down/upgrade its precisions.
\begin{comment}
instructed by the OS and user, it manages the resident model in four-way elasticity:
during inference, it down/upgrades the model precisions while executing inference on the fly by exploiting IO/compute parallelism; 
in the background, it de/inflates the resident model depthts and widths w.r.t. memory pressure.
\end{comment}
%it leverages available IO/memory resources to up/downgrade the resident model, both on and off the inference critical path.

%The resident model reconciles cold v.s. hot inference dichotomy by keeping the inference \textit{warm}: 
%%it provides a skeleton/backbone, just enough to warm up the next inference;
%%while always in-memory, it responds to OS memory pressure and is elastic -- low precision (resembling cold inference) to even full precision (resembling hot inference full model). 
%%it is always in memory, eliminating cold inference;
%%yet, it is resource-elastic -- depending on OS, it may expand to full precision, resembling full model in hot inference. 
%the inference is never cold, as it is always bootstrapped by the resident model;
%as long as memory permits, the resident model will keep being upgraded during rounds of (warm) inferences, eventually resembling a full model in hot inference.

\begin{comment}
First, from the full-fledged model the engine derives multiple lower-precisions versions on disk.
Instead of the full-fledged model, the engine starts with a small \textit{resident model} in memory. 
Such a resident model is fully elastic to OS resources: 
in the foreground during inference, the engine upgrades the resident model by loading extra versions from disk, whose IO overhead is hidden by overlapping with compute;
in the background, when the memory pressure is high, engine downgrades the resident model, as instructed by the OS.
The resident model reconciles cold v.s. hot dichotomy by keeping the inference \textit{warm}: 
%it provides a skeleton/backbone, just enough to warm up the next inference;
%while always in-memory, it responds to OS memory pressure and is elastic -- low precision (resembling cold inference) to even full precision (resembling hot inference full model). 
%it is always in memory, eliminating cold inference;
%yet, it is resource-elastic -- depending on OS, it may expand to full precision, resembling full model in hot inference. 
the inference is never cold, as it is always boosted by the in-memory resident model;
as long as system memory permits, resident model will keep being updated during rounds of (warm) inferences, eventually resembling a full model in hot inference.
%Instead of either preserving a full model file in memory or none at all, 
%To this end, the engine keeps a \textit{resident model} always in memory to kick start inferences. 
%To this end, the engine permanently deploys a \textit{resident model} in memory. 
%%To this end, the engine keeps a small \textit{resident model} always in memory (e.g. 5\% of the full model) to kick start inferences. 
%%Compared with prior dynamic models~\cite{layerdrop,edgebert,dynabert}, 
%A resident model is fully elastic to OS resources: in the foreground of the inference critical path, the engine leverages... 
\end{comment}

\begin{comment}
%% below useful
To this end, the engine derives multiple versions from the full-fledged model into different, lower precisions.
Instead of having the full model file either in memory or on disk, the engine keeps one version called \textit{resident model} always in memory, while leaving the rest on disk.
%A resident model is elastic and adaptive to system resources.
%a tiny portion (e.g. 5\%) of the original model, while keeping the rest \textit{XXX model} on disk (\Note{XXX} MB).
In the foreground, of the inference critical path, %invoked by the user, 
the engine uses the small resident model to kickstart inference while live patching it with on-disk versions for greater accuracy;
%the engine uses the resident model as a skeleton and live patches it with on-disk versions;
it hides the IO overhead of loading from disk by overlapping it with computing on the resident model. 
In the background, the engine adapts the elastic resident model structure to memory pressure as instructed by the OS. 
The resident model reconciles cold v.s. hot dichotomy by keeping the inference \textit{warm}: 
%it provides a skeleton/backbone, just enough to warm up the next inference;
%while always in-memory, it responds to OS memory pressure and is elastic -- low precision (resembling cold inference) to even full precision (resembling hot inference full model). 
%it is always in memory, eliminating cold inference;
%yet, it is resource-elastic -- depending on OS, it may expand to full precision, resembling full model in hot inference. 
the inference is never cold, as it is always boosted by the in-memory resident model;
as long as system memory permits, resident model will keep being updated during rounds of (warm) inferences, eventually resembling a full model in hot inference.
\end{comment}

%it is always in memory and can be directly used as-is;
%it is runtime elastic, adaptive to OS memory pressure;

%\Note{below}
%our key construct is a resident model ... (compressed form, always in memory)
%unlike static compression which lacks flexibility. resident model are more flexible..
%IT is meta model structure (bare minimum?)...
%decomp. on-demand...

%\Note{bring out planner, describe pipeline. Define goals.}
%\Note{merge below}
%Following the perspective, we present \textbf{S}peedy \textbf{T}ransformer \textbf{I}nference (\sys{}), a novel \tfm{} inference engine. 
%First, the engine derives multiple lower-precision versions \Note{this is to increase elasticity in IO of the pipeline...} from the full-fledged model and persists them on disk.
%It exposes an inference deadline $T$ and a memory threshold $M$ to user and OS respectively. 
%Bound by the two constraints, it manages the resident model while maximizing inference accuracy: 
%during inference, it loads parameters from versions which benefit most to current resident model accuracy under $T$; 
%in the background, it unloads the versions which hurt accuracy the least when $M$ decreases.

\begin{comment}
% below useful to explain why cold start happens for mobile platforms:
% constrained resources, inflexible memory structure, rigid inference engine design, ..
%
Cold start happens frequently on mobile platforms. 
First, mobile devices are resource-constrained. 
They usually have limited RAM, e.g. a few GBs~\cite{mengwei19www,dnn-mobile-imc}, much less than that of a desktop or server.
It is impractical to pin a \tfm{} model file into memory, only to respond to a bursty application use pattern~\cite{falakiDiversitySmartphoneUsage}. 
Second, multiple apps, along with their data, compete for the scarce memory.  
As a consequence, model files are swapped out frequently from filesystem page cache~\cite{dnn-mobile-lat-var}, leading to cold start inference from time to time when invoked. %next time they are invoked.
\end{comment}

%This is because during \textit{cold start}, the deep learning (DL) framework (e.g. PyTorch~\cite{pytorch-web}, TensorFlow~\cite{tensorflow-web}) must load the model file from the underlying storage medium (e.g. SD card, embedded flash) into memory before proceeding to inference computation. 

%Such high latency is unacceptable to user experience in interactive tasks.
%In comparison to \textit{hot start}, the \textit{cold start} inference happens when the deep learning (DL) framework (e.g. PyTorch~\cite{pytorch-web}, TensorFlow~\cite{tensorflow-web}) must load the model file from the underlying storage medium (e.g. SD card, embedded flash) into memory before proceeding to inference computation. 

\begin{comment}
% cold start breakdown. Vs hot inference is 26x higher. 
Figure~\ref{fig:motiv:lat-breakdown} shows the cold vs hot start inference latency of three models (i.e. \textbf{Mob}ileBERT~\cite{mobilebert}, \textbf{Dis}tilBERT~\cite{distilbert}, and \textbf{BERT}~\cite{bert}) running on Odroid~\cite{odroid-web} with PyTorch.
As can be seen, the cold start inference latency is as 26$\times$ higher than that of hot start. 
\Note{show more evidence on breakdown later}
\end{comment}


%Yet, the large size of a \tfm{} model (e.g. hundreds of MBs) imposes a significant \textit{cold start} inference latency of \tfm{}s on mobile/edge devices\footnote{Specifically, we target Arm devices with CPUs capable of floating point operations, e.g. Cortex-A73}, as high as a few seconds. 


%\input{fig-lat-breakdown}

\begin{comment}
\paragraph{Cold inference is not uncommon}
Cold inference happens when the model parameters are uncached in memory, a machine learning framework must load them from underlying flash/disk storage to execute an inference task. 
%Cold inference happens when the machine learning framework must load model parameters from underlying flash/disk storage. 
It is not uncommon for transformers on mobile platforms for the following two reasons:
\begin{myenumerate}
	\item 
	Mobile devices are resource-constrained; 
	they usually have limited RAM, e.g. a few GBs, much less than that of a desktop or server.
	Hence, to accommodate various applications in the narrow address space, cached files are frequently swapped in and out of memory\Note{cite}. 
	
	\item 
	They invoke transformer in an ad hoc and on-demand fashion, unlike a serving scenario in the cloud.
	Plus, transformer models are large (a few hundred MBs), making it uneconomic to always host them in memory.
\end{myenumerate}
\end{comment}



% \begin{myenumerate}
% 	\item 
% 	Mobile devices are resource-constrained; 
% 	they usually have limited RAM, e.g. a few GBs, much less than that of a desktop or server.
% 	Hence, to accommodate various applications in the narrow address space, cached files are frequently swapped in and out of memory\Note{cite}. 
% 	
% 	\item 
% 	They invoke transformer in an ad hoc and on-demand fashion, unlike a serving scenario in the cloud.
% 	Plus, transformer models are large (a few hundred MBs), making it uneconomic to always host them in memory.
% \end{myenumerate}

%This is because constrained by only a few GBs of RAM, mobile devices cannot afford long-live in-memory residency of model parameters;
%%unlike serving scenario on a server, they execute inference tasks sporadically, driven by applications; 
%to execute an inference task, they often load the parameters from persistent storage (i.e. cold), unlike serving scenario on a server which already hosts model file in memory (i.e. hot).


%In bringing on-device transformers inference to mobile/edge devices, the overwhelming model sizes of transformers give rise to a unique challenge: high \textbf{cold inference} latency -- as high as a few seconds and the it is dominated by IO (over 90\%) instead of compute, which we will characterize and provide more evidence in \sect{motiv}.
%The overwhelming model size of a transformer gives rise to a unique challenge for mobile/edge devices under a \textbf{cold-start} scenario. 
%The overwhelming transformer model size gives rise to a unique challenge for mobile/edge devices: high cold-start inference latency. 

%\paragraph{Design objectives}
%We seek to design a new system for reducing the \textit{cold start} inference latency of \tfm{}s on mobile devices. 
%We target two goals:
%\begin{itemize}
%	\item 
%	\textit{Latency.}
%	The system should withstand frequent cold start while still delivering the inference results with low latency.
%	
%	\item 
%	\textit{Accuracy.}
%	Meanwhile, the system should not compromise inference accuracy. 
%	It needs to maximize the accuracy, and ensure it is competitive to state-of-the-art models.
%
%%	\item 
%%	\textit{}
%
%\end{itemize}
%
%\Note{merge below}
%\textbf{Design goals:}
%\begin{myenumerate}
%	\item 
%	Fast cold inference latency
%	
%	\item 
%	Comparable hot inference accuracy
%	
%	\item 
%	Small memory footprint	
%\end{myenumerate}


% --- obsolete --- 
%\paragraph{Our approach}
%\Note{ideas... TODO}
%
%\textbf{First, model sharding.}
%The pretrained model must be partitioned into fine-grained pieces, which have the following properties:
%\begin{itemize}
%	\item 
%	Partial expressiveness of the full model.
%	The pieces must carry semantic information and language features, such that they can form subnets and be executed. 
%	
%	
%	\item 
%	Incremental accuracy. 
%	More pieces -> better accuracy. \Note{where to forecast execute incrementally?}
%	
%	
%	\item 
%	Minimum pipeline bubble.
%	\Note{actually should not be `close'}. 
%	Instead, should be as small as possible -- you can never ``starve'' IO because you can always load extra. 
%	
%	This is to create the pipeline which has high utilization and small bubbles. 
%	We donot want CPU to starve and wait for IO.   
%\end{itemize}
%
%\paragraph{Opportunities}
%We plan to exploit the following opportunities:
%\begin{myenumerate}
%	\item 
%	Need pipeline parallelism of io/compute. 
%	Currently the resources of a mobile SoC are under-utilized. 
%	Existing work focuses on compressing a model and reducing its size, e.g. via quantization~\cite{tenarybert}, knowledge distillation~\cite{distilbert}, weight sharing~\cite{albert};
%	they still wait for the model loading to finish to begin inference computation, during which time the CPU is idle. 
%	%	E.g. DistilBert~\cite{distilbert} has half the layers of a BERT~\cite{bert} model. Yet, it is still 400 MB large and takes at least 2 seconds to load. 
%	%	Alternative compression approaches such as quantization~\cite{q8bert,tenarybert,binarybert,bibert}, often has inferior performance. 
%	
%	\item 
%	Partial model execution: the model can execute based on only partial parameters and can be gradually loaded up. 
%	This is possible due to MHA redundancy. 
%	Unlike vision networks, \tfm{}s exhibit high redundancy in its attention heads~\cite{16heads}.
%	As a result, with only a few (e.g. 4) attention heads, the performance degradation is only less than 10\%~\cite{dynabert}. %of a \tfm{} model 	
%\end{myenumerate}


\paragraph{Contributions}
The paper makes the following contributions:
\begin{itemize}
\item Model sharding ... make elastic computation and IO time .. whole model as well as individual parts. 

\item Execution paradigm: a preload buffer for warming up pipeline; 
high efficient pipeline execution; 
execution with elastic IO and computation; minimized stalling; maximize computation and IO utilization. 

\item Planner: plan by selecting shard versions for execution. Based on accumulated IO budgets and shard importance. Multi step (stage) planning: computation (model depth and width; executable fraction; then iteratively allocate bitwidth to important shards; respect time constraints) 
\end{itemize}



==> recycle/intro-recycle-xzl.tex <==
% !TeX root = main.tex

\section{Introduction}
%\section{Motivations: high cold start inference latency of Transformers}
\label{sec:intro}

\Note{Fig1: mark the resource elasticity, prior work vs our work}


%\footnote{\textbf{XXX why need this?} Specifically, we target Arm devices with CPUs capable of floating point operations, e.g. Cortex-A73}~\cite{mengwei19www}. 

Interactive Natural Language Processing (NLP) tasks are popular on mobile devices. \xzlNote{cite}
A well-known application is Intelligent Personal Assistant (IPA), with which users verbally query information such as traffic~\cite{ipa-survey} and dictate tasks such as navigation~\cite{myersIntelligentPersonalAssistant2007}.
Under the hood, the application invokes modern language models such as the Transformer-based BERT \xzlNote{cite} in order to make inference on user input and generate response accordingly. 
% (which may or may not be based on NLP). 

IPA exemplifies the typical usage of mobile NLP: 
users request model execution in an impromptu fashion just as other mobile tasks ~\cite{falakiDiversitySmartphoneUsage,mobile-usage-imc15,mobile-usage-sigir20,mobile-usage-chi16}; 
each user engagement is brief, reported to constitute 2-3 interaction turns and last a few seconds~\cite{ipa-study-denmark}. 
%each utterance often has 10-20 words~\cite{tsaiFasterResponsesAre2019}. 
% To gain adoption, interactive NLP shall deliver latency lower than \xzlNote{XXX} ms, often mandated as a deadline~\cite{edgebert}. 
User-perceived delays are expected to be lower than \xzlNote{XXX} ms, often mandated as a deadline to NLP tasks~\cite{edgebert}. 

This paper targets NLP inference on devices such as smartphones. 
% optimizing for maximum inference accuracy under given deadlines. 
% We consider client devices such smartphones, for which 
To these devices, 
on-device execution crucially preserves user privacy and eliminates network trips to the cloud. \xzlNote{cite}
On-device NLP has the following characteristics. 
\Note{the two have some entanglement}
(1) \textit{IO as an integral part of execution.} 
As modern NLP models are large (several hundred MBs each, as compared to a few GBs of total physical memory) and each invocation of NLP is brief, it is inefficient to pin these models in memory permanently.  
Therefore, a model's parameters are likely to be out of memory in part or in full as an execution starts, requiring the model parameters to be loaded as the execution goes on. 
%Given the fragmented smartphone memory \xzlNote{cite}, a likely case is cold start, where execution starts with no weights in memory. 
%Transformers-based NLP models are memory hungry: 
%each model often has XXX--XXX MBs of parameters; 
%multiple models are needed for separate NLP tasks, e.g. one for sentiment classification and one for sequence tagging. 
%As it is impractical to pin NLP models in memory permanently
%While it may be possible to satisfy the memory demand \textit{temporarily} at the execution time (to store both parameters and activations), 
%it is impractical to pin these NLP models in memory permanently for future executions. 
%As a model is unlikely to be fully in memory as an execution starts, the model weights shall be loaded during the execution. 
%Given the fragmented smartphone memory \xzlNote{cite}, a likely case is cold start, where execution starts with no weights in memory. 
% IO for model loading will be an integral part of model execution. 
%Ideally, IO and computation should enjoy high pipeline parallelism, and IO should not starve the computation. 
% As we will show, IO is often the bottleneck, starving the computation. 
(2) In the background, NLP models move in and out of memory frequently -- in response to memory pressure or preload policies that NLP apps may implement. 
To summarize, on-device NLP needs orchestration of multiple resources -- compute, IO, and memory. 
% Of such an execution, a defining is that it demands multiple resources -- compute, IO, and memory. 


Our design goal is to maximize NLP inference accuracy under a deadline $T$. 
We identify two principles. 
(1) \textit{maximize utilization of multiple resources}. 
At execution time, higher CPU/GPU usage yields more GFLOPs; higher IO usage loads more (high fidelity) model parameters that are too large to be always \textit{resident} in memory; both lead to higher accuracy. 
%In the background, opportunistic preload of model parameters as memory becomes available, so that the upcoming inference execution starts with more model parameters in memory, which ... 
% It is also essential to preload/unload model parameters opportunistically as the available memory fluctuates, so that an inference execution starts with more model parameters in memory. 
(2) \textit{spend resources on a model's most important portions}. 
Modern language models are known over-parameterized and to contain redundant information \xzlNote{cite}. 
When executing a model in full cannot be done in $T$, the execution engine should execute model portions that have higher importances to accuracy. 

% computation, model memory footprint, and IO.
These principles call for elastic, joint management of resources: 
computation shall keep operating throughout the period until the deadline; 
% IO should form a pipeline with the computation, loading adequate parameters for the computation without starving it; 
IO should keep loading model parameters and feeding the computation, but not taking too long in case it may starve the computation; 
in the background, model parameters should be loaded and unloaded in small chunks according to memory availability. 

%While there exist techniques to scale individual resource types needed by an NLP model \xzlNote{cite}, there lacks a mechanism for managing the resources \textit{in a joint fashion}, result in low efficiency or low accuracy. 

Unfortunately, such resource management is absent under the current OS and ML frameworks.
%NLP execution under commodity frameworks lacks resource elasticity. 
(1) Model memory is managed in rigid, coarse granularity. 
A model's parameters are loaded/unloaded in pages, model layers, or even entirety, oblivious to how these parameters affect the model accuracy differently. 
% without accounting for the impact on model accuracy. 
% or subject to OS paging which is oblivious to the relative importance of weights. 
(2) IO and computation lack parallelism.
%IO blocks computation. 
An ML framework often loads an entire model or a layer prior to its execution.
While layerwise computation/IO pipelining is possible~\xzlNote{cite}, doing so with existing NLP models results in large pipeline bubbles and starves computation, as over-parameterized NLP models have highly skewed IO/compute ratios. 
As evidence, Section XXX characterizes the cold-start inference.

Recent techniques can scale resources for NLP execution~\xzlNote{cite} \textit{individually} but not jointly. 
% but there lacks a mechanism for managing the resources \textit{in a joint fashion}, result in low efficiency or low accuracy. 
For example, model compression reduces the model load IO~\cite{mobilebert,layerdrop,distilbert,bibert,binarybert,q8bert}, but offers no solution on how to alter the IO/compute skewness.
DynaBert~\cite{dynabert} and NestDNN~\cite{nestdnn} instantiates a model's multiple versions with variable compute demands; 
they however offer no solution on co-scheduling model execution and loading in parallel, which includes loading a version from scratch and loading the deltas between model versions.
%not accounting for IO delays that would interleave with the computations. 
These techniques are inadequate for our goal. 

%\input{intro-xzl-comment}

\paragraph{Our approach}
We present an inference engine called \sys{}. 
The key idea is to manage a language model as fine-grained, individually tunable shards for resource-elastic execution.
\Note{one exciting sentence}

\Note{diff with dynamic NNs -- In a model space, dynamic transformers provide coarse-grained waypoints which can have high accuracy under memory/latency constraints, our system 1) expands the waypoints by refining them into finer granularity, 2) and more importantly, provides a path (IO/computation planning) to connecting the waypoints}

Dynamic \tfm{}s sample the large model space in coarse, fixed granularity. 
Ours samples the space with finer granularity, and connects the samples...


%(2) that the inference engine judiciously assembles and tunes shards in order to orchestrate the demands for multiple resources. 
% (2) for each execution, the inference engine judiciously assembles and tunes shards according to available resources. 
This is illustrated in Figure~XXX. 

%We advocate for the inference engine to take on a greater role in orchestrating IO, compute, and memory resources, as illustrated in Figure~XXX. 

%\xzlNote{merge the below into ``our approach''?}
%\paragraph{Challenges \& solutions}
%Through retrofitting a suite of known machine learning techniques, 

% \paragraph{Managing model in fine, elastic granularity}
%\paragraph{Managing model memory in elastic granularity}
\paragraph{Managing model memory in elastic shards}
Built atop the dynamic Transformer model~\cite{dynabert}, 
\sys{} preprocesses a model: partitioning each of the $N$ model layers into a set of $M$ shards, where each shard spans one Transformer attention head and $1/M$ FFN neurons of this layer. 
For each shard, it creates $K$ fidelity versions, which are lower-bit representations of this shard's weights. 
For instance, a full-fidelity version that represents each weight with 32 bits, a two-bit version that does so with 2 bits. 
We therefore store $NxMxK$ shard versions on disk. 
The preprocessing is a one-time effort per model; being light transformation of an existing model without pre-training, it can be done on device at the model installation time. 

\xzlNote{shard importance -- ranking}

% \sys{} hosts a long-running service that maintains an elastic \textit{resident model} in memory. 
%\sys{} hosts an elastic \textit{resident model} in memory. 
Sharing allows \sys{} to selectively load shards from disk and assemble a \textit{resident model} in memory. 
The resident model comprises a subset of shards loaded from the disk, 
for which the engine can configure on three dimensions: 
select a subset of $n$ layers; 
for each selected layer, select a subset of $m$ shards; 
for each selected shard $i \in m \times n$, select a fidelity version $k_i$. 
\textit{Any concrete resident model in the configuration space will generate meaningful inference results}, albeit in different accuracies. 

The resident model is dynamic: 
in response to resource availability (e.g. memory pressure) and model execution requests, the engine loads or evicts shards as well as switching among a shard's multiple versions, hence managing multiple resources elastically. 
%Model shards allow the engine to manage multiple resources elastically. 
By adjusting $n$ and $m$, the engine scales the required computation close to the deadline; 
by setting fidelity versions 
%$\{k_i\},i=1..m \times n$ 
$\{k_{i=1..m \times n}\}$, the engine scales per shard IO delays (without affecting computation much), corrects the skewed IO/compute ratio, and therefore enjoy high IO/compute parallelism. 
% so that IO and computation can enjoy high pipeline parallelism. 
Tuning these knobs jointly, the engine adjusts the memory footprint of the resident model in response to the system memory pressure. 


%By selecting and assembling individual model shards, the engine tunes a resident model via three knobs: 
%1) \textit{widths}. 
%The engine adjusts the number of shards within a resident model layer.
%2) \textit{depths}.
%It stacks/unstacks resident model layers by adding/removing respective shards in their layers.
%3) \textit{fidelity}.
%For every single shard of the resident model, the engine may adjust its fidelity independently.  



%it may stack/unstack shards to \textit{de/inflate} the model size; 
%it may also tune individual shards to \textit{down/upgrade} the model precisions/fidelity.
%Instead of the rigid full-fledged model, the engine starts with a small \textit{resident model} in memory.
%Instructed by the OS and user, it manages the resident model in four-way elasticity: 
%depending on available IO/compute/memory resources, it may not only \textit{de/inflate} its depths and widths, but also \textit{down/upgrade} its precisions/fidelity;




\xzlNote{``reshape'' -- not necessarily accurate. e.g. we do not throw away the un-executable shards}

\paragraph{The engine}
The engine's primary service is foreground model load/execution (deadline T), for which the engine inflates the current resident model, meanwhile executing a computation/IO pipeline. 
The challenge is how to plan the resident model inflation and schedule the IO/computation pipeline towards maximum accuracy. 
The engine does so in two steps: 
it first plans for computation: determine the maximum model width and depth that can be executed within T (it favors a deeper model over a wider one). 
It then plans for IO: allocate the IO time budget $T$ to $ m \times n $ shards. 
The plan ensures high pipeline parallelism: each shard's IO must complete before the shard's computation starts, and the total IO times max out the budget T. 
The plan maximizes model accuracy with empirical heuristics: the engine prioritizes loading nonresident shards in low fidelity over upgrading resident shards to higher fidelity; 
to pick shards for loading or upgrading, it prioritizes shards with higher impact on accuracy, for which it profiles ahead of time. 
% it prioritizes shards at top model layers over shards at bottom layers. 

The engine also provides background model preload/unload, for which the engine inflates or deflates the resident model to a given memory budget $M$. 
It does so by tuning individual shards, including preloading new shards or unloading existing ones, as well as upgrading/downgrading their fidelities.
	 
As a result, we implement \sys{} on XXX dev board with Pytorch in XXX SLOC.
We conduct comprehensive benchmarks on GLUE benchmark...


%exploits IO/compute parallelism to upgrade the model while executing inference on the fly;

%instructed by the OS and user, it manages the resident model in full elasticity: depending on available IO/compute/memory resources, it may not only in/deflate its depths and widths, but also down/upgrade its precisions.
\begin{comment}
instructed by the OS and user, it manages the resident model in four-way elasticity:
during inference, it down/upgrades the model precisions while executing inference on the fly by exploiting IO/compute parallelism; 
in the background, it de/inflates the resident model depthts and widths w.r.t. memory pressure.
\end{comment}
%it leverages available IO/memory resources to up/downgrade the resident model, both on and off the inference critical path.

%The resident model reconciles cold v.s. hot inference dichotomy by keeping the inference \textit{warm}: 
%%it provides a skeleton/backbone, just enough to warm up the next inference;
%%while always in-memory, it responds to OS memory pressure and is elastic -- low precision (resembling cold inference) to even full precision (resembling hot inference full model). 
%%it is always in memory, eliminating cold inference;
%%yet, it is resource-elastic -- depending on OS, it may expand to full precision, resembling full model in hot inference. 
%the inference is never cold, as it is always bootstrapped by the resident model;
%as long as memory permits, the resident model will keep being upgraded during rounds of (warm) inferences, eventually resembling a full model in hot inference.

\begin{comment}
First, from the full-fledged model the engine derives multiple lower-precisions versions on disk.
Instead of the full-fledged model, the engine starts with a small \textit{resident model} in memory. 
Such a resident model is fully elastic to OS resources: 
in the foreground during inference, the engine upgrades the resident model by loading extra versions from disk, whose IO overhead is hidden by overlapping with compute;
in the background, when the memory pressure is high, engine downgrades the resident model, as instructed by the OS.
The resident model reconciles cold v.s. hot dichotomy by keeping the inference \textit{warm}: 
%it provides a skeleton/backbone, just enough to warm up the next inference;
%while always in-memory, it responds to OS memory pressure and is elastic -- low precision (resembling cold inference) to even full precision (resembling hot inference full model). 
%it is always in memory, eliminating cold inference;
%yet, it is resource-elastic -- depending on OS, it may expand to full precision, resembling full model in hot inference. 
the inference is never cold, as it is always boosted by the in-memory resident model;
as long as system memory permits, resident model will keep being updated during rounds of (warm) inferences, eventually resembling a full model in hot inference.
%Instead of either preserving a full model file in memory or none at all, 
%To this end, the engine keeps a \textit{resident model} always in memory to kick start inferences. 
%To this end, the engine permanently deploys a \textit{resident model} in memory. 
%%To this end, the engine keeps a small \textit{resident model} always in memory (e.g. 5\% of the full model) to kick start inferences. 
%%Compared with prior dynamic models~\cite{layerdrop,edgebert,dynabert}, 
%A resident model is fully elastic to OS resources: in the foreground of the inference critical path, the engine leverages... 
\end{comment}

\begin{comment}
%% below useful
To this end, the engine derives multiple versions from the full-fledged model into different, lower precisions.
Instead of having the full model file either in memory or on disk, the engine keeps one version called \textit{resident model} always in memory, while leaving the rest on disk.
%A resident model is elastic and adaptive to system resources.
%a tiny portion (e.g. 5\%) of the original model, while keeping the rest \textit{XXX model} on disk (\Note{XXX} MB).
In the foreground, of the inference critical path, %invoked by the user, 
the engine uses the small resident model to kickstart inference while live patching it with on-disk versions for greater accuracy;
%the engine uses the resident model as a skeleton and live patches it with on-disk versions;
it hides the IO overhead of loading from disk by overlapping it with computing on the resident model. 
In the background, the engine adapts the elastic resident model structure to memory pressure as instructed by the OS. 
The resident model reconciles cold v.s. hot dichotomy by keeping the inference \textit{warm}: 
%it provides a skeleton/backbone, just enough to warm up the next inference;
%while always in-memory, it responds to OS memory pressure and is elastic -- low precision (resembling cold inference) to even full precision (resembling hot inference full model). 
%it is always in memory, eliminating cold inference;
%yet, it is resource-elastic -- depending on OS, it may expand to full precision, resembling full model in hot inference. 
the inference is never cold, as it is always boosted by the in-memory resident model;
as long as system memory permits, resident model will keep being updated during rounds of (warm) inferences, eventually resembling a full model in hot inference.
\end{comment}

%it is always in memory and can be directly used as-is;
%it is runtime elastic, adaptive to OS memory pressure;

%\Note{below}
%our key construct is a resident model ... (compressed form, always in memory)
%unlike static compression which lacks flexibility. resident model are more flexible..
%IT is meta model structure (bare minimum?)...
%decomp. on-demand...

%\Note{bring out planner, describe pipeline. Define goals.}
%\Note{merge below}
%Following the perspective, we present \textbf{S}peedy \textbf{T}ransformer \textbf{I}nference (\sys{}), a novel \tfm{} inference engine. 
%First, the engine derives multiple lower-precision versions \Note{this is to increase elasticity in IO of the pipeline...} from the full-fledged model and persists them on disk.
%It exposes an inference deadline $T$ and a memory threshold $M$ to user and OS respectively. 
%Bound by the two constraints, it manages the resident model while maximizing inference accuracy: 
%during inference, it loads parameters from versions which benefit most to current resident model accuracy under $T$; 
%in the background, it unloads the versions which hurt accuracy the least when $M$ decreases.

\begin{comment}
% below useful to explain why cold start happens for mobile platforms:
% constrained resources, inflexible memory structure, rigid inference engine design, ..
%
Cold start happens frequently on mobile platforms. 
First, mobile devices are resource-constrained. 
They usually have limited RAM, e.g. a few GBs~\cite{mengwei19www,dnn-mobile-imc}, much less than that of a desktop or server.
It is impractical to pin a \tfm{} model file into memory, only to respond to a bursty application use pattern~\cite{falakiDiversitySmartphoneUsage}. 
Second, multiple apps, along with their data, compete for the scarce memory.  
As a consequence, model files are swapped out frequently from filesystem page cache~\cite{dnn-mobile-lat-var}, leading to cold start inference from time to time when invoked. %next time they are invoked.
\end{comment}

%This is because during \textit{cold start}, the deep learning (DL) framework (e.g. PyTorch~\cite{pytorch-web}, TensorFlow~\cite{tensorflow-web}) must load the model file from the underlying storage medium (e.g. SD card, embedded flash) into memory before proceeding to inference computation. 

%Such high latency is unacceptable to user experience in interactive tasks.
%In comparison to \textit{hot start}, the \textit{cold start} inference happens when the deep learning (DL) framework (e.g. PyTorch~\cite{pytorch-web}, TensorFlow~\cite{tensorflow-web}) must load the model file from the underlying storage medium (e.g. SD card, embedded flash) into memory before proceeding to inference computation. 

\begin{comment}
% cold start breakdown. Vs hot inference is 26x higher. 
Figure~\ref{fig:motiv:lat-breakdown} shows the cold vs hot start inference latency of three models (i.e. \textbf{Mob}ileBERT~\cite{mobilebert}, \textbf{Dis}tilBERT~\cite{distilbert}, and \textbf{BERT}~\cite{bert}) running on Odroid~\cite{odroid-web} with PyTorch.
As can be seen, the cold start inference latency is as 26$\times$ higher than that of hot start. 
\Note{show more evidence on breakdown later}
\end{comment}


%Yet, the large size of a \tfm{} model (e.g. hundreds of MBs) imposes a significant \textit{cold start} inference latency of \tfm{}s on mobile/edge devices\footnote{Specifically, we target Arm devices with CPUs capable of floating point operations, e.g. Cortex-A73}, as high as a few seconds. 


%\input{fig-lat-breakdown}

\begin{comment}
\paragraph{Cold inference is not uncommon}
Cold inference happens when the model parameters are uncached in memory, a machine learning framework must load them from underlying flash/disk storage to execute an inference task. 
%Cold inference happens when the machine learning framework must load model parameters from underlying flash/disk storage. 
It is not uncommon for transformers on mobile platforms for the following two reasons:
\begin{myenumerate}
	\item 
	Mobile devices are resource-constrained; 
	they usually have limited RAM, e.g. a few GBs, much less than that of a desktop or server.
	Hence, to accommodate various applications in the narrow address space, cached files are frequently swapped in and out of memory\Note{cite}. 
	
	\item 
	They invoke transformer in an ad hoc and on-demand fashion, unlike a serving scenario in the cloud.
	Plus, transformer models are large (a few hundred MBs), making it uneconomic to always host them in memory.
\end{myenumerate}
\end{comment}



% \begin{myenumerate}
% 	\item 
% 	Mobile devices are resource-constrained; 
% 	they usually have limited RAM, e.g. a few GBs, much less than that of a desktop or server.
% 	Hence, to accommodate various applications in the narrow address space, cached files are frequently swapped in and out of memory\Note{cite}. 
% 	
% 	\item 
% 	They invoke transformer in an ad hoc and on-demand fashion, unlike a serving scenario in the cloud.
% 	Plus, transformer models are large (a few hundred MBs), making it uneconomic to always host them in memory.
% \end{myenumerate}

%This is because constrained by only a few GBs of RAM, mobile devices cannot afford long-live in-memory residency of model parameters;
%%unlike serving scenario on a server, they execute inference tasks sporadically, driven by applications; 
%to execute an inference task, they often load the parameters from persistent storage (i.e. cold), unlike serving scenario on a server which already hosts model file in memory (i.e. hot).


%In bringing on-device transformers inference to mobile/edge devices, the overwhelming model sizes of transformers give rise to a unique challenge: high \textbf{cold inference} latency -- as high as a few seconds and the it is dominated by IO (over 90\%) instead of compute, which we will characterize and provide more evidence in \sect{motiv}.
%The overwhelming model size of a transformer gives rise to a unique challenge for mobile/edge devices under a \textbf{cold-start} scenario. 
%The overwhelming transformer model size gives rise to a unique challenge for mobile/edge devices: high cold-start inference latency. 

%\paragraph{Design objectives}
%We seek to design a new system for reducing the \textit{cold start} inference latency of \tfm{}s on mobile devices. 
%We target two goals:
%\begin{itemize}
%	\item 
%	\textit{Latency.}
%	The system should withstand frequent cold start while still delivering the inference results with low latency.
%	
%	\item 
%	\textit{Accuracy.}
%	Meanwhile, the system should not compromise inference accuracy. 
%	It needs to maximize the accuracy, and ensure it is competitive to state-of-the-art models.
%
%%	\item 
%%	\textit{}
%
%\end{itemize}
%
%\Note{merge below}
%\textbf{Design goals:}
%\begin{myenumerate}
%	\item 
%	Fast cold inference latency
%	
%	\item 
%	Comparable hot inference accuracy
%	
%	\item 
%	Small memory footprint	
%\end{myenumerate}


% --- obsolete --- 
%\paragraph{Our approach}
%\Note{ideas... TODO}
%
%\textbf{First, model sharding.}
%The pretrained model must be partitioned into fine-grained pieces, which have the following properties:
%\begin{itemize}
%	\item 
%	Partial expressiveness of the full model.
%	The pieces must carry semantic information and language features, such that they can form subnets and be executed. 
%	
%	
%	\item 
%	Incremental accuracy. 
%	More pieces -> better accuracy. \Note{where to forecast execute incrementally?}
%	
%	
%	\item 
%	Minimum pipeline bubble.
%	\Note{actually should not be `close'}. 
%	Instead, should be as small as possible -- you can never ``starve'' IO because you can always load extra. 
%	
%	This is to create the pipeline which has high utilization and small bubbles. 
%	We donot want CPU to starve and wait for IO.   
%\end{itemize}
%
%\paragraph{Opportunities}
%We plan to exploit the following opportunities:
%\begin{myenumerate}
%	\item 
%	Need pipeline parallelism of io/compute. 
%	Currently the resources of a mobile SoC are under-utilized. 
%	Existing work focuses on compressing a model and reducing its size, e.g. via quantization~\cite{tenarybert}, knowledge distillation~\cite{distilbert}, weight sharing~\cite{albert};
%	they still wait for the model loading to finish to begin inference computation, during which time the CPU is idle. 
%	%	E.g. DistilBert~\cite{distilbert} has half the layers of a BERT~\cite{bert} model. Yet, it is still 400 MB large and takes at least 2 seconds to load. 
%	%	Alternative compression approaches such as quantization~\cite{q8bert,tenarybert,binarybert,bibert}, often has inferior performance. 
%	
%	\item 
%	Partial model execution: the model can execute based on only partial parameters and can be gradually loaded up. 
%	This is possible due to MHA redundancy. 
%	Unlike vision networks, \tfm{}s exhibit high redundancy in its attention heads~\cite{16heads}.
%	As a result, with only a few (e.g. 4) attention heads, the performance degradation is only less than 10\%~\cite{dynabert}. %of a \tfm{} model 	
%\end{myenumerate}


\paragraph{Contributions}
The paper makes the following contributions:
\begin{myitemize}
	\item 
	It examines the existing inference engine design and identifies two key inefficiencies on mobile SoCs -- lack of resource management elasticity and coordination.
	It further presents a case study by characterizing the cold start inference of transformers, a tangible problem caused by the design inefficacies.
	%\st{on multiple platforms};
%	it will obtain diverse IO/Compute profiles measured on real hardwares, such as Odroid~\cite{odroid-web}, Raspberry Pi~\cite{rpi3-web}, and Beagleboard X15~\cite{x15-web}.
	
	\item 
	It presents a novel construct -- \textit{resident model}, allowing the engine to manage IO/compute/memory in full elasticity.
	Composed by model shards, the resident model offset the high skewness of IO vs compute of \tfm{}, enables the engine to construct an elastic inference pipeline to leverage IO/compute parallelism, and adapts to OS memory pressure in fine-granularity.
	
%	The idea of a resident model -- ... which unifies model loading and execution ... addressing cold start inference ..  
	
	\item 
	It presents a holistic inference engine design, \sys{}.
%	The inference engine design \sys{}... %for accelerating \tfm{} cold start inference of pretrained models on edge devices.
	It addresses two key challenges:
	1) \textit{how to structure a model shard?}
	\sys{} partitions the whole pretrained model into multiple attention heads, quantized into different bitwidths;
	2) \textit{how to plan shards for maximum accuracy?}
	\sys{} schedules shards based on their importance, profiled offline with XXX analysis..
	%for both low latency and maximum accuracy, based on the specific IO/Compute profile of the hardware and a deadline.
%		2) \textit{shard planning}, which schedules shards for both low latency and maximum accuracy, based on the specific IO/Compute profile of the hardware and a deadline.
	
	\item
	It presents the implementation and a comprehensive evaluation of \sys{}...
%	It will evaluate the system on the pretrained  BERT~\cite{bert} model using the GLUE benchmark suite~\cite{glue-benchmark}.
%	The implementation will be made open-source to facilitate future research on the cold start inference problem. 
	
	%	\begin{itemize}
	%		\item 
	%		Pipelining 
	%		
	%		\item 
	%		Deadline-driven dynamic bitwidth selection for encoder layers. 
	%		
	%		\item 
	%		Hierarchical word embedding cache layers. 
	%	\end{itemize}
	%	Backing the techniques is a co-designed system memory management layer.. 
	%	Compared with the vanilla page cache, it is model aware and finer grained: at the granularity of an attention head instead of whole model file; 
	%	cache replacement strategy is pipeline-aware...
	%	
	%	\item 
	%	Case studies of \sys{} on a wide range of devices that have diverse hardware characteristics. 
	
\end{myitemize}



==> recycle/intro-recycle.tex <==
% !TeX root = main.tex

\section{Introduction}
\Note{why mobile} -- resource constrained, latency sensitive. Shall we tie to mobile? Principle seems applicable to desktops?

\Note{what is cold start}

\Note{why care cold start}

\Note{why on-device but not offload to cloud}

\Note{define the term compute vs IO (model load?)/use consistently/}
An IO task: load model parameters from persistent storage.
A Compute task: matmuls/concate/reshape on the model with in-memory parameters. 

Transformers~\cite{transformer} have demonstrated a superior performance in Natural Language Processing (NLP) tasks such as Sentiment Analysis (SA), Question Answering (QA). 
The compelling expressiveness of transformers benefits from a larger and deeper model design, compared with Convolutional Neural Networks (CNNs). 
For instance, AlexNet~\cite{alexnet} has in total 11 layers with 62 Million parameters, whereas the commonly used BERT model~\cite{bert} contains in total 12 layers with 110 million parameters; 
larger models such as GPT-2~\cite{gpt-2} contains as many as 48 layers with over a billion parameters, a few orders of magnitude larger than a CNN.
A binary model file of a transformer model is hence easily of a few hundred MBs. 

In bringing on-device transformers inference to mobile/edge devices, the overwhelming model sizes of transformers give rise to a unique challenge: high \textbf{cold inference} latency -- as high as a few seconds and the it is dominated by IO (over 90\%) instead of compute, which we will characterize and provide more evidence in \sect{motiv}.
%The overwhelming model size of a transformer gives rise to a unique challenge for mobile/edge devices under a \textbf{cold-start} scenario. 
%The overwhelming transformer model size gives rise to a unique challenge for mobile/edge devices: high cold-start inference latency. 
Cold inference is not uncommon.
This is because constrained by only a few GBs of RAM, mobile devices cannot afford long-live in-memory residency of model parameters;
%unlike serving scenario on a server, they execute inference tasks sporadically, driven by applications; 
to execute an inference task, they often load the parameters from persistent storage (i.e. cold), unlike serving scenario on a server which already hosts model file in memory (i.e. hot).


\Note{clarify works that focus on parameter-efficient networks}
Existing approaches are inadequate for the following reasons. 
First, they mainly focus on reducing the computation latency, e.g. by compressing large models using quantization~\cite{q8bert}, distillation~\cite{distilbert}, depth/width scaling~\cite{dynabert,delight}, matrix factorization~\cite{panahiShapeshifterParameterefficientTransformer}, or early exit~\cite{edgebert} for meeting certain latency goals. 
In a cold inference, the reduction in computation is only marginal to that of IO, e.g. from \Note{XXX} seconds to \Note{YYY} seconds.
Second, their IO and compute are sequential and synchronous\Note{???}.
That is, the inference can only start as soon as all parameters are loaded, wasting a few seconds.  
%Third, they are oblivious to memory management, hence are memory-inefficient. 
%For instance, during a cold inference 


\paragraph{Approach \& challenges.} 
\Note{revise below XXX} -- one missing key principle is to load more parameters(layers) \textit{as} inference goes on. 
That is, early (cold) inferences use smaller sets of layer parameters while later (hot) inferences use more/full set of layer parameters. 
Will discuss dynamic BERT in design space exploration in \sect{motiv:design-explore}.

\textbf{Do not have to wait until all parameters are loaded.}

\textbf{Overlap compute with IO}

\textbf{Reuse already loaded parameters, use progressively}

To this end, our overarching approach is to start inference as soon as possible by overlapping compute with IO, analogous to pipelining.
Yet, the approach raises a twofold challenge:
\Note{specify we do on-device inference but not offloading}
\begin{myenumerate}
	\item 
	\textit{How to pipeline?}
	One may do layerwise pipelining.
	That is, progress the inference layer-by-layer and overlap compute of current layer with IO of \textit{next} layer, as done by CNNs\Note{cite mengwei's}. 
	However, unlike a CNN layer of only 1MB, a transformer layer (e.g. from BERT) is tens of MBs;
	loading one layer takes a few times or a few hundred times longer than computing on a layer, e.g. 6$\times$ for transformer, 100 $\times$ for embedding layer on our dev board. %varies on other platforms.
	This renders pipelining as-is barely beneficial due to large stalls, which we will evaluate in \sect{eval}. 
	
	\item 
	\textit{How to ensure accuracy?}
	To improve pipeline efficiency, one may compress a transformer layer to match its IO and compute time, e.g. applying a width multiplier~\cite{dynabert};
	in an optimal scenario, IO is completely overshadowed by compute.
	However, we will show in \sect{eval} that such a compression strategy shrinks a layer by tens of $\times$ (only 32 dimensions), leading to poor inference accuracy. 

\end{myenumerate}


\paragraph{Key ideas.}
To address the above challenges, we propose \sys{}, a novel transformer-OS co-design.
The mechanism is as follows.
\begin{myenumerate}
	\item
	Hierarchical, frequency-based word embedding storage. 
	To start as soon as possible, \sys{} caches XXX most recently used word embeddings in memory ($<1\%$, XXX KB) (Zipf law), and clusters the rest based on their frequency.
	\sys{} stores each cluster in a number sequential disk blocks (XXX MB, XXX words), which minimizes the loading latency for the platform\Note{platform aware...}.
	The hierarchical embedding reduces the latency by XX\%.

	
	\item 
	Progressive(evolutionary) weight sharing. 
	During cold inference, \sys{} only loads one transformer layer, whose parameters are shared across all others, inspired by~\cite{albert};
	upon each future inference, \sys{} loads one more transformer layer by overlapping its IO with compute on existing, loaded, and shared layers.  
	Such a model can be viewed as supernet of $N$ transformer layers, which consists of $N$ subnets, each of 1 to $N$ distinct layers.
		
	
	\item 
	Layer-aware page caching.
	To support \sys{}, we specialize kernel memory management. 
	It unifies the model file \textit{with} flatten/loaded model parameters\Note{XXX:forecast double copy}, making them a unified copy;
	instead of caching the model file as a whole, it caches individual transformer layers. 
	Doing so saves XXX\% memory during inference. 
	
	
	
\end{myenumerate}


\paragraph{Contribution.}
This paper makes the following contributions:

\begin{myitemize}
	\item 
	Identify the cold inference problem. 
	Characterize its overhead.
	Perform measuring on real hardware.
	

	\item 
	A novel transformer-kernel codesign, \sys{} which reduces cold inference latency by XXX\% while having negligible accuracy loss. 

	
	\item 
	A novel methods for training \sys{} transformer supernet. 
	
	\item 
	XXX
	
	
\end{myitemize}

%To enable on-device Natural Language Processing (NLP) inference such as Question Answering (QA) XXX, increasing \mobile{}s are being deployed with Transformer-based~\cite{transformer} deep learning models (e.g. MobileBert~\cite{mobilebert}, DistilBert~\cite{distilbert}) for their superior performance. 

%Yet, their inference on \mobile{}s is still largely on CPUs~\cite{fb-ml-edge-study}. The reasons are as follows. 
%1) Offloading to mobile GPUs offers little benefits. 
%Due to energy constraints, beefy GPUs are rarely seen on mobile SoCs; 
%on a median mobile SoC, its GPU is only as powerful as CPU in terms of peak FLOPs~\Note{cite}.
%2) Poor programmability hinders GPU adoption. 
%Despite OpenCL is shipped with most mobile GPU, the framework itself is not part of Android~\cite{android}.
%The result is a fractured driver support from vendors, contrasting the well-supported CUDA setup seen in desktop/server scenario. 
%3) \Note{XXX}. 

%Unfortunately, Transformer inference on mobile big.Little CPUs is $ $ inefficient.
%\Note{introduce bigLittle, cluster, XXX}
%Figure~\ref{XXX} shows the results of the performing sentiment analysis task on a XXX-word sentence with state-of-the-art models. 
%E.g. it takes XXX seconds with MobileBert~\cite{mobilebert}, a model specialized for resource-constrained devices. 
%
%The reason for the inefficiency is... 
%First, poor intra/inter-cluster scalability. 
%As shown in Figure~\ref{XXX}, running it with 1 big core vs 4 big cores offers only YYY $\times$ speedup whilest 1 Little core vs 2 Little cores has negligible speedup, 1 big core vs 1 big + 1 Little offers negligible speedup. 
%Second, hardware-asymmetry-unaware thread scheduling.
%1) task placement does not consider micro-architectural differences between the two clusters, causing the cache to thrash, as shown in Figure~\ref{xxx};
%\Note{misfit memory layout...}  
%2) inefficient work stealing. 
%Task migration between clusters are expensive because XXX...

















==> recycle/intro-recycle2.tex <==
% !TeX root = main.tex

\section{Introduction}
%\section{Motivations: high cold start inference latency of Transformers}
\label{sec:intro}

\Note{moved from memo, to merge}
\paragraph{Motivating scenario.}
\sys{} targets an interactive NLP scenario with intelligent personal assistant (IPA) on a multi-tenant mobile device.
In the scenario, a user typically interacts with the IPA for querying weather/personal emails/medical records~\cite{ipa-survey}, managing tasks~\cite{myersIntelligentPersonalAssistant2007} etc.
A typical interaction takes 2-3 turns and lasts for a few seconds~\cite{ipa-study-denmark};
during the interaction, the length of each utterance is often 10-20 words~\cite{tsaiFasterResponsesAre2019}. 

Under the hood, the IPA may run the pretrained Transformer language model to directly generate responses by running downstream tasks such as question answering~\cite{dynabert}, and dialog generation~\cite{dialogpt}.
Alternatively, it may generate responses from templates. 
It does so by filling the blanks in the templates~\cite{mdfn-aaai21} or selecting existing answers from its knowledge base, based on intent classification~\cite{dbpedia-chatbot} and sentiment analysis~\cite{yasudaDesigningChatbotSystem2021} results of the Transformer model.


%\Note{Mobile, interactive NLP, bursty, find mobile app use pattern, user-perceived latency is more important...}
%As the enabler for increasingly popular usage of voice assistant, 
On-device interactive Natural Language Processing (NLP) such as Sentiment Analysis (SA) and Question Answering (QA) have been increasingly popular~\cite{mengwei19www}. %thanks to advances in mobile CPUs.
In an interactive NLP task, a user follows a conversational model~\cite{conversational-model} -- s/he invokes a NLP model with a succinct, introductory phrase (e.g. ``Hello'') and proceeds with more complex communications;
the interactive process expects a low latency for user experience.
%Due to a strong performance, \tfm{}s~\cite{transformer} have demonstrated a superior performance and are becoming the de facto models in NLP tasks. 

Due to the strong performance, \tfm{}s~\cite{transformer} have become the de facto models in NLP tasks. 
%\Note{A motivational example -- it is widely used in interactive NLP, users use it for conversations, etc..}
The power of \tfm{}s comes from a unique self-attention design: each \tfm{} layer comprises a Multi-Head Attention (MHA) module, which extracts not only the contextual but also the intra-sentence features (i.e. self-attention). 
The architecture is shown in Figure~\ref{fig:motiv:transformer}.
By stacking the \tfm{} layers, a \tfm{} model encodes rich and profound language features, achieving great expressiveness. %than prior models. 
%\Note{mention MHA redundancy here}
%\Note{add an attention figure}
\input{fig-transformer}

Yet, the \tfm{} layer is known to be parameter-rich.
%Yet, the MHA module is parameter-inefficient.
Each layer draws parameters from four fully-connected matrix -- Query (Q), Key (K), Value (V), and a Feed-Forward Network (FFN), each having tens of thousands neurons. 
For this reason, \tfm{} models are often large;
a few to tens of layers are not uncommon, each layer having almost a million parameters.  
%\Note{Compared to traditional vision networks...}
For instance, BERT~\cite{bert}, as one of the most widely used \tfm{} models, contains 12 layers with in total 110 million parameters, which is 2$\times$ larger than Convolutional Neural Networks (CNN) AlexNet~\cite{alexnet} and Resnet-152~\cite{resnet}. %a known big Convolutional Neural Network (CNN). 
Larger-scale models used in cloud services (e.g. Google Translate~\cite{google-translate-blog}), such as GPT-2~\cite{gpt-2} contain as many as 48 layers with over a billion parameters. %a few orders of magnitude larger than a CNN.
Even for smaller models designed for mobile devices, e.g. MobileBERT~\cite{mobilebert} and DistilBERT~\cite{distilbert}, they comprise a few layers and in total tens of million parameters. 
With millions of parameters each stored as a 32-bit full-precision floating-point number, the pretrained model file of a \tfm{} is hence easily of a few hundred MBs.
%compared with Convolutional Neural Networks (CNNs).
%For instance, AlexNet~\cite{alexnet} has in total 11 layers with 62 Million parameters, whereas the commonly used BERT model~\cite{bert} contains in total 12 layers with 110 million parameters; 


\input{fig-lat-breakdown}

\paragraph{Problem statement}
%\Note{Multiple inferences not just oneshot, bursty nature: after cold start, the app may request a few more subsequent inferences...}
The large model imposes a significant \textit{cold start} inference latency of \tfm{}s on mobile/edge devices\footnote{Specifically, we target Arm devices with CPUs capable of floating point operations, e.g. Cortex-A73}, as high as a few seconds. 
This is because during \textit{cold start}, the deep learning (DL) framework (e.g. PyTorch~\cite{pytorch-web}, TensorFlow~\cite{tensorflow-web}) must load the model file from the underlying storage medium (e.g. SD card, embedded flash) into memory before proceeding to inference computation. 
Such high latency is unacceptable to user experience in interactive tasks.
%In comparison to \textit{hot start}, the \textit{cold start} inference happens when the deep learning (DL) framework (e.g. PyTorch~\cite{pytorch-web}, TensorFlow~\cite{tensorflow-web}) must load the model file from the underlying storage medium (e.g. SD card, embedded flash) into memory before proceeding to inference computation. 
Figure~\ref{fig:motiv:lat-breakdown} shows the cold vs hot start inference latency of three models (i.e. \textbf{Mob}ileBERT~\cite{mobilebert}, \textbf{Dis}tilBERT~\cite{distilbert}, and \textbf{BERT}~\cite{bert}) running on Odroid~\cite{odroid-web} with PyTorch.
As can be seen, the cold start inference latency is as 26$\times$ higher than that of hot start. 
\Note{show more evidence on breakdown later}

\textbf{The key bottleneck is IO...}


Cold start inference on mobile devices is not uncommon.
First, mobile devices are resource-constrained. 
They usually have limited RAM, e.g. a few GBs~\cite{mengwei19www,dnn-mobile-imc}, much less than that of a desktop or server.
It is impractical to pin a \tfm{} model file into memory, only to respond to a bursty application use pattern~\cite{falakiDiversitySmartphoneUsage}. 
Second, multiple apps, along with their data, compete for the scarce memory.  
As a consequence, model files are swapped out frequently from filesystem page cache~\cite{dnn-mobile-lat-var}, leading to cold start inference from time to time when invoked. %next time they are invoked.

\begin{comment}
\paragraph{Cold inference is not uncommon}
Cold inference happens when the model parameters are uncached in memory, a machine learning framework must load them from underlying flash/disk storage to execute an inference task. 
%Cold inference happens when the machine learning framework must load model parameters from underlying flash/disk storage. 
It is not uncommon for transformers on mobile platforms for the following two reasons:
\begin{myenumerate}
	\item 
	Mobile devices are resource-constrained; 
	they usually have limited RAM, e.g. a few GBs, much less than that of a desktop or server.
	Hence, to accommodate various applications in the narrow address space, cached files are frequently swapped in and out of memory\Note{cite}. 
	
	\item 
	They invoke transformer in an ad hoc and on-demand fashion, unlike a serving scenario in the cloud.
	Plus, transformer models are large (a few hundred MBs), making it uneconomic to always host them in memory.
\end{myenumerate}
\end{comment}



% \begin{myenumerate}
% 	\item 
% 	Mobile devices are resource-constrained; 
% 	they usually have limited RAM, e.g. a few GBs, much less than that of a desktop or server.
% 	Hence, to accommodate various applications in the narrow address space, cached files are frequently swapped in and out of memory\Note{cite}. 
% 	
% 	\item 
% 	They invoke transformer in an ad hoc and on-demand fashion, unlike a serving scenario in the cloud.
% 	Plus, transformer models are large (a few hundred MBs), making it uneconomic to always host them in memory.
% \end{myenumerate}

%This is because constrained by only a few GBs of RAM, mobile devices cannot afford long-live in-memory residency of model parameters;
%%unlike serving scenario on a server, they execute inference tasks sporadically, driven by applications; 
%to execute an inference task, they often load the parameters from persistent storage (i.e. cold), unlike serving scenario on a server which already hosts model file in memory (i.e. hot).


%In bringing on-device transformers inference to mobile/edge devices, the overwhelming model sizes of transformers give rise to a unique challenge: high \textbf{cold inference} latency -- as high as a few seconds and the it is dominated by IO (over 90\%) instead of compute, which we will characterize and provide more evidence in \sect{motiv}.
%The overwhelming model size of a transformer gives rise to a unique challenge for mobile/edge devices under a \textbf{cold-start} scenario. 
%The overwhelming transformer model size gives rise to a unique challenge for mobile/edge devices: high cold-start inference latency. 

\paragraph{Design objectives}
We seek to design a new system for reducing the \textit{cold start} inference latency of \tfm{}s on mobile devices. 
We target two goals:
\begin{itemize}
	\item 
	\textit{Latency.}
	The system should withstand frequent cold start while still delivering the inference results with low latency.
	
	\item 
	\textit{Accuracy.}
	Meanwhile, the system should not compromise inference accuracy. 
	It needs to maximize the accuracy, and ensure it is competitive to state-of-the-art models.

%	\item 
%	\textit{}

\end{itemize}
%
%\Note{merge below}
%\textbf{Design goals:}
%\begin{myenumerate}
%	\item 
%	Fast cold inference latency
%	
%	\item 
%	Comparable hot inference accuracy
%	
%	\item 
%	Small memory footprint	
%\end{myenumerate}

\paragraph{Our approach}
\Note{ideas... TODO}

\textbf{First, model sharding.}
The pretrained model must be partitioned into fine-grained pieces, which have the following properties:
\begin{itemize}
	\item 
	Partial expressiveness of the full model.
	The pieces must carry semantic information and language features, such that they can form subnets and be executed. 
	
	
	\item 
	Incremental accuracy. 
	More pieces -> better accuracy. \Note{where to forecast execute incrementally?}
	
	
	\item 
	Minimum pipeline bubble.
	\Note{actually should not be `close'}. 
	Instead, should be as small as possible -- you can never ``starve'' IO because you can always load extra. 
	
	This is to create the pipeline which has high utilization and small bubbles. 
	We donot want CPU to starve and wait for IO.   
\end{itemize}













\paragraph{Opportunities}
We plan to exploit the following opportunities:
\begin{myenumerate}
	\item 
	Need pipeline parallelism of io/compute. 
	Currently the resources of a mobile SoC are under-utilized. 
	Existing work focuses on compressing a model and reducing its size, e.g. via quantization~\cite{tenarybert}, knowledge distillation~\cite{distilbert}, weight sharing~\cite{albert};
	they still wait for the model loading to finish to begin inference computation, during which time the CPU is idle. 
	%	E.g. DistilBert~\cite{distilbert} has half the layers of a BERT~\cite{bert} model. Yet, it is still 400 MB large and takes at least 2 seconds to load. 
	%	Alternative compression approaches such as quantization~\cite{q8bert,tenarybert,binarybert,bibert}, often has inferior performance. 
	
	\item 
	Partial model execution: the model can execute based on only partial parameters and can be gradually loaded up. 
	This is possible due to MHA redundancy. 
	Unlike vision networks, \tfm{}s exhibit high redundancy in its attention heads~\cite{16heads}.
	As a result, with only a few (e.g. 4) attention heads, the performance degradation is only less than 10\%~\cite{dynabert}. %of a \tfm{} model 
	
	

	
	
\end{myenumerate}


\paragraph{Contributions}
The paper makes the following contributions:
\begin{myitemize}
	\item 
	It will identify and characterize the cold start inference problem on multiple platforms;
	it will obtain diverse IO/Compute profiles measured on real hardwares, such as Odroid~\cite{odroid-web}, Raspberry Pi~\cite{rpi3-web}, and Beagleboard X15~\cite{x15-web}.
	
	
	\item 
	A novel system design for accelerating \tfm{} cold start inference of pretrained models on edge devices.
	It features two novel techniques: 
	1) \textit{structured model sharding}, which partitions the whole pretrained model into multiple attention heads, quantized into different bitwidths;
	2) \textit{device heterogeneity-aware shard planning}, which schedules shards for both low latency and maximum accuracy, based on the specific IO/Compute profile of the hardware and a deadline.
	
	\item
	The implementation and evaluation of the proposed system.
	It will evaluate the system on the pretrained  BERT~\cite{bert} model using the GLUE benchmark suite~\cite{glue-benchmark}.
	The implementation will be made open-source to facilitate future research on the cold start inference problem. 
	
	%	\begin{itemize}
	%		\item 
	%		Pipelining 
	%		
	%		\item 
	%		Deadline-driven dynamic bitwidth selection for encoder layers. 
	%		
	%		\item 
	%		Hierarchical word embedding cache layers. 
	%	\end{itemize}
	%	Backing the techniques is a co-designed system memory management layer.. 
	%	Compared with the vanilla page cache, it is model aware and finer grained: at the granularity of an attention head instead of whole model file; 
	%	cache replacement strategy is pipeline-aware...
	%	
	%	\item 
	%	Case studies of \sys{} on a wide range of devices that have diverse hardware characteristics. 
	
\end{myitemize}



==> recycle/intro-recycle3.tex <==
% !TeX root = main.tex

\section{Introduction}
%\section{Motivations: high cold start inference latency of Transformers}
\label{sec:intro}

%\textbf{flow:}
%\begin{myitemize}
%	\item 
%	NLP inference, transformer model popular... 
%	
%	\item 
%	What is the problem? Latency variability, noticed by prior work... 
%	Caused by cold inference -- model file not in cache, load parameter from disk...
%	
%	\item 
%	The root cause: the conflicts between fluctuating memory pressure vs rigid inference engine design (separate load vs inference stage). 
%	
%	\item 
%	Existing approaches are inadequate. 
%	Two approaches: 
%	1) model compression. Mention dynabert (although can adjust model at runtime, but...) The inadequacy is that it is still (rigid).. Done deal for the model: whether it is in mem or not... Poor accuracy...
%	2) deadline driven inference. via early exit.. 
%	
%	\item 
%	Our paper -- the key construct is the \textit{resident model}, a ``meta model''... for bridging the rigid cold vs hot inference...
%	Describe what it is ...  
%	
%	\item 
%	We address two challenges in managing the resident model: first how to become elastic? existing approach -- dynamic width \& depth. why not work? because it is too coarse grained..
%	our solution -- shards.. second how to have high accuracy? our insight is to leverage spare IO...
%	
%	
%\end{myitemize}


%\Note{Mobile, interactive NLP, bursty, find mobile app use pattern, user-perceived latency is more important...}
%As the enabler for increasingly popular usage of voice assistant, 
On-device interactive Natural Language Processing (NLP) have been increasingly popular on mobile devices\footnote{Specifically, we target Arm devices with CPUs capable of floating point operations, e.g. Cortex-A73}~\cite{mengwei19www}. %thanks to advances in mobile CPUs.
In the scenario, the user interacts with the on-device Intelligent Personal Assistant (IPA) for querying weather/personal emails/medical records~\cite{ipa-survey}, managing tasks~\cite{myersIntelligentPersonalAssistant2007}, etc.
Under the hood, the IPA often runs \tfm{} language model due to its strong performance in NLP tasks. 
%It may directly generate responses by running downstream tasks such as question answering~\cite{dynabert}, and dialog generation~\cite{dialogpt}, by filling the templates~\cite{mdfn-aaai21}, by selecting existing answers from its knowledge base dependent on intent classification~\cite{dbpedia-chatbot} and sentiment analysis~\cite{yasudaDesigningChatbotSystem2021} results.

Like the usage pattern of many other mobile apps, the user also invokes the IPA in an on-demand, bursty manner~\cite{falakiDiversitySmartphoneUsage}, i.e. launch, use for a while, then quit.
A typical invocation constitutes 2-3 interaction turns and lasts for a few seconds~\cite{ipa-study-denmark};
during the interaction, the length of each utterance is often 10-20 words~\cite{tsaiFasterResponsesAre2019}. 
For a smooth and responsive experience, the user expects a consistent and low latency.

\begin{comment}
% lwg: useful -- describes the actual transformer tasks. 

%Under the hood, the IPA often runs \tfm{} language model due to its strong performance. 
%It may directly generate responses by running downstream tasks such as question answering~\cite{dynabert}, and dialog generation~\cite{dialogpt}, by filling the templates~\cite{mdfn-aaai21}, by selecting existing answers from its knowledge base dependent on intent classification~\cite{dbpedia-chatbot} and sentiment analysis~\cite{yasudaDesigningChatbotSystem2021} results. 
\end{comment}

%Alternatively, it may generate responses from templates. 
%It does so by filling the blanks in the templates~\cite{mdfn-aaai21} or selecting existing answers from its knowledge base, based on intent classification~\cite{dbpedia-chatbot} and sentiment analysis~\cite{yasudaDesigningChatbotSystem2021} results of the Transformer model.

%In an interactive NLP task, a user follows a conversational model~\cite{conversational-model} -- s/he invokes a NLP model with a succinct, introductory phrase (e.g. ``Hello'') and proceeds with more complex communications;
%the interactive process expects a consistent and low latency for a responsive user experience.
%Due to a strong performance, \tfm{}s~\cite{transformer} have demonstrated a superior performance and are becoming the de facto models in NLP tasks. 

% ---- move below to transformer primer ----
\begin{comment}
Due to the strong performance, \tfm{}s~\cite{transformer} have become the modern model such tasks. 
%\Note{A motivational example -- it is widely used in interactive NLP, users use it for conversations, etc..}
The power of \tfm{}s comes from a unique self-attention design: each \tfm{} layer comprises a Multi-Head Attention (MHA) module, which extracts not only the contextual but also the intra-sentence features (i.e. self-attention). 
The architecture is shown in Figure~\ref{fig:motiv:transformer}.
By stacking the \tfm{} layers, a \tfm{} model encodes rich and profound language features, achieving great expressiveness. %than prior models. 
%\Note{mention MHA redundancy here}
%\Note{add an attention figure}
\input{fig-transformer}

Yet, the \tfm{} layer is known to be parameter-rich.
%Yet, the MHA module is parameter-inefficient.
Each layer draws parameters from four fully-connected matrix -- Query (Q), Key (K), Value (V), and a Feed-Forward Network (FFN), each having tens of thousands neurons. 
For this reason, \tfm{} models are often large;
a few to tens of layers are not uncommon, each layer having almost a million parameters.  
%\Note{Compared to traditional vision networks...}
For instance, BERT~\cite{bert}, as one of the most widely used \tfm{} models, contains 12 layers with in total 110 million parameters, which is 2$\times$ larger than Convolutional Neural Networks (CNN) AlexNet~\cite{alexnet} and Resnet-152~\cite{resnet}. %a known big Convolutional Neural Network (CNN). 
Larger-scale models used in cloud services (e.g. Google Translate~\cite{google-translate-blog}), such as GPT-2~\cite{gpt-2} contain as many as 48 layers with over a billion parameters. %a few orders of magnitude larger than a CNN.
Even for smaller models designed for mobile devices, e.g. MobileBERT~\cite{mobilebert} and DistilBERT~\cite{distilbert}, they comprise a few layers and in total tens of million parameters. 
With millions of parameters each stored as a 32-bit full-precision floating-point number, the pretrained model file of a \tfm{} is hence easily of a few hundred MBs.
%compared with Convolutional Neural Networks (CNNs).
%For instance, AlexNet~\cite{alexnet} has in total 11 layers with 62 Million parameters, whereas the commonly used BERT model~\cite{bert} contains in total 12 layers with 110 million parameters; 
\end{comment}

\Note{problem at a higher-lv? Challenge: 1) large model, cannot be held for now, all-or-nothing situation; 2) long IO delay to load the model; problem -- rigid model loading -- define goals: given ddl, io should adjust elastically xx..}

\Note{elasticity in 3 dimensions: IO (precisions) and compute (dep and wid), memory}

\Note{theme: rigid vs elasticity. At what dimensions are we more elastic compared with prior work? }


\xzlNote{problems}: 
\begin{itemize}
\item 
1. large NLP models -- cannot be always, 100\% in memory (waste of resources) -- memory management problem. Current: model is stored as a whole or by layer; 
mm -- oblivious to model's internal structures, page in/out (by layers at best)

2. loading \& execution -- execution request is bursty. Model has to be loaded and executed. 
Current: no pipelining or rigid pipelining. Reason: skewed compute/IO ratio. Compute starvation. 

\end{itemize}

\paragraph{Problem: lack of elasticity in resource scheduling}
There are three dimensions of elasticity in inference: IO, Compute, and memory. 
Existing engine design: rigid separation, no coordination, oblivious to OS management..
The inefficiency manifests in model loading phase -- too long time to load.


\paragraph{Problem: cold start inference}
%\Note{Multiple inferences not just oneshot, bursty nature: after cold start, the app may request a few more subsequent inferences...}
However, existing mobile NLP inference engine fails to respond to user invocations in a consistent and timely manner due to \textit{cold start}~\cite{dnn-mobile-char}.
During cold start, the engine must load the large model file (e.g. hundreds of MBs) from the disk\footnote{By convention, we use ``disk'' to refer to storage medium such as SD card and flash on mobile devices.} into memory before proceeding to inference computation.
On a commodity dev board, we measured such a process takes as many as a few seconds, which is unacceptable to user experience;
%On a commodity dev board we measured such a process takes as many as a few seconds due to the large size of the \tfm{} model (e.g. hundreds of MBs), which is unacceptable to UX;
it also happens frequently, increasing latency variability~\cite{dnn-mobile-lat-var}.

% lwg: root causes for cold start inference
% constrained resources, inflexible memory structure (not quite true -- dynabert has some flexibity), rigid inference engine design, ..
%\Note{we discover a key inefficiency in resource utilization of the inference engine: 1) lack of system-app memory coordination; 2) lack of IO-compute coordination; 3) large model files further...}
Why does cold start occur often?
We discover two key inefficiencies of resource utilization in existing inference engines. 
%\Note{lack of resource elasticity?? what order?}
\Note{move forward -- these are the high level challenges}
\begin{myitemize}
	\item 
	First, lack of OS-engine memory coordination.
	As tenant apps compete for the scarce memory (e.g. a few GBs~\cite{mengwei19www,dnn-mobile-imc}), the OS tends to reclaim the large model files which occupy up to 20\% of kernel page cache; 
	the process is oblivious to the engine.
	As a result, \tfm{} model files are swapped out frequently from kernel page cache, causing cold start from time to time.
%	Mobile devices only have constrained memory (e.g. only a few GBs~\cite{mengwei19www,dnn-mobile-imc}). 
%	The heavy competition of tenant apps leads to memory pressure fluctuation\Note{cite}. 
%	\Note{XXX: resident model is much smaller thus can afford to be long lived in memory...}
	
	\item
	Second, lack of IO-compute parallelism.
	Existing inference engines impose a rigid separation between the two stages, model loading and inference computation.
	The computation hence can only start as soon as the full model file is loaded, which accounts over 90\% of time.
	The large size of the \tfm{} model file and medium to low storage throughput (tens of MB/s) further exacerbates the delay.
\end{myitemize}
%First, mobile devices only have constrained memory (e.g. only a few GBs~\cite{mengwei19www,dnn-mobile-imc}). 
%The heavy competition of tenant apps leads to memory pressure fluctuation\Note{cite}. 
%As a result, \tfm{} model files are swapped out frequently from kernel page cache, causing cold start from time to time.
%\Note{XXX: resident model is much smaller thus can afford to be long lived in memory...}
%must compete for the scarce memory . 
%It is impractical to pin a \tfm{} model file into memory, only to respond to a bursty application use pattern~\cite{falakiDiversitySmartphoneUsage}. 
%As a consequence, model files are swapped out frequently from kernel page cache~\cite{dnn-mobile-lat-var}, leading to cold start from time to time. %next time they are invoked.
%much less than that of a desktop or server.
%Second, existing inference engine imposes a rigid separation between model loading and inference computation.
%As a result, the computation can only start as soon as the full model file is loaded, which accounts over 90\% of time.
%Last but not least, the large size of the \tfm{} model file and medium to low storage throughput (tens of MB/s) further exacerbates the situation.
%Compared with commodity vision networks~\cite{alexnet} (tens of MB), a \tfm{} model is easily hundreds of MBs. 

\paragraph{Existing techniques are inadequate}
Model compression, for example, is a common technique for reducing model size, facilitating faster loading;
it includes model structure~\cite{layerdrop,distilbert} and feature pruning~\cite{mobilebert}, and quantization which reduces full-precisions (32bit) parameters into low-bit (e.g. 2bit) representations~\cite{bibert,binarybert,q8bert}. 
Alternatively, one may deploy dynamic \tfm{}s which adapt to varied memory or latency constraints by correspondingly configuring model widths and/or depths~\cite{dynabert,edgebert}. 
\Note{native pipelining is insufficient...layerwsie, etc.}

\Note{then define our goals must cover background and foreground -- efficient pipelining (no starvation), maximum accuracy, elastic and fine-grained memory management}

\Note{lack of elasticity in memory management, data parallelism}
Without considering the above inefficiencies, existing approaches are inadequate.  
This is because however small they may reduce the model files to, static or dynamic, it still remains oblivious to OS memory management decisions (i.e. get swapped out and become cold again), and contributes significant loading overhead during next inference.
%it still remains oblivious to OS memory pressure fluctuation, gets swapped out of page cache (i.e. become cold again), and contributes significant loading overhead during next inference.
%one compresses a large \tfm{} model file (e.g. BERT~\cite{bert}), such that it is a few $\times$ smaller and hence faster to load.


%Alternatively, one may 

\Note{need something more ``meta'' on the high level idea. thoughts: resident model: in memory; backup model: on disk; a model hierarchy to fit storage hierarchy which balances out io compute...respond to user/OS with two primitives: up/downgrade or de/inflate.}
\paragraph{Our approach}
\Note{one sentence summary of our idea ... manage composable tunable components...tune for maximum accuracy (for future inferences)}
In response, we advocate for a fresh perspective of inference engine design, which takes on a greater role in orchestrating IO, compute, and memory resources, as illustrated in Figure~XXX.
Instead of the full-fledged model, the engine starts with a small \textit{resident model} in memory.
Instructed by the OS and user, it manages the resident model in four-way elasticity: 
\Note{data structure}depending on available IO/compute/memory resources, it may not only \textit{de/inflate} its depths and widths, but also \textit{down/upgrade} its precisions;
\Note{operation} at inference run time, it exploits IO/compute parallelism to upgrade the model while executing inference on the fly. \Note{when memory pressure changes...et,c}
%instructed by the OS and user, it manages the resident model in full elasticity: depending on available IO/compute/memory resources, it may not only in/deflate its depths and widths, but also down/upgrade its precisions.
\begin{comment}
instructed by the OS and user, it manages the resident model in four-way elasticity:
during inference, it down/upgrades the model precisions while executing inference on the fly by exploiting IO/compute parallelism; 
in the background, it de/inflates the resident model depthts and widths w.r.t. memory pressure.
\end{comment}
%it leverages available IO/memory resources to up/downgrade the resident model, both on and off the inference critical path.
The resident model reconciles cold v.s. hot inference dichotomy by keeping the inference \textit{warm}: 
%it provides a skeleton/backbone, just enough to warm up the next inference;
%while always in-memory, it responds to OS memory pressure and is elastic -- low precision (resembling cold inference) to even full precision (resembling hot inference full model). 
%it is always in memory, eliminating cold inference;
%yet, it is resource-elastic -- depending on OS, it may expand to full precision, resembling full model in hot inference. 
the inference is never cold, as it is always bootstrapped by the resident model;
as long as memory permits, the resident model will keep being upgraded during rounds of (warm) inferences, eventually resembling a full model in hot inference.

\begin{comment}
First, from the full-fledged model the engine derives multiple lower-precisions versions on disk.
Instead of the full-fledged model, the engine starts with a small \textit{resident model} in memory. 
Such a resident model is fully elastic to OS resources: 
in the foreground during inference, the engine upgrades the resident model by loading extra versions from disk, whose IO overhead is hidden by overlapping with compute;
in the background, when the memory pressure is high, engine downgrades the resident model, as instructed by the OS.
The resident model reconciles cold v.s. hot dichotomy by keeping the inference \textit{warm}: 
%it provides a skeleton/backbone, just enough to warm up the next inference;
%while always in-memory, it responds to OS memory pressure and is elastic -- low precision (resembling cold inference) to even full precision (resembling hot inference full model). 
%it is always in memory, eliminating cold inference;
%yet, it is resource-elastic -- depending on OS, it may expand to full precision, resembling full model in hot inference. 
the inference is never cold, as it is always boosted by the in-memory resident model;
as long as system memory permits, resident model will keep being updated during rounds of (warm) inferences, eventually resembling a full model in hot inference.
%Instead of either preserving a full model file in memory or none at all, 
%To this end, the engine keeps a \textit{resident model} always in memory to kick start inferences. 
%To this end, the engine permanently deploys a \textit{resident model} in memory. 
%%To this end, the engine keeps a small \textit{resident model} always in memory (e.g. 5\% of the full model) to kick start inferences. 
%%Compared with prior dynamic models~\cite{layerdrop,edgebert,dynabert}, 
%A resident model is fully elastic to OS resources: in the foreground of the inference critical path, the engine leverages... 
\end{comment}

\begin{comment}
%% below useful
To this end, the engine derives multiple versions from the full-fledged model into different, lower precisions.
Instead of having the full model file either in memory or on disk, the engine keeps one version called \textit{resident model} always in memory, while leaving the rest on disk.
%A resident model is elastic and adaptive to system resources.
%a tiny portion (e.g. 5\%) of the original model, while keeping the rest \textit{XXX model} on disk (\Note{XXX} MB).
In the foreground, of the inference critical path, %invoked by the user, 
the engine uses the small resident model to kickstart inference while live patching it with on-disk versions for greater accuracy;
%the engine uses the resident model as a skeleton and live patches it with on-disk versions;
it hides the IO overhead of loading from disk by overlapping it with computing on the resident model. 
In the background, the engine adapts the elastic resident model structure to memory pressure as instructed by the OS. 
The resident model reconciles cold v.s. hot dichotomy by keeping the inference \textit{warm}: 
%it provides a skeleton/backbone, just enough to warm up the next inference;
%while always in-memory, it responds to OS memory pressure and is elastic -- low precision (resembling cold inference) to even full precision (resembling hot inference full model). 
%it is always in memory, eliminating cold inference;
%yet, it is resource-elastic -- depending on OS, it may expand to full precision, resembling full model in hot inference. 
the inference is never cold, as it is always boosted by the in-memory resident model;
as long as system memory permits, resident model will keep being updated during rounds of (warm) inferences, eventually resembling a full model in hot inference.
\end{comment}

%it is always in memory and can be directly used as-is;
%it is runtime elastic, adaptive to OS memory pressure;

%\Note{below}
%our key construct is a resident model ... (compressed form, always in memory)
%unlike static compression which lacks flexibility. resident model are more flexible..
%IT is meta model structure (bare minimum?)...
%decomp. on-demand...

\Note{bring out planner, describe pipeline. Define goals.}
Following the perspective, we present \textbf{S}peedy \textbf{T}ransformer \textbf{I}nference (\sys{}), a novel \tfm{} inference engine. 
First, the engine derives multiple lower-precision versions \Note{this is to increase elasticity in IO of the pipeline...} from the full-fledged model and persists them on disk.
It exposes an inference deadline $T$ and a memory threshold $M$ to user and OS respectively. 
Bound by the two constraints, it manages the resident model while maximizing inference accuracy: 
during inference, it loads parameters from versions which benefit most to current resident model accuracy under $T$; 
in the background, it unloads the versions which hurt accuracy the least when $M$ decreases.

\paragraph{Challenges \& solutions}
Through retrofitting a suite of known machine learning techniques, we have addressed following two challenges in managing a resident model, which sets us apart from prior dynamic \tfm{} work.

\noindent
%\textbf{First, how to construct the elastic resident model?}
\textbf{1) Management granularity of the resident model.}
As the engine exploits IO/compute parallelism to upgrade the resident model with on-disk models, it must select a proper granularity: 
the upgraded parameters must carry additional semantic features to improve resident model accuracy; 
to hide the IO overhead, loading time must be on a par with compute time.

To this end, \sys{} partitions the model into vertical slices, grouped by individual layers.
Each vertical slice, dubbed a \textit{model shard}, constitutes one attention head plus a set of FFN neurons and resembles the dynamic ``width'' of the \tfm{} model~\cite{dynabert};
with one shard being a few MBs, the time to load one shard vs compute is similar.
\sys{} further compresses the full-fledged shards into lower precisions, inspired by a Gaussian-outlier-based quantization technique~\cite{quantization-survey}.
With model shards as the key building block, \sys{} manages a resident model by adjusting the number of shards per layer, and by up/downgrading precisions of individual shards.

\noindent
%\textbf{Second, how to plan for maximum accuracy?}
\textbf{2) Optimal accuracy under constraints $T$ and $M$.}
The engine manipulates model shards of the resident model in both the foreground (i.e. during inference) and background.
It must decide judiciously a configuration which satisfies $T$ and $M$, and achieves an optimal accuracy.
Yet, the configuration space grows combinatorially with total number of shards, making it possible to exhaust. 

To address the challenge, we formulate the problem as a search problem, guided by a set of heuristics for runtime efficiency. 
To devise the heuristics, our key insight is to follow the gradient of information gain/loss, that is, choose whichever configuration that gains most/loses least in model information.
The rationale is to compensate information loss caused by quantization.
To this end, we measure the information gain of shards using hessian trace, a known technique....
At a higher level, \sys{} uses the following heuristics.
In reshaping the resident model, it favors depths over widths;
in upgrading the individual shards, it favors more important shards, i.e. with most information.

As a result, we implement \sys{} on XXX dev board with Pytorch in XXX SLOC.
We conduct comprehensive benchmarks on GLUE benchmark...

\begin{comment}
% below useful to explain why cold start happens for mobile platforms:
% constrained resources, inflexible memory structure, rigid inference engine design, ..
%
Cold start happens frequently on mobile platforms. 
First, mobile devices are resource-constrained. 
They usually have limited RAM, e.g. a few GBs~\cite{mengwei19www,dnn-mobile-imc}, much less than that of a desktop or server.
It is impractical to pin a \tfm{} model file into memory, only to respond to a bursty application use pattern~\cite{falakiDiversitySmartphoneUsage}. 
Second, multiple apps, along with their data, compete for the scarce memory.  
As a consequence, model files are swapped out frequently from filesystem page cache~\cite{dnn-mobile-lat-var}, leading to cold start inference from time to time when invoked. %next time they are invoked.
\end{comment}

%This is because during \textit{cold start}, the deep learning (DL) framework (e.g. PyTorch~\cite{pytorch-web}, TensorFlow~\cite{tensorflow-web}) must load the model file from the underlying storage medium (e.g. SD card, embedded flash) into memory before proceeding to inference computation. 

%Such high latency is unacceptable to user experience in interactive tasks.
%In comparison to \textit{hot start}, the \textit{cold start} inference happens when the deep learning (DL) framework (e.g. PyTorch~\cite{pytorch-web}, TensorFlow~\cite{tensorflow-web}) must load the model file from the underlying storage medium (e.g. SD card, embedded flash) into memory before proceeding to inference computation. 

\begin{comment}
% cold start breakdown. Vs hot inference is 26x higher. 
Figure~\ref{fig:motiv:lat-breakdown} shows the cold vs hot start inference latency of three models (i.e. \textbf{Mob}ileBERT~\cite{mobilebert}, \textbf{Dis}tilBERT~\cite{distilbert}, and \textbf{BERT}~\cite{bert}) running on Odroid~\cite{odroid-web} with PyTorch.
As can be seen, the cold start inference latency is as 26$\times$ higher than that of hot start. 
\Note{show more evidence on breakdown later}
\end{comment}


%Yet, the large size of a \tfm{} model (e.g. hundreds of MBs) imposes a significant \textit{cold start} inference latency of \tfm{}s on mobile/edge devices\footnote{Specifically, we target Arm devices with CPUs capable of floating point operations, e.g. Cortex-A73}, as high as a few seconds. 


%\input{fig-lat-breakdown}

\begin{comment}
\paragraph{Cold inference is not uncommon}
Cold inference happens when the model parameters are uncached in memory, a machine learning framework must load them from underlying flash/disk storage to execute an inference task. 
%Cold inference happens when the machine learning framework must load model parameters from underlying flash/disk storage. 
It is not uncommon for transformers on mobile platforms for the following two reasons:
\begin{myenumerate}
	\item 
	Mobile devices are resource-constrained; 
	they usually have limited RAM, e.g. a few GBs, much less than that of a desktop or server.
	Hence, to accommodate various applications in the narrow address space, cached files are frequently swapped in and out of memory\Note{cite}. 
	
	\item 
	They invoke transformer in an ad hoc and on-demand fashion, unlike a serving scenario in the cloud.
	Plus, transformer models are large (a few hundred MBs), making it uneconomic to always host them in memory.
\end{myenumerate}
\end{comment}



% \begin{myenumerate}
% 	\item 
% 	Mobile devices are resource-constrained; 
% 	they usually have limited RAM, e.g. a few GBs, much less than that of a desktop or server.
% 	Hence, to accommodate various applications in the narrow address space, cached files are frequently swapped in and out of memory\Note{cite}. 
% 	
% 	\item 
% 	They invoke transformer in an ad hoc and on-demand fashion, unlike a serving scenario in the cloud.
% 	Plus, transformer models are large (a few hundred MBs), making it uneconomic to always host them in memory.
% \end{myenumerate}

%This is because constrained by only a few GBs of RAM, mobile devices cannot afford long-live in-memory residency of model parameters;
%%unlike serving scenario on a server, they execute inference tasks sporadically, driven by applications; 
%to execute an inference task, they often load the parameters from persistent storage (i.e. cold), unlike serving scenario on a server which already hosts model file in memory (i.e. hot).


%In bringing on-device transformers inference to mobile/edge devices, the overwhelming model sizes of transformers give rise to a unique challenge: high \textbf{cold inference} latency -- as high as a few seconds and the it is dominated by IO (over 90\%) instead of compute, which we will characterize and provide more evidence in \sect{motiv}.
%The overwhelming model size of a transformer gives rise to a unique challenge for mobile/edge devices under a \textbf{cold-start} scenario. 
%The overwhelming transformer model size gives rise to a unique challenge for mobile/edge devices: high cold-start inference latency. 

%\paragraph{Design objectives}
%We seek to design a new system for reducing the \textit{cold start} inference latency of \tfm{}s on mobile devices. 
%We target two goals:
%\begin{itemize}
%	\item 
%	\textit{Latency.}
%	The system should withstand frequent cold start while still delivering the inference results with low latency.
%	
%	\item 
%	\textit{Accuracy.}
%	Meanwhile, the system should not compromise inference accuracy. 
%	It needs to maximize the accuracy, and ensure it is competitive to state-of-the-art models.
%
%%	\item 
%%	\textit{}
%
%\end{itemize}
%
%\Note{merge below}
%\textbf{Design goals:}
%\begin{myenumerate}
%	\item 
%	Fast cold inference latency
%	
%	\item 
%	Comparable hot inference accuracy
%	
%	\item 
%	Small memory footprint	
%\end{myenumerate}


% --- obsolete --- 
%\paragraph{Our approach}
%\Note{ideas... TODO}
%
%\textbf{First, model sharding.}
%The pretrained model must be partitioned into fine-grained pieces, which have the following properties:
%\begin{itemize}
%	\item 
%	Partial expressiveness of the full model.
%	The pieces must carry semantic information and language features, such that they can form subnets and be executed. 
%	
%	
%	\item 
%	Incremental accuracy. 
%	More pieces -> better accuracy. \Note{where to forecast execute incrementally?}
%	
%	
%	\item 
%	Minimum pipeline bubble.
%	\Note{actually should not be `close'}. 
%	Instead, should be as small as possible -- you can never ``starve'' IO because you can always load extra. 
%	
%	This is to create the pipeline which has high utilization and small bubbles. 
%	We donot want CPU to starve and wait for IO.   
%\end{itemize}
%
%\paragraph{Opportunities}
%We plan to exploit the following opportunities:
%\begin{myenumerate}
%	\item 
%	Need pipeline parallelism of io/compute. 
%	Currently the resources of a mobile SoC are under-utilized. 
%	Existing work focuses on compressing a model and reducing its size, e.g. via quantization~\cite{tenarybert}, knowledge distillation~\cite{distilbert}, weight sharing~\cite{albert};
%	they still wait for the model loading to finish to begin inference computation, during which time the CPU is idle. 
%	%	E.g. DistilBert~\cite{distilbert} has half the layers of a BERT~\cite{bert} model. Yet, it is still 400 MB large and takes at least 2 seconds to load. 
%	%	Alternative compression approaches such as quantization~\cite{q8bert,tenarybert,binarybert,bibert}, often has inferior performance. 
%	
%	\item 
%	Partial model execution: the model can execute based on only partial parameters and can be gradually loaded up. 
%	This is possible due to MHA redundancy. 
%	Unlike vision networks, \tfm{}s exhibit high redundancy in its attention heads~\cite{16heads}.
%	As a result, with only a few (e.g. 4) attention heads, the performance degradation is only less than 10\%~\cite{dynabert}. %of a \tfm{} model 	
%\end{myenumerate}


\paragraph{Contributions}
The paper makes the following contributions:
\begin{myitemize}
	\item 
	For the first time it identifies and characterizes the cold start inference of transformers \st{on multiple platforms};
%	it will obtain diverse IO/Compute profiles measured on real hardwares, such as Odroid~\cite{odroid-web}, Raspberry Pi~\cite{rpi3-web}, and Beagleboard X15~\cite{x15-web}.
	
	\item 
	The idea of a resident model -- ... which unifies model loading and execution ... addressing cold start inference ..  
	
	\item 
	The inference engine design \sys{}... %for accelerating \tfm{} cold start inference of pretrained models on edge devices.
	It features two novel techniques: 
	1) \textit{model shards}, which partitions the whole pretrained model into multiple attention heads, quantized into different bitwidths;
	2) \textit{shard planning}, which schedules shards for both low latency and maximum accuracy, based on the specific IO/Compute profile of the hardware and a deadline.
	
	\item
	The implementation and evaluation of the proposed system.
%	It will evaluate the system on the pretrained  BERT~\cite{bert} model using the GLUE benchmark suite~\cite{glue-benchmark}.
%	The implementation will be made open-source to facilitate future research on the cold start inference problem. 
	
	%	\begin{itemize}
	%		\item 
	%		Pipelining 
	%		
	%		\item 
	%		Deadline-driven dynamic bitwidth selection for encoder layers. 
	%		
	%		\item 
	%		Hierarchical word embedding cache layers. 
	%	\end{itemize}
	%	Backing the techniques is a co-designed system memory management layer.. 
	%	Compared with the vanilla page cache, it is model aware and finer grained: at the granularity of an attention head instead of whole model file; 
	%	cache replacement strategy is pipeline-aware...
	%	
	%	\item 
	%	Case studies of \sys{} on a wide range of devices that have diverse hardware characteristics. 
	
\end{myitemize}



==> recycle/motiv-bkgn-recycle.tex <==
% !TeX root = main.tex
\subsection{\Tfm{} on mobile device}
\label{sec:motiv:primer}
%\Note{TODO: use formula}
%
%\Note{Explain: width (dimension, hidden dimension), depth (\# of stacked layers), what is the common scale of parameters}

\input{fig-transformer}

\paragraph{A primer on \tfm{}}
Figure~\ref{fig:motiv:transformer}
shows the architecture of Transformer~\cite{transformer}, the modern NN developed for NLP tasks.  
Compared with prior NNs (e.g. LSTM~\cite{lstm}), it features a unique Multi-Headed Attention (MHA) mechanism. %i.e. Multi-Headed Attention (MHA). 
MHA extracts features at sequence dimension by modeling pairwise word interactions through many \textit{attention heads} (typically 12), backed by three fully-connected (i.e. linear) layers, namely Query (Q), Key (K), Value (V).
Given an input, each attention head independently contributes an attention score as one representation of the feature space.
%space of the input.
Scores across attention heads are concatenated and then projected into higher feature dimensions by two linear layers in the point-wise Feed-Forward Network (FFN) module. %which feature dimensions. 

Due to the large number of fully connected layers, a \tfm{} based model contains as many as over 100 million parameters. 
Despite many parameters are highly redundant~\cite{head-prune-acl19}, a typical pretrained model in a few hundred MBs of model size (e.g. BERT~\cite{bert} model size is over 400MB).  
% and there exist many such layers (e.g. 12  layers~\cite{bert}). 
%into a high-dimensional (e.g. 512) feature space using attention map. 
%Different from prior NNs, Transformer deploys a unique attention module, which extracts features of words within a sentence and across sentences into a high-dimensional (e.g. 512) feature space using attention map. 

%Inside the attention module are many \textit{attention heads}, which are backed by three linear (i.e. fully connected) modules, Query (Q), Key (K), Value (V).
%Given an input, each attention head independently contributes its own attention score, which is pooled and processed by two fully connected layers of the FFN module to capture the textual pattern. 
%
%A \tfm{} model has high parameter redundancy, as there are large number of fully connected layers within each layer~\cite{head-prune-acl19}, and there exist many such layers (e.g. 12  layers~\cite{bert}). 
%, a \tfm{} layer has high parameter redundancy

%When a new sentence is fed into a Transformer, individual words are looked up and encoded as word embeddings, each containing as many as 758 dimensions.  
%The resultant embedding matrix for the sentence is then sent to a Transformer layer.
%A transformer layer first process the embedding matrix with the attention module, which consists of three linear modules dubbed as Query, Key, Value. \Note{Multi-Head Attention (MHA)}
%With their own weights, Q, K, V independently computes on the embedding matrix;
%the results are an attention score, given by the formula $Atten=QKV...$.
%The attention score is then fed into Feed Forward Neural (FFN) layer which captures the textual pattern of the sentence at current layer.
%For smaller networks, such as BERT~\cite{bert}, the process repeats for 12 stacked transformer layers while for larger ones, the process can repeat up to 96 layers. 
%\Note{Merge below}
%MHA \& FFN focus on two different dimensions, sequence and feature dimensions respectively. 
%To process Q,K,V, the attention module incorporates three linear layers with own weights;
%to speed up, it splits the matrices across multiple attention-heads, which computes in parallel. 
%The final results of the three linear layers is then combined as an attention score, for the input. 

%Encoder/decoder...
%Residue weights...
%Many variants have since emerged...

\paragraph{Key resources of a mobile device} are latency T and memory M. 
On one hand, mobile app interactions are brief, for less than a minute~\cite{livelab};
interactions with IPAs are even shorter, for only a few seconds~\cite{ipa-study-denmark,tsaiFasterResponsesAre2019}.
During such a short period, human attention is a scarce resource~\cite{proj-aura}.
It is vital that the system be responsive and rapid upon invocations, for a smooth user experience~\cite{falcon-mobisys12}. 




\paragraph{Why cold inference matters?}
\Note{to characterize:}
Multiple platforms
io/compute latency: per layer/per component
io/compute speed: what is the storage throughput, what is the CPU frequency?

Mobile app interactions are brief, for less than a minute~\cite{livelab};
interactions with IPAs are even shorter, for only a few seconds~\cite{ipa-study-denmark,tsaiFasterResponsesAre2019}.
During such a short period, human attention is a scarce resource~\cite{proj-aura}.
It is vital that the system be responsive and rapid upon invocations, for a smooth user experience~\cite{falcon-mobisys12}. 

Existing cold inference latency of \tfm{} inference, however, is far from ideal.
As shown in Figure~\ref{fig:motiv:lat-breakdown}, on a commodity embedded SoC the cold inference is as high as 4 seconds, which has already exceeded the typical duration of interactions with IPAs.
This is unacceptable to user experience.

Hence for the interactive NLP tasks we target, \sys{} aims to reduce its cold inference latency to the same level as \textbf{human interactions}.
That is, the latency (i.e. set by the deadline) is only a few hundred milliseconds~\cite{human-latency-study}, with hundred-milliseconds breaks between utterances.


==> recycle/motiv-recycle.tex <==
The workloads demonstrate two key properties:
\begin{myenumerate}
	\item 
	\textbf{IO dominates inference latency.}
	On average, model loading (IO time) contributes to over 90\% cold inference latency, as can be seen in Figure~\ref{fig:motive-char}.
	This is due to large parameters transformer models have -- tens of million, surpassing a commonly used CNN by tens of X, e.g. MobileNet has XXX parameters with XXX MB file. 
	\Note{XXX: IO is the key bottleneck}
	
	\item 
	\textbf{Divers io/compute capability}
	The ratio varies across devices due to different hardwares they have. 
	For instance, 10:1 on Odroid, XX:1 on Rpi3, and XX:1 on X15. 
\end{myenumerate}


\paragraph{Design implications}
\Note{cast the sentiment that we will do overlap IO vs Compute }
To minimize cold inference latency, 
%we can not afford to wait for the full model loading completion to start inference due to the large (synchronous) IO;
we must prioritize reducing the cost of IO task (i.e. model loading), which constitutes over 90\% of cold inference latency;
\Note{we cannot afford to wait for the model loading completion; 
we set to overlap IO vs Compute...}
In the meantime, we must take into consideration that the IO/Compute tasks are also hardware-dependent. 
%hardwares have various IO vs Compute ratio, suggesting the mileage may vary on different platforms. 
%different hardwares have various IO vs Compute ratio, calling for careful treatment of different platforms. 
%we must consider different IO/Compute due to hardware differences. 


\Note{merge below ....}
\paragraph{IO is the key bottleneck}
To understand the high latency of transformer cold inference, we use DistilBert, MobileBert, and \Note{XXX} which are designed for mobile/edge devices; 
larger model, e.g. RoberTa even fails to execute due to out of memory. 
We characterize the cold inference latency by layers and IO/Compute tasks, on three different platforms -- Odroid, Odroid, and X15.
Their hardware configurations are detailed in Table~\ref{tab:platforms}.



==> recycle/planning-recycle.tex <==
% !TeX root = main.tex

\section{Planning shard pipeline for heterogeneous devices}
\label{sec:design:planning}


\paragraph{\textit{Problem \& objectives}}
The user sets up a deadline for cold start inferences. 
To reduce the latency and to ensure meeting the deadline, our proposed system exploits the missed opportunity of overlapping IO (i.e. shard loading) with Compute (i.e. matrix multiplications and additions in MHA modules) tasks, resembling the pipelining idea~\cite{recnn,pipeline-cpu-gpu,pipeline-edge}.


\paragraph{Challenges}
Yet, it faces a key question: how to schedule an IO and Compute task? 
% the trade off between accuracy and latency...
The challenge is twofold.
\underline{First,} how to schedule for low latency on different devices?
As IO and Compute time is device-specific, it takes a cautious planning not to starve either for different devices, in order to meet the deadline timely. 
%The IO time of an uncompressed shard is a few $\times$ larger than the compute time on it, which we will show in preliminary results.
\underline{Second,} how to schedule for a maximum accuracy? 
As cold start inference latencies are amortized by loading and executing the model partially with shards, so is the model accuracy.
Our system sets to ramp up the accuracy as fast as possible while maintaining the high accuracy. 

\input{fig-planning}

\paragraph{Design.}
For a given deadline, we propose to dynamically plan the shard pipeline, which maximizes the inference accuracy while considering device heterogeneity, e.g. different IO/Compute capability. 

The approach comprises two steps. 
\underline{First, offline profiling}.
Our proposed system profiles time for an IO and Compute task on the corresponding platform in an offline fashion, out of the execution path of the inferences. 
For IO, the system measures the latency of loading an uncompressed shard from storage and derives the latency for the compressed shards, which is linear to their bitwidths.
%from the uncompressed latency, the system derives IO time of compressed shards, which is linear to their bitwidths.
For Compute, the system does a dry run with different number of heads and measures the layerwise latency. 
The rationale of profiling IO and Compute offline is they are data-independent~\cite{driverlet,asymo,tinystack}, whose latency hence is deterministic at run time. 
%both model loading and NN inference depends , 
%execution is solely dependent on the NN model itself. 
\underline{Second, online planning}. 
The proposed system executes the inferences in layers and overlaps the IO and Compute at each layer. 
%Deciding the Compute task is trivial, the system simply uses computes on shards.
To achieve a high accuracy, it schedules the IO and Compute based on two key ideas: 1) depths over widths. 
The system prioritizes loading and executing the \textbf{full} 12 layers, as long as the deadline permits.
2) first high-precision then low-precision. 
The system favors shards with higher precisions in top layers;
if possible, the system loads up a minimal number of \textit{full-precision} heads (typically 3 heads). 
The rationale is the weight distribution of \tfm{}s:
attention heads within each layer are redundant;
outlier weights are centered on top layers, requiring higher precisions.
%For a given deadline, 


\paragraph{\textit{Preliminary results}}
Our principle is based on measured per-layer outlier distribution of pretrained DynaBERT model.
As shown in Figure~\ref{fig:prelim:weight}, top layers have more outliers thus calling for higher precision.
We have also characterized the IO and Compute time of BERT~\cite{bert} on an Odroid dev board~\cite{odroid-web} as a sample IO/Compute profile, shown in Figure~\ref{fig:prelim:load}.
We have also profiled the per-component inference latency of BERT on an x86 machine for convenience, shown in Figure~\ref{fig:prelim:breakdown}. 
These preliminary results suggest a sublinear increase in Compute time as the number of attention heads (i.e. the sharding granularity) increase.
They will be as a key heuristic in planning the shard pipeline.

\input{fig-prelim-planning}


==> recycle/related-recycle.tex <==
% !TeX root = main.tex
\section{Related work}

We next discuss related work which have not been covered so far.

\xzlNote{moved to related work?}
The capability to tune $R$ on the basis of individual shards gives the resident model unprecedented elasticity needed by fine-grained management.
It sets us apart from prior dynamic \tfm{}s -- once loaded in memory, their fidelity version is fixed~\cite{haq} and that they must configure the same width for all layers~\cite{dynabert,hat}, respecting a ``rectangular'' shape because they are expected to be readily executable.
In comparison, our fidelity can adapt on-the-fly by replacing shard versions, and that it can have variable number of shards per layer.


\xzlNote{to merge}


\paragraph{Existing techniques are inadequate}
They cannot achieve our design goals because...
\begin{myitemize}
	\item 
	\textbf{Model compression.} 
	E.g. model structure~\cite{layerdrop,distilbert} \& feature pruning~\cite{mobilebert}; quantization~\cite{bibert,binarybert,q8bert}. 
	
	\textbf{Inadequacy:} cannot achieve both goals.
	Only IO elasticity (load a smaller size). 
	No compute/memory elasticity: once loaded become rigid; will be swapped in/out again.
		
	\item 
	\textbf{Dynamic NN.} E.g. Dynabert~\cite{dynabert}, NestDNN~\cite{nestdnn}, 
	
	\textbf{Inadequacy:} still has cold start; MM is coarse grained, etc. only depths \& widths. 
	only CPU/memory elasticity, which adapts to runtime constraint. 
	No IO elasticity because need to load the ``supernet'' to prune from. 
	No IO/compute parallelism. 
	
	\item 
	\textbf{(naive) Pipelining.} EdgePipe~\cite{edgepipe}.
	
	\textbf{Inadequacy:} cannot achieve both goals. 
	Only IO/compute parallelism. 
	Naive layerwise, no elasticity. 

\end{myitemize}


\xzlNote{moved}


\Note{diff with dynamic NNs -- In a model space, dynamic transformers provide coarse-grained waypoints which can have high accuracy under memory/latency constraints, our system 1) expands the waypoints by refining them into finer granularity, 2) and more importantly, provides a path (IO/computation planning) to connecting the waypoints}

\Note{Why our engine faces unique challenges?}
\begin{myitemize}
	\item 
	AutoML (NAS), notably~\cite{hat,haq,hawq}, may efficiently sample the search space and find an optimal $R'$ (a point in the solution space). 
	They do not answer the question of how to connect it ($R'$) with current point $R$, under runtime constraints $T$ and $M$ in the context of pipelining...
	
	\item 
	NestDNN~\cite{nestdnn} may switch between models by leveraging a multi-capacity model at runtime.
	However, the switching is still rigid, i.e. simply by calculating the delta between two models. 
	It does not consider pipelining nor explore solution space at runtime.
\end{myitemize}



Recent techniques can scale resources for NLP execution~\xzlNote{cite} \textit{individually} but not jointly. 
For example, model compression reduces the model load IO~\cite{mobilebert,layerdrop,distilbert,bibert,binarybert,q8bert}, but offers no solution ... highly parallel IO/computation pipeline ... 
managing important model parameters in memory. 
DynaBert~\cite{dynabert} and NestDNN~\cite{nestdnn} instantiates a model's multiple versions with variable compute demands; 
they however offer no solution on co-scheduling model execution and loading in parallel, which includes loading a version from scratch and loading the deltas between model versions.
%not accounting for IO delays that would interleave with the computations. 
These techniques are inadequate for our goal. 


% moved from intro
Model compression, for example, is a common technique for reducing model size, facilitating faster loading;
it includes model structure~\cite{layerdrop,distilbert} and feature pruning~\cite{mobilebert}, and quantization which reduces full-precisions (32bit) parameters into low-bit (e.g. 2bit) representations~\cite{bibert,binarybert,q8bert}. 
Alternatively, one may deploy dynamic \tfm{}s which adapt to varied memory or latency constraints by correspondingly configuring model widths and/or depths~\cite{dynabert,edgebert}. 


\Note{Compare with automated mixed-precision quantization}

Key difference: 
\begin{myitemize}
	\item 
	Theirs: search for the quantization precision setup of the model. Offline, heuristics  -- hessian, entropy, contrastive,  goal: accuracy, hot inference only
	
	\item
	Ours: similarly also a search problem. Diff: Online, heuristics -- weight distribution, goal: accuracy under latency and IO constraint, cold/warm inference 
\end{myitemize}

In this section we discuss the work related to our proposed system and our goal of reducing cold inference latency.

\paragraph{Compressing \tfm{}s}
One may compress a \tfm{}-based model, such that its model has fewer parameters and/or requires less compute bandwidth (e.g. from floating point to integer computation), reducing both IO and Compute time. 
From a higher level, the key difference (also the novelty) of our proposed system is we address the cold inference process, which they overlook, by overlapping IO and Compute of \tfm{} shards. 

Nevertheless, we describe our differences in the following specific compression approaches.
%There are following approaches in doing so. 
\ul{Structured pruning} prunes a \tfm{} model along two axes: width~\cite{liDSNetDynamicWeight2021,liDynamicSlimmableNetwork2021,mccarleyStructuredPruningBERTbased2021,mobilebert} and depth~\cite{layerdrop, dynabert,elbayadDepthAdaptiveTransformer2020,distilbert}. 
Inspired by them, our proposed sharding strategy is also structured, i.e. attention head-based, which is the \textit{width} of a \tfm{} layer.
Different from them, the width and depth of our system is dynamically decided by the pipeline scheuler (\S\ref{sec:design:planning}), which targets at both accuracy and latency.
\ul{Weight sharing} reduces the \tfm{} parameters by sharing paramters across attention heads~\cite{albert} or different layers~\cite{universal-transformer}. 
Similar to them, the larger \tfm{} subnets in our proposed system also shares with parameters (i.e. in shards) with those of smaller subnets.
Differently, our proposed system does not require retraining or fine-tuning. 
\ul{Quantization} reduces the full precision of parameters (often in 32 bits) to low bits.
Some quantize the whole model to a fixed bitwidth, e.g. 2 bits~\cite{binarybert,bibert}. 
Differently, our proposed shards of a model have different bitwidths. 
Some quantize the model layers in mixed-precision to achieve latency goal~\cite{haq}, energy goal~\cite{mixed-quantization-energy} by searching for optimal bitwidth configurations~\cite{emq,hawq}.
Inspired by them, our system also features a mixed-precision model and adopts known quantization techniques~\cite{cnn-weight-share,gobo};
compared with them, the precision configurations are decided w.r.t. the given deadline and hardware capability. 



%fake quantization\cite{cnn-weight-share} is close to our approach.

\paragraph{Systems for accelerating NN inference}
On the other hand, offerings form systems community focus on improving the efficiency of computation.
Asymo~\cite{asymo} accelerates inference by tailoring matrix multiplication operations for the architectural characteristics of the Arm heterogeneous multi-processing (HMP) cores;
similarly,~\cite{transformer-cpu} optimizes the operations on x86 CPUs.
EdgeBERT~\cite{edgebert} also targets at an inference deadline by adopting an early exit approach, in the same spirit as depth compression of a \tfm{} model.
Compared with them~\cite{asymo,transformer-cpu,edgebert}, our proposed system shares the same overarching goal of reducing the inference latency.
Their techniques are complementary to our proposed system, i.e. in hot inferences, but are not applicable in cold inferences, where IO is the key bottlneck instead of compute. %they do not consider 
%Differently, we address the cold inference  
EdgePipe~\cite{edgepipe} partitions a \tfm{} model, pipelines the stages of inference, and dispatches the stage onto different devices. 
Compared with it, we have a similar idea of partitioning and pipelining a \tfm{} model.
Yet, we focus on on-device inference and exploit the IO/Compute parallelism of a single device.

%NNV12~\cite{nnv12}
 
\paragraph{Pipeline parallelism for ML}
Pipelining has been extensively used to accelerate ML. 
Prior work mainly uses it to scale out ML to multiple machines (overcome limit of single machine resource). 
Notably for training, PP is used to distribute a model or training data over a cluster of machines, improving data locality and hiding delays of data move. 
\xzlNote{cite GPipe, PipeDream, etc.}
For inference, ....
The major innovations include ways to split data batches and partition models. 
We share a similar goal of maximizing pipeline utilization and minimizing bubbles.  
Unlike that they focus on a pipeline of computations (forward/backward passes of different inputs) or network/computation, our pipeline consists of disk IO tasks and computation. 
our approach towards high efficiency is through adjusting IO workloads of model shards to the computation. 

\textbf{GPipe}: split a model into sublayers to be distributed across multiple machines. Problem: layer dependencies; forward/backward passes dependencies. Solution: split minibatches into microbatches, create pipeline parallelism. 
Difference: pipeline parallelism is our baseline, we increase the parallelism through tuning fidelity (hence IO delays) of each shard. 



%\paragraph{Mixed-precision quantization}
%
%The line of work~\cite{haq,bitmixer,mixed-quantization-energy,emq} focuses on selects an optimal quantization bit-width for each layer out of latency~\cite{haq}, accuracy, energy~\cite{mixed-quantization-energy} goal, by using NAS~\cite{X} or evolutionary search~\cite{emq}, or based on Hessian score~\cite{hawq}.

==> recycle/sharding-recycle.tex <==
% !TeX root = main.tex

\section{Building an elastic IO/compute pipeline}
\label{sec:design:sharding}

\Note{Challenges:}
\begin{myitemize}
	\item 
	Highly skewed io/compute time of a transformer layer
	
	\item 
	Device heterogeneity. Various Deadline.
\end{myitemize}


\paragraph{Challenges}
In hindsight, one naive approach to exploiting the pipeline parallelism is to overlap io 


We set to shard \textit{pretrained} language models (e.g. BERT) without retraining. 
The \underline{first} research question is at what granularity? 
To do so, there are two design choices. 
One is \textit{unstructured} sharding~\cite{gordonCompressingBERTStudying2020,ladabert}, that is, viewing the whole (over 100 million) parameters as a large flat data array and splitting it in trunks. % which is common in network pruning
The other is \textit{structured} sharding, where shards conform to a network structure, e.g. a layer~\cite{layerdrop,edgebert}, a CNN filter~\cite{cnn-filter-pruning}, or a \tfm{} attention head~\cite{dynabert}. 
The \underline{second} research question is how to compress the shards?
Broadly, three techniques can be used to compress the shards:
shards may be pruned and discarded~\cite{cnn-entropy-filter-pruning, cnn-prune-nvidia}; 
they may share weights with each other~\cite{transformer-attention-share,nn-weight-share};
they may be quantized into a lower bitwidth~\cite{binarybert,ibert,bibert}.
%Our system must navigate through the compression techniques to ensure that shards 
Our system must shard a model cautiously, navigate through the compression techniques, and ensure a decent model performance. %shards should work well with each other

\input{fig-sharding}

\paragraph{\textit{Our ideas}}
For pretrained \tfm{} models, we propose a retraining-free sharding approach, which is a novel combination of width-adaptive \tfm{} and outlier-aware quantization.
%\textbf{structured}, \textbf{outlier-aware quantization} approach for sharding the pretrained \tfm{} model. 

Our key idea is to shard the model by layers, and by their attention heads.
For each layer, the system uses outlier-aware quantization, similar to~\cite{gobo}. 
It first fits its weights into a Gaussian model.
It uses the Gaussian model to find out a group of ``outliers'' parameters and preserve them in full precision.
For the rest, the system quantizes them into $n$-bit integers (e.g. typically 2 to 4) using \textit{simulated quantization}~\cite{quantization-survey}, where each integer points to a full-precision FP32 value called a centroid, representing a group of original weights.
The system decides the centroids by dividing the non-outlier parameters into $2^n$ groups and calculating their arithmetic means.
\ul{The key difference to prior work} is our system does not quantize the attention heads uniformly into $n$-bit. 
Instead, each shard may be quantized into different bitwidths; 
the eventual model comprises shards with different precisions. 
Figure~\ref{fig:design:sharding} shows the idea.

Our rationale for the sharding strategy is as follows.
First, an attention head is an atomic structure of the MHA mechanism~\cite{transformer}, which is learned at training time;
shards conforming to the structure preserves the same mechanism.
%shards can work seamlessly with each other. 
Second, attention head weights are heavily redundant~\cite{16heads}.
%Most need only a few bits~\cite{ibert,binarybert} while only outliers need high-precision.
Preserving the few outliers (e.g. 0.01\%~\cite{gobo}) while representing the most others with a small number of values ensures performance.

\input{fig-prelim-sharding}

\paragraph{\textit{Preliminary results}}
We have done preliminary experiments on the pretrained model from DynaBERT~\cite{dynabert}. 
Figure~\ref{fig:prelim:sharding} validates the importance of outliers with SST-2 frrom GLUE benchmark~\cite{glue-benchmark}, a dual-class sentiment classification task. %to evaluate the model performance of the proposed sharding strategy.
It shows our proposed quantization technique achieve near original model performance (less than 1\% degradation when quantized into 4 bits) while without outliers the quantized model performance drops to 50\% (i.e. random guess).
Figure~\ref{fig:prelim:others} shows the proposed quantization technique also achieves decent performance in two other tasks (less than 1\% degradation when quantized into 5 bits), STS-B and MNLI in GLUE~\cite{glue-benchmark}.
Figure~\ref{fig:prelim:heads} shows the attention-head granularity achieves a decent performance and scales with number of heads, as expected.


 



==> related.tex <==
% !TeX root = main.tex
\balance
\section{Related work}


%We next discuss related work.  %not covered so far.

%However, we are the first to have the capability to tune fidelities on the basis of individual shards, in order to adapt to both memory and latency constraints. %gives us unprecedented elasticity %needed by fine-grained 
%Inspired by them, we adapt to latency constraints by adjusting submodel sizes. 
%However, we are the first to have the capability to tune fidelities on the basis of individual shards, in order to adapt to both memory and latency constraints. %gives us unprecedented elasticity %needed by fine-grained management.
%It sets us apart from prior dynamic \tfm{}s -- once loaded in memory, their fidelity version is fixed~\cite{haq} and that they must configure the same width for all layers~\cite{dynabert,hat}, respecting a ``rectangular'' shape because they are expected to be readily executable.
%In comparison, our fidelity can adapt on-the-fly by replacing shard versions, and that it can have variable number of shards per layer.

%Moreover, they offer no solution on co-scheduling model execution and loading in parallel, which includes loading a version from scratch and loading the deltas between model versions.

%NestDNN~\cite{nestdnn} may switch between models by leveraging a multi-capacity model at runtime.
%However, the switching is still rigid, i.e. simply by calculating the delta between two models. 
%It does not consider pipelining nor explore solution space at runtime.
%\Note{diff with dynamic NNs -- In a model space, dynamic transformers provide coarse-grained waypoints which can have high accuracy under memory/latency constraints, our system 1) expands the waypoints by refining them into finer granularity, 2) and more importantly, provides a path (IO/computation planning) to connecting the waypoints}

%\paragraph{Automated quantization} searches for an optimal (mixed) quantization strategy of a network, often on a per layer basis.
%HAQ~\cite{haq} adopts a RL approach;
%HAWQ~\cite{hawq} chooses Hessian trace as a measure for optimal bit-widths;
%EMQ~\cite{emq} uses evolutionary search to find the optimal bit-widths combinations of layers.
%%Bit-Mixer~\cite{bitmixer} trains a meta-quantized network and allows the bit-widths of individual layers can be selected at run time. 
%Similarly, our \tfm{} is also mixed-precision.
%Compared with them, we do not need any fine-tuning, which is time-consuming. 
%Also, the decisions are finer grained, e.g. per-shard and must be done at run time.
%%\paragraph{Efficient \tfm{}s}



%for improving data locality and hiding delays of data move

%\xzlNote{cite GPipe, PipeDream, etc.}

%% Merged
%Gpipe~\cite{gpipe}: split a model into sublayers to be distributed across multiple machines. Problem: layer dependencies; forward/backward passes dependencies. 
%Solution: split minibatches into microbatches, create pipeline parallelism. 
%Difference: pipeline parallelism is our baseline, we increase the parallelism through tuning fidelity (hence IO delays) of each shard. 
%
%Pipedream~\cite{pipedream}: partitioning layers and scheduling forward/backward passes which respects data dependencies for maximizing pipeline throughput, minimizing stalls. 
%
%EdgePipe~\cite{edgepipe} partitions a \tfm{} model, pipelines the stages of inference, and dispatches the stage onto different devices. 
%Compared with it, we have a similar idea of partitioning and pipelining a \tfm{} model.
%Yet, we focus on on-device inference and exploit the IO/Compute parallelism of a single device.
%
%PipeTransformer~\cite{pipetransformer}: achieves elastic pipelining during training by 1) adaptively freezing layers on the fly, removing the layers from the pipeline. 2) allocating more resources to remaining layers. 
% 
%DART~\cite{dart}: partitions layers among CPU/GPU and maximizes the co-utilization of inference job execution. (Compute/Compute pipeline)
%
%For inference, ....
%The major innovations include ways to split data batches and partition models. 
%We share a similar goal of maximizing pipeline utilization and minimizing bubbles.  
%Unlike that they focus on a pipeline of computations (forward/backward passes of different inputs) or network/computation, our pipeline consists of disk IO tasks and computation. 
%our approach towards high efficiency is through adjusting IO workloads of model shards to the computation. 



\begin{comment}

\xzlNote{to merge}
\paragraph{Existing techniques are inadequate}
They cannot achieve our design goals because...
\begin{myitemize}
	\item 
	\textbf{Model compression.} 
	E.g. model structure~\cite{layerdrop,distilbert} \& feature pruning~\cite{mobilebert}; quantization~\cite{bibert,binarybert,q8bert}. 
	
	\textbf{Inadequacy:} cannot achieve both goals.
	Only IO elasticity (load a smaller size). 
	No compute/memory elasticity: once loaded become rigid; will be swapped in/out again.
		
	\item 
	\textbf{Dynamic NN.} E.g. Dynabert~\cite{dynabert}, NestDNN~\cite{nestdnn}, 
	
	\textbf{Inadequacy:} still has cold start; MM is coarse grained, etc. only depths \& widths. 
	only CPU/memory elasticity, which adapts to runtime constraint. 
	No IO elasticity because need to load the ``supernet'' to prune from. 
	No IO/compute parallelism. 
	
	\item 
	\textbf{(naive) Pipelining.} EdgePipe~\cite{edgepipe}.
	
	\textbf{Inadequacy:} cannot achieve both goals. 
	Only IO/compute parallelism. 
	Naive layerwise, no elasticity. 

\end{myitemize}


\xzlNote{moved}


\Note{Why our engine faces unique challenges?}
\begin{myitemize}
	\item 
	AutoML (NAS), notably~\cite{hat,haq,hawq}, may efficiently sample the search space and find an optimal $R'$ (a point in the solution space). 
	They do not answer the question of how to connect it ($R'$) with current point $R$, under runtime constraints $T$ and $M$ in the context of pipelining...
	
	\item 

\end{myitemize}



Recent techniques can scale resources for NLP execution~\xzlNote{cite} \textit{individually} but not jointly. 
For example, model compression reduces the model load IO~\cite{mobilebert,layerdrop,distilbert,bibert,binarybert,q8bert}, but offers no solution ... highly parallel IO/computation pipeline ... 
managing important model parameters in memory. 
DynaBert~\cite{dynabert} and NestDNN~\cite{nestdnn} instantiates a model's multiple versions with variable compute demands; 

%not accounting for IO delays that would interleave with the computations. 
These techniques are inadequate for our goal. 


% moved from intro



\Note{Compare with automated mixed-precision quantization}

Key difference: 
\begin{myitemize}
	\item 
	Theirs: search for the quantization precision setup of the model. Offline, heuristics  -- hessian, entropy, contrastive,  goal: accuracy, hot inference only
	
	\item
	Ours: similarly also a search problem. Diff: Online, heuristics -- weight distribution, goal: accuracy under latency and IO constraint, cold/warm inference 
\end{myitemize}

In this section we discuss the work related to our proposed system and our goal of reducing cold inference latency.

\paragraph{Compressing \tfm{}s}
One may compress a \tfm{}-based model, such that its model has fewer parameters and/or requires less compute bandwidth (e.g. from floating point to integer computation), reducing both IO and Compute time. 
From a higher level, the key difference (also the novelty) of our proposed system is we address the cold inference process, which they overlook, by overlapping IO and Compute of \tfm{} shards. 

Nevertheless, we describe our differences in the following specific compression approaches.
%There are following approaches in doing so. 
\ul{Structured pruning} prunes a \tfm{} model along two axes: width~\cite{liDSNetDynamicWeight2021,liDynamicSlimmableNetwork2021,mccarleyStructuredPruningBERTbased2021,mobilebert} and depth~\cite{layerdrop, dynabert,elbayadDepthAdaptiveTransformer2020,distilbert}. 
Inspired by them, our proposed sharding strategy is also structured, i.e. attention head-based, which is the \textit{width} of a \tfm{} layer.
Different from them, the width and depth of our system is dynamically decided by the pipeline scheuler (\S\ref{sec:design:planning}), which targets at both accuracy and latency.
\ul{Weight sharing} reduces the \tfm{} parameters by sharing paramters across attention heads~\cite{albert} or different layers~\cite{universal-transformer}. 
Similar to them, the larger \tfm{} subnets in our proposed system also shares with parameters (i.e. in shards) with those of smaller subnets.
Differently, our proposed system does not require retraining or fine-tuning. 
\ul{Quantization} reduces the full precision of parameters (often in 32 bits) to low bits.
Some quantize the whole model to a fixed bitwidth, e.g. 2 bits~\cite{binarybert,bibert}. 
Differently, our proposed shards of a model have different bitwidths. 
Some quantize the model layers in mixed-precision to achieve latency goal~\cite{haq}, energy goal~\cite{mixed-quantization-energy} by searching for optimal bitwidth configurations~\cite{emq,hawq}.
Inspired by them, our system also features a mixed-precision model and adopts known quantization techniques~\cite{cnn-weight-share,gobo};
compared with them, the precision configurations are decided w.r.t. the given deadline and hardware capability. 



%fake quantization\cite{cnn-weight-share} is close to our approach.

\paragraph{Systems for accelerating NN inference}
On the other hand, offerings form systems community focus on improving the efficiency of computation.
Asymo~\cite{asymo} accelerates inference by tailoring matrix multiplication operations for the architectural characteristics of the Arm heterogeneous multi-processing (HMP) cores;
similarly,~\cite{transformer-cpu} optimizes the operations on x86 CPUs.
EdgeBERT~\cite{edgebert} also targets at an inference deadline by adopting an early exit approach, in the same spirit as depth compression of a \tfm{} model.
Compared with them~\cite{asymo,transformer-cpu,edgebert}, our proposed system shares the same overarching goal of reducing the inference latency.
Their techniques are complementary to our proposed system, i.e. in hot inferences, but are not applicable in cold inferences, where IO is the key bottlneck instead of compute. %they do not consider 
%Differently, we address the cold inference  


%NNV12~\cite{nnv12}
 




%\paragraph{Mixed-precision quantization}
%
%The line of work~\cite{haq,bitmixer,mixed-quantization-energy,emq} focuses on selects an optimal quantization bit-width for each layer out of latency~\cite{haq}, accuracy, energy~\cite{mixed-quantization-energy} goal, by using NAS~\cite{X} or evolutionary search~\cite{emq}, or based on Hessian score~\cite{hawq}.
\end{comment}

==> scripts/Makefile <==
# batch convert all .pptx files in a directory to .pdf  
# files and crop them. 
# 
# to be used in conjunction with ppt.vbs, which converts
# a .pptx file into a pdf. 
#
# usage: copy this file and ppt.vbs to figs/ and run make
# there
#
# environment: win 10 cmd
#

docobjects := $(patsubst %.docx,%.pdf,$(wildcard *.docx)) $(patsubst %.dox,%.pdf,$(wildcard *.dox))
pptobjects := $(patsubst %.pptx,%.pdf,$(wildcard *.pptx))

current_dir  := $(shell cd)

all : check_overlap $(docobjects) $(pptobjects) 

	
docx : $(docobjects)

pptx : $(pptobjects)

clean :
	del /Q $(docobjects) $(pptobjects)

check_overlap :
	@echo "$(current_dir)"
		
		
%.pdf.uncrop : %.docx
	"c:\Windows\SysWOW64\cscript.exe" "$(scriptDir)\docx.vbs" "$(current_dir)\$^" "$(current_dir)\$@"

%.pdf.uncrop : %.dox
	"c:\Windows\SysWOW64\cscript.exe" "$(scriptDir)\docx.vbs" "$(current_dir)\$^" "$(current_dir)\$@"

%.pdf.uncrop : %.pptx
	"c:\Windows\SysWOW64\cscript.exe" "$(scriptDir)\ppt.vbs" "$(current_dir)\$^" "$(current_dir)\$@"

%.pdf: %.pdf.uncrop
	"$(scriptDir)\bin\pdfcrop.exe" $^ $@
	
	
.PHONY: check_overlap all docx pptx

==> scripts/bin/pdfcrop <==
#!/usr/bin/env perl
use strict;
$^W=1; # turn warning on
#
# pdfcrop.pl
#
# Copyright (C) 2002, 2004, 2005, 2008-2012 Heiko Oberdiek.
#
# This program may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.2
# of this license or (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.2 or later is part of all distributions of LaTeX
# version 1999/12/01 or later.
#
# See file "README" for a list of files that belong to this project.
#
# This file "pdfcrop.pl" may be renamed to "pdfcrop"
# for installation purposes.
#
my $prj         = 'pdfcrop';
my $file        = "$prj.pl";
my $program     = uc($&) if $file =~ /^\w+/;
my $version     = "1.38";
my $date        = "2012/11/02";
my $author      = "Heiko Oberdiek";
my $copyright   = "Copyright (c) 2002-2012 by $author.";
#
# Reqirements: Perl5, Ghostscript
# History:
#   2002/10/30 v1.0:  First release.
#   2002/10/30 v1.1:  Option --hires added.
#   2002/11/04 v1.2:  "nul" instead of "/dev/null" for windows.
#   2002/11/23 v1.3:  Use of File::Spec module's "devnull" call.
#   2002/11/29 v1.4:  Option --papersize added.
#   2004/06/24 v1.5:  Clear map file entries so that pdfTeX
#                     does not touch the fonts.
#   2004/06/26 v1.6:  Use mgs.exe instead of gswin32c.exe for MIKTEX.
#   2005/03/11 v1.7:  Support of spaces in file names
#                     (open("-|") is used for ghostscript call).
#   2008/01/09 v1.8:  Fix for moving the temporary file to the output
#                     file across file system boundaries.
#   2008/04/05 v1.9:  Options --resolution and --bbox added.
#   2008/07/16 v1.10: Support for XeTeX added with new options
#                     --pdftex, --xetex, and --xetexcmd.
#   2008/07/22 v1.11: Workaround for open("-|").
#   2008/07/23 v1.12: Workarounds for the workaround (error detection, ...).
#   2008/07/24 v1.13: open("-|")/workaround removed.
#                     Input files with unsafe file names are linked/copied
#                     to temporary file with safe file name.
#   2008/09/12 v1.14: Error detection for invalid Bounding Boxes.
#   2009/07/14 v1.15: Fix for negative coordinates in Bounding Boxes
#                     (David Menestrina).
#   2009/07/16 v1.16: Security fixes:
#                     * -dSAFER added for Ghostscript,
#                     * -no-shell-escape added for pdfTeX/XeTeX.
#   2009/07/17 v1.17: Security fixes:
#                     * Backticks and whitespace are forbidden
#                       for options --(gs|pdftex|xetex)cmd.
#                     * Validation of options --papersize and --resolution.
#   2009/07/18 v1.18: * Restricted mode added.
#                     * Option --version added.
#   2009/09/24 v1.19: * Ghostscript detection rewritten.
#                     * Cygwin: `gs' is preferred to `gswin32c'.
#   2009/10/06 v1.20: * File name sanitizing in .tex file.
#   2009/12/21 v1.21: * Option --ini added for IniTeX mode.
#                     * Option --luatex and --luatexcmd added for LuaTeX.
#   2009/12/29 v1.22: * Syntax description for option --bbox fixed
#                       (Lukas Prochazka).
#   2010/01/09 v1.23: * Options --bbox-odd and -bbox-even added.
#   2010/08/16 v1.24: * Workaround added for buggy ghostscript ports
#                       that print the BoundingBox data twice.
#   2010/08/26 v1.25: * Fix for the case that the PDF file contains
#                       an entry /CropBox different to /MediaBox.
#                     * \pageinclude implemented for XeTeX.
#                     * XeTeX: --clip does not die, but this option
#                       is ignored, because XeTeX always clip.
# 2010/08/26 v1.26: * XeTeX's \XeTeXpdffile expects keyword
#                     `media', not `mediabox'.
#                   * New option --pdfversion.
#                     Default is `auto' that means the PDF version
#                     is inherited from the input file. Before
#                     pdfcrop has used the TeX engine's default.
#                   * Option --luatex fixed (extra empty page at end).
# 2010/09/03 v1.27: * Workaround of v1.24 fixed.
# 2010/09/06 v1.28: * The Windows registry is searched if Ghostscript
#                     is not found via PATH.
#                   * Windows only: support of spaces in command
#                     names in unrestricted mode.
# 2010/09/06 v1.29: * Find the latest Ghostscript version in registry.
# 2010/09/15 v1.30: * Warning of pdfTeX because of \pdfobjcompresslevel
#                     avoided when reducing \pdfminorversion.
#                   * Fix for TeX syntax characters in input file names.
# 2010/09/17 v1.31: * Passing the input file name via hex string to TeX.
#                   * Again input file names restricted for Ghostscript
#                     command line, switch then to symbol link/copy
#                     method.
# 2011/08/10 v1.32: * Detection for gswin64c.exe added.
# 2012/02/01 v1.33: * Input file can be `-' (standard input).
# 2012/04/18 v1.34: * Format of --version changed
#                     from naked version number to a line with
#                     program name, date and version.
# 2012/10/15 v1.35: * Additional debug infos added for Perl version.
# 2012/10/16 v1.36: * More error codes added.
# 2012/10/16 v1.37: * Extended error messages if available.
#                   * Fix for broken v1.36.
# 2012/11/02 v1.38: * Fix for unsufficient cleanup, if function `cleanup' is
#                     prematurely called in `eval' for `symlink' checking.

### program identification
my $title = "$program $version, $date - $copyright\n";

### error strings
my $Error = "!!! Error:"; # error prefix

### make ENV safer
delete @ENV{qw(IFS CDPATH ENV BASH_ENV)};

# Windows detection (no SIGHUP)
my $Win = 0;
$Win = 1 if $^O =~ /mswin32/i;
$Win = 1 if $^O =~ /cygwin/i;
use Config;
my $archname = $Config{'archname'};
$archname = 'unknown' unless defined $Config{'archname'};

### extended error messages
sub exterr () {
    chomp(my $msg_errno = $!);
    chomp(my $msg_extended_os_error = $^E);
    if ($msg_errno eq $msg_extended_os_error) {
        $msg_errno;
    }
    else {
        "$msg_errno/$msg_extended_os_error";
    }
}

### string constants for Ghostscript run
# get Ghostscript command name
$::opt_gscmd = '';
sub find_ghostscript () {
    return if $::opt_gscmd;
    if ($::opt_debug) {
        print "* Perl executable: $^X\n";
        if ($] < 5.006) {
            print "* Perl version: $]\n";
        }
        else {
            printf "* Perl version: v%vd\n", $^V;
        }
        if (defined &ActivePerl::BUILD) {
            printf "* Perl product: ActivePerl, build %s\n", ActivePerl::BUILD();
        }
        use Config;
        printf "* Pointer size: $Config{'ptrsize'}\n";
        printf "* Pipe support: %s\n",
                (defined($Config{'d_pipe'}) ? 'yes' : 'no');
        printf "* Fork support: %s\n",
                (defined($Config{'d_fork'}) ? 'yes' : 'no');
    }
    my $system = 'unix';
    $system = "dos" if $^O =~ /dos/i;
    $system = "os2" if $^O =~ /os2/i;
    $system = "win" if $^O =~ /mswin32/i;
    $system = "cygwin" if $^O =~ /cygwin/i;
    $system = "miktex" if defined($ENV{"TEXSYSTEM"}) and
                          $ENV{"TEXSYSTEM"} =~ /miktex/i;
    print "* OS name: $^O\n" if $::opt_debug;
    print "* Arch name: $archname\n" if $::opt_debug;
    print "* System: $system\n" if $::opt_debug;
    my %candidates = (
        'unix' => [qw|gs gsc|],
        'dos' => [qw|gs386 gs|],
        'os2' => [qw|gsos2 gs|],
        'win' => [qw|gswin32c gs|],
        'cygwin' => [qw|gs gswin32c|],
        'miktex' => [qw|mgs gswin32c gs|]
    );
    if ($system eq 'win' or $system eq 'cygwin' or $system eq 'miktex') {
        if ($archname =~ /mswin32-x64/i) {
            my @a = ();
            foreach my $name (@{$candidates{$system}}) {
                push @a, 'gswin64c' if $name eq 'gswin32c';
                push @a, $name;
            }
            $candidates{$system} = \@a;
        }
    }
    my %ext = (
        'unix' => '',
        'dos' => '.exe',
        'os2' => '.exe',
        'win' => '.exe',
        'cygwin' => '.exe',
        'miktex' => '.exe'
    );
    my $candidates_ref = $candidates{$system};
    my $ext = $Config{'_exe'};
    $ext = $ext{$system} unless defined $ext;
    use File::Spec;
    my @path = File::Spec->path();
    my $found = 0;
    foreach my $candidate (@$candidates_ref) {
        foreach my $dir (@path) {
            my $file = File::Spec->catfile($dir, "$candidate$ext");
            if (-x $file) {
                $::opt_gscmd = $candidate;
                $found = 1;
                print "* Found ($candidate): $file\n" if $::opt_debug;
                last;
            }
            print "* Not found ($candidate): $file\n" if $::opt_debug;
        }
        last if $found;
    }
    if (not $found and $Win) {
        $found = SearchRegistry();
    }
    if ($found) {
        print "* Autodetected ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
    else {
        $::opt_gscmd = $$candidates_ref[0];
        print "* Default ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
}

sub SearchRegistry () {
    my $found = 0;
    eval 'use Win32::TieRegistry qw|KEY_READ REG_SZ|;';
    if ($@) {
        if ($::opt_debug) {
            print "* Registry lookup for Ghostscript failed:\n";
            my $msg = $@;
            $msg =~ s/\s+$//;
            foreach (split /\r?\n/, $msg) {
                print "  $_\n";
            }
        }
        return $found;
    }
    my $open_params = {Access => KEY_READ(), Delimiter => '/'};
    my $key_name_software = 'HKEY_LOCAL_MACHINE/SOFTWARE/';
    my $current_key = $key_name_software;
    my $software = new Win32::TieRegistry $current_key, $open_params;
    if (not $software) {
        print "* Cannot find or access registry key `$current_key'!\n"
                if $::opt_verbose;
        return $found;
    }
    print "* Search registry at `$current_key'.\n" if $::opt_debug;
    my %list;
    foreach my $key_name_gs (grep /Ghostscript/i, $software->SubKeyNames()) {
        $current_key = "$key_name_software$key_name_gs/";
        print "* Registry entry found: $current_key\n" if $::opt_debug;
        my $key_gs = $software->Open($key_name_gs, $open_params);
        if (not $key_gs) {
            print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
            next;
        }
        foreach my $key_name_version ($key_gs->SubKeyNames()) {
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            print "* Registry entry found: $current_key\n" if $::opt_debug;
            if (not $key_name_version =~ /^(\d+)\.(\d+)$/) {
                print "  The sub key is not a version number!\n" if $::opt_debug;
                next;
            }
            my $version_main = $1;
            my $version_sub = $2;
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            my $key_version = $key_gs->Open($key_name_version, $open_params);
            if (not $key_version) {
                print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
                next;
            }
            $key_version->FixSzNulls(1);
            my ($value, $type) = $key_version->GetValue('GS_DLL');
            if ($value and $type == REG_SZ()) {
                print "  GS_DLL = $value\n" if $::opt_debug;
                $value =~ s|([\\/])([^\\/]+\.dll)$|$1gswin32c.exe|i;
                my $value64 = $value;
                $value64 =~ s/gswin32c\.exe$/gswin64c.exe/;
                if ($archname =~ /mswin32-x64/i and -f $value64) {
                    $value = $value64;
                }
                if (-f $value) {
                    print "  EXE found: $value\n" if $::opt_debug;
                }
                else {
                    print "  EXE not found!\n" if $::opt_debug;
                    next;
                }
                my $sortkey = sprintf '%02d.%03d %s',
                        $version_main, $version_sub, $key_name_gs;
                $list{$sortkey} = $value;
            }
            else {
                print "  Missing key `GS_DLL' with type `REG_SZ'!\n" if $::opt_debug;
            }
        }
    }
    foreach my $entry (reverse sort keys %list) {
        $::opt_gscmd = $list{$entry};
        print "* Found (via registry): $::opt_gscmd\n" if $::opt_debug;
        $found = 1;
        last;
    }
    return $found;
}

# restricted mode
my $restricted = 0;
if ($0 =~ /rpdfcrop/ or $0 =~ /restricted/) {
    $restricted = 1;
}

# "null" device
use File::Spec::Functions qw(devnull);
my $null = devnull();

### variables
my $inputfile   = "";
my $outputfile  = "";
my $tmp = "tmp-\L$program\E-$$";

### paper sizes

my @papersizes = qw[
  11x17 ledger legal letter lettersmall
  archE archD archC archB archA
  a0 a1 a2 a3 a4 a4small a5 a6 a7 a8 a9 a10
  isob0 isob1 isob2 isob3 isob4 isob5 isob6
  c0 c1 c2 c3 c4 c5 c6
  jisb0 jisb1 jisb2 jisb3 jisb4 jisb5 jisb6
  b0 b1 b2 b3 b4 b5
  flsa flse halfletter
];
my %papersizes;
foreach (@papersizes) {
    $papersizes{$_} = 1;
}

### option variables
my @bool = ("false", "true");
$::opt_version    = 0;
$::opt_help       = 0;
$::opt_debug      = 0;
$::opt_verbose    = 0;
$::opt_pdftexcmd  = "pdftex";
$::opt_xetexcmd   = "xetex";
$::opt_luatexcmd  = "luatex";
$::opt_tex        = "pdftex";
$::opt_margins    = "0 0 0 0";
$::opt_clip       = 0;
$::opt_hires      = 0;
$::opt_papersize  = "";
$::opt_resolution = "";
$::opt_bbox       = "";
$::opt_bbox_odd   = "";
$::opt_bbox_even  = "";
$::opt_initex     = 0;
$::opt_pdfversion = "auto";

sub usage ($) {
    my $ret = shift;
    find_ghostscript();
    my $usage = <<"END_OF_USAGE";
${title}Syntax:   \L$program\E [options] <input[.pdf]> [output file]
Function: Margins are calculated and removed for each page in the file.
Options:                                                       (defaults:)
  --help              print usage
  --version           print version number
  --(no)verbose       verbose printing                         ($bool[$::opt_verbose])
  --(no)debug         debug informations                       ($bool[$::opt_debug])
  --gscmd <name>      call of ghostscript                      ($::opt_gscmd)
  --pdftex | --xetex | --luatex
                      use pdfTeX | use XeTeX | use LuaTeX      ($::opt_tex)
  --pdftexcmd <name>  call of pdfTeX                           ($::opt_pdftexcmd)
  --xetexcmd <name>   call of XeTeX                            ($::opt_xetexcmd)
  --luatexcmd <name>  call of LuaTeX                           ($::opt_luatexcmd)
  --margins "<left> <top> <right> <bottom>"                    ($::opt_margins)
                      add extra margins, unit is bp. If only one number is
                      given, then it is used for all margins, in the case
                      of two numbers they are also used for right and bottom.
  --(no)clip          clipping support, if margins are set     ($bool[$::opt_clip])
                      (not available for --xetex)
  --(no)hires         using `%%HiResBoundingBox'               ($bool[$::opt_hires])
                      instead of `%%BoundingBox'
  --(no)ini           use iniTeX variant of the TeX compiler   ($bool[$::opt_initex])
Expert options:
  --restricted        turn on restricted mode                  ($bool[$restricted])
  --papersize <foo>   parameter for gs's -sPAPERSIZE=<foo>,
                      use only with older gs versions <7.32    ($::opt_papersize)
  --resolution <xres>x<yres>                                   ($::opt_resolution)
  --resolution <res>  pass argument to ghostscript's option -r
                      Example: --resolution 72
  --bbox "<left> <bottom> <right> <top>"                       ($::opt_bbox)
                      override bounding box found by ghostscript
                      with origin at the lower left corner
  --bbox-odd          Same as --bbox, but for odd pages only   ($::opt_bbox_odd)
  --bbox-even         Same as --bbox, but for even pages only  ($::opt_bbox_even)
  --pdfversion <1.x> | auto | none
                      Set the PDF version to 1.x, 1 < x < 8.
                      If `auto' is given as value, then the
                      PDF version is taken from the header
                      of the input PDF file.
                      An empty value or `none' uses the
                      default of the TeX engine.               ($::opt_pdfversion)

Input file: If the name is `-', then the standard input is used and
  the output file name must be explicitly given.
Examples:
  \L$program\E --margins 10 input.pdf output.pdf
  \L$program\E --margins '5 10 5 20' --clip input.pdf output.pdf
In case of errors:
  Try option --verbose first to get more information.
In case of bugs:
  Please, use option --debug for bug reports.
END_OF_USAGE
    if ($ret) {
        die $usage;
    }
    else {
        print $usage;
        exit(0);
    }
}

### process options
my @OrgArgv = @ARGV;
use Getopt::Long;
GetOptions(
  "help!",
  "version!",
  "debug!",
  "verbose!",
  "gscmd=s",
  "pdftexcmd=s",
  "xetexcmd=s",
  "luatexcmd=s",
  "pdftex" => sub { $::opt_tex = 'pdftex'; },
  "xetex"  => sub { $::opt_tex = 'xetex'; },
  "luatex" => sub { $::opt_tex = 'luatex'; },
  "initex!",
  "margins=s",
  "clip!",
  "hires!",
  "papersize=s",
  "resolution=s",
  "bbox=s",
  "bbox-odd=s" => \$::opt_bbox_odd,
  "bbox-even=s" => \$::opt_bbox_even,
  "restricted" => sub { $restricted = 1; },
  "pdfversion=s" => \$::opt_pdfversion,
) or usage(1);
!$::opt_help or usage(0);

if ($::opt_version) {
    print "$prj $date v$version\n";
    exit(0);
}

$::opt_verbose = 1 if $::opt_debug;

@ARGV >= 1 or usage(1);

print $title;

print "* Restricted mode: ", ($restricted ? "enabled" : "disabled"), "\n"
        if $::opt_debug;

$::opt_pdfversion =~ /^(|none|auto|1\.([2-7]))$/
        or die "!!! Error: Invalid value `$::opt_pdfversion' for option `--pdfversion'!\n";
print "* Option `pdfversion': $::opt_pdfversion\n" if $::opt_debug;
$::opt_pdfversion = $2 if $2;
$::opt_pdfversion = '' if $::opt_pdfversion eq 'none';

find_ghostscript();

if ($::opt_bbox) {
    $::opt_bbox =~ s/^\s+//;
    $::opt_bbox =~ s/\s+$//;
    $::opt_bbox =~ s/\s+/ /;
    if ($::opt_bbox =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box: $::opt_bbox\n" if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox \"$::opt_bbox\")!\n";
    }
}
if ($::opt_bbox_odd) {
    $::opt_bbox_odd =~ s/^\s+//;
    $::opt_bbox_odd =~ s/\s+$//;
    $::opt_bbox_odd =~ s/\s+/ /;
    if ($::opt_bbox_odd =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for odd pages: $::opt_bbox_odd\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-odd \"$::opt_bbox_odd\")!\n";
    }
}
if ($::opt_bbox_even) {
    $::opt_bbox_even =~ s/^\s+//;
    $::opt_bbox_even =~ s/\s+$//;
    $::opt_bbox_even =~ s/\s+/ /;
    if ($::opt_bbox_even =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for even pages: $::opt_bbox_even\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-even \"$::opt_bbox_even\")!\n";
    }
}

@ARGV <= 2 or die "$Error Too many files!\n";

### input file
$inputfile = shift @ARGV;

if ($inputfile eq '-') {
    @ARGV == 1 or die "$Error Missing output file name!\n";
    print "* Input file: <stdin>\n" if $::opt_debug;
}
else {
    if (! -f $inputfile) {
        if (-f "$inputfile.pdf") {
            $inputfile .= ".pdf";
        }
        else {
            die "$Error Input file `$inputfile' not found!\n";
        }
    }
    print "* Input file: $inputfile\n" if $::opt_debug;
}

### output file
if (@ARGV) {
    $outputfile = shift @ARGV;
}
else {
    $outputfile = $inputfile;
    $outputfile =~ s/\.pdf$//i;
    $outputfile .= "-crop.pdf";
}

print "* Output file: $outputfile\n" if $::opt_debug;

### margins
my ($llx, $lly, $urx, $ury) = (0, 0, 0, 0);
if ($::opt_margins =~
        /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
    ($llx, $lly, $urx, $ury) = ($1, $2, $3, $4);
}
else {
    if ($::opt_margins =~ /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
        ($llx, $lly, $urx, $ury) = ($1, $2, $1, $2);
    }
    else {
        if ($::opt_margins =~ /^\s*([\-\.\d]+)\s*$/) {
            ($llx, $lly, $urx, $ury) = ($1, $1, $1, $1);
        }
        else {
            die "$Error Parse error (option --margins)!\n";
        }
    }
}
print "* Margins: $llx $lly $urx $ury\n" if $::opt_debug;

### papersize validation (security)
if ($::opt_papersize ne '') {
    $::opt_papersize =~ /^[0-9A-Za-z]+$/
            or die "$Error Invalid papersize ($::opt_papersize)!\n";
    $papersizes{$::opt_papersize}
            or die "$Error Unknown papersize ($::opt_papersize),"
                   . " see ghostscript's documentation for option `-r'!\n";
}

### resolution validation (security)
if ($::opt_resolution ne '') {
    $::opt_resolution =~ /^\d+(x\d+)?$/
            or die "$Error Invalid resolution ($::opt_resolution),"
                   . " see ghostscript's documentation!\n";
}

### command name validation (security)
my %cmd = (
    'gscmd' => \$::opt_gscmd,
    'pdftexcmd' => \$::opt_pdftexcmd,
    'luatexcmd' => \$::opt_luatexcmd,
    'xetexcmd' => \$::opt_xetexcmd
);
foreach my $cmd (keys %cmd) {
    my $cmd_ref = $cmd{$cmd};
    $$cmd_ref =~ s/^\s+//;
    $$cmd_ref =~ s/\s+$//;
    my $val = $$cmd_ref;
    next unless $val;
    next unless $val;
    if ($val =~ /`/) {
        die "$Error Forbidden backtick for option `--$cmd' ($val)!\n";
    }
    if ($val =~ /\s/) {
        my $err = 0;
        if ($restricted or not $Win) {
            $err = 1;
        }
        else {
            $err = 1 if $val =~ /\.exe.*\s/i;
            $err = 1 if $val =~ /\s[-\/@+]/;
        }
        die "$Error Forbidden whitespace for option `--$cmd' ($val)!\n" if $err;
    }
}
if ($restricted) {
    if ($::opt_pdftexcmd and $::opt_pdftexcmd ne 'pdftex') {
        die "$Error pdfTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_xetexcmd and $::opt_xetexcmd ne 'xetex') {
        die "$Error XeTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_luatexcmd and $::opt_luatexcmd ne 'luatex') {
        die "$Error LuaTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_gscmd) {
        $::opt_gscmd =~ /^(gs|mgs|gswin32c|gs386|gsos2)$/
        or $::opt_gscmd =~ /^gs[\-_]?(\d|\d[\.-_]?\d\d)c?$/
        or die "$Error: Invalid Ghostscript program name in restricted mode!\n";
    }
}
if ($Win and $::opt_gscmd =~ /\s/) {
    $::opt_gscmd = "\"$::opt_gscmd\"";
}

### cleanup system
my @unlink_files = ();
my $exit_code = 1;
sub clean {
    print "* Cleanup\n" if $::opt_debug;
    if ($::opt_debug) {
        print "* Temporary files: @unlink_files\n";
    }
    else {
        for (; @unlink_files>0; ) {
            unlink shift @unlink_files;
        }
    }
}
sub cleanup {
    clean();
    exit($exit_code);
}
$SIG{'INT'} = \&cleanup;
$SIG{'__DIE__'} = \&clean;

### Calculation of BoundingBoxes

# use safe file name for use within cmd line of gs (unknown shell: space, ...)
# and XeTeX (hash, curly braces, ...)
my $inputfilesafe = $inputfile;
if ($inputfile eq '-') {
    $inputfilesafe = "$tmp-stdin.pdf";
    print "* Temporary input file: $inputfilesafe\n" if $::opt_debug;
    push @unlink_files, $inputfilesafe;
    open(OUT, '>', $inputfilesafe)
            or die sprintf "$Error Cannot write `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    binmode(OUT);
    my $size = 0;
    my $len = 0;
    my $buf = '';
    my $buf_size = 65536;
    do {
        $len = read STDIN, $buf, $buf_size;
        if (not defined $len) {
            my $msg = exterr;
            die "$Error Reading standard input ($msg)!\n";
        }
        print OUT $buf
                or die sprintf "$Error Writing `%s` (%s)!\n",
                               $inputfilesafe, exterr;
        $size += $len;
    }
    while ($len);
    close(OUT);
    print "* File size (STDIN): $size\n" if $::opt_debug;
}
elsif (not $inputfile =~ /^[\w\d\.\-\:\/@]+$/) { # /[\s\$~'"#{}%]/
    $inputfilesafe = "$tmp-img.pdf";
    push @unlink_files, $inputfilesafe;
    my $symlink_exists = eval {
        local $SIG{'__DIE__'};
        symlink("", "");
        1;
    };
    print "* Input file name `$inputfile' contains special characters.\n"
          . "* " . ($symlink_exists ? "Link" : "Copy")
          . " input file to temporary file `$inputfilesafe'.\n"
            if $::opt_verbose;
    if ($symlink_exists) {
        symlink($inputfile, $inputfilesafe)
            or die sprintf "$Error Link from `%s' to `%s' failed (%s)!\n",
                           $inputfile, $inputfilesafe, exterr;
    }
    else {
        use File::Copy;
        copy($inputfile, $inputfilesafe)
                or die sprintf "$Error Copy from `%s' to `%s' failed (%s)\n",
                               $inputfile, $inputfilesafe, exterr;
    }
}

if ($::opt_pdfversion eq 'auto') {
    open(IN, '<', $inputfilesafe)
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    my $buf;
    read(IN, $buf, 1024)
            or die sprintf "!!! Error: Cannot read the header of `%s' failed (%s)!\n",
                           $inputfilesafe, exterr;
    close(IN);
    if ($buf =~ /%PDF-1.([0-7])\s/) {
        $::opt_pdfversion = $1;
        print "* PDF header: %PDF-1.$::opt_pdfversion\n" if $::opt_verbose;
        $::opt_pdfversion = 2 if $::opt_pdfversion < 2;
    }
    else {
        die "!!! Error: Cannot find PDF header of `$inputfilesafe'!\n";
    }
}
print '* Using PDF minor version: ',
      ($::opt_pdfversion ? $::opt_pdfversion : "engine's default"),
      "\n" if $::opt_debug;

my @gsargs = (
    "-sDEVICE=bbox",
    "-dBATCH",
    "-dNOPAUSE"
);
push @gsargs, "-sPAPERSIZE=$::opt_papersize" if $::opt_papersize;
push @gsargs, "-r$::opt_resolution" if $::opt_resolution;
push @gsargs,
    "-c",
    "save",
    "pop",
    "-f",
    $inputfilesafe
;

my $tmpfile = "$tmp.tex";
push @unlink_files, $tmpfile;
open(TMP, ">$tmpfile")
    or die sprintf "$Error Cannot write tmp file `%s' (%s)!\n",
                   $tmpfile, exterr;
print TMP <<'END_TMP';
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
END_TMP
my $pdffilehex = unpack 'H*', $inputfilesafe;
$pdffilehex = "\U$pdffilehex\E";
print TMP "\\def\\pdffilehex{$pdffilehex}\n";
print TMP <<'END_TMP';
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
END_TMP
if ($::opt_tex eq 'luatex') {
    print TMP <<'END_TMP';
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname directlua\endcsname\relax
  \errmessage{LuaTeX not found!}%
\else
  \begingroup
    \newlinechar=10 %
    \endlinechar=\newlinechar %
    \ifnum0%
        \directlua{%
          if tex.enableprimitives then
            tex.enableprimitives('TEST', {
              'luatexversion',
              'pdfoutput',
              'pdfcompresslevel',
              'pdfhorigin',
              'pdfvorigin',
              'pdfpagewidth',
              'pdfpageheight',
              'pdfmapfile',
              'pdfximage',
              'pdflastximage',
              'pdfrefximage',
              'pdfminorversion',
              'pdfobjcompresslevel',
            })
            tex.print('1')
          end
        }%
        \ifx\TESTluatexversion\UnDeFiNeD\else 1\fi %
        =11 %
      \global\let\luatexversion\luatexversion %
      \global\let\pdfoutput\TESTpdfoutput %
      \global\let\pdfcompresslevel\TESTpdfcompresslevel %
      \global\let\pdfhorigin\TESTpdfhorigin %
      \global\let\pdfvorigin\TESTpdfvorigin %
      \global\let\pdfpagewidth\TESTpdfpagewidth %
      \global\let\pdfpageheight\TESTpdfpageheight %
      \global\let\pdfmapfile\TESTpdfmapfile %
      \global\let\pdfximage\TESTpdfximage %
      \global\let\pdflastximage\TESTpdflastximage %
      \global\let\pdfrefximage\TESTpdfrefximage %
      \global\let\pdfminorversion\TESTpdfminorversion %
      \global\let\pdfobjcompresslevel\TESTpdfobjcompresslevel %
    \else %
      \errmessage{%
        Missing \string\luatexversion %
      }%
    \fi %
  \endgroup %
\fi
END_TMP
}
if ($::opt_tex eq 'pdftex' or $::opt_tex eq 'luatex') {
    print TMP <<'END_TMP_HEAD';
\pdfoutput=1 %
\pdfcompresslevel=9 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1<5 %
      \pdfobjcompresslevel=0 %
    \else
      \pdfobjcompresslevel=2 %
    \fi
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#1\relax
    }%
  }{%
    \pdfminorversion=#1\relax
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
END_TMP_HEAD
    print TMP "\\setpdfversion{$::opt_pdfversion}\n" if $::opt_pdfversion;
}
else { # XeTeX
    print TMP <<'END_TMP_HEAD';
\expandafter\ifx\csname XeTeXpdffile\endcsname\relax
  \errmessage{XeTeX not found or too old!}%
\fi
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \shipout\hbox{%
    \kern-1in%
    \kern-#2bp%
    \vbox{%
      \kern-1in%
      \kern#3bp%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \page {#1} [#2 #3 #4 #5]%
}
\def\pageinclude#1{%
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \kern-1in%
    \vbox{%
      \kern-1in%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
END_TMP_HEAD
}

print "* Running ghostscript for BoundingBox calculation ...\n"
    if $::opt_verbose;
print "* Ghostscript call: $::opt_gscmd @gsargs\n" if $::opt_debug;

my @bbox;
my @bbox_all;
my @bbox_odd;
my @bbox_even;
if ($::opt_bbox) {
     $::opt_bbox =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_all = ($1, $2, $3, $4);
}
if ($::opt_bbox_odd) {
     $::opt_bbox_odd =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_odd = ($1, $2, $3, $4);
}
if ($::opt_bbox_even) {
     $::opt_bbox_even =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_even = ($1, $2, $3, $4);
}

sub getbbox ($$$$$) {
    my $page = shift;
    my $a = shift;
    my $b = shift;
    my $c = shift;
    my $d = shift;
    if ($page % 2 == 1) {
        if ($::opt_bbox_odd) {
            return @bbox_odd;
        }
    }
    else {
        if ($::opt_bbox_even) {
            return @bbox_even;
        }
    }
    if ($::opt_bbox) {
        return @bbox_all;
    }
    return ($a, $b, $c, $d);
}
my $page = 0;
my $gs_pipe = "$::opt_gscmd -dSAFER @gsargs 2>&1";
$gs_pipe .= " 1>$null" unless $::opt_verbose;
$gs_pipe .= " |";

open(GS, $gs_pipe)
        or die sprintf "$Error Cannot call ghostscript `%s' (%s)!\n",
                       $::opt_gscmd, exterr;
my $bb = ($::opt_hires) ? "%%HiResBoundingBox" : "%%BoundingBox";
my $previous_line = 'Previous line';
# Ghostscript workaround for buggy ports that prints
# the bounding box data twice on STDERR.
while (<GS>) {
    print $_ if $::opt_verbose;
    if (/^$bb:\s*(-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+)/o) {
    }
    else {
        $previous_line = $_;
        next;
    }
    next if $previous_line eq $_;
    $previous_line = $_;
    $page++;
    @bbox = getbbox($page, $1, $2, $3, $4);

    my $empty = 0;
    $empty = 1 if $bbox[0] >= $bbox[2];
    $empty = 1 if $bbox[1] >= $bbox[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: Empty Bounding Box is returned by Ghostscript!
!!!   Page $page: @bbox
!!! Either there is a problem with the page or with Ghostscript.
!!! Recovery is tried by embedding the page in its original size.

END_WARNING
        print TMP "\\pageinclude{$page}\n";
        next;
    }

    print "* Page $page: @bbox\n" if $::opt_verbose;

    my @bb = ($bbox[0] - $llx, $bbox[1] - $ury,
             $bbox[2] + $urx, $bbox[3] + $lly);

    $empty = 0;
    $empty = 1 if $bb[0] >= $bb[2];
    $empty = 1 if $bb[1] >= $bb[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: The final Bounding Box is empty!
!!!   Page: $page: @bb
!!! Probably caused by too large negative margin values.
!!! Recovery by ignoring margin values.

END_WARNING
        print TMP "\\page $page [@bbox]\n";
        # clipping shouldn't make a difference
        next;
    }
    if ($::opt_clip) {
        print TMP "\\pageclip $page [@bbox][$llx $lly $urx $ury]\n";
    }
    else {
        print TMP "\\page $page [@bb]\n";
    }
}
close(GS);

if ($? == -1) {
    die sprintf "$Error Ghostscript failed to execute (%s)!\n",
                exterr;
}
elsif ($? & 127) {
    die sprintf  "$Error Ghostscript died with signal %d!\n",
                 ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error Ghostscript exited with error code %d!\n",
                $? >> 8;
}

print TMP "\\csname \@\@end\\endcsname\n\\end\n";
close(TMP);

if ($page == 0) {
    die "$Error Ghostscript does not report bounding boxes!\n";
}

### Run pdfTeX/XeTeX

push @unlink_files, "$tmp.log";
my $cmd;
my $texname;
if ($::opt_tex eq 'pdftex') {
    $cmd = $::opt_pdftexcmd;
    $texname = 'pdfTeX';
}
elsif ($::opt_tex eq 'luatex') {
    $cmd = $::opt_luatexcmd;
    $texname = 'LuaTeX';
}
else {
    $cmd = $::opt_xetexcmd;
    $texname = 'XeTeX';
}
$cmd = "\"$cmd\"" if $Win and $cmd =~ /\s/;
$cmd .= ' -no-shell-escape';
if ($::opt_initex) {
    $cmd .= ' --ini --etex';
}
if ($::opt_verbose) {
    $cmd .= " -interaction=nonstopmode $tmp";
}
else {
    $cmd .= " -interaction=batchmode $tmp";
}
print "* Running $texname ...\n" if $::opt_verbose;
print "* $texname call: $cmd\n" if $::opt_debug;
if ($::opt_verbose) {
    system($cmd);
}
else {
    `$cmd`;
}
if ($? == -1) {
    die sprintf "$Error %s run failed to execute (%s)!\n",
                $texname, exterr;
}
elsif ($? & 127) {
    die sprintf "$Error %s run died with signal %d!\n",
                $texname, ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error %s run failed with value %d!\n",
                $texname, ($? >> 8);
}

### Check pdf version of temp file
if ($::opt_pdfversion) {
    open(PDF, '+<', "$tmp.pdf")
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    my $header;
    read PDF, $header, 9
            or die sprintf "!!! Error: Cannot read header of `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    $header =~ /^%PDF-1\.(\d)\s$/ or die "!!! Error: Cannot find header of `$tmp.pdf'!\n";
    if ($1 ne $::opt_pdfversion) {
        seek PDF, 7, 0
                or die sprintf "!!! Error: Cannot seek in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print PDF $::opt_pdfversion
                or die sprintf "!!! Error: Cannot write in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print "* PDF version correction in output file: 1.$::opt_pdfversion\n"
                if $::opt_debug;
    }
    close(PDF);
}

### Move temp file to output
if (!rename("$tmp.pdf", $outputfile)) {
    use File::Copy;
    move "$tmp.pdf", $outputfile or
            die "$Error Cannot move `$tmp.pdf' to `$outputfile'!\n";
}

print "==> $page page", (($page == 1) ? "" : "s"),
      " written on `$outputfile'.\n";

$exit_code = 0;
cleanup();

__END__


==> tab-baselines.tex <==
% !TEX root = main.tex
\begin{table}[t]
	\centering
	\caption{
		Baselines for evaluation and their positions in the design space.
	}
	\includegraphics[width=0.48\textwidth{}]{./figs/baselines-pptx}
%	\vspace{-2em}
	\label{tab:baselines}
%	\vspace{-3em}
\end{table}


==> tab-eval-distilbert.tex <==
% !TeX root = main.tex

\begin{table}
	\centering
	\begin{tabular}{llllll} 
		\hline
		& SST-2 & RTE  & QNLI & QQP &  Time (s) \\ 
		\hline
		Vanilla-Distil & 91.3  & 59.9 & 89.2 & 88.5  &  >3
	\end{tabular}
	\caption{Vanilla DisilBERT results. It takes over 3s to finish execution on both Odroid and Jetson due to large IO. 
	It fails to meet all target latencies due to its size is not configurable.}
	\label{tab:eval:distil}
\end{table}

==> tab-eval-odroid-acc.tex <==
% !TeX root = main.tex

\begin{table*}[h!]
	\centering
	\caption{Model execution accuracies; given target latencies, ours are the best or the closest to the best. 	
		|S|: preload buffer size. 
		Gold accuracy from DistilBERT~\cite{distilbert}, 
		which exceed all target latencies.
		End-to-end DistilBERT execution delays: 3.7s on Odroid, of which IO=3.1s; 
		3.36s on Jetson, of which IO=3.0s. 
		%DistilBERT latencies: 3.7s on Odroid, IO/computation=3.1s/0.6s; 3.36s on Jetson, IO/computation=3.0s/0.36s.
	}
	\includegraphics[width=1\textwidth{}]{./figs/tab_accu}
	%	\vspace{-2em}
	\label{tab:accu}
%	\vspace{-2em}
\end{table*}


%\begin{table*}
%	\centering
%	\begin{tabular}{l|lll|lll|lll|lll} 
%		\hline
%		\multicolumn{1}{l}{Task:}   & \multicolumn{3}{c|}{SST-2 (accu.)}            & \multicolumn{3}{c|}{RTE (accu.)}              & \multicolumn{3}{c|}{QNLI (accu.)}             & \multicolumn{3}{c}{QQP (accu. + F1)}           \\ 
%		\hline
%		\multicolumn{1}{l}{T (ms):} & 150           & 200           & 400           & 150           & 200           & 400           & 150           & 200           & 400           & 150           & 200           & 400            \\ 
%		\hline
%		Load\&Exec                     & 50.9          & 50.9          & 78.8          & 47.3          & 47.3          & 47.7          & 44.8          & 44.8          & 59.4          & 45.4          & 45.9          & 42.9           \\
%		NaivePL                         & 50.9          & 50.9          & 78.8          & 47.3          & 47.3          & 47.7          & 44.8          & 44.7          & 59.4          & \textbf{45.4} & 45.9          & 42.9           \\
%		NaivePL-2                       & 74.7          & 67.8          & 89.3          & 46.9          & 47.3          & 51.6          & 51.2          & 50.6          & 53.0          & 33.9          & 31.6          & 55.2           \\
%		NaivePL-6                       & 78.8          & 78.0          & 91.7          & 47.3          & 47.7          & 67.9          & 59.3          & 54.1          & 88.9	 & 41.6          & 44.7          & 88.2           \\
%		AllInMem                      & 78.8          & 87.2          & \textbf{92.0} & \textbf{47.7} & 52.3          & 68.2          & 59.4          & \textbf{72.7} & 88.8          & 42.9          & 81.2          & 88.1           \\
%		AllInMem-6                    & 78.8          & 87.2          & 92.0          & 47.3          & \textbf{52.7} & 67.5          & 59.3          & 69.7          & 88.9          & 41.6          & 80.7          & 88.2           \\
%		Ours (1MB)                  & \textbf{79.8} & \textbf{87.2} & 91.9          & 47.3          & 52.0          & \textbf{68.2} & \textbf{60.0} & 71.2          & \textbf{89.0}          & 42.4          & \textbf{81.3} & \textbf{88.2} 
%	\end{tabular}
%	\caption{\sys{} accu. on Odroid (CPU). 		All models used are DynaBERT because we need to configure the sizes;		Vanilla-DistilBERT results in Table~\ref{tab:benchmarks}.		Unless specified, fidelities used are full 32-bit.  (XXX present Nano results???XXX}
%	\label{tab:eval:accu-odroid}
%\end{table*}

%\input{tab-eval-distilbert}

==> tab-gptloraSc1.tex <==
% !TeX root = main.tex



\begin{table}[t]
	\centering
	\caption{
		The forward time, backward time on different devices during fine-tuning (LoRA) GPT2-large with the batch size of 16.}
		%		Gold accuracy measured from DistilBERT~\cite{distilbert}.
	
	\includegraphics[width=0.48\textwidth{}]{figs/gptloraSc1.pdf}
%	\vspace{-1em}
	\label{tab:gptloraSc1}
%	\vspace{-3em}
\end{table}

==> tab-gptwoloraSc1.tex <==
% !TeX root = main.tex



\begin{table}[t]
	\centering
	\caption{
		The forward time, backward time on different devices during fine-tuning (without LoRA) GPT2-large with the batch size of 16.}
		%		Gold accuracy measured from DistilBERT~\cite{distilbert}.
	
	\includegraphics[width=0.48\textwidth{}]{figs/gptwoloraSc1.pdf}
%	\vspace{-1em}
	\label{tab:gptwoloraSc1}
%	\vspace{-3em}
\end{table}

==> tab-network-confs.tex <==
% !TeX root = main.tex
\begin{table}[h]
		\caption{Sizes (depth$\times$width) of submodels selected under different target latencies. A large submodel means more FLOPs executed, suggesting a higher accuracy. 
		%		benchmarks have the same submodel size given the same T.
		\sys{} is able to run the largest submodel.
		}
		\includegraphics[width=0.48\textwidth{}]{./figs/tab_networks}
		\label{tab:network-confs}
\end{table}

%\begin{table}
%	\centering
%	\footnotesize
%	\begin{tabular}{l|cccc|cccc}
%		& \multicolumn{4}{c|}{T (ms) on Odroid (CPU)}                                                     & \multicolumn{4}{c}{T (ms) on Jetson (GPU)}  \\
%		& 300                   & 600                    & 900                   & 1200                   & 50 & 100 & 150 & 200                        \\ 
%		\hline
%		V-Distil                                                                                  & \multicolumn{8}{c}{6x12 (not configurable)~}                                                                                                  \\ 
%		\hline
%		\multirow{2}{*}{V/N-Dyna}                                                                 & \multirow{2}{*}{3x3~} & \multirow{2}{*}{5x3}   & \multirow{2}{*}{7x3~} & \multirow{2}{*}{9x3}   &    &     &     &                            \\
%		&                       &                        &                       &                        &    &     &     &                            \\ 
%		\hline
%		\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}N-Dyna-2b,\\O-Dyna(-2/6b),\\Ours\end{tabular}} & \multirow{3}{*}{8x3~} & \multirow{3}{*}{12x4~} & \multirow{3}{*}{12x8} & \multirow{3}{*}{12x12} &    &     &     &                            \\
%		&                       &                        &                       &                        &    &     &     &                            \\
%		&                       &                        &                       &                        &    &     &     &                            \\
%		\cline{2-9}
%	\end{tabular}
%	\caption{Submodel sizes decided by \sys{} compute planning... Vanilla/NPP-dyna share sizes because both IO dominate pipeline (compute negligible), NPP-Dyna-2b...Ours share the same submodel because all are compute-bound...}
%\label{tab:network-confs}
%\end{table}

\begin{comment}
\begin{table*}
	\centering
%	\footnotesize
	\begin{tabular}{l|lllll|l|llllll}
		& \multicolumn{6}{c|}{Odroid (CPU)}                                                                                                & \multicolumn{6}{c}{Jetson Nano (GPU)}  \\ 
		\cline{2-13}
		\diagbox{Baselines}{T (ms)} & 300                   & 600                    & 900                   & 1200                   & T\_cold                 & Mem. & 50 & 100 & 150 & 200 & T\_cold & Mem.  \\ 
		\hline
		Vanilla-Distil              & \multicolumn{5}{c|}{6x12 (not configurable)}                                                                              & 0    & \multicolumn{5}{c}{6x12}       & 0     \\ 
		\cline{2-13}
		Vanilla-Dyna                & \multirow{2}{*}{3x3~} & \multirow{2}{*}{5x3}   & \multirow{2}{*}{7x3~} & \multirow{2}{*}{9x3}   & \multirow{2}{*}{12x12~} & 0    &    &     &     &     &         & 0     \\
		NPP-Dyna                    &                       &                        &                       &                        &                         & 0    &    &     &     &     &         & 0     \\ 
		\hline
		NPP-Dyna-2b                 & \multirow{5}{*}{8x3~} & \multirow{5}{*}{12x4~} & \multirow{5}{*}{12x8} & \multirow{5}{*}{12x12} & \multirow{5}{*}{12x12}  & 0    &    &     &     &     &         & 0     \\
		Oracle-Dyna                 &                       &                        &                       &                        &                         & 440  &    &     &     &     &         & 50    \\
		Oracle-Dyna-2b              &                       &                        &                       &                        &                         & 28   &    &     &     &     &         & 1     \\
		Oracle-Dyna-6b              &                       &                        &                       &                        &                         & 80   &    &     &     &     &         & 1     \\
		Ours                        &                       &                        &                       &                        &                         & 1-5  &    &     &     &     &         & 1     \\
		\hline
	\end{tabular}
	\label{tab:network-confs}
	\caption{Choice of target latencies and baselines...}
\end{table*}
\end{comment}

==> tab-platform.tex <==
% !TEX root = main.tex
\begin{table}[t]
	\centering
	\caption{
		Platforms in evaluation.
		Benchmarks run on Odroid's CPU (its GPU lacks Pytorch support) and Jetson's GPU. 
		%		Nano -- should be 32GB storage
	}
	\includegraphics[width=0.4\textwidth{}]{./figs/platform}
%	\vspace{-2em}
	\label{tab:platform}
%	\vspace{-3em}
\end{table}


==> tab-roomTemperature.tex <==
% !TeX root = main.tex



\begin{table}[t]
	\centering
	\caption{
		The temperature of the room where each device is.
		%		Gold accuracy measured from DistilBERT~\cite{distilbert}.
	}
	\includegraphics[width=0.4\textwidth{}]{figs/roomTemperature.pdf}
%	\vspace{-1em}
	\label{tab:roomTemperature}
%	\vspace{-3em}
\end{table}

==> tab-scenarioConfig.tex <==
% !TeX root = main.tex



\begin{table}[t]
	\centering
	\caption{
		Possible scenarios of different workloads on different testbeds. 
		%		Gold accuracy measured from DistilBERT~\cite{distilbert}.
	}%\xzlNote{Dec 5: why different precision?}
	\includegraphics[width=0.48\textwidth{}]{figs/scenarioConfig.pdf}
%	\vspace{-1em}
	\label{tab:scenarioconfig}
%	\vspace{-3em}
\end{table}

==> tab-shard-param.tex <==
% !TeX root = main.tex
\begin{table}
	\centering
	\caption{The weight composition of a shard. $M$ is number of attention heads. 
		The $M$ shards equally slices a \tfm{} layer, where each shard of the layer can be uniquely identified by its vertical slice index $i = 0 \dots M-1$.}
	\begin{tabular}{l|c|c|c}
		& Attn (Q,K,V,O)         & FFN1                        & \multicolumn{1}{l}{FFN2}     \\ 
		\hline
		Transformer Layer & $d\times d $           & $d_{ff} \times d$             & $d \times d_{ff}$              \\ 
		\hline
		Shard (vertical slice)      & $d \times \frac{d}{M}$ & $\frac{d_{ff}}{M} \times d$ & $d \times \frac{d_{ff}}{M}$  \\
		\hline
	\end{tabular}
	\label{tab:vertical_slice}
\end{table}

==> tab-shard-selection.tex <==
% !TeX root = main.tex

\begin{table}[t]
	\centering
	\caption{Model accuracies resultant from allocating additional IO budget within a 5x3 submodel of 2-bit shards. Our method shows much higher accuracies than random shard selection.}
	\includegraphics[width=0.48\textwidth{}]{./figs/plot/shard-selection/tab}
	%	\vspace{-2em}
%	\caption{Accuracies when progressively upgrading a 2-bit 5x3 submodel to 6-bit.
%	2/6bit accu. are the accuracies when the submodel has all shards in 2 or 6 bitwidths.
%	Ours has significantly better accuracies than importance-unaware random selection.}
%	2/6bit accu. are the accuracies when the submodel has all shards in 2 or 6 bitwidths.
%	Ours has significantly better accuracies than importance-unaware random selection.}
	\label{tab:eval:shard-selection}
%	\vspace{2em}
\end{table}

==> tab-shards-size.tex <==
% !TeX root = main.tex

\begin{table}[h!]
	\centering
	\begin{tabular}{llllll} 
		\hline
		Fidel. ver. (bit) & 2     & 3     & 4    & 5    & 6     \\ 
		\hline
		Comp. ratio ($\times$)   & 15.66 & 10.52 & 7.92 & 6.35 & 5.30 
	\end{tabular}
	\caption{SST-2 model compression ratios at different fidelities (0.15\% outliers).
	Others have similar compression ratios (CoLa, RTE outliers: 0.14\%, QQP outliers: 0.17\%).}
\label{tab:eval:shard-size}
\end{table}

==> tab-trainingTimeSc1.tex <==
% !TeX root = main.tex



\begin{table}[t]
	\centering
	\caption{
		The forward time, backward time on different devices during training whisper.medium with the batch size of 4.
	}
	\includegraphics[width=0.48\textwidth{}]{figs/trainingTimeSc1.pdf}
%	\vspace{-1em}
	\label{tab:trainingTimeSc1}
%	\vspace{-3em}
\end{table}

==> tab-trainingTimeSc2.tex <==
% !TeX root = main.tex



\begin{table}[t]
	\centering
	\caption{
		The forward time, backward time on different devices during training whisper.medium with the batch size of 4 when CUDA devices are applied with Zero-Offload. 
		%		Gold accuracy measured from DistilBERT~\cite{distilbert}.
	}%\xzlNote{Dec 5: why different precision?}
	\includegraphics[width=0.48\textwidth{}]{figs/trainingTimeSc2.pdf}
%	\vspace{-1em}
	\label{tab:trainingTimeSc2}
%	\vspace{-3em}
\end{table}

==> tab-trainingTimeSc2gptxllora.tex <==
% !TeX root = main.tex



\begin{table}[t]
	\centering
	\caption{
		The forward time, backward time on different devices during training GPT2-XL with the batch size of 16, with LoRA, when CUDA devices are applied with Zero-Offload. 
		%		Gold accuracy measured from DistilBERT~\cite{distilbert}.
	}%\xzlNote{Dec 5: why different precision?}
	\includegraphics[width=0.48\textwidth{}]{figs/trainingSc2gptxllora.pdf}
%	\vspace{-1em}
	\label{tab:trainingTimeSc2gptlora}
%	\vspace{-3em}
\end{table}

==> tab-trainingTimeSc2gptxllora__Feng_Dahua_____________________2024-12-23_.tex <==
% !TeX root = main.tex



\begin{table}[t]
	\centering
	\caption{
		The forward time, backward time on different devices during training GPT2-XL with the batch size of 16, without LoRA, when CUDA devices are applied with Zero-Offload. 
		%		Gold accuracy measured from DistilBERT~\cite{distilbert}.
	}%\xzlNote{Dec 5: why different precision?}
	\includegraphics[width=0.48\textwidth{}]{figs/trainingSc2gptxlwolora.pdf}
%	\vspace{-1em}
	\label{tab:trainingTimeSc2gptlora}
%	\vspace{-3em}
\end{table}

==> tab-trainingTimeSc2gptxlwolora.tex <==
% !TeX root = main.tex



\begin{table}[t]
	\centering
	\caption{
		The forward time, backward time on different devices during training GPT2-XL with the batch size of 16, without LoRA, when CUDA devices are applied with Zero-Offload. 
		%		Gold accuracy measured from DistilBERT~\cite{distilbert}.
	}%\xzlNote{Dec 5: why different precision?}
	\includegraphics[width=0.48\textwidth{}]{figs/trainingSc2gptxlwolora.pdf}
%	\vspace{-1em}
	\label{tab:trainingTimeSc2gptwolora}
%	\vspace{-3em}
\end{table}

==> tab-workloadScenario__Feng_Dahua_____________________2024-12-23_.tex <==
% !TeX root = main.tex



\begin{table}[t]
	\centering
	\caption{
		The workloads we used in our experiments, with AdamW optimizer. 
		%		Gold accuracy measured from DistilBERT~\cite{distilbert}.
	}%\xzlNote{Dec 5: why different precision?}
	\includegraphics[width=0.48\textwidth{}]{figs/scenarioConfig.pdf}
%	\vspace{-1em}
	\label{tab:workload}
%	\vspace{-3em}
\end{table}

==> tab_benchmarks.tex <==
% !TEX root = main.tex
\begin{table}[t]
	\centering
	\caption{
		GLUE benchmarks~\cite{glue-benchmark} used in evaluation.
		%		Gold accuracy measured from DistilBERT~\cite{distilbert}.
	}
	\includegraphics[width=0.48\textwidth{}]{./figs/benchmarks}
%	\vspace{-1em}
	\label{tab:benchmarks}
%	\vspace{-3em}
\end{table}


==> thoughts.tex <==
% !TeX root = main.tex

\section*{Thoughts}

\paragraph{Benefits of being retraining free}
No need to fine tune, which is time-consuming. 
Does not need access to training data, which is often private and proprietary. 
\Note{needs to be careful about this:} we cannot do arbitrary pretrained model. Need to use dynabert as a backbone network. 


\paragraph{What are key innovations?}
The key contribution of \sys{} is: 
1) it identifies the model shards which have elastic IO time, as the proper building block for the IO/compute pipeline of transformer inference \Note{novel approach for constructing the elastic pipeline};
2) based on model shards, it proposes a novel planning algorithm that maximizes the inference accuracy while meeting a user-set deadline on different devices.

We do not claim: 1) quantization techniques used to generate shards, and 2) IO/compute pipeline as our contribution since these techniques are well-known. 

\paragraph{How does the IO/compute pipeline work with shards?}
The number of shards per layer can be regarded as the ``width'' of the \tfm{} model during an inference;
it is the same across all layers during one inference.
Prior to each inference, \sys{} decides how many shards and the bitwidth of each shard to be used, depending on the deadline and device-specific IO/compute capability. 
For one inference, \sys{} constructs the IO/compute pipeline in the following way: it first loads the initial set of shards for layer 1; it then begins computing on shards of layer 1, while overlapping shard loading for layer 2, and so on and so forth.

\paragraph{Why do partial model composed of shards give meaningful results?}
Because of the parameter redundancy of \tfm{} models: 
a \tfm{} model may still give meaningful results even if attention heads are reduced from full sixteen to a few~\cite{16heads}, or layers share the same set of parameters~\cite{albert}. 
In \sys{}, one shard is a vertical slice of the transformer layer, comprising one attention head plus a set of FFN neurons; 
it preserves the structure on which the model is trained and the learned features. 
By stacking them in layers, the resultant model resembles a partial model with a smaller width~\cite{dynabert, liDynamicSlimmableNetwork2021}, hence still giving meaningful results.



\paragraph{\sys{} seems a generic model compression technique, why target cold inference only?}
To clarify: the model compression technique used by \sys{} is not new~\cite{gobo};
it acts only as an enabling tool for \sys{} to generate shards as the IO/compute pipeline building block.

\sys{}'s key ideas are tailored to cold inference due to the deadline constraint, where IO is the bottleneck.
The compression, however, does not affect compute time w.r.t. a full-precision model.
It hence has little benefits in a hot inference scenario, i.e. same latency but inferior accuracy than a full-precision model.

\paragraph{Can a GPU help reduce cold inference latency?}
No. 
This is because during cold inference, IO is the bottleneck, dominating over 90\% of the latency.
By simply offloading the compute to GPU, the IO keeps blocking compute and still results in high cold inference latency.

\paragraph{Why not offload to cloud?}
First, on-device inference ensures better privacy. 
The query as well as content being queried (e.g. medical records) do not have to be exposed to cloud.
Second, it is more reliable where spotty network connections are common on mobile devices~\cite{livelab,backgnd-in-wild2}.
Third, cloud offloading is a complementary approach, e.g. for other non-private queries, the user can always offload to cloud.

\paragraph{Can we leverage idle intervals between IPA interactions to load model?}
This is an orthogonal approach.
The idea is to prefetch the model file prior to inference.
Its challenge is twofold: 1) it is unclear how well IPA invocations can be predicted, while misprediction leads to excessive memory usage and poor user experience.
2) coordinating with other apps which compete for memory may be challenging, e.g. the already prefetched model file may be swapped out due to contention.


\paragraph{Why sacrifice accuracy for latency?}
Because in the scenario we target, reducing the latency from seconds to milliseconds significantly improves user experience.
Meanwhile, the accuracy loss is only 1\%, which is considered negligible in NLP literature~\cite{albert,nagarajanOptimizingTransformersApproximate}.
Prior study on IPAs~\cite{tsaiFasterResponsesAre2019} support our design, advocating ``faster responses are better responses''. 

==> todo.tex <==
% !TeX root = main.tex

TODO: 
1. decompession time... not universal. depending on bitwidth
2. our use of board.. pretty wimpy. so our target delays are higher than prior work (edgebert which uses jetson...)


\Note{High level ideas}
\begin{myitemize}
	\item 
	Memory-resident model. 
	A high level ``specification'' -- depths \& widths. 
	
	\item 
	Resource-elasticity. Can respond to 
	1. diff. latency constraint (thru tuning specification); 2. diff. memory constraints: deflating/inflating like VMM memory balloon.
\end{myitemize}



\Note{Thoughts on spare IO:}
The key theme of \sys{} is how to leverage the spare IO, which is the key missing component in prior work.
Cold inference problem is a only small entry point -- because it does not leverage spare IO, it suffers from long delay.

``Resource-elastic'', tied to IO (key difference, an IO planner)
In-memory state transformer -- give bits to different parameters, depending on spare IO or not, can upgrade or throw away accordingly. 

Do not have to consider model always in memory -- our solution provides a middle ground in between

\Note{selection of quantization granularity}
Weird for odd-bit? E.g. 3-bit seems rarely used.
May use 2,4,8,16? Albeit more coarse-grained.
But keep in mind this ties to the pipeline elasticity and should fit what the device needs (what its io/compute capability is)


\Note{STI reconciles accuracy with latency...}

\Note{todo:} make a case for suboptimal accuracy during first inferences

\Note{Critical vs non-critical path:}
Critical path (i.e. during during inference): 
1. overlap io/compute. 
2. for those do not have compute or multiple stages to overlap (e.g. embedding) -- minimize io (e.g. fixed-precision embedding). 

non-critical path (i.e. background thread) can allow for some  extra work. 
Examples include:
1. embedding matrix update. 
Based on frequency, update the corresponding block positions.
2. shards upgrade.
Existing already loaded shards can be replaced by full-precision. 


